End-to-end interstellar communication system design for power efficiency

Radio communication over interstellar distances is studied, accounting for noise, dispersion, scattering and motion. Large transmitted powers suggest maximizing power efficiency (ratio of information rate to average signal power) as opposed to restricting bandwidth. The fundamental limit to reliable communication is determined, and is not affected by carrier frequency, dispersion, scattering, or motion. The available efficiency is limited by noise alone, and the available information rate is limited by noise and available average power. A set of five design principles (well within our own technological capability) can asymptotically approach the fundamental limit; no other civilization can achieve greater efficiency. Bandwidth can be expanded in a way that avoids invoking impairment by dispersion or scattering. The resulting power-efficient signals have characteristics very different from current SETI targets, with wide bandwidth relative to the information rate and a sparse distribution of energy in both time and frequency. Information-free beacons achieving the lowest average power consistent with a given receiver observation time are studied. They need not have wide bandwidth, but do distribute energy more sparsely in time as average power is reduced. The discovery of both beacons and information-bearing signals is analyzed, and most closely resembles approaches that have been employed in optical SETI. No processing is needed to account for impairments other than noise. A direct statistical tradeoff between a larger number of observations and a lower average power (including due to lower information rate) is established. The "false alarms" in current searches are characteristic signatures of these signals. Joint searches for beacons and information-bearing signals require straightforward modifications to current SETI pattern recognition approaches.

==> ICH-capacity.TEX <==

\begin{abstract}
The end-to-end design of an interstellar communication system
taking into account all known impairments due to radio propagation in the interstellar medium (attenuation, noise, dispersion, and scattering) and source/observer motion
is undertaken.
A fundamental tradeoff between signal power
(which relates to transmit and receive antenna gains and transmit power)
and signal bandwidth is established, and our design minimizes power
at the expense of bandwidth.
The fundamental limit to power efficiency
(signal power divided by information rate)
is determined by noise alone, and constrains all civilizations no matter how advanced
their technology.
This limit reveals that signal designs previously assumed in SETI observations
require about 50 times higher average power than required.
A set of five simple and practical power-efficient design principles can shrink and
eliminate this gap.
First, information is communicated by on-off patterns of energy bundles.
Second, the transmit signal is chosen to circumvent as many impairments as possible.
It is shown that by restricting the bandwidth and time duration of the waveform conveying one energy bundle,
all impairments save additive (thermal) noise and 
multiplicative noise (scintillation) are avoided.
We call this the ''interstellar coherence hole'', 
and its parameters are characterized in terms of the various impairments.
No processing related to impairments other than noise and scintillation
is required in either transmitter or receiver.
Third, information is embedded in the location of energy bundles in time or frequency.
This is illustrated using the example of M-ary FSK, in which $\log_{2} M$ bits of information are
conveyed by transmitting an energy bundle shifted by one of $M$ frequency offsets.
Fourth, scintillation is countered by time-diversity combining.
This is not pursued here in favor of a simpler outage strategy.
Fifth, energy is conserved by utilizing a low duty cycle (on-to-off ratio),
leading to highly intermittent signals.
The reliable discovery of power-efficient signals is shown to be feasible at
much lower power levels than required for information extraction.
Since this is at the expense of multiple independent observations,
there is a tradeoff between processing power and antenna collection area
in discovery.
Signals that are power-optimized for discovery can be reliably discovered
at power levels on the order of 99\% to 99.99\% lower than previously assumed.
Common algorithms can detect either information-bearing signals
or information-free beacons; however, the beacon possesses no advantages
in power or reliability.
Power-efficient design principles have profound implications for both METI and SETI,
as they significantly affect both transmitted signals and receiver discovery techniques.
First, power-efficient signals dictate
multiple independent observations in discovery to deal with their intermittent nature as well as scintillation.
Second, that intermittent character also dictates distinctive post-observation pattern recognition algorithms.
\end{abstract}

%\comment{Old abstract}
%The end-to-end design of an interstellar radio communication system is undertaken taking into account all known impairments due to radio propagation in the interstellar medium (attenuation, noise, dispersion, and scattering) and source/observer motion. 
%Recognizing the tradeoff between spectral efficiency  (information rate divided by bandwidth) and power efficiency (information rate divided by received power), power efficiency is emphasized.
%It is shown that the maximum possible power efficiency is determined by noise alone, and not affected by any other impairments.
%This is proven by showing that a transmit signal structured around the coherence hole (defined shortly)
%can achieve the fundamental limit on power efficiency.
%Optimal approaches to signal discovery establish that scintillation allows such a signal to be discovered
%with arbitrary reliability for any false alarm probability and signal level (provided the
%receiver makes repeated independent observations), obviating the need for an
%attention-attracting beacon.
%As both ISM impairments and fundamental limits are timeless, a more advanced civilization 
%cannot improve on this approach.
%An interstellar coherence hole is the largest bandwidth and time duration of an elemental signal for which most ISM and motion impairments can be neglected, and has a size (coherence bandwidth and coherence time)
%which depends on physical parameters observable by both transmitter and receiver. 
%When the transmitted signal is structured about the coherence hole, the remaining
%impairments observed by the receiver are noise and scintillation (flat fading),
%and any and all impairment-specific processing in transmitter and receiver
%(save noise and scintillation) are avoided.
%Because it preserves the average received signal power,
%scintillation due to scattering does not affect the achievable power efficiency, and is beneficial to signal discovery.
%The concrete design of an interstellar communication system based on the coherence hole, 
%without channel coding (opening up a gap to the maximum achievable power efficiency), 
%and using an outage strategy to deal with scintillation reveals numerous insights.
%The most power efficient modulation is binary on-off keying OOK, and power efficiency is maximized with 63\% outage time, placing a burden on reliable recovery of messages. 
%At higher information rates, the signal design  must have a multicarrier structure. 
%The receiver's search space is beneficially constrained by the coherence hole parameters, 
%which are dominated by the electron density and component of acceleration along the line sight.
%It is argued that these results have profound implications for both passive and active SETI, as they place strong constraints on the structure and parameterization of any information-bearing signal that seeks to approach the highest achievable power efficiency.


%\comment{Short project desc.}
%
%This project will explore for the first time a search of the radio spectrum for information-bearing signals of extraterrestrial origin.  We have overcome several off-stated objections. (a) The transmit signal structure can circumvent the dispersive and multipath phenomena of the interstellar medium (ISM) and avoid any special processing. (b) The parameterization of the receiver's search is dramatically narrowed. (c) Fundamental limits on power efficiency are approached, precluding any superior approach. 
%
%Our communication engineering methodology achieves coordination of transmitter/receiver through end-to-end design taking into account the interstellar medium (ISM) propagation characteristics. Except for scintillation, the ISM is transparent to a waveform confined to an ''interstellar coherence hole'' (ICH) determined by observable physical parameters of the ISM [a]. Associating information units (e.g. one bit) with an ICH is moderately bandwidth inefficient (acceptable because of the broad microwave window [b]). The unavoidable scintillation phase incoherence narrowly constrains the modulation choice. Minimizing peak power determines how ICH-based information units should be staged in time and frequency [c]. Waveform design is tightly constrained by immunity to radio-frequency interference [d]. Overall, we find that the signal structure and parameterization is tightly constrained.
%
%In summary, interstellar communication is quite easy when bandwidth is plentiful. The exceptions are (a) the large transmit powers and high antenna gain (an issue for a transmitter designer), (b) the lack of coordination between transmitter and receiver designers, and (c) the ''needle in a haystack'' problem of discovering such a signal at the receiver. Fortunately, addressing (a) by maximizing the power efficiency also addresses (b) by tightly constraining the structure and modulation and also (c) by dramatically reducing the signal parameterization based on observable parameters. In this research we will develop and deploy a SETI search strategy based on ''ICH analysis''.  A requirement-consistent set of modulation schemes and signal waveforms will be studied. Search algorithms will be developed emphasizing computational efficiency and parallelism. Simulation in a controlled environment will establish correctness and computational requirements. Finally, code will be ported to the production environment on the Mopra telescope platform and applied to actual observational data. The resulting production software will then be available for porting and deployment to other observation platforms used for SETI observations, such as seti@home and the Allen Telescope Array. We hope the results of this project will serve as a foundation for wideband SETI observations for many years to come.
%
%[a] D.G. Messerschmitt, ''The interstellar coherence hole and its role in interstellar communication'', working paper, May 30, 2012 (available at https://www.sugarsync.com/pf/D72382_988784_63193905).
%
%[b] H. W. Jones, ''Optimum signal modulation for interstellar communication,'' in Astronomical Society of the Pacific Conference Series., vol. 74, 1995, p. 369.
%
%[c] G. S. Shostak, ''SETI at wider bandwidths?'' Progress in the Search for Extraterrestrial Life, ed.G.Seth Shostak, ASP Conference Series, vol. 74, 1995.
%
%[d] D. G. Messerschmitt, ''Interstellar communication: The case for spread spectrum,'' arXiv:1111.0547v1 [astro-ph.IM], Nov. 2, 2011.

%\section{ISM coherence hole}
%
%It is a well established principle that over short periods of time the integrity of a monochromatic
%wave is preserved by the ISM, with the exceptions of  Doppler (a frequency shift
%due to motion) and scintillation 
%(a random phase and amplitude shift due to propagation losses and scattering).
%This concept is generalized to waveforms with finite bandwidth,
%establishing a ''interstellar coherency hole'' (ICH) characterized by 
%a maximum ''coherence bandwidth''
%and a maximum ''coherence time''.
%Together the coherence bandwidth and time constitute the ''size'' of an ICH,
%and this size depends on carrier frequency, line of sight, and the accuracy criterion
%for coherence.
%For all practical purposes,
%the ISM is transparent to any transmit waveform falling within a single ICH,
%with the exception of two Doppler consequences (a shift in carrier frequency and a time dilation)
%and scintillation (a random phase and amplitude essentially fixed within one ICH but which
%varies across ICH's non-overlapping in time and frequency).
%
%\section{Interstellar communication based on the ICH}
%
%Information can be transferred though the ISM using a multiplicity of ICH's
%that are non-overlapping in both time and frequency.
%Such information can be recovered
%at a receiver essentially without degradation due to impairments introduced
%in the ISM and without processing in transmitter or receiver related to the ISM.
%The notable exceptions to this are noise and scintillation.
%Also, such an information-bearing signal can be discovered with \emph{greater}
% reliability than recovery of its embedded information because scintillation sometimes
% results in a higher received power than is necessary for communication.
% Conversely any attempt to communicate a unit of information
%using a signal with bandwidth or time duration that is too great
%to fall within a single ICH will cause the discovery sensitivity to deteriorate,
%creating a situation in which a signal cannot be discovered in spite of
%its viability for conveying information.
%During communication, the effect of scintillation is to create periods of
%outage during which reliable extraction of information is not possible.
%
%\section{An interstellar communication system}
%
%The use of ICH's non-overlapping in time and frequency as the basis for
%an interstellar communication results in a modest bandwidth inefficiency,
%but this should not be an issue in light of the wide bandwidth of the
%microwave window.
%A benefit is that
%neither transmitter nor receiver require any special processing
%related to the ISM (other than noise and scintillation)
%and thus such a system is also dramatically simpler (at the level of
%modulation and detection and receive signal processing) than
%any existing terrestrial wireless communication system
%(which typically go to extremes to reduce bandwidth).
%Such is the benefit of assuming an unconstrained bandwidth for the ISM.
%
%\section{Comparison to fundamental limits}
%
%This communication system is compared to fundamental limits
%on the power efficiency (total information rate divided by received power)
%in the presence of noise and scintillation, and it is shown that
%with one bit per ICH (or more) it operates at a fixed gap (independent
%of rate and power) that could in principle be closed using sophisticated
%channel coding techniques.
%The size (time duration and bandwidth) of an individual ICH is irrelevant to
%the power efficiency and to this gap.
%Thus, other than reducing the size of this gap through 
%modulation and coding, it would be iimpossible
%to construct an interstellar communication system 
%that operates at greater power efficiency.
%
%\section{Conclusions}
%
%In light of the above, the assumption that any interstellar communication
%transmitter would be designed according to these principles is compelling.
%This has profound implications to the discovery of such a signal,
%because these design principles dramatically narrow the possibilities
%for the structure of the transmitted signal
%(a framework based on the ICH),
%the modulation used (which must counter noise and scintillation
%and radio-frequency interference, but no other impairments in the ISM),
%and the signal parameterization (time duration and bandwidth
%associated with individual units of information).
%Regarding the latter point, a major parameter of the signal is the
%size of an ICH, which is based on physical parameters
%that can be observed and measured (with some uncertainty) 
%by both transmitter and receiver for a given
%line of sight, and this results in a dramatic reduction in the receiver's search space.
%
%\newpage
%\comment{Following is the old abstract.}
%
%Interstellar communication must contend with dispersion caused by an interstellar low-density plasma resulting in a frequency-dependent group delay. The effect of dispersion on the discovery of and communication using digital amplitude-modulated signals is studied. It is shown that a per-carrier bandwidth larger than the coherence bandwidth (the largest bandwidth over which there is little phase variation) reduces discovery sensitivity, resulting in signals which reliably convey information but cannot be reliably discovered. This argues that the maximum information rate per subcarrier should be limited to the coherence bandwidth, which in turn is a characteristic of dispersion and scattering. Higher higher information rates can be achieved using multiple carrier frequencies (called multicarrier modulation) as proposed for interstellar communication by S. Shostak in 1995. An information-bearing signal of this type has several characteristics that distinguish it from astronomical sources of energy. The resulting receiver (for both discovery and communication) is implemented as if there were no dispersion, and in particular does not require the de-dispersion algorithms used in pulsar astronomy. The receiver can operate at the fundamental limits of noise sensitivity, and embedded spread spectrum can yield RFI immunity at the expense of a lower information rate per subcarrier and correspondingly more subcarriers. There is no constraint on frequency band, permitting the use of bands most favorable for atmospheric attenuation and noise. The greatest power efficiency (information rate per unit power) is achieved by biphase modulation, and the aggregate information rate (unaffected by dispersion) is then proportional to the received power. The information rate per subcarrier is lower bounded by the coherence time, which is determined by scattering and Doppler (addressed in a forthcoming paper). This minimum-rate design is attractive because it requires the lowest power and achieves the greatest RFI immunity. Dispersion makes interstellar communication easier because it provides specific guidance on modulation, and because it greatly reduces the search parameter space during discovery by specifying a bandwidth per carrier, carrier spacing, and (for the lowest rate design) information rate per subcarrier based on observable dispersion and scattering parameters. The minimum-rate subcarrier is also an attractive alternative to a narrowband information-free beacon (the basis of most current SETI searches) because it requires the same receive power for discovery, embeds information, and has greater RFI immunity. It is notable that past and present narrowband and pulse searches would fail to discover such a signal. When multiple subcarriers of this type are received, signals too weak for reliable communication can still be discovered based on the larger aggregate power.

\include{introduction}

\chapter{Introduction}
\label{sec:introduction}

A fundamental characteristic of the Milky Way is its capability to support the sharing of information using electromagnetic radiation among intelligent civilizations separated by interstellar distances. This capability is subject to various intrinsic physical impairments such as large spreading loss, natural sources of noise, dispersion and scattering of electromagnetic radiation in the interstellar medium (ISM) and time-varying effects due to relative source/observer motion. This paper explores this information-carrying capability, both in terms of its fundamental limits and in practical terms. This is the first attempt to comprehensively take into account impairments in the ISM an end-to-end design of an interstellar communication system employing the techniques and experience of communication engineering.

Prominent among the obstacles to establishing communication is the impossibility of prior coordination between the designers of a transmitter and a receiver \citeref{583}. 
The transmitter chooses a specific signal structure and parameterization, and to achieve high sensitivity a receiver discovering that signal (and subsequently extracting information) must also assume a specific signal structure and search over a large parameter space including spatial, frequency, and temporal variables. 
Yet prior to the establishment of communication there is no feasible way to directly coordinate these choices.
Fridman recently asserted that
''In each epoch we can only use our current technical knowledge to predict what kind of signals an ETI could send''
\citeref{602}.
We are far more optimistic than this, as from a communication engineering perspective
two pieces of this puzzle are timeless.
First, any civilization is constrained by mathematically provable fundamental limits on communication.
Second, the impairments encountered within the ISM remain fundamentally unchanging over
time periods dramatically longer than the joint epoch of a transmitting and receiving
civilization (which is governed by the interstellar propagation delay).
Together these two invariants serve as a powerful form of coordination.
As shown here, the fundamental limits are governed by attenuation and noise,
and not affected by any other impairments.
Approaching fundamental limits is feasible, but only if the various impairments are circumvented.
The resulting signal is
highly constrained as to structure by the impairments and as to parameterization by observable physical quantities.
A third, albeit less fundamental point of coordination is reasonable presumptions about costs and objectives, assuming that less transmit power is preferable to more,
greater distance is preferable to less, and that the bandwidth supported by
both the propagation and by the the transmitter and receiver is relatively plentiful.

A second serious practical obstacle to communication is the ''needle in a haystack'' challenge in discovering a signal originating from an extraterrestrial source. At minimum the receiver has to search for a signal over starting time and carrier frequency. If the dimensions of search are expanded beyond this, the result is increased computational load (increasing costs) and increased probability of false alarm (reducing sensitivity by necessitating a more strict criterion for a detection).
Since this is a set of challenges that must be overcome at the receiver, one might surmise
that the transmitter designer will not take this into account.
We disagree with this, as an altruistic motivation would suggest that the transmitter has an
interest in maximizing the chances that their signal will be discovered.
Making a signal more ''discoverable'' in the sense of cost as well as performance measures (like
false alarm probability) offers another wealth of information that a receiver can use to infer
characteristics of the transmitted signal.


Assumptions about resource constraints are especially influential in the issue of
power vs. bandwidth. At fundamental limits there is a tradeoff between power efficiency (the information rate divided by received average power) and the spectral efficiency (the information rate divided by the transmit signal bandwidth). 
It was observed by Jones in 1995 \citeref{196} that the bandwidth of the ISM is very large due to the large microwave window. 
We would add that our terrestrial technologies are increasingly capable in their ability to
accommodate broadband signals.
On the other hand, the transmit power levels and transmit/receive antenna gains must be very high to account for the spreading losses of large distances, and these are expected to be a major source of both operational costs and capital expenditures for the two civilizations.
More recently Fridman asserted specifically that power is surely a bigger issue than bandwidth \citeref{602}.
Concurring with this,
this paper makes the strong assumption that
power efficiency takes precedence over spectral efficiency,
which we term \emph{power-efficient design}.
Stated in more practical terms, as the information rate is increased it is assumed that the transmitter will exhaust its power budget before it exhausts its bandwidth budget. 

\textbox
	{Interstellar communication is conceptually simpler than terrestrial}
	{
The dominance of power efficiency over spectral efficiency makes interstellar communications quite distinctive from terrestrial wireless communications, which usually emphasize minimizing signal bandwidth due to the high economic value associated with the radio spectrum spectrum (principally due to the scarcity of regulatory spectral allocations).
This suggests that an interstellar communication system will be spectrally inefficient, 
or in other words consume a bandwidth that is relatively large relative to the information rate.
This is flatly contradictory to the Cyclops report, which initiated the
modern era of SETI observation programs \citeref{142}.
The Cyclops report begins with a simple (although flawed) argument that leads to the conclusion that
``we would expect interstellar contact signals to be highly monochromatic'',
and this principle has largely guided SETI observation programs since then.
This conclusion fails to recognize the principles of power efficient design, one of which is
that power-efficient signals must fundamentally be broadband.
Ironically, at the time the Cyclops report was written, power-efficient design was already fully
understood, including both fundamental limits and specific design principles to approach those limits.
The authors of Cyclops were understandably not aware of this relatively recent research,
and unfortunately the issue has never been revisited until today.
The overwhelming attention to spectrally efficient design in the commercial sector
has also been overly influential on the SETI literature. \\

Power-efficient design is a good choice for interstellar communication for other practical reasons.
Power-efficient design principles are conceptually and practically
simple when compared with known techniques for obtaining spectral efficiency.
This is a significant advantage in interstellar communication because of the
lack of coordination between transmitter and receiver,
and also as a way to minimize computational requirements.
The latter is especially significant to discovery, where computational requirements
are a limiting factor in the speed of a search.
	}

Our methodology first establishes a fundamental limit on power efficiency, and then seeks to attain that limit.
Based on this many of the characteristics of the signal design are
determined, which is reassuring since a significantly more technologically
advanced civilization would not be able to do better.
In this context, power is defined as the average signal power at the same point
that noise is measured, which is at the output of the receive antenna.
This power is determined by transmit power, transmit and receive antenna gains, and
propagation distance.
Increased power efficiency can be exploited in any of these dimensions:
lower transmit power, reduced antenna gains and collection area, 
and greater propagation distance.
All these improvements except distance come with either capital or
operational cost savings for transmitter, to receiver, or both.

Using an end-to-end model that we show is 
directly relevant to interstellar communications,
 R. Kennedy in 1969 proposed a set of relatively simple principles for power-efficient
design \citeref{}, and proved that the fundamental limit 
on power efficiency can be approached by a combination of those principles.
We apply Kennedy's principles to interstellar communication as well as
interstellar beacon design.
The result is a substantial reduction in average power required at a given
performance level.
The potential reduction in average power for information-bearing signals
is about 98\%,
and using simple practical approaches we are able to obtain a 90\% reduction.

Information-bearing signals have to operate at a minimum power level
as determined by information rate and power efficiency,
but signals designed for discovery alone have no fundamental
lower limit on average power.
Rather, the limitation is
the number of independent observations necessary to obtain a
given detection reliability.
Thus, the limit on average power is a practical one, related to
the computational resources available at the receiver.
Relative to the beacons being sought in past SETI programs,
we demonstrate average power reductions on the order of 99.9\% to 99.99\%
at a computational cost that may be considered reasonable.
This result also demonstrates a useful tradeoff for the receiver designer
between smaller antenna collection area and larger computational resources.
We also demonstrate that with, respect to discovery,
power-optmized beacons have no advantage over
power-efficient information bearing signals, and both types of signals can
be discovered using a common set of algorithms.
This suggests a receiver strategy based on 
discovery using a relatively small antenna collection area,
followed by an upgrade in collection area to extract information from
any signal that is discovered.

Given the current state of spacecraft and propulsion technology \citeref{617}, there is no possibility of our own direct experimentation with interstellar communication except with the cooperation of intelligent civilizations elsewhere in our galaxy. Fortunately astrophysical models and astronomical observations (especially from pulsar astronomy \citeref{212}) provide relevant models that can be used as a basis of design and predictions of performance.
In particular, it is a well established principle in astrophysics that over relatively short periods of time the integrity of a monochromatic wave is preserved by the ISM, with the exceptions of a frequency shift (due to Doppler) and scintillation (time variations in phase and amplitude due to scattering in the interstellar medium) \citeref{132}.
This concept is generalized here to waveforms with finite bandwidth, establishing an ''interstellar coherence hole'' (ICH) characterized by a maximum ''coherence bandwidth'' and a maximum ''coherence time''.
It is shown, with some compromise in spectral efficiency, how a transmitted signal in an interstellar communication system can be structured to take advantage of the ICH.
Such a system does not require any specific signal processing related to other ISM
impairments (such as dispersion, scattering, and source/observer motion),
in either transmitter or receiver
and during discovery or communication.
This is a necessary step to approaching fundamental limits on power
efficiency, because that avoided processing is inevitably associated with noise
enhancement, meaning an added deleterious effect due to thermal noise.
Approaching fundamental limits does require
matched filtering in the receiver, which presumes that the intra-ICH waveform can be guessed (the receiver may also search over multiple possibilities at some cost in increased false-alarms).

The fundamental limit on power efficiency is not 
affected by the coherence bandwidth or coherence time
of the ICH, and thus does not depend on carrier frequency.
It also is not affected by any impairments other than thermal noise,
including scintillation.
 It is shown that fundamental limits on power efficiency for interstellar communication are the same
 as fundamental limits on power efficiency for ICH-structured communication,
 and thus the design approach of structuring the transmit signal design around the ICH
 cannot be improved upon, either by us or by a more advanced civilization,
 as long as power efficiency takes precedence over spectral efficiency.
 
These ideas are illustrated by a concrete end-to-end design, drawing in part of
a wealth of theory, experience, and practice with terrestrial wireless
impairments that parallel the interstellar variety \citeref{574}. 
Modeling of such a system illustrates how the ICH structure
and the wealth of knowledge of the ISM based on astronomical observations
 heavily constrains both the structure and parameterization
of the received information-bearing signal, 
and thus dramatically reduces the search space in the attempted discovery of that signal,
 providing a level of implicit coordination between the transmit and receiver designs \citeref{583}.

Other authors have considered the effects of ISM impairments on signals,
although none as comprehensively as here or emphasizing the methodology of communication engineering.
Clancy was notable as the first author to suggest the combination of a broadband
(in his case a narrow pulse) signal combining with dispersion in the ISM \citeref{578}.
A couple of authors have proposed, as we do here, transmit signals specifically tailored to circumvent
effects introduced in interstellar radio propagation, including
Cordes and Sullivan \citeref{123} and Shostak \citeref{127}.
In particuar,
Shostak notes the significance of dispersion and scattering and suggests that it may be necessary to limit the per-carrier bandwidth, and suggested working around that limitation using multiple carriers, each modulated with a narrower bandwidth . 
This is called \emph{multicarrier modulation} (MCM) \citeref{612},
and is a necessary outgrowth of the ICH signal structure proposed here.
Harp et. al. propose a receiver autocorrelation technique supported by the transmit signal that can limit the
effect of ISM impairments \citeref{581}.
Morrison also asserts, as we do here, that discovery of broadband signals is feasible
by highlighting a specific example \citeref{577}.
Other authors have suggested some benefits for using wider bandwidth.
In addition to those previously mentioned \citerefthree{196}{578}{602}, 
Cohen and Charlton advocated the use of
wideband signals to overcome frequency-selective fading in improving the chances of discovery \citeref{140},
as did Cordes and Sullivan \citeref{123}.
In our own work, the ability of broadband signals to improve immunity to radio-frequency
interference was advocated \citeref{211}.


%While no similar end-to-end design of an interstellar communication system has been published,
%some earlier authors have pursued some ideas about information bearing and wider-bandwidth in interstellar communication \citerefsix{196}{578}{140}{581}{127}{602}. Of the previous papers, only \citeref{127} considered ISM propagation effects. These papers have anticipated some of the results that arise here. Observing the wide bandwidth available in the ISM, block orthogonal modulation techniques have been suggested \citeref{196}, but without consideration of the ISM. The power limitation on information rate is prominently addressed in \citeref{616}, but specific modulation techniques are not considered. Others have suggested \citereftwo{140}{578} that the frequency diversity due to wider bandwidth can improve the reliability of detection of an attention-attracting but information-free beacon.


%\chapter{Summary}
%
%We address the search of the radio spectrum for information-bearing signals of extraterrestrial origin. Such signals are necessarily of wider bandwidth than the extremely narrowband signals that have been sought over the past decades and more complex than the narrow pulses that have been given recent attention. Serious speculation as to the possibility of finding information-bearing wideband signals goes back about 15 years, but there have always been two objections that seemed to largely rule out the possibility. (a) Wideband signals are affected by dispersive and multipath phenomena in the interstellar medium (ISM), distorting such signals and thus obfuscating them. (b) The number of parameters characterizing such a signal is so large that the already-large receiver search space (at minimum angle of arrival, starting time, and carrier frequency) expands beyond reason, increasing the computational cost and the false alarm probability. Because of these objections and lack of resources, nobody has seriously pursued this option. In this paper, we completely circumvent the first objection, and largely (although not entirely) overcome the second.
%
%We follow the methodologies of communication engineering rather than experimental physics, which in itself is novel for SETI research. We pursue the conceptual design of an end-to-end interstellar communication system, incorporating the expanding understanding of the interstellar medium (ISM) arising largely from pulsar astronomy. We have also exploited the wide and varied experience with terrestrial wireless communication of the past couple decades. What we have uncovered has surprised and delighted us.
%
%In an end-to-end design, the first step is to understand the impairments in the ''channel'' (in this case, radio propagation through the ISM). The transmitter design is then undertaken, designing the waveforms, modulation, and coding of information that will be as immune to these impairments as possible. This circumvention of propagation impairments dramatically narrows the transmitter design possibilities. If the receiver designer (us in this case) follows a similar approach by first conceptually designing a transmitter, then a certain level of implicit coordination has been achieved between transmitter and receiver designs. The receiver can then search over remaining degrees of freedom for which the propagation impairments offer little insight or constraint (such as starting time and carrier frequency and signal parameterizations).
%
%We have thus examined all known channel impairments in some depth based on models appearing in the astrophysics and astronomy literature. These include ISM impairments (noise, plasma dispersion, and scattering), impairments due to the motion of transmitter and receiver (Doppler time-warping and frequency shifting), and interactions between scattering and Doppler (what astronomers call scintillation and communication engineers call fading). The breakthrough came when we realized that these impairments can actually be avoided (with one exception, scintillation), without compromises in performance, and without any impairment-specific processing required in either transmitter or receiver. 
%
%In particular, it is a well established principle that over short periods of time the integrity of a monochromatic wave is preserved by the ISM, with the exceptions of Doppler (a frequency shift due to motion) and scintillation (a random phase and amplitude shift due to propagation losses and scattering). What we realized is that this concept generalizes to waveforms with finite bandwidth, establishing a ''interstellar coherence hole'' (ICH) characterized by a maximum ''coherence bandwidth'' and a maximum ''coherence time''. Together the coherence bandwidth and time constitute the ''size'' of an ICH, and this size depends on carrier frequency, line of sight, and the exact requirements for ''coherence''. For all practical purposes, the ISM is transparent to any transmit waveform falling within a single ICH, with the exception of two Doppler consequences (a shift in carrier frequency and a time dilation) and scintillation (a random phase and amplitude that remains essentially fixed within one ICH but which varies across ICH's non-overlapping in time and frequency). Information can be transferred though the ISM without material distortion if the integrity of the ICH is maintained in the design of the transmit signal. By this we mean that each unit of data (say even a single bit) is embedded in a modulated waveform that is confined to a single ICH. A stream of data can be communicated using a multiplicity of ICH's that are non- overlapping in both time and frequency. Because no receiver processing related to ISM impairments is required, whole dimensions of search are avoided and the receiver's discovery of the signal is relatively simple.
%
%The second breakthrough came when we were able to divorce our thinking from our terrestrial experience, and consider bandwidth as unconstrained. Avoiding distortion introduced by the propagation is a strategy never used in terrestrial wireless systems, where spectrum (bandwidth) is always scarce and valuable. The wide microwave bandwidth window and the lack of competition for that window when high-gain transmit and receive antennas are employed, was pointed out by H. Jones in 1995. Using a signal structure based on the ICH is moderately inefficient in its consumption of bandwidth, but we do not believe that to be a disadvantage for interstellar communication.
%
%We then investigated how efficient such an interstellar communication system based on the ICH design principle could be. What we found is remarkable. Assuming unconstrained bandwidth, the major scarce resource is transmit power because of the large attenuation at interstellar distances. Thus, we believe the appropriate definition of ''efficiency'' is power efficiency, defined as information rate divided by the receive power required to detect that information reliably (low error probability). Remarkably, the size of an ICH is irrelevant to the resulting power efficiency. We found that the power efficiency of such a system can approach fundamental limits for any communication system (called ''channel capacity'') as established by Claude Shannon in 1948. Even very simple modulation schemes can achieve an information rate that is proportional to the received power, tracking the fundamental limit with a fixed gap that can be reduced (and conceptually even reduced to zero) by using more sophisticated modulation and coding.  There is no danger that a more advanced civilization can higher power efficiency with a more ''sophisticated'' approach, because they are subject to the same fundamental limits as we are.
%
%In practice, a transmitter designer will wish to minimize the peak power requirement, which can be achieved with a stream of ICH-based information elements sharing a single carrier frequency. There is a maximum information rate this can achieve (as limited by the coherence bandwidth), but if additional transmit power is available this rate can be doubled by sending a second stream at a different carrier frequency, tripled with a third carrier frequency, etc. This approach, called ''multicarrier modulation'', has become a standard technique in terrestrial wireless standards, and was actually suggested in the context of SETI by S. Shostak in 1995. The unconstrained bandwidth means, in practical terms, that transmit power is exhausted before bandwidth is exhausted.
%
%There is a strong (and arguably overwhelming) imperative to structure an information-bearing transmission based on the ICH. Any transmitter designer attempting to violate the ICH structure will be penalized by reduced sensitivity during a search, creating a situation in which a signal cannot be discovered in spite of its viability for conveying information. This design will also impose vastly greater computational requirements not he receiver.
%
%Scintillation, or a variation in received signal level due to the interaction of transmitter/receiver motion with interstellar scattering, cannot be avoided. This is actually fortunate for the receiver's signal discovery because there are periods when the signal strength is actually increased by constructive interference in the ISM propagation. However, during communication communication will inevitably cause periods of ''outage'', as routinely experienced in terrestrial wireless systems. We show that the outage probability should be very high (63\%) for maximum power efficiency.
%
%A remarkable advantage of structuring a signal based on the ICH is that both the transmitter and receiver can estimate with some uncertainty the size (coherence bandwidth and coherence time) of an ICH based on observable physical quantities for a give carrier frequency, line of sight, and modulation scheme, and they should arrive at similar (although not identical) conclusions. As a result, the receiver's search space is dramatically reduced in scope, because it need take into account only its and the transmitter's uncertainty. In addition, the remaining scintillation tightly constrains modulation schemes due to the resulting phase incoherence of the signal, further reducing the number of possibilities the receiver need search. A remaining issue is the choice of waveform used as the basis of the modulation. In earlier work we proposed waveform design strategies based on considerations of immunity to radio-frequency interference, but there are other possibilities to explore.
%
%In summary, we have concluded that interstellar communication is rather easy compared to the terrestrial variety, chiefly because of the generous bandwidth available. The exceptions to this simplicity are (a) the large transmit powers and high antenna gain (an issue for a transmitter designer), (b) the lack of coordination between transmitter and receiver designers, and (c) the ''needle in a haystack'' problem of discovering such a signal at the receiver. Fortunately, addressing (a) by maximizing the power efficiency without bandwidth constraint also addresses (b) by tightly constraining the structure and even detailed modulation schemes and also (c) by dramatically reducing the range of parameterization of the signals. In retrospect, we are extremely fortunate that nature has provided us with ISM impairments, because they directly assist in the coordination of transmitter and receiver designs and receiver searches without (and this is the amazing part) affecting performance or requiring transmitter or receiver processing directly related to the ISM impairments.

\chapter{Power-efficient design}
\label{sec:powerefficient}

The designer and builder of a transmitter for interstellar communication
is faced with large propagation distances and therefore large spreading loss
proportional to distance squared.
This coupled with the inevitable thermal noise accompanying the signal at the
receiver, as well as possibly other impairments, implies very large
radiated power in the direction of maximum transmit antenna gain.
This large radiated power can be obtained through a tradeoff between
two elements, both of them the source of significant cost.
One is the signal power at the antenna input, which requires
high-power electronics and significant ongoing costs of energy consumption.
The second is the antenna gain, which is related to antenna size
as well as other characteristics.
The cost of both building and operating a transmitter will be dominated by
this radiated power requirement.
It is therefore reasonable to assume that the transmitter designer will be
motivated to reduce the transmitted power to the lowest levels possible
consistent with the desire for reliable extraction of information from the
received signal.
This is called \emph{power-efficient design}, which is the subject of this report.

The receiver designer experiences related issues.
Reliably discovering the signal in the first place, or later extracting
information from it,
dictates a minimum power level in the signal at receive antenna output, 
that power related to the level of thermal noise at that same point.
The receiver designer can exploit a power-efficient signal
design by using a smaller receive antenna gain and collection area,
also saving costs.
However, a significant cost to the receiver is the large computational
resources required at the discovery stage due to the ''needle in a
haystack'' challenge of searching over a large parameter space.
Thus, the computational requirements imposed by the discovery
of a power-efficient signal is also an issue to the receiver designer.

One of our conclusions is that signals can be reliably discovered at
very lower power levels.
This raises two possibilities that need to be explored.
One is the possibility of using a dual-antenna approach, in which
a smaller antenna collection area is used for discovery and a larger
collection area is used for information extraction.
This would open up a two-stage investment strategy, in which
the larger collection area was constructed only when its need
was justified by the discovery of a candidate signal.
Another is designing a signal optimized for discovery at low
power levels without the constraint that it embed information.
This latter option is called a \emph{interstellar beacon}, which
is like a lighthouse in that it is intended to attract attention without
conveying additional information.
We will find that the beacon is not a compelling idea, since
information bearing signals at similar power levels can be discovered
as easily and reliably.

The major competitor for power-efficient design is spectrally efficient design,
where the major design objective is to minimize the bandwidth
or range of frequencies occupied by the transmit signal.
In fact, we will demonstrate a fundamental tradeoff between power efficiency
and spectral efficiency,
implying that power efficient designs are spectrally inefficient and vice versa.
Present and past SETI observations at radio frequencies have been
strongly influenced by terrestrial communication
(with one notable exception \citeref{196}).
Terrestrial is usually subject to fixed regulatory spectral allocation,
and economic forces favor achieving the highest information rates within the
assigned bandwidth.
Terrestrial thus generally follow
design principles that emphasize spectral efficiency.
However, interstellar communication is generally not subject to
the same economic forces that favor smaller bandwidth, and the
microwave window available for such communication is quite broad.
Further, power limitations will likely limit information rates
to be relatively low, and the resulting bandwidth requirements are not technologically 
challenging.

Spectrally efficient design emphasizes conveying information
as much as possible through the
\emph{amplitude} of a signal because this does not consume
extra bandwidth.
Spectral efficiency is also gained by making maximum utilization of time,
implying that a signal will be transmitted continually.
In contrast, power-efficient design typically limits the signal amplitude to
two levels, the minimum possible.
To reduce average power, power-efficient design emphasizes two techniques.
One is to convey information through the \emph{location} of the signal
in time and/or frequency because, with respect to energy consumption,
location comes for free.
The second is to
limit the \emph{duty cycle} of the signal, which is the on-time to off-time.
Limiting the duty cycle reduces the average power, although it does not
reduce peak power.
Power-efficient design thus makes poor utilization of time, resulting
in excess use of bandwidth.
As a result of this, power-efficient signals are intermittent,
implying that they cannot be counted on to be present in every observation
and their persistence cannot be counted on.
This simple comparison makes it obvious that power efficiency takes us in a very
different design direction from spectral efficiency.
Especially significant for interstellar communication is the challenge of
initial discovery of a signal, whether it be information-bearing or a beacon.
Algorithms chosen for the discovery of power-efficient signals will not work well for
spectrally-efficient signals, and vice versa.

\section{Basic building block: Energy bundles}
\label{eq:energybundles}

Power-efficient design uses energy bundles as a basic building block.
A bundle of energy is transmitted, and the receiver detects this bundle
by observing its excess energy over and above the noise.
The ''carrier'' for an energy bundle is a waveform $\sqrt{\energy_h} \, h(t)$,
which is assumed to have some time duration $T$ and some bandwidth $B$.
The waveform $h (t)$ is assumed to have unit energy, defined as
\begin{equation}
\int_{0}^{T} | h(t) |^2 \, dt = 1 \,,
\end{equation}
so that the energy is $\energy_h$.
The number of \emph{degrees of freedom} of $h(t)$ is defined as
\begin{equation}
K = B \, T \,,
\end{equation}
must satisfy $K \ge 1$ as discussed further in Chapter \ref{sec:fundamental}.

In the presence of thermal noise, the best method for detecting the excess
energy represented by $h(t)$ is
a filter matched to $h(t)$.
This \emph{matched filter} MF is illustrated in Figure \ref{fig:mfillustrate} and discussed in detail in Chapter \ref{sec:detection}.
Matched filtering is essential to approaching the fundamental limit on power efficiency,
but it is significant that in order to apply an MF the receiver must know (or be able to guess)
the waveform chosen by the transmitter.
Alternatively, as part of a discovery search strategy the receiver
(at the expense of additional computation) can trial more than one waveform $h(t)$.

\incfig
	{mfillustrate}
	{1}
	{An illustration of a bundle of energy as it appears in OOK, FSK, or PPM.
	It consists of a waveform $h(t)$ shown on the left, which can be simple
	or complicated.
	The remainder of the
	figure illustrates how this bundle of energy can be detected using a matched
	filter, which consists of a convolution
	(represented by $\convolve$)
	 with a time-reversed and conjugated version $\cc h (-t)$ (illustrated in the middle),
	with the result equal to the autocorrelation of $h(t)$ (shown on the right). 
	This autocorrelation at zero lag equals the total energy of $h(t)$.
	Various types of $h(t)$ can be used as the basis for an energy bundle, but arguably 
	the most useful are the segment of a sinusoid (on top) and the segment of
	a noise-like signal (shown on the bottom).}


Impairments introduced in the interstellar medium (ISM) 
and due to the relative motion of the transmitter and receiver can have a
deleterious effect on the detection of energy bundles.
This can take the form of smearing the bundle out in time or in frequency.
However, by placing an upper bound on both $T \le T_c$ and $B \le B_c$ these
effects can be rendered negligible, as discused in Chapter \ref{sec:incoherence}.
The largest values $T_c$ and $B_c$ are called respectively the
\emph{coherence time} and \emph{coherence bandwidth} of the ISM,
and a waveform that meets this constrain is said to fall in an
\emph{interstellar coherence hole} (ICH).
Fortunately it is shown in Chapter \ref{sec:incoherence} that for the ISM and motion impairments
$B_{c} \, T_{c} \gg 1$ so there is no
difficulty choosing an $h(t)$ that satisfies this constraint.
The ICH exists, a fact that renders power-efficient interstellar communication feasible.
Nature has been kind to us, as well as civilizations that might wish to communication with us.

It is significant that the shape of the waveform $h(t)$ does not matter,
as long as it conforms to the constraints $T \le T_c$ and $B \le B_c$.
Two cases that are particularly interested illustrated in Figure \ref{fig:mfillustrate}
are a piece of a sinusoid and a noise-like-waveform.
The considerations that enter the choice of $h(t)$ are discussed further
in Chapter \ref{sec:detection}.
The immunity to noise is not impacted by $h(t)$, but the
immunity to radio-frequency interference (RFI) that may be present at
the receiver is the major consideration.
In particular, the sinusoid (although conceptually simple) is highly susceptible
to interference, where a properly designed noise-like waveform is maximally immune
to interference \citeref{211}.
Another conceptually simple choice is a narrow pulse, and this option has also been
pursued in SETI searches \citereftwo{605}{631}.
However, the narrow pulse violates the coherence bandwidth constraint and thus is
not of interest in power-efficient design.

Within the ICH there are two impairments of note remaining,
impairments that cannot be rendered negligible by restricting $T$ and $B$.
These are additive noise (of thermal origin) and multiplicative
noise (due to scintillation), and they are discussed in Chapter \ref{sec:fundamental}.
Scintillation manifests itself as a variation in phase and amplitude of
the signal at the output of the MF from one ICH to another.
Scintillation is called \emph{fading} in communications, and is a common
phenomenon in radio communications in the presence of motion.

An energy estimate is generated by taking the magnitude-squared
of the MF output.
This energy estimate is not sensitive to the phase of scintillation
nor to the unknown phase of the carrier.
This estimate is influenced by the noise and by the scintillation.


\section{Design of power-efficient information-bearing signals}
\label{sec:illustrations}

We have asserted that there is a tradeoff between power and bandwidth.
This tradeoff will now be illustrated by some concrete examples.

\subsection{On-off keying}

A simple baseline case, which is neither power-efficient nor spectrally efficient,
is the on-off keying (OOK) as illustrated in Figure \ref{fig:ookIllustrate}.
In OOK the presence or absence of a bundle of energy is used to represent
one bit of information.
In the $k$th time slot of width $T$, the signal is 
$A_{k} \cdot \sqrt{\energy_h}\, h(t - k T)$
where $A_{k} = 0$ or $A_{k} = 1$
depending on the information bit.
The spectral efficiency of OOK can be improved
as illustrated in Figure \ref{fig:mmkIllustrate}.
In this multilevel keying,
$\log_2 M$ bits of information is represented
at each time by using $M$ different levels of energy
(the case shown is $M = 8$, corresponding to $\log_2 8 = 3$ bits).
This is spectrally efficient because each bundle of energy consumes the
same time and bandwidth as OOK, but conveys more information.
However, this is inefficient in its use of power because the
average power is increased by a factor proportional to $M^2$
in order to maintain the same noise immunity as OOK,
but the information rate is increased by only a factor of $\log_2 M$.
	
\incfig
	{ookIllustrate}
	{1}
	{In on-off keying (OOK), in each time slot
	the presence or absence of a bundle of energy represents
	a single bit of information.}
	
\incfig
	{mmkIllustrate}
	{1}
	{Spectrally efficient design is illustrated by multilevel keying.
	At each time slot, a
	bundle of energy assumes one of $M = 8$ values (including zero),
	and thus represents $\log_2 M = 3$ bits of information. }

\subsection{M-ary frequency-shift keying}

The power efficiency can be improved relative to OOK by
M-ary frequency-shift keying (FSK),
which is illustrated in Figure \ref{fig:fskIllustrate}.
In this approach,  $\log M$ bits of information
is represented in each time slot by a single bundle of energy at 
 at one of $M$ different frequencies
(the case shown is $M = 64$, corresponding to $\log_2 64 = 8$ bits of information).
The transmitted signal takes the form $\sqrt{\energy_h} \, h(t) \, e^{\,i\, 2 \pi A_{k} f_{0} t}$,
where $A_{k} \in \{ 0, 1, \dots \, M-1 \}$
and $f_{0}$ is the frequency spacing, typically equal to $f_{0} = B$
so that the energy bundle locations do not overlap.
Compared to OOK, this requires $M$ times as much bandwidth,
so it is spectrally less efficient.
However, it is more power-efficient than OOK because the 
average power is the same, but each time slot communicates
 $\log_2 M$ times as much information.
One general principle of power-efficient design is to convey 
information by the \emph{location}
of a bundle of energy rather than the \emph{amount} of energy.
While consuming extra bandwidth, this conserves energy.

\incfig
	{fskIllustrate}
	{1}
	{Power-efficient design is illustrated by M-ary FSK.
	In each time slot, a bundles of energy assumes one of $M=64$ different frequencies,
	representing $\log_{2} M = 8$ bits of information.}

\subsection{M-ary pulse-position modulation}

While M-ary FSK represents information by the the location of
energy bundles in frequency, an alternative is
M-ary \emph{pulse-position modulation} (PPM), as illustrated in
Figure \ref{fig:ppmIllustrate}.
In PPM information is conveyed by the position of an energy bundle in time.
The transmitted signal is of the form $\sqrt{\energy_h} \, h(t - A_{k}/ M T)$,
where $A_{k} \in \{ 0, 1, \dots \, M-1 \}$.
Typically the bandwidth is expanded due to the shorter time duration of
each energy bundle. 

There is one substantive difference between FSK and PPM.
The FSK signal is transmitting energy continuously,
whereas PPM is intermittent.
For FSK the average and peak transmitted powers are the same, but in PPM
the peak transmitted power is higher than the average.
In PPM the same energy is transmitted in less time,
so the peak power is $M$ times larger than FSK.
While the cost of energy consumption will be comparable,
there is a significant difference in the implementation of the
power circuitry in the transmitter, and this may affect the capital cost.
The goal of power-efficient design is to reduce the average power,
but it should be kept in mind that some approaches can have the
side effect of increasing the peak power as illustrated by PPM.

\incfig
	{ppmIllustrate}
	{1}
	{
	Power-efficient design is also illustrated by
	pulse-position modulation (PPM).
	Time is divided into codewords with $M=8$ positions each, and $\log_{2} M = 3$ bits
	of information are conveyed by the location of a single pulse within
	each codeword.
	}

\subsection{Reducing the average power}

For either FSK or PPM the information rate (in bits per second) is
$\rate = \log_2 M /T$.
If an energy bundle uses a waveform $h(t)$ that spreads the energy
uniformly over $[0,T]$, the power during an energy bundle is
$\energy_h / T$.
This equals the average power $\power$.
The power efficiency $\powere$ is defined as
\begin{equation}
\label{eq:power}
\powere = \frac{\rate}{ \power} = \frac{\log_2 M}{\energy_h}
\end{equation}
The reliability with which an energy bundle can be detected in the presence
of noise depends on the value of $\energy_h$, so generally this
parameter should be held fixed.
From \eqref{eq:power} the power efficiency is
not affected by $T$, implying that $\power \propto \rate$.
Thus, reducing $\power$ also reduces $\rate$ by and equivalent factor.
As we will see, this is a straightforward tradeoff that is 
characteristic of power-efficient design.

Now suppose the power budget does not allow the use of FSK or PPM as
just described.
The value of $\power$ is simply too large.
An easy way to reduce $\power$ is to increase the value of $T$.
The fixed energy $\energy_h$ is spread over a greater time,
so the power is reduced.
However, there is a limit $T \le T_c$ imposed by the ICH, so $\power$
cannot be reduced indefinitely in this manner.
Specifically the constraints are
\begin{equation}
\power \ge \frac{\energy_{h}}{T_{c}}
\ \ \ \ \text{and} \ \ \ \  \rate \ge \frac{\log_{2} M}{T_{c}} \,.
\end{equation}
However, once $T = T_c$ is reached, $\power$ can be reduced
further by introducing a \emph{duty cycle} $0 < \delta <1$,
which equals the fraction of the time that the signal is transmitted.
By putting a minimum gap between energy bundles, $\delta < 1$ can be achieved.
A duty cycle of $\delta = 1/4$ is illustrated by Figure \ref{fig:fskIllustrateDutyCycle}.

\incfig
	{fskIllustrateDutyCycle}
	{1}
	{
	Figure \ref{fig:fskIllustrate} is repeated with a duty cycle $\delta = 1/4$.
	While retaining the same power efficiency $\powere$, both the
	average power $\power$ and information rate $\rate$ are reduced by $\delta$.
	}

For a duty cycle $\delta$, all else being equal $\power$ will be
reduced by $\delta$, and $\rate$ will also be reduced by $\delta$.
Thus, using the duty cycle trick does not affect the power efficiency $\powere$.
Reducing the average power by reducing the duty cycle is another
common technique in power-efficient design to reduce the average power.
Note, however, that whoever $\delta < 1$ the peak power must be higher than the average
power.
The duty cycle approach would never be used if spectral efficiency is a high priority,
because it makes inefficient use of time and hence of bandwidth.

\subsection{Exploiting larger average power}

Now suppose it is desired to increase the information rate $\rate$ rather than reduce it.
An easy way to do this is reduce $T$, but eventually (maybe even initially) $B$
will inevitably increase as $T$ decreases due to the constraint $B \, T \ge 1$.
Then as $T$ decreases further $B$ will reach the limit 
$B \le B_{c}$, so $h(t)$ can no longer fit in the coherence hole.
The smallest feasible $T$ is determined by the constraints $B \, T \ge 1$ and
$B \le B_{c}$, implying that the maximum power and information rate
that are feasible on a single carrier M-ary FSK signal is
\begin{equation}
\power \le \energy_{h} \, B_{c}
\ \ \ \ \text{and} \ \ \ \  \rate \le B_{c} \, \log_{2} M
\end{equation}
When this constraint is reached, there is an alternative path to larger $\rate$, which is to transmit
a parallel sequence of energy bundles at another carrier frequency spaced far enough
apart that there is no frequency overlap.
This is called \emph{multicarrier modulation} MCM \citeref{612}, and is illustrated in Figure \ref{fig:ppmIllustrateMCM}.
In 1995 Shostak anticipated the importance of
MCM, motivated (as here) by its immunity to ISM impairments \citeref{127}.
MCM increases $\rate$ with a proportional increase in $\power$, so the power efficiency is unchanged.

\incfig
	{ppmIllustrateMCM}
	{1}
	{Figure \ref{fig:ppmIllustrate} is repeated, with PPM signals transmitted on three different
	carrier frequencies.
	This is an
	illustration of multicarrier modulation (MCM), a way to increase
	$\power$ and information rate $\rate$ proportionally by transmitting parallel sequences
	of energy bundles on different frequencies.
	}

%The rate $F$ (and hence $\rate$) for the single-carrier approach of Figure \ref{fig:IUstructure}(b) is constrained by the requirement that each IU fit within an ICH,
%\begin{equation}
%\label{eq:constantpowerbounds}
%\frac{1}{T_{c}} \le F = \frac{1}{T_{0}} \le B_{c} = \frac{K_c}{T_c} \,.
%\end{equation}
%The lower bound follows from $T_0 \le T_c$,
%and the upper bound follows from
%$B_0 \le B_c$ and $B_0 T_0 \ge 1$.
%For a large $K_c$, \eqref{eq:constantpowerbounds} 
%gives us a considerable range to adjust $F$ and $\rate$,
%but it does constrain the possibilities.
%There are, however, easy ways to operate outside these bounds.
%To get lower rates, the IU's can be spread out in time as shown in Figure \ref{fig:IUstructure}(c),
%with the side effect that the peak power becomes larger than the average power.
%To get higher rates, $M$ parallel single-carrier sequences can be transmitted at
%different carrier frequencies as shown in Figure \ref{fig:IUstructure}(d).
%This \emph{multicarrier modulation} (MCM) \citeref{612},
%and is a natural outgrowth of an ICH-structured transmit signal.
%In 1995 Shostak anticipated the importance of
%multicarrier, motivated (as here) by its immunity to ISM impairments \citeref{127}.

\textbox
	{Multicarrier modulation}
	{
Multicarrier modulation (MCM) is widely used because it is recognized to have a number of advantages.
Immunity to dispersion is only one. 
If the distinct carrier frequencies deliberately violate frequency coherence,
the scintillation experienced by
different carriers will be unrelated to one another (this is called \emph{frequency-selective fading}).
This observation can be used to improve the reliability for communication as well as discovery,
for example by creating data redundancy across different carriers.
The relative powers allocated to different carriers can be adjusted
to accommodate frequency-dependent phenomena such as a planet's
larger atmospheric noise due to water vapor (concentrated at $f_c \gg 15$ GHz).
The power allocated to one (and only one) subcarrier can be artificially increased
to make discovery easier with only a small power penalty overall.
MCM also lends itself to parallelism in transmitter implementation.
For example, any collection of subcarrier signals can be transmitted independently
of the others using separate
RF electronics and antennas, each optimized for its own carrier frequency.
A transmitter designer on a limited budget can 
expand total information rate over time by increasing $M$, 
with a capital cost that scales no faster than $\rate$.
As discussed in Chapter \ref{sec:discovery}, MCM can also improve
the discovery sensitivity.
Both transmit and receive implementations lend themselves to
joint subcarrier manipulation at baseband using discrete Fourier
transform techniques \citeref{612}.

For many of the same motivations, MCM is widely used in terrestrial wireless communications.
The first commercial application (The Collins Radio Kineplex) in 1957
\citeref{623} exploited multiple carriers to counter selective fading in military communications.
Because terrestrial bandwidth is a scarce resource, terrestrial applications use a clever form of MCM in which the subcarrier signals have a 50\% overlap in frequency without interference (this idea was patented in 1970 \citeref{611} and gained traction in the 1990's \citeref{612}). A specific realization called orthogonal frequency-division modulation (OFDM) \citeref{613} appears in wireless communication standards such as ''wireless fidelity'' (WiFi), ''worldwide interoperability for microwave access'' (WiMAX), and the 4G digital cellular standard ''long term evolution'' (LTE). 
These standards typically combine MCM with spread spectrum \citereftwo{615}{621} for RFI mitigation.
These numerous applications give us some additional confidence in this as an approach for
interstellar communication, as well as provides relevant design experience.
	}


\section{Power efficiency vs. spectral efficiency}
\label{sec:tradeoff}

The last section described an approach to the design of
power-efficient information-bearing signals.
One notable feature of the design approach is that the restriction of
an energy bundle waveform $h(t)$ to the ICH implies that
no signal processing related to ISM and motion impairments is
required in either transmitter or receiver,
with the exceptions of noise and scintillation.
Another notable characteristic of FSK, PPM,
reducing average power using a duty cycle, and
increasing average power using multiple carriers
is that they all lead to the same conclusion.
The power efficiency $\powere$ defined in \eqref{eq:power}
remains constant as the $\power$ and $\rate$
are changed, as long as $M$ remains fixed.
This implies that $\power \propto \rate$.
The question naturally arises whether this linear tradeoff between rate and power is the best that can be achieved.
We will now show that
this proportionality is characteristic
of the fundamental limit on power efficiency, although there remains the
issue of the constant of proportionality.

\textbox
	{A word about terminology and nomenclature}
	{
This paper deals with both physical models and communications.
Generally we use a nomenclature consistent with the astrophysics literature
when dealing with physical models, and a notation consistent with the communications
engineering literature when dealing with communications.
For example, the dispersion measure is $\dm$, but the $K$-factor for a Rician
fading model is $\kappa$.
A similar division is used for terminology, for example in dealing with
scintillation and fading (which are similar phenomena with different
names in astrophysics and communications).

Generally deterministic signals are denoted by a lower-case letter and
random signals by upper case (like $z(t)$ vs $Z(t)$).
Physical constants are usually denoted by a Greek letter, unless the
convention in the physics or communications literature is different
(for example the dispersion measure $\dm$ or noise power spectral density $N_{0}$).
The probability of an event $A$ is denoted by $\prob{A}$.
For a random variable $X$, the $f_{X} (x)$ is the probability density function
and $F_{X} (x)$ is the cumulative distribution function,  so the two are related by
\begin{equation*}
F_{X} (x) = \prob{X \le x} = \int_{- \infty}^{x} f_{X} (u) \, du 
\ \ \ \ \text{and} \ \ \ \ 
f_{X} (x) = \frac{d}{d x} F_{X} (x)
\,.
\end{equation*}
The averaging or expectation operator is denoted as $\expec{\cdot}$
(whereas in the physics literature the alternative notation $< \cdot > \equiv \expec{\cdot}$
is often used).
For example
\begin{equation*}
\expec{X^{2}} = \int x^{2} \, f_{X} (x) \, dx \,.
\end{equation*}
The variance of a random variable $X$ is denoted as
$\var{X} = \expec{X^{2}} - ( \expec{X} )^{2}$,
and the standard deviation of $X$ is $\sqrt{\var{X}}$.
	}

%The previous examples illustrate how signals can be designed to prioritize
%power efficiency or spectral efficiency, each at the expense of the other.
%The question arises as to whether this is coincidence, or a fundamental
%property of information-bearing signals.
%In fact this tradeoff cannot be avoided,
%as we now show by considering the fundamental limits to communication.

For information-bearing signals, 
the power efficiency was defined in \eqref{eq:power}.
Power efficiency has the units of bits per Joule.
In place of $\powere$ it is often useful to work with its reciprocal,
\begin{equation}
\label{eq:energybit}
\energybit = \frac{1}{\powere} \,,
\end{equation}
which is the received signal energy per information bit.
Two schemes requiring the same $\energybit$ have the same $\powere$, and vice versa.
A similar definition applies to spectral efficiency,
\begin{equation}
\spectrale = \frac{\rate}{B_{\text{total}}}
\end{equation}
where $B_{\text{total}}$ is the total bandwidth of the information-bearing signal.
$\spectrale$ and has the units of bits per sec per Hz, or simply bits.
The spectral efficiency is determined by the transmitter through its choice
of a signal structure and parameterization.

We now show that there is a fundamental tradeoff between $\powere$
and $\spectrale$ for a particular channel model that captures one of the
two unavoidable impairments in interstellar communication,
which is noise of thermal origin.
The incompleteness of this model is addressed in Chapter \ref{sec:channelmodel},
where this fundamental limit in the presence of both noise and scintillation is addressed.
The striking conclusion there is that scintillation has no effect on the fundamental limit
on power efficiency.

\subsection{Additive white Gaussian noise}

The end-to-end path for the transmitted signal
as it arrives at the receiver is called a \emph{communications channel}.
It is beneficial to use the simplest model for the channel that captures the
essential \emph{impairments}, 
which are characteristics of the channel that limit the ability to communicate reliably.
The impairments relevant to interstellar communication are covered in
some detail in Chapters \ref{sec:channelmodel} and \ref{sec:incoherence}.
We find that the most important of these is
additive noise of thermal origin that originates from black body radiation,
background radiation, and the finite temperature of the receiver.
This is usually modeled as 
\begin{equation}
\label{eq:awgnchannel}
Y(t) = X (t) + N(t) \,,
\end{equation}
where $Y(t)$ is the received signal corrupted by noise, 
$X(t)$ is the portion of $Y(t)$ attributable to the transmitter, and
$N(t)$ is  additive white Gaussian noise (AWGN) with power spectral density $N_{0}$.
For purposes of this chapter, this will be the channel model considered.

\subsection{Channel capacity}

 C. Shannon developed the concept of \emph{channel capacity} in 1948,
which is a mathematically provable upper bound on the information
rate $\rate$ that can be achieved reliably for a given channel model \citeref{164}.
More modern developments of Shannon's results are found in \citereftwo{171}{172}.
Although channel capacity is a general concept,
for the AWGN channel of \eqref{eq:awgnchannel} the result is
particularly simple to derive, and
this is the first case that Shannon considered.
Unless the average power of $X(t)$ is constrained, the capacity becomes
infinite, so it is assumed that $\expec{X^{2} (t)} \le \power$.
It is important to note that the average signal power $\power$ is referenced
to the same point as the noise in \eqref{eq:awgnchannel}, which is usually
chosen to be at the receive antenna output and before baseband signal processing.
The transmitter, of course, has to adjust the transmit power to achieve
received power $\power$, taking into account 
also the transmit and receive antenna gains.
In contrast, it is not necessary to constrain the signal bandwidth $B_{t}$.

Shannon's famous formula is
\begin{equation}
\label{eq:capacity}
\rate \le  B_{t} \, \log_{\,2} \left( 1 + \frac{\power}{N_{0} \, B_{t}} \right) \text{   bits/sec}
%\ \ \overset{B \to \infty}{\longrightarrow} \ \ 
%\capacityinf = \frac{1}{\log_{\,e} 2} \, \frac{\power}{N_0}
\,.
\end{equation}
His proof of this result comes in two parts.
First, when $\rate$ satisfies this bound,
there exist channel codes such that the probability of error in
communication $\pe$ can be made arbitrary small.
Hence reliable communication is possible.
The idea of a channel code will be described shortly.
Second, when the bound of \eqref{eq:capacity} is violated,
$\pe$ is necessary bounded away from zero, or reliable communication
is not possible.


%Shannon's channel capacity formula \citereftwo{171}{172} provides a theoretical upper bound
%on the rate of reliable information transfer for the channel of \eqref{eq:awgnchannel}.\footnote{
%$\capacity$ is the highest rate at which it is possible to achieve
%arbitrarily small error probability $\pe$.
%Conversely, for $\rate > \capacity$,  it can be shown that $\pe$ is bounded
%away from zero.
%Thus, it may be possible to communicate at higher rates than $\capacity$,
%but it is impossible to communicate \emph{reliably} at these higher rates.
%The derivation of this bound assumes that information is transmitted over
%infinite time, and both the delay introduced from input information
%to decoded information and the complexity of the receiver are unconstrained.
%}
%The \emph{capacity} is defined as the largest achievable information rate
%that can be communicated reliably,
%\begin{equation}
%\label{eq:capacity}
%\capacity = B \, \log_{\,2} \left( 1 + \frac{\power}{N_{0} \, B} \right) \text{   bits/sec}
%%\ \ \overset{B \to \infty}{\longrightarrow} \ \ 
%%\capacityinf = \frac{1}{\log_{\,e} 2} \, \frac{\power}{N_0}
%\,.
%\end{equation}
%This expresses a tradeoff between the maximum possible rate $\rate \le \capacity$,
%the received power $\power$, and the bandwidth $B$.

\textbox
	{Fundamental limits were a revelation}
		{
This idea that communication was subject to fundamental physical limits
was a revelation when Shannon introduced it in 1948.
Prior to that time, it was expected that more and more complicated and sophisticated
techniques could achieve higher and higher information rates.
As it turns out there is a hard limit on the information rate that can be achieved.
Also, it was assumed that perfectly reliable communication with $\pe \to 0$
would be impossible at any rate due to the deleterious effect of noise.
In fact, it is theoretically possible to achieve arbitrarily low $\pe$ for any information
rate, as long as that rate is less than capacity.

The existence of a fundamental limit is a great asset for interstellar communication.
This limit alerts us to the fact that relative to the types of signals typically considered
for interstellar communication to date,
a substantial improvement in power efficiency is feasible.
The fundamental limit also constrains what any civilization can achieve,
no matter how advanced.
If we can achieve a practical design that approaches the fundamental
limit, we know that no other civilization can do significantly better.
We also find that a design that approaches the fundamental limit becomes
strongly constrained, reducing design freedom and 
providing specific guidance on signal structure to both transmitter and receiver.
Thus, the fundamental limit proves valuable as a form of implicit coordination
between transmitter and receiver \citeref{583}.
	}

\subsection{Fundamental limit on power efficiency}
\label{sec:pelimit}

The bound of \eqref{eq:capacity} can be algebraically manipulated
to create an equivalent bound on power efficiency $\powere$
expressed in terms of spectral efficiency $\spectrale$,
\begin{equation}
\label{eq:powerVsSpectral}
\powere \le \powerenoise \cdot g( \spectrale )
\end{equation}
where the two factors are
\begin{equation}
\label{eq:powerenoise}
\powerenoise =  \frac{\log_{2} e}{N_{0}}
\ \ \ \ \text{and} \ \ \ \ \
g( x ) =  \frac{x \, \log_{\,e} 2}{2^{\,x}-1} \,.
\end{equation}
The factor $ g( \spectrale )$ represents the fundamental reduction in $\powere$
that must be sacrificed to achieve a given $\spectrale$, and the region represented by
\eqref{eq:powerVsSpectral} is plotted in Figure \ref{fig:powerVsSpectral}.

Figure \ref{fig:powerVsSpectral} harbors several interesting insights.
Substantial increases in power efficiency $\powere$ are feasible only
by allowing spectral efficiency $\spectrale$ to get small, or equivalently
for a given information $\rate$ reducing power $\power$ dictates increasing bandwidth $B_{t}$.
There is, however, a global maximum $\powerenoise$ can can be achieved.
This is the fundamental limit to which we should aspire in designing our interstellar
communication system.
Another insight is that spectral efficiency $\spectrale$ can be increased
\emph{without bound}, but only at the expense of reducing $\powere$.
One conclusion for interstellar communication is that relatively poor spectral efficiency
is an expected and fundamental consequence of seeking high power efficiency.

\incfig
	{powerVsSpectral}
	{1}
	{In the presence of white Gaussian noise (characteristic of natural
	sources of thermal noise), Shannon proved that reliable
	communication is possible within the shaded region of 
	$\{ \powere/\powerenoise , \, \spectrale \}$ and not possible outside that region.
	The horizontal axis is the spectral efficiency $\spectrale$ and the
	vertical axis the power efficiency $\powere$ normalized by the global
	maximum possible power efficiency $\powerenoise$.
	Commercial terrestrial wireless systems invariably operate in the
	spectrally efficient regime where $\spectrale$ is favored at the expense of $\powere$.
	Interstellar communication should operate in the power-efficient regime where
	$\powere$ is favored at the expense of of $\spectrale$.
	As a result, we would expect an interstellar communication system to use
	a relatively wide bandwidth relative to the information rate.
	 The global maximum power efficiency $\powerenoise$ can only be achieved
	 as $\spectrale \to 0$, or equivalently the total signal bandwidth $B_{\text{total}}$ is unconstrained.}

Terrestrial communication usually emphasizes high spectral efficiency $\spectrale$ 
due to the high commercial value attached to spectrum allocations.
Thus, terrestrial designs typically operate in the lower right region
of Figure \ref{fig:powerVsSpectral}, where $\spectrale$ is high and $\powere$ is low.
Interstellar communication should operate in the upper left region, where $\powere$ is high
but $\spectrale$ is low.
Thus, an interstellar communication signal can be expected to consume relatively
wide bandwidths relative to the information rate.
This reflects a significant difference in objectives between interstellar and
terrestrial communication, as well as a significant distinction in practical
design techniques.

The global limit on power efficiency from  \eqref{eq:powerenoise} is
\begin{equation}
\label{eq:poweremaxAWGN}
\powere \le \powerenoise = \frac{\log_{2} e}{N_{0}} \,.
\end{equation}
At this fundamental limit,
$\rate \propto \power$, or every increase in $\rate$ demands a proportional
increase in $\power$.
This is exactly the same tradeoff that was seen in the practical designs
(M-ary FSK and PPM) in Section \ref{sec:illustrations}, although we expect the constant
of proportionality to be smaller than the fundamental limit.
Expressed in terms of the energy per bit as defined in \eqref{eq:energybit},
\eqref{eq:poweremaxAWGN} becomes
\begin{equation}
\label{eq:ecrawgn}
\frac{\energybit}{N_0} \ge \log_e 2 = 0.69
\ \ \ ( - 1.6 \ \text{dB}) \,.
\end{equation}
Thus, there exists a global minimum
energy that is required to convey each information bit reliably
in the presence of AWGN.

A different interpretation follows from consideration of the \emph{signal-to-noise ratio}, or SNR.
An SNR, in contrast to an energy contrast ratio, is a ratio of signal power to noise power.
The SNR of interest right now is referenced to the input to the MF, where the SNR is
\begin{equation}
\snrin = \frac{\power}{N_{0} B_{t}} \,,
\end{equation}
since $\power$ is the received power
$N_{0} B_{t}$ is the total input noise in bandwidth $B_{t}$.
Assume $\snrin \approx 0$ since $B_{t}$ is very large, in which case
 \eqref{eq:capacity} can be expanded in a Taylor series as
 \begin{equation}
 \label{eq:capproxBlarge}
\rate \le \frac{\power \, \log_{2} e}{N_{0}} \cdot
\left( 1 - \frac{\snrin}{2} + \frac{\snrin^{\,2}}{3} - \dots \right) 
\underset{\snrin \to 0}{\longrightarrow}  
\frac{\power \, \log_{2} e}{N_{0}} 
\,.
\end{equation}
Thus, another characteristic of power-efficient communication is
a very small $\snrin$ because of a large $B_{t}$,
and in this special case \eqref{eq:capacity} simplifies
to \eqref{eq:capproxBlarge}, in which $\rate \propto \power$ at the fundamental limit.

This last interpretation emphasizes that to approach the fundamental limit on
power efficiency $\powere$ the bandwidth $B_{t}$ must be
\emph{unconstrained}.
It is important to note that unconstrained bandwidth is different than \emph{unlimited} bandwidth, because
the bandwidth actually utilized in any practical design
(such as those in Section \ref{sec:illustrations} will always be finite.
Unconstrained bandwidth merely assumes
that bandwidth is not a consideration in the transmitter's signal design.

\subsection{Wake-up call from the fundamental limit}

To gain some perspective on significance of \eqref{eq:ecrawgn}, it is
useful to relate it to a simple but concrete modulation scheme, OOK as illustrated
in Figure \ref{fig:ookIllustrate}.
Recall that OOK is a simple but ''middle of the road'' option,
one that is neither particularly energy efficient nor power efficient.
It is characteristic of the type of signals that have been the subject of
SETI discovery searches over the past five decades.
OOK is analyzed in Chapter \ref{sec:infosignals}, where its probability of error
$\pe$ is determined as a function of $\ecrb$, and the result in
plotted in Figure \ref{fig:gapFundamental}.
As expected, $\pe$ decreases rapidly as the signal energy $\energybit$
increases in relation to the noise energy $N_0$.
Also shown, as a vertical line, is the fundamental limit
on $\ecrb$ at minus 1.6 dB, as given by \eqref{eq:ecrawgn}.
This plot reveals a substantial gap between OOK and the fundamental
limit.
That gap depends on the reliability that we demand, but at a moderate
reliability of $\pe = 10^{-4}$ it is 17.6 dB.
This reveals that a substantial improvement
in power efficiency relative to OOK is possible on the AWGN channel.
Specifically, for a given information rate $\rate$, there is an opportunity to reduce
the transmit and receiver power by a factor of 50, or a 98\% reduction in power.
In Chapter \ref{sec:infosignals} we will find that this gap grows larger when scintillation is added to the AWGN.
This seems well worth going after.

\incfig
	{gapFundamental}
	{.8}
	{A log plot of the error probability $\pe$ vs bit energy contrast ratio $\ecrb$
	for the baseline on-off keying (OOK) modulation of Figure \ref{fig:ookIllustrate}.
	To achieve a reliability of $\pe = 10^{-4}$, $\ecrb \approx 16$ dB is required.
	The gap to the global minimum power efficiency of $\ecrb = -1.6$ dB is then 17.6 dB at this
	level of reliability, implying that a factor of $\approx 50$
	increase in power efficiency $\powere$  
	(factor of $50$ reduction in received average power $\power$)
	can be achieved relative to OOK while achieving arbitrarily small $\pe$.}

%The existence of fundamental limits to communication is itself significant
%from several perspectives.
%The technological advancement
%of the transmitting civilization may greatly exceed that of the receiving civilization,
%but no civilization can circumvent fundamental limits.
%Further, as the transmitter and receiver attempt to circumvent
%a shared set of physical impairments
% in an attempt to reach the fundamental limits,
%they should arrive at compatible conclusions about the
%design of an end-to-end system, and this narrows the ambiguity that each perceives in the
%design perpetrated by the other.
	

\subsection{Approaching channel capacity: channel coding}

The M-ary FSK and PPM examples of Section \ref{sec:illustrations}
are simple examples of a more general concept called \emph{channel coding}.
Their characteristic that makes them a channel code is that they
map $M$ information bits onto a signal, rather than doing that mapping
one bit at a time.
The resulting signal is a function of all $M$ bits, and there is no way to examine
that signal and determine just a single bit.
Shannon introduced the idea of channel coding,
and showed that it is necessary to approach the capacity.

Channel coding is another area where power-efficient and spectrally efficient design
differ dramatically.
Power-efficient design is conceptually very simple by comparison, and effective
channel codes are correspondingly easy to find.
For this reason, power-efficient design was attacked first during the 1950's and 1960's.
In fact, it shown by Fano in 1961 that
M-ary FSK and PPM both approach fundamental limits on power efficiency on the AWGN channel
as $M \to \infty$ \citeref{639}.
These are special cases of a more general class of \emph{orthogonal codes} that
all have that nice property.
In contrast, for spectrally efficient design it took almost five decades of research and
incremental improvement to approach fundamental limits, culminating in
the very complex \emph{turbo codes} \citeref{618} proposed in 1993.
FSK and PPM are very useful weapons in the power-efficient design arsenal,
but as will be seen in Chapters \ref{sec:channelmodel} and \ref{sec:infosignals} they are not sufficient by themselves
because they do not account for scintillation.

\subsection{From fundamental limits to practical interstellar communication}

%In extending these examples to practical schemes for interstellar communication,
%there are several issues that must be dealt with.
%There is a serious question about how to detect a bundle of energy in the presence of
%several different types of impairments due to the interstellar medium (ISM) and due to the relative
%motion of the transmitter and receiver.
%Power-efficient design chooses a signal that is least susceptible to these impairments.
%In Chapter \ref{sec:channelmodel} it is shown that all but two impairments can be rendered
%insignificant by limiting the bandwidth $B$ and time duration $T$ of the energy bundle waveform
%$h(t)$.
%The maximum $\{ B , T \}$ pair is called the interstellar coherence hole (ICH), and is fundamentally
%important to power-efficient design.
%The two exceptions are thermal noise of the form \eqref{eq:awgnchannel} and \emph{scintillation}, 
%which is a random
%variation in the received signal power due to scattering effects in the ISM.

The AWGN channel model considered here is a useful teaching tool, but
it is too simple to accurately capture all the ISM and motion impairments.
It is shown in Chapter \ref{sec:incoherent} that almost all of those impairments
can be rendered negligible with an appropriate signal design by the  transmitter,
with noise and scintillation remaining.
Chapter \ref{sec:channelmodel}
develop a resulting channel model for interstellar communication 
incorporating both noise and scintillation and, based on that result revisits the
fundamental limit on power efficiency.
The result is a bit surprising -- scintillation does not affect the fundamental limit of $\powere$ of \eqref{eq:poweremaxAWGN}, but it does profoundly affect the
design techniques needed to approach that fundamental limit.
It no longer suffices to use M-ary FSK or PPM and let $M \to infty$,
but other techniques are needed to deal with the scintillation.
It has been shown that combining M-ary FSK with time diversity combining and
a low duty cycle can approach the fundamental limit \citereftwo{637}{638}, and this is discussed in Chapter \ref{sec:channelmodel}.

Chapter \ref{sec:infosignals} pursues a concrete design example for interstellar communication.
This report does not attempt to use time diversity, but rather a simple outage strategy is adopted
as a way to deal with scintillation.
In an outage strategy,
no attempt to made to extract information from the signal during periods of lower received amplitude.
As a way to achieve
high power efficiency during periods of non-outage,
a design based on M-ary FSK using phase-incoherent detection is chosen.
The resulting power efficiency is compared to the fundamental limit, and the size of the remaining gap
due to the outage strategy and phase-incoherence is quantified.
It is established that this simple approach can increase power efficiency by a factor of about 10 relative to OOK,
leaving another factor of five to be extracted by more complicated additions
such as time diversity.

\section{Discovery}
\label{eq:multipleobservations} 

Extraction of information from an information bearing signal is only possible once
the presence of that signal has been established.
That is the role of \emph{discovery},
which is addressed in Chapter \ref{sec:discovery}.
Discovery is actually the most difficult aspect of interstellar communication
because of the ''needle in a haystack'' challenge of searching a large parameter
space consisting of spatial, frequency, and time variables.
Another reason it is difficult is the absence of prior knowledge of any
characteristics of the signal, such as power level, repetition time,
modulation technique (FSK or PPM or something else?), duty cycle, etc.
However, if we assume that the transmitter is motivated to maximize power efficiency,
then the discovery challenge is considerably simplified since we know that
;power-efficient signals are composed of streams of energy bundles.
It is only the arrangement of those energy bundles in time and frequency that is affected by the
choice of channel coding.
Thus, the first stage of discovery focuses on detecting individual energy bundles.
The detection of individual energy bundles is addressed in Chapter \ref{sec:detection},
including issues like the absence of knowledge or uncertainty about the amount of energy 
that may be present in bundles and the power of the noise.

When one energy bundle is detected, then the discovery algorithms can
shift to a pattern recognition mode, in which additional energy bundles
are sought at the same location or at nearby location 
(meaning direction and frequency).
This is where the discovery of power-efficient signals differs from past
practice, because they are intermittent.
One energy bundle is almost certainly not immediately followed by another energy bundle,
and may occur at nearby carrier frequencies (as seen in the case of M-ary FSK).
That same intermittent nature of the signal also implies that a discovery strategy
cannot expect to be successful with a single observation.
Multiple observations in the same location 
(line of sight and carrier frequency) are necessary to have a reasonable
chance of an observation interval overlapping an actual energy bundle.
Scintillation is another reason for using multiple observations, because
sometimes scintillation amplifies the received signal amplitude, and
sometimes attenuates it.
To take advantage of scintillation, observations need to be spaced temporally far
apart, with time spacing large relative to the coherence time of the ISM.
This critical role of multiple observations in combating scintillation
was pointed out by Cordes, Lazio, and Sagan in 1993 \citereftwo{122}{121}.

In Chapter \ref{sec:discovery} it is assumed that $L$
observations are made in each location, and the goal is
to design a signal that insures a reasonable change of discovery for a given $L$
at the lowest possible received power $\power$.
This is a significantly different criterion from maximizing power efficiency
for an information-bearing signal, and thus the fundamental limits on the latter
do not apply.
In fact, there is no lower limit on the received power necessary for
reliable discovery, although the number of observations the receiver is
willing to deploy places a practical limit.
The characteristics of the transmit signal can be explicitly designed
to minimize $L$; such a signal is said to be \emph{power-optimized for discovery}.
We show that power optimization is critically important if the goal is to
achieve average power that are as low as possible.
For a given value of $L$, the average power can be reduced substantially
at a given reliability of discovery by power optimization.
For a low average signal power, the value of
$L$ can be reduced by many orders of magnitude through power optimization.

Of course power-optimized signals display a tradeoff between a larger $L$
required for reliable discovery
and lower average received signal power.
The fundamental limit on power efficiency of \eqref{eq:ecrawgn}
gives a strong hint as to that tradeoff.
Discovery of a signal is essentially equivalent to extracting
one bit of information (whether the signal present or absent), and \eqref{eq:ecrawgn}
predicts that reliably extracting this one bit of information requires a certain
total energy.
Thus, it is a reasonable hypothesis (confirmed in Chapter \ref{sec:discovery})
that the total energy of the energy bundles that overlap the $L$ observations
must be above some threshold to achieve reliable discovery.

This is true of a signal that is power-optimized for discovery.
A transmitter that wishes to minimize the power at which its signal is discovered
must first establish a minimum $L$ that is necessary to reliably discover its signal,
and this in turn establishes the received power that is necessary.
It is shown in Chapter \ref{sec:discovery} that
power optimization for discovery does not require any sacrifice in power efficiency for
information extraction.
Rather, an information-bearing signal that is power optimized for discovery
simply has the very low information rate $\rate$ commensurate with
its small power $\power$.

\subsection{Two principles of discovery}

Table \ref{tbl:twoprindisc}

\doctable
	{\normalsize}
	{twoprindisc}
	{xx}
	{l p{12cm}}
	{
	\toprule
	\textbf{Principle} & \textbf{Definition}
	\\
	\addlinespace[3pt]
	\cmidrule{1-2}
	\textbf{Bundle energy} &
	The reliability with which a single energy bundle can detected
	is determined by the ratio of the energy in a bundle $\energy_{h}$ and the noise power $N_{0}$.
	\\
	\addlinespace[3pt]
	\cmidrule{1-2}
	\textbf{Total energy} &
	When each individual bundle energy $\energy_{h}$ is sufficiently
	large for reliable detection of individual bundles, the reliability with which a collection
	of energy bundles can be detected is determined by the total
	number the bundles that overlap the observation time, or equivalently the
	total energy of the bundles that overlap the observation time.
	\\
	\bottomrule
	}
	
% Five arguments:
		% Size, which can be any of
			% '\tiny', `\scriptsize', `\footnotesize', `\small', `\normalsize'
			%`\large', `\LARGE', `\huge', `\Huge'
	     % Label for cross-references
	     % Caption
	     % Column formatting directives
	     % Column content


\subsection{Power-optimized beacons}

An interstellar beacon is designed to attract attention, but not embed
any more information than that.
Beacons were prescribed in the Cyclops study \citeref{142}
because of their presumed simplicity of discovery.
Thus, it is natural to ask how a beacon can be power-optimized for discovery
(meaning that it displays the most favorable tradeoff between average
power and the required number of observations) and whether a beacon
offers any advantage over an information-bearing signal.

As a simple example of a baseband design, the Cyclops beacon
is a sinusoid
transmitted continually a single carrier frequency.
This prescription is equivalent
to a continuous sequence of energy bundles where the chosen waveform $h(t)$
is a sinusoid, and where the duty cycle is $\delta = 1$.
This Cyclops beacon is illustrated in Figure \ref{fig:beaconIllustrate}.
Of course, with an appropriate filter matched to $h(t)$ in the receiver, that
sinusoid can be replaced by any $h(t)$ that falls within the ICH constraints.


%Because it is not conveying information at a continuous rate $\rate$,
%the Shannon capacity limits do not apply, nor does the concept
%of power efficiency.
%Yet, the motivation to minimize the transmit power of a beacon
%is clearly relevant.
%This raises the question of how much transmit power is sufficient for
%a beacon?
%If the transmitter designer had the luxury of knowing when the
%receiver would be observing the beacon, a short-term transmission
%would suffice.
%Normally we expect that a beacon has to be transmitted ''continuously''
%so that the receiver retains complete flexibility on when to observe.
%
%Suppose the receiver makes one observation intended to detect
%whether a beacon is present.
%In the absence of a beacon the \emph{false alarm} probability $\pfa$
%captures how how often a beacon is falsely detected because the noise has some
%similarly to the expected beacon.
%For operational reasons, the receiver typically sets a small value
%for $\pfa$.
%It is entirely a choice of the receiver as to what $\pfa$ to choose,
%with the discipline that a lower $\pfa$ inevitably implies a smaller
%detection probability $\pd$, the probability of a valid detection of
%a beacon.
%
%Now suppose a beacon is present in the receiver's observation.
%The transmitter has no idea when the receiver is going to be
%observing its beacon, so it must keep transmitting the beacon
%indefinitely.
%If and when the receiver makes one observation in the location
%of the beacon,
%there is a \emph{detection} probability $\pd$ for the correct
%detection of that beacon.
%$\pd$ depends on the received beacon power,
%and is therefore largely determined by the transmitter.
%One answer to the question ''how much beacon power is enough''
%is a power level $\power$ that results in $\pd \approx 1$.
%However, the transmitter also realizes that if the receiver
%were to make a second independent observation, then the
%chances of detecting the beacon is improved.
%This is particularly true for interstellar beacons because of the
%effects of the scintillation described in Chapter \ref{sec:channelmodel}.
%Scintillation sometimes attenuates the beacon, and at other times
%actually magnifies it, so two independent observations improves the chances
%of the latter.
%By \emph{independent} we mean statistically independent,
%so the observations are far apart enough in time that they do not
%experience the same or correlated scintillation.
%
%In fact, if the receiver makes $L$ independent observations,
%the resulting net probability of detection is
%\begin{equation}
%\label{eq:independentobs}
%1 - ( 1 - \pd )^L \to 1
%\ \ \ \text{as} \ \ \ \ 
%L \to \infty \,.
%\end{equation}
%Starting at any (even low) $\pd$, the effective detection
%probability can be improved as much as desired.
%Because \eqref{eq:independentobs} is valid for any
%$\pd > 0$, there is no
%minimum power required in order for a beacon to be detected reliably.
%It all depends on the number of observations $L$ that the
%receiver is willing to make, and
%the chosen $L$ determines the
%$\power$ that will be reliably detected.
%This is not a contradiction of Shannon's fundamental limits,
%because as $L \to \infty$ the total energy available to the
%receiver to detect the single bit of information embedded in the
%beacon increases without bound.
%That is, $\energybit \to \infty$ as $L \to \infty$.
%The transmitter has a reasonable expectation that the
%receiver make multiple independent observations, because
%the cost to the transmitter to generate a larger $\power$
%indefinitely is much greater than the receiver's one-time cost
%of repeating its observation multiple times.
%
%The transmitter does have considerable control over what
%$L$ is required to reliably detect its beacon in its design of
%the transmit signal.
%A ''good'' beacon design is thus one that minimizes the $L$
%required for detection.
%We can therefore state a criterion for beacons that is analogous
%to power efficiency for information bearing signals.
%A power efficient beacon minimizes the value of $L$
%required to achieve a given detection probability under the
%constraint $\expec{X^{2} (t)} \le \power$.

\incfig
	{beaconIllustrate}
	{.8}
	{
	Illustration of a beacon of the type proposed by Cyclops study  \citeref{142},
	consisting of a sequence of contiguous (unity duty cycle) energy bundles
	at a single frequency.
	}
	
Our experience with power-efficient design of information-bearing signals
suggests that a low duty cycle $\delta \ll 1$ is one way to power-optimize a beacon.
This type of beacon is illustrated in Figure \ref{fig:peBeaconIllustrate}.
For a fixed average power $\power$, the energy of each bundle can be increased
by a factor of $1/\delta$.
There are two competing factors that must be taken into
account in choosing $\delta$.
Only a fraction $\delta$ of observations overlaps a given observation,
assuming that the observation time duration is on the order of $T$, the
time duration of one energy bundle.
This factor increases the $L$ required to achieve a given reliability of discovery.
On the other hand, for those observations that overlap an energy bundle,
the probability of detection is improved
because of the larger amount of energy in that bundle, and this reduces
the required $L$.
These two factors working against one another result in
an optimum choice of $\delta$ for each value of received power $\power$,
if the goal is to minimize the $L$ required to discovery a beacon reliably at that $\power$.

\incfig
	{peBeaconIllustrate}
	{1}
	{
	Relative to the Cyclops beacon of Figure \ref{fig:beaconIllustrate},
	the amount of energy in each energy bundle can be increased
	by decreasing the duty cycle $\delta$ while keeping the average power fixed.
	In this illustration, the duty cycle is $\delta = 0.1$, in which 
	case each bundle can have an energy $1/\delta = 10$ times higher
	at the same average power.
	}

In practice the transmitter chooses a value for $\delta$ and the
receiver chooses a value for $L$, and these two choices are not coordinated.
These choices together determine the minimum average power
at which a beacon can be reliably discovered.
Fortunately, it is generally true that the smaller $\delta$ and the larger $L$ the
lower the average power level at which the beacon can be discovered.
This case is investigated in Chapter \ref{sec:discovery}.
The reliability of discovery of
a continuously transmitted ($\delta = 1$) and a low-duty-cycle
($\delta = 3$\%) beacon are compared in Figure \ref{fig:beaconCompare},
where the power-optimzed beacon also 
assumes a much larger number of observations ($L = 848$ vs $3$).\footnote{
The values of $\delta$ and $L$ were were power-optimized at $\xi = 1$ (0 dB) corresponding to the
vertical line on the left to achieve a miss probability of $1 - \pd =10^{-4}$.}
The power-optimized beacon combined with a larger number of observations
achieves considerably better reliability of discovery at all average powers levels.
In particular, as shown the intermittent beacon achieves the same reliability
(miss probability $1 - \pd =10^{-4}$) at an average received power level that is 28 dB lower,
corresponding to a reduction in power by a linear factor of $631$, or a 99.84\% reduction.
even lower powers can be reliably discovered by making $L$ larger.

The design of power-efficient beacons is considered further
in Chapter \ref{sec:discovery}.
A typical result is illustrated in Figure \ref{fig:beaconCompare},
where two beacon designs are compared.
One is a beacon with continuous transmission,
which can be considered typical of the beacons
that are sought in the current and past SETI discovery searches.
It uses a 100\% duty cycle ($\delta = 1$) and relatively few
independent observations ($L = 3$). 
The second is a beacon design that is optimized to be discovered
at much lower average received power 
while achieving the same performance objective.
It uses a 3\% duty cycle ($\delta = 0.03$) chosen by the transmitter and a
relatively large number of independent observations 
$L = 1000$ implemented by the receiver.
Corresponding to the low duty cycle, the peak received signal power is
much higher in the second case, by a factor of $1/\delta = 32$ ($15$ dB).
The second design permits a transmitted and 
received average power that is 28.5 dB lower,
or a 99.86\% reduction in power (linear factor of 708).
This power advantage is reduced for smaller $L$, or can be increased at will by
choosing a larger $L$.
To the extent that they have depended on the persistence
of beacon energy as part of the search strategy and make relatively few independent observations,
current and past SETI searches will fail to detect beacons that have been
power-optimized for discovery.

\incfig
	{beaconCompare}
	{.8}
	{A log plot of the miss probability $(1 - \pd)$ for two cases (both
	achieving  false alarm probability $\pfa = 10^{-12}$) plotted against 
	$\xi_0$ (which is proportional to average power) in dB.
	For the continuous-beacon case, 
	energy bundles are transmitted continuously ($\delta = 1$)
	and the number of receiver observations is small ($L = 3$).
	For the intermittent-beacon case, the energy bundles are transmitted with
	a low duty cycle ($\delta = 0.03$ or 3\%)
	and the number of observations is large ($L = 1000$).
	The horizontal axis is the energy contrast ratio $\xi_{0}$ for each energy bundle
	in the continuous beacon, 
	with the amount of energy in each bundle for the intermittent
	case being a factor of $1/0.03 = 33.3$ (15.2 dB) larger.
	At a miss probability of $1-\pd=10^{-4}$, the reduction in beacon
	power is 28.5 dB (a linear factor of 708, or a 99.86\% reduction).
	}

\subsection{Replacing a beacon with an information-bearing signal}

In the power-optimized and power-efficient regime, discovery of a beacon
and an information-bearing signal are essentially the same.
Both concentrate on the detection of an individual energy bundle
by making a relatively large number of observations in the same location.
Following the detection of one energy bundle, those observations should
be extended at that location, including nearby frequencies.
A pattern-recognition algorithm operating over extended period of time
can then distinguish a false alarm from a signal of extraterrestrial origin,
and also discern from the pattern of locations the nature of the signal.

Since the discovery technique is so similar, the question arises whether
an information-bearing signal is as good as a beacon from a discovery perspective.
Both can be discovered, so
this comes down to the question of whether a beacon can be discovered
at lower average power than an information-bearing signal.
This question is addressed in Chapter \ref{sec:discovery}, and the
answer is a bit complicated.
It comes down to this:
\begin{description}
\item[Discovery is possible at lower average power.]
In extracting information from a signal, the multiple-observation trick
cannot be used.
The absence or presence of an energy bundle is detected to
extract one or $M$ bits of information from the signal.
By using multiple observations, an information-bearing signal can
always be discovered at considerably lower average power than
is necessary for reliable information recovery.
\item[Beacon optimized for discovery.]
The optimization of a beacon for discovery is a matter of
adjusting the duty-cycle $\delta$ according to the combination of
minimum average power and number of observations $L$
at which that beacon can be reliably discovered.
\item[Information-bearing signal optimized for discovery.]
Taking a power-optimized beacon design and embedding
additional information within it does not compromise its discovery.
In so doing, the main constraint is to retain the same duty cycle.
This information-bearing signal can then have as good a
power efficiency as any information-bearing signal.
However, its rate $\rate$ is constrained by the choice of
duty cycle, which was determined by its discovery properties.
\end{description}
The bottom line is that we would expect all discovered signals
to be information-bearing.
However, those information-bearing signals designed specifically to be detected
at low average power level $\power$ will have correspondingly low information rate $\rate$
(recall that, at constant power efficiency, the two are proportional $\rate \propto \power$).
More generally, power-efficient information-bearing signals are designed to have
lower average power for the same reliability.
This does not make them more difficult to discover, however, because the
reliability criterion places a floor on the amount of energy required in each
energy bundle.
Power-efficient information-bearing signals are, however, more sparse in the density of these
energy bundles in time and frequency, and therefore they do mandate a larger
number of observations $L$ to discover reliably.

\textbox
	{Why transmit a beacon?}
	{
One basic question that SETI researchers have always faced is
whether to expect to find a beacon rather than an information-bearing signal.
Generally this question has been resolved by expecting a beacon,
the logic being that beacons are simpler and thus easier to discover.
This logic has some validity in the regime of spectrally efficient signals,
because achieving high spectral efficiency requires very complex
channel coding techniques.
At minimum this makes them difficult to reverse engineer to extract
the embedded information, but it may also interfere with their discovery.
At minimum all this complexity does not contribute to discoverability
in any constructive way.

Within the regime of power-efficient design, in contrast, there is no
big distinction between a beacon and an information-bearing signal.
Both have the same basic structure consisting of a sparse assembly
of energy bundles.
Generally the way to achieve power efficiency for an information-bearing
signal and power optimization for a beacon is the same:
Keep the amount of energy in each energy bundle constant while making
them more sparse.
Thus, both can be discovered in the same way, by first detecting an
energy bundle and then continuing the observations looking for more energy bundles in the
same vicinity.
Essentially the distinction between the two types of signals disappears,
and it seems unlikely that a civilization going to all the trouble of
transmitting a high power signal would neglect to embed information within
that signal at a rate $\rate$ consistent with that power $\power$.
Embedding that information does not help discovery, but does not harm it either.
Further, once that information has been successfully decoded the statistical
argument for technological and intelligent origin of that signal is vastly improved.
%
%Why would a transmitter choose to transmit a beacon when it can
%just as easily transmit an information-bearing signal?
%The correct answer is that because it is not subject to the fundamental
%limits on power efficiency of information-bearing signals,
%a beacon can get away with significantly less transmit power,
%reducing both capital and operational expenses.
%This places the extra burden on the receiver that it must perform
%more observations.
%From an economics point of view this is a sensible tradeoff.
%The transmitter has no idea when the receiver is observing, and thus
%must suffer the expense of added power essentially in perpetuity.
%The added receiver cost is one-time, and it is the receiver which
%derives all the value from a successful discovery of a beacon.
%
%Generally SETi searches have chosen to search for beacons,
%but the reasoning behind this is flawed.
%In some sense beacons are considered to be ''easier'' to discover.
%Our finding here is that identical search strategies can
%discover power-efficient beacons and power-efficient
%information-bearing signals, the only difference being that
%beacons can be detected at much lower power levels
%since they are not subject to the same fundamental limits.
%Thus, it makes sense to search for beacons if the receiver
%is willing to invest more independent observations seeking
%low-power beacons.
%At received powers large enough to detect with one or a few
%observations, there is essentially no savings in either complexity
%or cost to search for a beacon.
	}

\subsection{Receiver tradeoffs in discovery}
\label{sec:discantennaobs}

The lower average received power required for discovery of either a beacon
or an information-bearing signal can be leveraged in one of several
ways.
The transmitter can reduce the transmitted power, or the receiver
can reduce the gain (collection area) of its receive antenna,
or the propagation distance can be increased.
During the communication phase, the average received power has
a floor that is dictated by the fundamental limit on power efficiency $\powere$.
However, during the discovery phase there is no such floor, and
there is an additional opportunity to decrease the average received power
by increasing the number of independent observations $L$, essentially
taking advantage of scintillation.

This insight opens up a useful opportunity for the receiver designer,
since at a given received signal flux (which is determined by the transmit
power, transmit antenna gain, and propagation distance), the receiver
designer can trade off his antenna collection area against the number
of observations in each direction and frequency.
This is a tradeoff between the cost of the antenna against the
cost of the computation involved in received signal processing, and it
can be resolved by considering the capital and operational costs
associated with both.
Once an information-bearing signal is discovered, a receiver designer
relying heavily on computation will likely have to increase the receive
antenna collection gain in order to reliably extract information from that signal.
However, it is attractive to defer this investment until after
a credible signal of extraterrestrial origin has been discovered.

\section{Average vs peak transmitted power}

Signals power-optimized for discovery and designed for power efficiency in
information extraction have the character that the amount of energy in each
energy bundle is not decreased nearly so much as the sparsity of the energy bundles
in time or frequency.
This has implications for the transmitter design, because it implies that the
peak transmitted power will generally be larger than the average transmitted
power.
This has both design and technological implications for the transmitter designer.
The peak transmitted power can be reduced by extending the time duration of
each energy bundle $T$ as much as feasible, but there is the time coherency
limit $T \le T_{c}$ that limits that opportunity.

High-peak-power transmission is commonplace, for example in radar transmitters.
Research into the applicability of the underlying technologies for interstellar
transmission would be welcome.
There is another opportunity that is perhaps less obvious.
Often a transmitter will want to transmit in multiple directions simultaneously
if it has little or no prior knowledge of where the signal may be received.
Aperture syntheses in a radio interferometer could be used for transmission as
well as reception, allowing multiple directions to be scanned using a common radio transmitter.
In this way, a continuous transmit power would be directed in multiple directions,
resulting in an intermittent low-duty cycle signal from the perspective of each receiver location.
For a given aggregate transmit power, multiple receive locations could be scanned.

\section{Five principles of power-efficient design}
\label{sec:principles}

By 1970 the challenge of achieving fundamental limits in power
efficiency had been theoretically solved
for the Rayleigh fading channel with AWGN, and this model is
shown in Chapter \ref{sec:channelmodel} to apply directly to interstellar communication.
The following
five straightforward principles of power-efficient design,
used in appropriate combination, were shown to be sufficient to achieve this goal.
\begin{description}
\item[On-off signals.]
Spectral efficiency uses multiple levels of signals, but this makes inefficient use of power.
Power efficiency is achieved by conveying information through the presence or absence of 
a bundle of energy.
This is evident in M-ary FSK, which is used in the design example of Chapter \ref{sec:infosignals}.
\item[Design transmitted signal to circumvent impairments.]
Spectrally efficiency is achieved by accommodating dispersive impairments
in the channel and overlapping signals in time and frequency, making up for the
resulting ambiguity by extensive signal processing in the receiver.
Power efficient design, at some expense in bandwidth, designs a transmit signal to
circumvent as many impairments in the channel as feasible.
Not only does this avoid all receiver processing that might otherwise be required to
compensate for impairments, but that processing would inevitably come at a penalty
in enhancement of noise.
This will be illustrated in Chapters \ref{sec:channelmodel} and \ref{sec:incoherence} 
by the many impairments in the interstellar medium and
due to source/observer motion, only two of which (noise and scintillation) cannot be circumvented
by appropriate signal choice in the transmitter.
\item[Convey information by location rather than amplitude.]
Multiple bits of information can be conveyed using only a single bundle of energy
by using location rather than amplitude, in the process conserving energy.
An illustration of this is M-ary FSK, which is used in the design example of Chapter \ref{sec:infosignals}.
\item[Time diversity combining.]
To combat scintillation, the same information can be redundantly transmitted
at time spaced by more than the coherence time, and the receiver can phase-incoherently average
the energy from those redundant transmissions.
\item[Use low duty cycle.]
At the expense of a peak transmitted power that is greater than the average power,
average power can be reduced by transmitting a signal only part of the time.
This technique is inevitable for low-information-rate signals, where power and
information rate are reduced by transmitting only when needed, and where
signals cannot be spread out too much in time due to the time incoherence of the channel.
This design approach is also very relevant to
the design of power-efficient beacons as discussed in Chapter \ref{sec:discovery}.
In that case, the benefit comes from trading off lower duty cycle
for higher power in the energy bundles that are transmitted, more effectively overcoming
noise and scintillation at a given average power level.
\end{description}


\section{History of power-efficient design}

%Power efficiency is important to interstellar communication because of
%the large propagation distance and resulting signal attenuation.
%For a given spreading loss and information rate,
%a communication system design that results in a lower $\powere$ 
%then requires a higher transmit signal power or higher transmit (and receive) antenna gain,
%but these resources are the major source of both capital and operational cost.
%Other authors have argued that spectral efficiency is a secondary consideration
%in interstellar communication due to the broad microwave window \citereftwo{196}{602}.
%We agree with this, and add that the cost of bandwidth in baseband and RF circuitry
%is decreasing rapidly in our terrestrial technologies.
%
%RFI immunity
%is defined as the degree of consistent attenuation of
%RFI overlapping the signal spectrum in time and frequency.
%RFI is a prominent problem in terrestrial radio astronomy,
%particularly due to orbital spacecraft,
%and a transmitter designer sympathetic to this issue
%can easily tailor $h(t)$ to be less susceptible.
%Increasing either bandwidth or time duration of $h(t)$ or both,
%together with a noise-like signal design, provides
%greater suppression of RFI \citeref{211}.
%Thus, one benefit of the relaxed spectral efficiency for interstellar communication
%is that it can be exchanged for increased RFI immunity.


The origin of power-efficient communication is the insight of
Shannon into fundamental limits to communication \citeref{164}.
First applied to the AWGN, this theory clearly demonstrated the tradeoff
between power efficiency and spectral efficiency.
 Further, is highlighted the fact that substantial progress was
 possible in both regimes because of a gap between best practices at the time
 and fundamental limits.
 While the proof of Shannon's theorem is not constructive, it
 provided a general direction to close that gap while not
 giving any specific prescription.
 
 Early and rapid progress in the power-efficient regime 
 came relatively early
because it is conceptually and practically simpler.
It was shown in 1961 that orthogonal coding
 could achieve capacity asymptotically on the AWGN channel
 \citeref{639}.
 M-ary FSK and PPM are examples of  the more general
 class of orthogonal codes, all of which exhibit identical
 $\pe$ performance.
 Also directly relevant to interstellar communication and discussed in
 Chapter \ref{sec:channelmodel},
 the capacity of a Rayleigh fading channel (equivalent to scintillation in the ISM)
 was established to be
 the same as the AWGN by 1969 \citeref{637}.
 The proof was constructive, based on demonstrating a combination of
 techniques that asymptotically achieved the AWGN capacity.
 
 This flurry of activity in power-efficient design was primarily of theoretical
 interest because of the relative conceptual simplicity of the challenge.
 Little research on power-efficient design has appeared in
 the literature since 1970, as the problem was essentially solved by then.
 Attention focused on the much more theoretically challenging
 (and commercially important) spectrally efficient domain.
 Most practical applications demanded spectral efficiency because of the
 limited overall capacity of the radio spectrum for a growing set of
 applications and growing traffic.
 As a reflection of the much greater difficulty,
 channel coding in the spectrally efficient regime
 required many decades of research and incremental improvement
 before the \emph{turbo codes} that were demonstrated in 1993
 finally closed the gap to channel capacity \citeref{618}
 on the AWGN.
 On the other hand, power-efficient design is widely used in
 optical communications, often in the form of PPM \citeref{640},
 because spectral efficiency is hardly a consideration.
 Optical communication thus serves as a better practical validation of power-efficient design
  than terrestrial wireless communication.
 
 Due to the emergence of battery-operated mobile terminals,
 there has been much recent attention to ''energy-efficient''
 wireless communication \citeref{641}.
 In this case energy efficiency refers to extending the battery life.
 Because the radio communications demands spectral efficiency,
 battery life is dominated by the extensive processing required
 in the terminals for signal processing and protocol implementation,
 and the power devoted to radio-frequency transmission is small
 by comparison.
 Thus, this recent work focuses mostly on protocol design for
 lower power consumption in the receiver computation, and has little relevance to
 interstellar communication, where discovery rather than communication
 is the major contributor to computational burden.
 
 
%Power efficiency is much simpler to achieve than spectral efficiency.
%After the birth of modern communications with the
%achievements of Shannon in establishing fundamental limits,
%considerable research on power efficient communication was
%undertaken because theoretical results were easier to attain.
%However, this flurry of activity was soon supplanted by spectrally efficient
%design, both because power efficiency was relatively easy to understand
%and because of the much greater relevance to commercial design.
%For this reason, most references on power efficiency date to the
%1950's and 1960's, and little research has been performed since.
%
%The insights most relevant to interstellar communication are
%due to Kennedy \citeref{}.
%He established the fundamental limits on power efficiency on
%the Rayleigh fading channel, which we will see in Chapter \ref{}
%is a model for interstellar communication in the strong scattering regime.
%His approach to establishing these limits was constructive, by
%demonstrating techniques that can actually achieve fundamental limits.
%This is quite different from spectral efficiency, where fundamental limits were
%established by other means, but concrete ways of approaching those limits
%took four decades of intense effort.

\chapter{Interstellar channel model}
\label{sec:channelmodel}

In Chapter \ref{sec:powerefficient} a fundamental limit was established on
the power efficiency obtainable on the AWGN channel.
However, noise is only one a number of impairments due to the ISM
and due to relative motion between source and observer.
These impairments are listed in Table \ref{tbl:impairments}.
It is, however, possible to choose transmitted signal that avoid many of them.
Avoiding impairments by signal choice is one of the principles of
power-efficient design, since compensating for them at the receiver
typically brings with it a noise penalty.
The interstellar coherence hole (ICH) is a constraint on the bandwidth and
time duration of a signal such that it suffers the minimum possible
change (or impairment) in propagation through the interstellar medium (ISM)
and after being affected by the relative motion of the source and observer.
The ICH provides guidance on how to convey individual
energy bundles in a power-efficient manner.

The appropriate channel model for energy bundles includes
only impairments encountered by a signal falling within an ICH.
From Table \ref{tbl:impairments} these include noise and scintillation, which
are further characterized in this chapter.
In addition, the model must include the possibility of a frequency offset
between one ICH signal and another, although this frequency offset can
avoided if both the source and observer compensate for their relative
acceleration due to their respective planetary motion.
The remaining impairments can be neglected in the channel model, 
but due to their importance in determining the size of the ICH
they are chacterized in Chapter \ref{sec:incoherence}.

%The idea of the ICH is based on an elemental complex-valued baseband waveform $h(t)$ that is
%limited in both time duration and bandwidth.
%The methodology is to design a receiver 
%to detect a transmitted waveform $h(t)$, after modulation and demodulation, pretending that the ISM
%introduces only additive noise of thermal origin.
%Then all the other ISM and motion impairments are introduced one at a time
%to characterize their impact on the receiver performance.
%The question is whether the waveform $h(t)$ can be chosen to
%avoid some or all of these impairments.
%The ICH is defined as a set of constraints on $h(t)$ such
%that as many ISM and motion impairments are avoided as possible.
%Those impairments that cannot be eliminated through the judicious choice of
%$h(t)$ become a characteristic of the ICH model itself.

\doctable
	{\small}
	{impairments}
	{
	A list of the impairments affecting interstellar communication.
	They are divided into three categories:
	Intra-ICH impairments apply to signals falling within
	the interstellar coherence hole (ICH).
	Inter-ICH impairments apply to two signals that each fall within the ICH
	but are fairly widely separated in time.
	Extra-ICH impairments can apply to signals with bandwidth and time duration
	too large to fall in the ICH.
	}
	{l p{2cm} p{11cm}}
	{
	\textbf{Source} & \textbf{Impairment} & \textbf{Symptom and cause}\\
	\toprule
	\addlinespace[3pt]
	Intra-ICH & Noise
	& Additive white Gaussian noise (AWGN) of thermal origin from
	background radiation, emission, and the receiver temperature
	(Section \ref{sec:noiseICH})
	\\
	\addlinespace[3pt]
	\cmidrule{2-3}
	& Scintillation &
	Variation in signal flux at the observer due to the constructive and
	destructive interference of different paths through the scattering medium
	that varies with time due to the component of relative velocity of
	source and observer perpendicular to the line of sight
	(Section \ref{sec:scintillation})
	\\
	\addlinespace[3pt]
	\cmidrule{1-3}
	Inter-ICH & Frequency \newline offset &
	Signals separated in time may be observed with a relative frequency offset
	due to the component of relative acceleration in the direction of the line of sight
	(Section \ref{sec:freqoffset})
	\\
	\addlinespace[3pt]
	\cmidrule{1-3}
	Extra-ICH & Delay \newline spread &
	A relative variation in delay for different signal components due to
	wavelength-dependent group delay for paths passing
	through a scattering medium (Section \ref{sec:dispersion}),
	and also due to the different propagation delays of separate paths though the
	scattering medium (Section \ref{sec:scattering})
	\\
	\addlinespace[3pt]
	\cmidrule{2-3}
	& Carrier \newline phase shift &
	A variation of carrier phase with time due to the relative acceleration of
	source and observer (Section \ref{sec:doppler})
	\\
	\addlinespace[3pt]
	\bottomrule
	}

\section{Definition of the coherence hole}

The concept of an ICH is illustrated
in Figure \ref{fig:ICHidea}.
A complex-valued baseband signal $h(t)$ was defined
in Section \ref{eq:energybundles},
including unit energy, Fourier transform confined to $f \in [0,B]$, 
time confined to $t \in [0,T]$, and time=bandwidth product $K = B T$.
After modulation to carrier frequency $f_{c}$, the real part $\Re \{ h(t) \}$
becomes the in-phase signal, and the imaginary part  $\Im \{ h(t) \}$
becomes the quadrature signal.
After experiencing the ISM impairments at passband and demodulation back to
baseband in the receiver, the matched filter (MF) with impulse response $\cc h (-t)$ is applied.
(See Appendix \ref{sec:moddemod} for an analysis of the modulation and demodulation
and Chapter \ref{sec:detection} for a detailed analysis of the MF.)
The MF does not account for any impairments other than AWGN, so the question is
how other impairments affect the MF output $z(t)$.
Our goal is to establish the simple model for $z(0)$ shown whenever
$h(t)$ falls within an ICH.
This model adds scintillation, but no other impairments, and is justified in
Chapter \ref{sec:incoherence}.


\textbox
	{Simultaneous bandlimiting and time-limiting}
	{
Strictly speaking a waveform cannot be simultaneously bandlimited
and time limited.
However, a classical uncertainty principle of Fourier transforms \citereftwo{599}{625}
states that if $K = B T \gg 1$ then waveforms exist with
most of their energy concentrated in $f \in [0,B]$ and $t \in [0,T]$,
and ''most'' approaches ''all'' as  $K  \to \infty$.
This should not be surprising in light of the sampling theory, which says
that an $h(t)$ precisely confined to $f \in [0,B]$ can be sampled
at rate $1/B$ without losing any information.
If only $K$ consecutive samples are non-zero (the remaining infinity of samples are all zero)
then the waveform is
approximately (although not precisely) confined to time interval $T = K/B$.
	}


\incxy
	[@C=.6cm] 
	{ICHidea}
	{
	The three diagrams from top to bottom represent 
	(a) the radio channel from input $\sqrt{\recenergy} \, h(t)$ to output $r(t)$
	including modulation and demodulation,
	(b) the optimum baseband receiver processing assuming the ISM propagation
	is not present,
	and (c) the simplified end-to-end model taking account of all ISM impairments assuming
	and source/observer motion, but assuming that the bandwidth and time duration
	of $h(t)$ are sufficiently small to fall within an interstellar coherence hole (ICH).
	The scintillation is represented by a multiplicative noise $S$,
	which like additive noise $M$ is complex-valued.
	For the special case of strong scattering, $S$ is Gaussian
	with identically distributed and statistically independent real and
	imaginary parts.
	All signals represented by a single arrow ($\longrightarrow$) are real-valued,
	and all signals represented by a double arrow ($\Longrightarrow$) are complex-valued.
	}
	{
	% First diagram
 	\sqrt{\recenergy} \, h(t) \ar@{=>}[r] 
	&
	*{\bigotimes} \ar@{=>}[r] 
	&
	*+<1pc>[F-,]{2 \,\Re \{ \cdot \}} \ar@{->}[r] 
	&
	*+<1pc>[F-,]{
	\begin{matrix}
	\text{ISM} \\
	\text{impairments}
	\end{matrix}
	} \ar@{->}[r] 
	&
	*{\bigotimes} \ar@{=>}[r] 
	&
	*+<1pc>[F-,]{\begin{matrix}\text{LPF} \\ f \in [0,B] \end{matrix}} \ar@{=>}[r] 
	&
	r(t)
	\\
	& 
	\displaystyle e^{\, i \, ( 2 \pi \, f_{c} t + \theta)} \ar@{=>}[u] 
	&&&
	\displaystyle e^{ - \, i \, 2 \pi \, f_{c} \, t } \ar@{=>}[u]
	% Second diagram
	\\
	&
	r(t)  \ar@{=>}[r]
	&
	*+<1pc>[F-,]{
	\begin{matrix}
	\text{Matched filter} \\
	\cc h (-t)
	\end{matrix}
	} \ar@{=>}[r]
	&
	z(t)
	% Third diagram
	\\
	&
	\sqrt{\recenergy} \ar@{->}[r] 
	&
	*{\bigotimes} \ar@{=>}[r] 
	&
	*{\bigoplus} \ar@{=>}[r] 
	&
	z(0)
	\\
	&& 
	S \ar@{=>}[u] 
	& 
	M \ar@{=>}[u] 
	}


Having defined a receiver structure appropriate for noise-only, it is appropriate to
return to Figure \ref{fig:ICHidea} and ask what happens when 
other impairments are introduced,
including propagation impairments in the ISM and effects due to the
relative motion of source/observer.
There is a good understanding of the ISM and its effects on radio propagation
arising from natural phenomena such as pulsars \citeref{214}.
In particular, the ISM is populated by clouds of low-density plasma
consisting principally of hydrogen ions and free electrons,
and thus it is a conductive medium that affects radio propagation.
Based on these observations, together with theoretical modeling
based on an understanding of the underlying physics of plasmas
and Doppler effects, good models are available for this propagation.
The models in the astrophysics literature are commonly monochromatic, 
and tell us that the effect of ISM propagation
on a monochromatic signal is group delay, spreading loss, and scintillation.
Group delay is primarily due to the speed-of-light propagation over large distances.
Spreading loss is due to the spherical spreading of energy during propagation, with only
a tiny portion of that energy captured by the receiving antenna.
Scintillation will be addressed shortly.

A waveform $h(t)$
is affected in similar ways to a sinusoid, but with additional complications
due to its non-zero bandwidth.
However, if the bandwidth $B$ of $h(t)$ is restricted, it would not be surprising if we
reached a point at which the distortion of $h(t)$ due to these complicated
effects simplified to be similar to those experienced by a monochromatic signal.
Further, if we shrink the time duration $T$ of $h(t)$, it would not
be surprising if the time-varying effects like Doppler
became insignificant.
These effects are still manifested, but for sufficiently small $T$ their time-varying nature
can be neglected.
Like a sinusoid, the remaining impairments of a fixed delay, a spreading loss, additive noise and scintillation
remain, and these are characteristics of the ICH.
This intra-ICH impairments will now be further characterized.
The significant physical parameters for interstellar communication
are listed in Table \ref{tbl:assumptions}, including values
that will be used for numerical examples.
The nature and significance of these parameters will be explained as we proceed.

%When all the impairments are taken into account, not just additive noise,
%it is appropriate to divide them into two distinct categories.
%Category I impairments are those that 
%moderate as $B$ and/or $T$ are decreased, 
%and for sufficiently small $B$ and $T$ can be neglected.
%The \emph{coherence bandwidth} $B_c$ and the \emph{coherence time} $T_c$
%are determined by the $B$ and $T$ that render \emph{all}
%Category I impairments insignificant enough to be neglected.
%The ICH is defined as all
%waveforms $h(t)$ with bandwidth $B \le B_{c}$ and $T \le T_{c}$.
%An important qualification is that
%Category I impairments don't disappear suddenly as $B$ and $T$ decrease.
%Thus, the choice of $B_{c}$ and $T_{c}$ is inevitably influenced to some degree by whatever
%we are trying to accomplish with the ICH.
%The two parameters $B_{c}$ and $T_{c}$ define the \emph{size} of an ICH.
%Category II impairments, on the other hand, are those that 
%remain essentially unchanged as both $B$ and $T$ are decreased.
%Thus these impairments cannot be neglected for $h(t)$
%that fall inside an ICH, and are characteristic of the ICH itself.
%
%The primary Category II impairments are scintillation and noise.
%Scintillation is a random fluctuation in amplitude and phase of the sinusoid with time
%as corrupted by the propagation and seen by the observer.
%Scintillation is due to inhomogeneities in the ISM, which results in the signal energy
%following multiple paths, interacting with motion effects.
%The time-varying constructive and destructive interference of these different
%paths results in a random amplitude and phase for their superposition,
%with the exact character of that interference changing with time due to motion
%of the turbulent clouds and the source/observer motion.
%Since scintillation is apparent as $B \to 0$, it is a Category II impairment,
%as is the additive noise of thermal origin due to the cosmic background radiation
% and natural emitters of thermal energy such as stars.
% As we will see, the noise energy at the MF output is independent of $B$ and $T$.
% 
% Other impairments fall into Category I.
% The group delay of the propagation through a plasma has some wavelength dependencies,
% causing $h(t)$ to be smeared out in time.
% This \emph{plasma dispersion} is moderated for small bandwidth $B$.
% The inhomogeneities in the turbulent clouds of the ISM cause
% diffractive and refractive effects in the propagation.
% The distances involved are very large in relation to a wavelength,
% and thus the physics of geometrical optics governs these impairments,
% and hence the use of terminology from optics like ''refraction''.
% The effect is energy traveling from source to observer with different
% path lengths, and hence group delays, and then superimposing themselves
% prior to observation.
% This is called \emph{multipath} distortion.
% As the bandwidth $B$ of $h(t)$ decreases, the multipath itself is not affected
% but its effect on $h(t)$ is moderated and eventually can be neglected.
%The relative motion of the source and observer cause time-variation in the
%carrier frequency and baseband signal phase, but these effects becomes insignificant
%for sufficiently small $T$. 
%However, the interaction of multipath with motion causes \emph{fading},
%which is the time variation in signal magnitude manifested by Category I scintillation.
%While the time-variation of scintillation falls in Category I, the observation of a random
%signal magnitude and phase at any single point in time is a Category II impairment.
%
%The Category II impairments, those that characterize the ICH, will now be described.
%It is important to understand them because they determine the fundamental limits on
%discovery (Chapter \ref{sec:discovery}) and communication (Chapter \ref{sec:fundamental}), 
%and are influential in the design of
%a communication system (Chapter \ref{sec:channelmodelstructure})..
%Category I impairments are addressed in Chapter \ref{sec:incoherence}.
%They are less important because they affect only the size of the ICH,
%and as we will see the achievable power efficiency is not affected by that size
%as long as $K_{c} \gg 1$.

\doctable
	{\small}
	{assumptions}
	{All the significant physical parameters determining the
	strength of impairments in
	interstellar communication, together with
	numerical values used in examples.
	Generally the values are chosen to minimize the ICH size.}
	{l c p{12cm}}
	{
	\textbf{Source} & \textbf{Parameter} & \textbf{Description}\\
	\toprule
	\addlinespace[3pt]
	ISM & $\dm$ &
	The dispersion measure equals the total column density of
	free electrons along the line of sight (Section \ref{sec:dispersion}).
	\\
	&& $\dm = 1000$ is
	approximately the largest $\dm$ observed in pulsar astronomy;
	$\dm$ will be much smaller for most lines of sight.
	\\
	&& Pre-equalization in either transmitter or receiver can
	reduce the effective value to the uncertainty $\Delta \dm$ 
	(Appendix \ref{sec:equalization}).
	\\
	\addlinespace[3pt]
	\cmidrule{2-3}
	& $D$ &
	A distance-of-propagation measure. 
	In Figure \ref{fig:scattering-iD-illustration},
	$D$ is the distance from screen to observer, and
	more generally it is defined by \eqref{eq:d12}.
	\\
	&&The coherence bandwidth of scattering decreases with $D$
	and the scattering becomes stronger,
	so we use a relatively large value of
	 $D = 250$ light years
	 (this corresponds to $D_{1} = D_{2} = 500$ light years)
	\\
	\addlinespace[3pt]
	\cmidrule{2-3}
	& $\rdiff$&
	The diffraction scale characterizes the turbulent clouds of 
	interstellar plasma, and equals the range of $x$ at the scattering screen
	over which the phase introduced by the screen is is approximately constant.
	\\
	&&It is wavelength-dependent, with $\rdiff \propto f_{c}^{\,6/5}$,
	with a typical value of $\rdiff = 10^{\,7}$ meters at $f_{c} = 0.3$ GHz \citeref{598}.
	\\
	\addlinespace[3pt]
	\cmidrule{1-3}
	Motion & $P$ &
	Period of circular motion, either diurnal rotation about axis or orbital motion around star.
	\\
	&& $P= 1$ day ($8.6 \times 10^{4}$ sec)  for the diurnal rotation of the Earth.
	\\
	\addlinespace[3pt]
	\cmidrule{2-3}
	& $R$ &
	Radius of circular motion, either diurnal rotation about axis or orbital motion around star.
	\\
	&& $R = 6.38 \times 10^{6}$ meters for the diurnal rotation of the Earth.
	\\
	\addlinespace[3pt]
	\cmidrule{2-3}
	& $v_{\bot}$&
	The velocity of the observer transverse to the line of sight.
	\\
	&& Although \citeref{122} estimates a typical value $v_{\bot} = 10  \ \text{km s}^{-1}$,
	we conservatively adopt $v_{\bot} = 50  \ \text{km s}^{-1}$.
	\\
	\addlinespace[3pt]
	\bottomrule
	}


\section{Model of a coherence hole}
\label{sec:modelICH}

If a signal $h(t)$ falls within an ICH, then the model of its propagation through the
ISM simplifies to that shown in Figure \ref{fig:ICHidea}
and is captured by the equation
\begin{equation}
\label{eq:ICHmodel}
Z(0) =  \sqrt{\recenergy} \, e^{\,i\,\theta} \, S+ M \,.
\end{equation}
where $S$ is the multiplicative scintillation noise and
$M$ is the additive noise.
The unknown carrier phase $\theta$ is can be omitted,
since $S$ also has a random phase.
The scintillation can be written in terms of magnitude and
phase as
\begin{equation}
S = \sqrt{\flux} \, e^{\,i\,\Phi}
\end{equation}
where $\flux$ is the received signal flux and $\Phi$
is a random phase that is uniformly distributed on $[ 0 , \, 2 \pi ]$.
This model omits spreading loss and propagation delay, which can be considered separately.

While $\Phi$ does not add any new uncertainty on the phase,
since the carrier phase is unknown anyway, it does imply a more rapid phase fluctuation
between two ICH's that are non-overlapping in time.
The scintillation flux $\flux$ is the significant new element of the model.
The magnitude of the signal is affected by the received energy $\recenergy$
in the absence of scintillation, and the scintillation \emph{flux} $\flux$.
These are both energy measures, so their contribution to the signal magnitude
is the square root.
In the absence of scintillation, by convention $\flux = 1$.
In the presence of scintillation, the received signal energy is multiplied by $\flux$,
becoming $\recenergy \cdot \flux$,
and it is possible to have $\flux > 1$ or $\flux < 1$ implying that
scintillation results in either an increase or a decrease in signal level.
The presence of the random phase term $e^{\,i\,\Phi}$ 
in the signal renders 
the phase of $Z(0)$ basically useless, but the magnitude $|Z(0)|^{2}$
contains useful information about the presence of a signal ($\recenergy > 0$)
or the absence of a signal ($\recenergy = 0$).

In the model of \eqref{eq:ICHmodel}, by definition
$\expec{\flux} = \vs$ and $\expec{|M|^{2}} = N_{0}$.
The \emph{energy contrast ratio} $\xi$ is
defined as the average signal energy divided by the average noise energy
at the output of the MF,
\begin{equation}
\label{eq:ecrs}
\ecrs =  \frac{\recenergy \cdot \expec{\flux}}{N_{0}}
= \frac{\recenergy \, \vs}{N_{0}} \,.
\end{equation}
In both fundamental limits and concrete communication design,
this ratio appears repeatedly.
Generally speaking the parameters $\{ \recenergy, \vs, N_{0} \}$
are not as individually significant as their 
contribution to the ratio as expressed in \eqref{eq:ecrs}.
If the signal energy $\recenergy$ and noise power density $N_{0}$
are increased by the same factor
(they both have the units of energy),
generally speaking it can be said that the performance remains constant.

A useful parameter of the scintillation is the \emph{modulation index},
defined as
\begin{equation}
\label{eq:modulationindex}
m_{\flux} = \frac{\sqrt{\var{\flux}}}{\expec{\flux}} \,.
\end{equation}
This index is a measure of the typical variation in the flux $\flux$
(as measured by standard deviation)
in relation to its mean-value.
Thus when $m_{\flux} \approx 0$ there is a very small variation in
signal level due to scintillation (at least in relation to the average signal level)
and when $m_{\flux} \approx 1$ the standard deviation is
equal to the mean value.

%a multiplicative \emph{scintillation} $(\ms+S)$  
%and an 
%additive \emph{thermal noise} $M$.
%The $\ms$ is a complex-valued constant, and 
%represents a non-random component to the signal.
%Both $S$ and $M$ are complex-valued zero-mean Gaussian random variables, and
%thus $Z$ is also a complex-valued zero-mean Gaussian random variable.
%The real- and imaginary parts of both $S$ and $M$ are independent, and hence their
%parts have mean-value zero and variance $vs/2$ and $N_{0}/2$ respectively.
%Other important parameters of the model are the mean-square scintillation $E |S|^{2} = \vs$
%and the mean-square additive noise $E |M|^{2} = N_{0}$.
%
%The effect of the multiplicative scintillation term $(\ms+S)$ is to introduce a random phase
%unknown to the receiver.
%As a result, the ''raw'' MF output $Z(0)$ has all the characteristics of noise, but 
%the receiver will always calculate the energy $|Z(0)|^{2}$ to render the subsequent
%processing independent of this random phase.
%Fortunately $|Z(0)|^{2}$ contains information about the signal energy $\recenergy$
%(for example, its mean value is dependent on the parameters
%$\{ \recenergy, \ms, \sigma_{s}, N_{0} \}$).
%The distribution of $|Z(0)|^{2}$ does not depend on the phase of $\ms$, so $\ms$
%can be taken to be real-valued without loss of generality.
%
%Considered separately of noise $M$, the scintillation magnitude-squared $Y = |\ms + S|^{2}$ 
%is a measure of the intensity of the random signal, and in physics this
%is called the \emph{signal flux}.
%
%$Y$ has a non-central $\chi^{2}$ distribution, while
%$|M|^{2}$ has a central $\chi^{2}$ distribution.
%A characteristic of $Y$ is its \emph{modulation index}, which measures the
%size of the variation in $Y$ relative to its mean.
%The index $m_{Y}$ is defined as the ratio of standard deviation to mean, or
%\begin{equation}
%m_{Y} = \frac{\sqrt{\,\text{Var}[Y]\,}}{E[Y]} =
%\frac{\sqrt{\, \vs (\vs + 2 \ms^{\,2}) \,}}{\vs + \ms^{\,2}} \,,
%\end{equation}
%and is a measure of how much random fluctuation there is in
%$Y$ relative to its non-zero mean-value.
%The maximum possible value is $m_{Y} = 1$ when $\ms = 0$,
%so the standard deviation of $Y$ is always smaller than the mean value of $Y$
%(except they are equal when $\ms = 0$).
%In words, the maximum variation in $Y$ is equal to the mean value of $Y$. 

This simple model of \eqref{eq:ICHmodel} is now related to the physics of scattering \citeref{598}
followed by noise of thermal origin.

\subsection{Scattering within a coherence hole}
\label{sec:scintillation}

Scattering is due to variations in electron density within the turbulent interstellar clouds.
Because the distance scales are so large, even at radio frequencies
the phenomenon can be modeled by geometrical optics
using a ray approximation to the radio propagation.
This is illustrated by a simple one-dimensional model in Figure \ref{fig:scattering-iD-illustration}.
Although reality is considerably more complicated, with the conductive medium in turbulent clouds
spread through three dimensions, this model captures the essential features.
A thin one-dimensional \emph{scattering screen} is placed in the path of a plane wave,
and an observer views the resulting intensity at distance $D$.
The essential feature that causes scattering is the non-homogeneity of the screen
which has a group delay $\tau (x)$ that depends on the position $x$ on the screen.
The resulting diffractive and refractive effects at the observer result from
constructive or destructive interference among rays passing through different $x$
that influence the signal level.

\incfig
	{scattering-iD-illustration}
	{.8}
	{Illustration of the geometry of scattering using a simplified one-dimensional
	scattering screen. Rays pass through the screen
	(located at distance $D$ from the observer) at different lateral distances $x$ and
	encounter different group delays and phase shifts due to small variations in electron density.}

The phase shift encountered by a given ray is affected by (a) the phase shift encountered at the
screen, (b) the phase shift due to propagation from point $x$ on the screen to the observer,
and (c) changes in the latter phase shift with time due to the observer's motion.
Although (b) and (c) are deterministic and easily modeled, (a) is unknown and subject only to
statistical analysis based on a model of turbulent motion of interstellar clouds.
An essential characteristic of this model is the \emph{diffraction scale} $\rdiff$,
which measures the range of $x$ over which the phase is statistically likely to remain fairly constant.
It is these ''coherent patches'' of stationary phase that contribute most strongly to the
energy that arrives at the observer.
Other areas on the screen without coherent phase tend not to contribute much net energy,
since they result in a jumble of phases that destructively interfere.

A second essential scale is the
\emph{Fresnel scale} $\rf$,
given by
\begin{equation}
\label{eq:rf}
\rf (f) = \sqrt{\lambda_{c} D } =  \sqrt{\frac{c \, D}{f_{c}}}
\end{equation}
where $\lambda_{c}$ is the wavelength and $f_{c}$ is the frequency of the carrier,
 $c$ is the speed of light.
 The Fresnel scale
 $\rf$ is the distance over which the phase shift due to the triangular geometry is small,
having nothing to do
 with the phase shift of  the scattering screen.
 The phase shifts as a function of $x$ are small over a scale $|x| \le \rf$
 (called the first Fresnel zone)
 because over this scale the variation in propagation distance is small relative
 to one wavelength.
 Along with coherence of phase introduced by the screen, coherence of phase
 due to the geometry is another necessary condition for the constructive interference
 of rays and hence a significant contribution to the energy arriving at the observer.
 
There is an important interplay between $\rdiff$ and $\rf$ that determines the
character of the resulting signal impairment.
The regime where $\rdiff \gg \rf$ is called \emph{weak scattering},
and $\rdiff \ll \rf$ is called \emph{strong scattering}.
Interstellar communication can encounter both types of scattering
as determined primarily by the interaction between the parameters $D$ and $f_{c}$.
The scales follow $\rdiff \propto  f_{c}^{\,6/5}$ and $\rf \propto f_{c}^{\,- 1/2}$,
and hence $\rdiff / \rf \propto f_{c}^{\, 17/10}$, and in addition $\rdiff /\rf \propto D^{-1/2}$ \citeref{598}.
The boundary between these regimes is illustrated in Figure \ref{fig:weakVsStrong},
where strong scattering occurs for lower $f_{c}$ and larger $D$.

The character of scintillation is very distinctive for strong and weak scattering,
so they are now considered separately.

\incfig
	{weakVsStrong}
	{.8}
	{A log-log plot showing the boundary between weak and strong scattering for variation of the
	distance $D$ in light years (according to the definition of \eqref{eq:d12}) and the carrier frequency $f_{c}$.
	The numerical value of $\rdiff$ given in Table \ref{tbl:assumptions} is assumed.}

\subsubsection{Strong scattering regime}

See Figure \ref{fig:scattering-strongvsweak} for an illustration of the distinctive
geometries that separate strong vs. weak scattering.
In the strong scattering regime of Figure \ref{fig:scattering-strongvsweak}a, 
$\rdiff \ll \rf$, and thus the typical coherent patch
of stationary phase is at a scale much shorter than $\rf$.
Within the first Fresnel zone the geometric variation in phase
is not much of a factor, but
even coherent patches occurring outside the first Fresnel zone are significant contributors
to the received flux,
albeit at a reduced level, because the geometric contribution to phase variation can
still be small over the smaller $\rdiff \ll \rf$ scale.
In fact, there is a longer \emph{refraction scale} $\rref > \rf$ over which coherence patches
make a significant contribution (it happens that $\rref = \rf^{\,2} / \rdiff$).
Within the refraction scale there are multiple distinct coherent patches,
each contributing energy with a propagation delay that increases with $x$.
The maximum delay that is a significant contributor roughly corresponds to $x = \rref$.
In strong scattering there is \emph{multipath distortion} due to the multiple
pathways that arrive at the observer, each corresponding to a distinct coherent
patch, and each having a distinct delay.

\incfig
	{scattering-strongvsweak}
	{.8}
	{An illustration of the difference in geometries between (a) strong scattering
	and (b) weak scattering. The $x$ scale is exaggerated relative to the $z$ scale
	to magnify the distinction.}

To model the ICH, the question is what the effect of this multipath distortion
is on a finite bandwidth waveform $h(t)$.
To develop a simple model, assume that there are $N$ paths
corresponding to distinct coherent patches, where
the $n$th path is characterized by an amplitude
$r_k$ and a phase shift $\phi_{n}$.
Although $h(t)$ will also be distorted by plasma dispersion (see Section \ref{sec:dispersion}),
within an ICH this effect can be neglected.
Although there is some smearing of energy over time due to the
geometric variation of propagation delay within a single coherent path,
neglect this effect to lump all this energy into a single discrete delay $\tau_{n}$.
Although the exact amplitudes are unknown, it is the
phases that are very random.
Phase is very sensitive to slight perturbations
of conditions over such long distances and those perturbations can easily be large
relative to one wavelength.

In our simple model,
the observation consists of a superposition of these paths,
\begin{equation}
\label{eq:multipathsum}
r(t) = \sqrt{\recenergy} \cdot \sum_{n=1}^{N}  r_k \, e^{\,i\,\Phi_{n}} \, h( t - \tau_{n} ) \,.
\end{equation}
Altough the parameterization is likely to be very different, this basic model is
very familiar in terrestrial wireless communication,
where the multipath distortion is due to radio waves bouncing over
various obstacles like buildings and mountains \citeref{574}.
There are two distinct effects to consider: the delays $\{ \tau_{n} \}$
and the phases $\{ \phi_{n} \}$.

Consider first the delays  $\{ \tau_{n} \}$.
As seen from geometric reasoning, all $\tau_{n} < \infty$
since as $x$ increases (and equivalently propagation delay increases)
eventually a point is reached where the geometric variation in phase
across a coherent patch yields an insignificant observed net flux.
Thus, define the \emph{delay spread} $\tau_{s}$ of the scattering as
the maximum of the $\{ \tau_{n}, \, 1 \le \tau \le N \}$.
Recall that in the model of the ICH of Figure \ref{fig:ICHidea}
it is the response of an MF to the reception $r(t)$ that matters.
The response of the MF to a single term $h(t - \tau_{n})$ is
\begin{equation}
\label{eq:multipath}
\int_{0}^{T} \, h(t - \tau_{n}) \cc h (t) \, dt
=  \int_{0}^{B} | H(f) |^{2} \, e^{-\,i\,2 \pi f \, \tau_{n}} \, d f \,.
\end{equation}
The effect of delay $\tau_{n}$ is reflected
in the frequency-domain by the phase term $e^{-\,i\,2 \pi f \, \tau_{n}}$.
This term can be ignored (and hence $\tau_{n}$ can be neglected) if
the total phase shift variation across $f \in [0,B]$ is less than $\alpha \pi$, or
\begin{equation}
\label{eq:delaycbw}
2 \, B \, \tau_{s} \ll \alpha \,,
\end{equation}
where $0 \le \alpha \le 1$ is a parameter chosen to adjust the
strictness of the criterion.
Intuitively, the ''width'' or rate of change of $h(t)$ is limited by $B$; the larger
$B$, the faster can be the variations in $h(t)$.
As long as $\tau_{s}$ is less than $\alpha/2B$, the effect on $h(t)$ is
hardly noticeable because the waveform of $h(t)$ is changing too slowly to
see the effects of that delay.

This establishes delay spread as a frequency coherence issue, in that
its effects are mitigated and eventually can be neglected as bandwidth $B$ is decreased.
Thus, within an ICH it can be assumed that \eqref{eq:delaycbw} is satisfied
and \eqref{eq:multipathsum} simplifies to
\begin{equation}
\label{eq:scinmulti}
Z(0) = \left. r(t) \convolve \cc h (-t) \right|_{t = 0} 
= \sqrt{\recenergy} \cdot \sum_{n=1}^{N} r_{n} \, e^{\,i\,\Phi_{n}}
\,,
\end{equation}
which is consistent with \eqref{eq:ICHmodel} without the noise.
In \eqref{eq:scinmulti} the magnitude and phase of the scintillation are,
\begin{equation}
\label{eq:S}
 \sqrt{\flux} \, e^{\,i\,\Phi} = S = \sum_{n=1}^{N} r_{n} e^{\,i\,\Phi_{n}}\,.
\end{equation}
A new complex-valued random variable $S$ has been introduced, capturing
both the magnitude and phase of the scintillation.

The flux $\flux$ is the average observed energy associated with unit-energy waveform $h(t)$ after it is 
intercepted by the screen, and this is the origin of the term flux.
No reduction in $B$ and/or $T$ can rid us of $\flux$,
and thus scintillation is a Category II impairment that is a characteristic of the ICH model.
It even affects even the limiting case of a monochromatic signal ($B \to 0$) \citerefthree{121}{122}{132}.
The phase shifts of different paths are a very sensitive function of
the physical parameters, including plasma density and path length.
For example, differences in the $\{ \tau_{n} \}$ too small to cause frequency incoherence
will still have a big effect on the $\{ \Phi_{n} \}$.
On the other hand, the $\{ r_n \}$ can be expected to vary reasonably slowly with time,
since they are dependent on the large-scale geometry of multiple paths of propagation
through the ISM.
Thus, in \eqref{eq:scinmulti} the liberty has been taken to make the $\{ r_n \}$
constants and the $\{ \Phi_n \}$ are random variables.

Working back from these assumed statistics of the $\{ \Phi_{n} \}$ it is straightforward to show
(Appendix \ref{sec:withoutmod}) that $S$ is zero mean
($\expec{S} = 0$), and by a Central Limit Theorem argument it is a Gaussian
random variable with second order statistics
\begin{equation}
\label{eq:strongsecorder}
\expec{S^{2}} = 0
\ \ \ \text{and} \ \ \ \ 
\vs = \expec{|S|^{2}} = \sum_{n=1}^{N} r_n^{\,2} \,.
\end{equation}
The condition $\expec{S^{2}} = 0$ implies that 
$\Re \{ S \}$ and $\Re \{ S \}$ 
are independent and each have variance $\vs/2$.
In different ICH's that do not overlap in time or in frequency, the values of $S$
may have some statistical dependency, more so in magnitude than in phase
because the $\{ r_{n} \}$ are determined primarily by turbulence in the interstellar
clouds and the motion of the receiver.
The effect of motion is considered in more detail in Section \ref{sec:fading},
where it is shown that it results in a Category I time incoherence that can be
neglected for sufficiently small $T$.

From the Gaussian distribution of $S$ and \eqref{eq:strongsecorder}, it follows that
$\expec{\flux} = \vs$ and $\var{\flux} = \sigma_{s}^{\,4}$,
and thus from \eqref{eq:modulationindex}
the modulation index is $m_{\flux} = 1$.
Thus, the standard deviation of flux equals its mean, independent of $\vs$.
However, a deeper examination of the physics reveals that \citeref{598}
\begin{equation}
\label{eq:sigmasone}
\expec{\flux} = \vs = 1 \,.
\end{equation}
Thus, neither weak nor strong scattering affects the
energy contrast ratio $\ecrs$ in \eqref{eq:ecrs}.

For strong scattering $\sqrt{\flux}$ has a Rayleigh
distribution, and thus this type of scintillation is
called \emph{Rayleigh fading} in the communications literature.
There is a wealth of relevant experience in designing wireless mobile communication
systems that encounter Rayleigh fading.

%The random variable $|S|$ represents the current magnitude of the
%signal, and has a Rayleigh distribution,
%\begin{equation}
%\prob{|S| \le \lambda} = 1 -  \exp \left( - \frac{\lambda^{2}}{\vs} \right) \,, \ \ \lambda \ge 0 \,.
%\end{equation}
%The fact that $\arg S$ is uniformly distributed on $[ - \pi , \pi ]$ is also significant,
%although the carrier phase is already unknown so this adds no additional challenge.
%In view of the logic above, $S$ can be considered a fixed random variable within
%one ICH.
%However, if we compare $S$ between two ICH's that
%are non-overlapping in time and frequency, we would expect
%$|S|$ to be highly correlated if the two ICH's are close to one another,
%but we would expect $\arg S$ to be statistically independent.
%This observation does add an additional challenge, because while the unknown carrier
%phase may be relatively stable over time, scintillation adds a source of phase instability.
%
%Because the scintillation magnitude has a Rayleigh distribution, 
%a similar phenomenon to scintillation in terrestrial mobile and wireless systems
%is called ''flat Rayleigh fading'',
%and there is a wealth of relevant experience in designing wireless mobile communication
%systems that encounter Rayleigh fading.

\subsubsection{Weak scattering regime}

Returning to Figure \ref{fig:scattering-strongvsweak}b,
in weak scattering (where $\rdiff \gg \rf$) the scale of coherent patches
is large relative to the Fresnel scale.
This implies that geometric effects are dominant in the sense that
the delay spread and received flux are determined by the geometry
more than the coherence patches, although the latter remain very
significant in determining whether the flux is high (a coherence patch
overlaps the observer's first Fresnel zone) or low (the observer's first Fresnel
zone falls in a region of chaotic phase or transition).
For weak scattering, the modulation index is less than unity \citeref{598},
\begin{equation}
\label{eq:mfluxRician}
m_{\flux} = \left( \frac{\rf}{\rdiff} \right)^{\,5/6} < 1 \,,
\end{equation}
or the variations in flux $\flux$ are smaller than the mean.
Since $m_{\flux} = 1$ for a completely random scintillation, this implies
that $\flux$ has a deterministic component that 
contributes to $\expec{\flux}$ but does not contribute to $\sqrt{\var{\flux}}$.

In communications the case $m_{\flux} < 1$ is called \emph{Rician fading},
because $\sqrt{\flux}$ has a Rice distribution.
The model used in communications for Rician flux is \citeref{574}
\begin{align}
\label{eq:ricianflux}
&\sqrt{\flux} \, e^{\,i\,\Phi} =\sqrt{\gamma\,} \, \sigma_{s} \, e^{\,i\,\Psi}
+ \sqrt{1-\gamma\,} \, S \\
&\gamma = \frac{\kappa}{1 + \kappa}
 \,,
\end{align}
where $S$ has the same statistics as in Rayleigh fading.
Comparing with \eqref{eq:S}, there is the addition of
a \emph{specular} term which has a constant magnitude
(it is not Gaussian) and a random phase $\Psi$ that is uniformly
distributed on $[0, 2 \pi ]$ and independent of $S$.
A parameter
$0 \le \kappa < \infty$ called the $K$-factor controls
how much of the energy is in the constant-magnitude term vs the random term,
all the while maintaining a constant average flux $\expec{\flux} = \vs$.
The modulation index
\begin{equation}
\label{eq:mfluxRicianK}
m_{\flux} = \frac{\sqrt{1 + 2 \, \kappa}}{1 + \kappa} \,,
\end{equation}
is plotted in Figure \ref{fig:scinMod}.
The Rayleigh fading case (strong scattering) corresponds to $\kappa = 0$,
while $m_{\flux}$ decreases as $\kappa$ increases.
Rayleigh fading is therefore ''worst case'' in the sense of ''largest modulation index''.

Rician fading is characteristic of wireless propagation when there is an unobstructed specular path
from source to observer that contributes a constant flux
(albeit with random phase $\Psi$), accompanied by a multiple random
paths that contributes to a variation in flux.
In order to get proper articulation between weak and strong scattering at the
transition ($\rdiff = \rf$), we must have $\vs = 1$ in \eqref{eq:ricianflux}.
For a given value of $m_{\flux}$ from \eqref{eq:mfluxRician},
the appropriate $\kappa$ can be read off of Figure \ref{fig:scinMod}
or calculated from \eqref{eq:mfluxRicianK}.

\incfig
	{scinMod}
	{.6}
	{The modulation index $m_{\flux}$ of Rician fading as a function of the
	$K$-factor $\kappa$.}

%The unknown carrier phase $\theta$ is omitted
%from the ICH model of Figure \ref{fig:ICHidea} is because
%it has no influence in the face of the random phase of $S$.
%
%The implication of $\Theta$ is that there is no information
%present in the phase of MF output $Z = z(0)$.
%Only the magnitude $|Z|$ has relevance to questions like
%whether $\recenergy > 0$ or estimating the value of $\recenergy$.
%
%The magnitude of scintillation $R$ is, on the other hand, extremely significant
%to interstellar communication.
%Because it has a Rayleigh distribution, the similar phenomenon to scintillation
%is called ''flat Rayleigh fading'' by communication engineers.
%
%More specifically, $S$ is a complex-valued zero-mean circularly 
%symmetric Gaussian random variable
%with $E | S |^{2} = \vs$.
%If the ISM impairments were removed the effect would be $S = 1$,
%and hence we expect that $E | S |^{2} = \vs < 1$.
%It follows that the distribution of $R$ is
%\begin{equation}
%\label{eq:rayleighdist}
%f_{R} (r) = \frac{2 \, r}{\vs} \, \exp \left( - \frac{r^{2}}{\vs} \right)
%\ \ \ \ \text{and} \ \ \ \ \ 
% F_{R} (r) = 1 -  \exp \left( - \frac{r^{2}}{\vs} \right)
%\end{equation}
%The first and second moments of $R$ are
%\begin{equation}
%E [ R] = \frac{\sqrt{\pi \,  \vs}\,}{2}
%\ \ \ \ \text{and} \ \ \ \ \ 
%E [ R^{2}] = \vs
%\end{equation}

\subsection{Noise within a coherence hole}
\label{sec:noiseICH}

Suppose that the ISM introduces AWGN $N(t)$
with power spectral density $N_{0}$ into $r(t)$.
Then the noise at the MF output in Figure \ref{fig:ICHidea} is
\begin{equation}
\label{eq:noiseICH}
M = \int_{0}^{T} e^{-\,i\, 2 \pi \, f_{c} \, t} \, \cc h (t) \, dt \,.
\end{equation}
This random variable is (Appendix \ref{sec:modelICH}) zero-mean Gaussian with
variance $E|M|^{2} = N_{0}$, and
further $\Re \{ M \}$ and $\Im \{ M \}$ are independent and
have the same variance $N_{0}/2$.

It is significant that neither $B$ nor $T$ affects the statistics of $M$.
Thus, the statistics of the noise at the MF output do not change as $B$ and $T$ decrease, and thus
noise remains an important Category II impairment within an ICH.
The intuitive explanation for this is that within bandwidth $B$ the
total noise power is $N_0 B$, and thus the total noise energy within
time $T$ is $N_0 B T = N_0 K$.
Although this \emph{total} noise energy increases with $K$, the MF
extracts the noise in only one of those degrees of freedom and rejects the 
noise in the remaining $K-1$ degrees of freedom,
leaving a total noise energy in the direction of $h(t)$ equal to $N_0$
and independent of $K$.

\section{Frequency offset due to acceleration}
\label{sec:freqoffset}

When multiple energy bundles are transmitted, each bundle may experience
a different scintillation phase $\Phi$ and flux $\flux$.
In addition, the carrier frequency is offset according to any uncorrected acceleration
between source and observer along the line of sight.
This phenomenon is modeled in Chapter \ref{sec:incoherence}.
The significant sources of acceleration are the diurnal rotation of
a planet or moon about its axes and the orbital motion of a planet about its
host star or a moon about its host planet.
A transmitter and a receiver can readily correct the signal to remove the effects of
this acceleration based on their knowledge of the local orbital mechanics.
However, if either fails to make this correction, acceleration becomes more
important than scintillation in determining the coherence time $T_{c}$.
In addition, acceleration results in a carrier frequency offset between
two energy bundles separated in time.
If the receiver suspects or assumes the presence of acceleration,
this will affect the energy bundle pattern recognition algorithms in discovery,
and even more significantly the extraction of information from the signal.

\section{Time-bandwidth product and degrees of freedom}
\label{sec:channelmodeldof}

An important secondary parameter of the ICH is its time-bandwidth product
$K_{c} = B_c T_c$, which is called the \emph{degrees of freedom} (DOF).
$K_{c}$ is the number of complex numbers
that are required to fully specify any waveform $h(t)$ that falls in an ICH.
$K_{c}$ depends
on the specific line of sight (LOS) and the carrier frequency $f_{c}$.
If $K_{c} \le 1$, then interstellar communication becomes very difficult because
for all practical purposes the ICH does not exist, or putting it another way
the inherent incoherence of interstellar propagation between a source and observer
in relative motion severely distorts virtually any waveform $h(t)$ that we attempt to transmit.
This would be particularly problematic for discovery, since there is no opportunity
to estimate $h(t)$ in advance nor even observe the current ISM ''weather'' conditions
to infer some of its likely properties.
If on the other hand, if $K_{c} \gg 1$, then interstellar communication becomes
relatively straightforward, as will be shown in the remainder of this paper.
In Chapter \ref{sec:incoherence},
$K_{c}$ is estimated using the numerical values of Table \ref{tbl:assumptions}
and the result is shown in Figure \ref{fig:dofICH}.
It ranges from about $K_c = 1000$ to $10^5$ for the range $0.5 \le f_c \le 60$ GHz.
Thus, interstellar communication is quite feasible for all values of $f_c$ shown.
In addition, if both the transmitter and receiver correct for their respective accelerations
in the direction of the line of sight, then $T_{c}$ (and hence $K_{c}$) increases substantially.

\incfig
	{dofICH}
	{.8}
	{A log-log plot of $K_c = B_c T_c$, the degrees of freedom for an ICH,
	vs the carrier frequency $f_c$ for the numerical values of
	Table \ref{tbl:assumptions}.
	A safety factor of $\alpha = 0.1$ is assumed, except for acceleration
	where the safety factor is $\alpha = 0.01$.
	The components $B_c$ and $T_c$ are shown in Figure \ref{fig:btCoherence}.}


%In choosing an $h(t)$, we can choose $K = K_{c}$, so that the waveform
%essentially ''fills up'' the ICH, or alternatively we can choose $K \ll K_{c}$
%so that the DOF's of $h(t)$ is much smaller than the ICH would permit.
%Since a waveform $h(t)$ with bandwidth $B$ and time duration $T$ has $K = B T$
%DOF's, there is a great deal of freedom in choosing $h(t)$ unless $K \approx 1$.
%Choosing $h(t)$ is equivalent to choosing (a) a set of $K$ basis functions
%and (b) a set of $K$ complex-valued numbers that weight those basis functions.
%The sampling theorem argument specifies one particular set of basis functions,
%namely the time translates of a $\text{sinc} (\cdot)$ function.
%More generally, we can choose any set of $K$ basis functions
%$\{ g_{k} (t) , \, 1 \le k \le K \}$ which have the orthonormality property
%\begin{equation}
%\label{eq:basis}
%\int_{0}^{T} g_{m} (t) \, \cc g_{n} (t) \, dt =
%\begin{cases}
%1, & m = n \\
%0, & m \ne n \,.
%\end{cases}
%\end{equation}
%The $\text{sinc} (\cdot)$ functions of the sampling theorem have this
%property, and so do the complex exponentials $e^{\,i\,2 \pi \, k t /T}$ of a Fourier
%series expansion of a waveform precisely time-limited to $t \in [0,T]$.

The choice of $h(t)$ is of considerable importance from two perspectives.
First, the choice should be a waveform that the receiver can guess
in order to apply a matched filter, because
there is no possibility of conveying the precise $h(t)$ to the receiver prior to discovery.
Second, while the choice of $h(t)$ has no relevance to the
power efficiency of the system,
it does have considerable significance to the RFI immunity of the signal,
which argues for choosing as large a $K$ as possible \citeref{211}.
Of course, the largest value is $K = K_{c}$ consistent with the ICH.

\section{Some observations about the ICH}

We can consider ourselves fortunate that the ISM and source/observer motion
introduce impairments from the perspective of implicit coordination of transmitter and
receiver \citeref{583}.
The source and observer can independently
estimate $\{ T_{c} , B_{c} \}$ and the resulting $K_{c}$ based on common observable physical
characteristics of line of sight, and they should arrive at similar (although not identical) estimates.
This provides source and observer a common reference in choosing some free parameters
in the transmit signal $h(t)$, and reduces the ambiguity and the size of a discovery search
at the receiver.
In addition to RFI immunity, this is another strong argument for choosing $K = K_{c}$,
as this choice minimizes the ambiguity in $K$ between transmitter and receiver.
At the same time as ambiguity is reduced, ISM and motion impairments
(with the exceptions of noise and scintillation) do not adversely affect our ability
to communicate or introduce any added processing requirements.

The estimate of $\{ T_{c} , B_{c} \}$ depends on several circumstances:
\begin{description}
\item[Definition of coherence.]
Coherence improves gradually as $\{ T , B \}$ are decreased,
but perfection is not attainable.
How much coherence is enough depends to some extent on the usage; for example,
some information-representation schemes are more sensitive to incoherence 
(and to particular
types of incoherence) than others.
Thus the transmitter and receiver will adjust their definitions of coherence
somewhat (fortunately in compatible ways) based on other aspects of the system design.
\item[The line of sight and observer motion.]
Dispersion and scattering
and source/observer motion depend on the line of sight.
In particular, the relevant parameters of the line of sight from Table \ref{tbl:assumptions}
are the dispersion measure $\dm$, the diffraction scale $\rdiff$, and the distance $D$.
Astronomical observations yield considerable information \citeref{214}, but with some residual uncertainty.
A lot is also known about the motion impairments, which depend on the
radial acceleration $a_{\parallel}$ and the transverse velocity $v_{\bot}$.
This is particularly true of $a_{\parallel}$ because acceleration can be inferred from
an accelerometer or equivalently from modeling of the dominant sources of acceleration,
which are the orbit of a planet about its star as well as the revolution about its axis.
\item[Carrier frequency.]
All impairments depend on the wavelength (carrier frequency) in use.
\end{description}
Inevitably there will be some discrepancy between the source and observer estimates,
particularly in reference to the density of electrons along their line of sight
and the nature of their inhomogeneity.
Information about this is presumably due primarily to pulsar observations,
and the source and observer must base their estimates on pulsars that typically
have a different orientation relative to the line of sight.

There are also two forms of compensation that can be performed at the transmitter
and that have the effect of increasing the size of the ICH:
one is for acceleration and the other equalizes for the best-case dispersion
alone the line of sight (Chapter \ref{sec:incoherence}).
The receiver designer must therefore account for the possibility that the
transmitter may have compensated for one or both of these effects, or not.

One recurring question addressed in the following sections
is the significance of the numerical value of $K_{c}$ to interstellar communications.
What we will uncover is that $K_{c} \gg 1$ doesn't affect power efficiency
because the noise at the output of the MF does not depend on any aspect of
the shape of $h(t)$, including $B$ or $T$.
On the other hand, the effect of a filter matched to $h(t)$ on sources of RFI depends
on the detailed characteristics of the $h(t)$ waveform, and thus $K_{c}$ does
impact RFI immunity.
In the following sections ways of structuring a transmit information-bearing signal
based on the ICH will be described, followed by a calculation of fundamental limits,
and this point should then become clearer.


%\incxy
%	[@C=1cm] 
%	{coherenceholemodel}
%	{
%	An input-output model for the case where 
%	a transmit signal $A \, \sqrt{\energy_{t}} \, h(t)$ with energy $\energy_{t}$ falls within a coherence hole
%	and a matched filter is applied to that signal in the receiver.
%	The output $Z$ (which is essentially the same as $z(0)$ in
%	Figure \ref{fig:coherenceholetest}) is a complex-valued random variable which
%	can be used as the basis for making a decision about the value of $A$.
%	The impairments which cannot be eliminated by restricting $\{ B, T \}$ to $\{ B_{c}, T_{c} \}$
%	include a multiplicative
%	scintillation factor $S$ and an additive thermal noise $M$.
%	Of course the receive energy $\recenergy$ also reflects all sources of
%	attenuation during propagation through the ISM.
%	}
%	{
% 	A \, \sqrt{\recenergy} \ar@{=>}[r] 
%	&
%	*{\bigotimes} \ar@{=>}[r] 
%	&
%	*{\bigoplus} \ar@{=>}[r] 
%	&
%	Z
%	\\
%	& 
%	S \ar@{=>}[u] 
%	& 
%	M \ar@{=>}[u] 
%	}

\chapter{The fundamental limit}
\label{sec:fundamental}

As shown in Chapter \ref{sec:channelmodel},
most impairments can be circumvented by basing energy bundles
on a waveform $h(t)$ that falls within the
interstellar coherence hole (ICH).
The resulting channel model includes not only noise, but also
scintillation.
If it is to apply to the interstellar channel model, the fundamental
limit on power efficiency of Section \ref{sec:pelimit}
must be extended to include scintillation.
That is done in this chapter.
Our conclusion is that a similar tradeoff between spectral efficiency and
power efficiency holds, and the limit on power efficiency is not
changed by scintillation.
However, to approach that limit have to do more than
use M-ary FSK or M-ary PPM as described in Chapter \ref{sec:powerefficient}.

\section{Channel models}

Fundamental limits are based on particular channel models,
which hopefully are faithful to the underlying physical channel.
The first step is adding scintillation to the noise model of \eqref{eq:awgnchannel},
which does not yet model the interstellar channel because it fails to take
into account all the impairments other than noise and scintillation.
The second step is to deal with those other impairments by rendering them
insignificant through restriction of the channel model to base signals on the
interstellar coherence hole (ICH) described in Section \ref{sec:modelICH}.
The question is whether this restriction changes the fundamental limit,
and we demonstrate that it does not.

\subsection{Adding scintillation to noise}

Now add a multiplicative time-varying scintillation term $S(t)$ to the signal in \eqref{eq:awgnchannel},
\begin{equation}
\label{eq:scintillationchannel}
Y(t) = S(t) \cdot X (t) + N(t) \,,
\end{equation}
where $S(t)$ and $N(t)$ are statistically independent.
Note that the average power is
\begin{equation}
\expec{\left| S(t) \cdot X (t) \right|^{2}} = \expec{| S(t) |^{2} \cdot \expec{| X(t)|^{2}}}
= \vs \, \expec{| X(t)|^{2}}  = \expec{| X(t)|^{2}} \,,
\end{equation}
from \eqref{eq:sigmasone}.
Thus a constraint on the received average power $\power$ including the influence of
scintillation flux not affected by scintillation,
namely $\expec{X^{2} (t)} \le \power$.

\subsection{Basing communication on the coherence hole}

The ICH can form the basis for a practical interstellar communication system.
Suppose that a waveform $h(t)$ meets the constraints of an ICH.
This waveform can be transmitted repeatedly
with different time and frequency offsets.
In particular, let the $k$th repetition have time offset $\tau_k$
and frequency offset $f_k$, so it equals $h(t-\tau_k) \, e^{\,i\,2 \pi \, f_k t}$.
If these repetitions do not overlap one another
in time or frequency during transmission, then
a filter matched to one repetition
will have no response to any of the others.
Examples of this include M-ary FSK and M-ary PPM on a single carrier,
as well as replicating these signals on multiple carriers, as described in
Chapter \ref{sec:powerefficient}.

%This is very different from how terrestrial wireless communication systems
%are structured.
%There the primary goal is good spectral efficiency rather than power efficiency,
%and therefore the repetitions of $h(t)$ are always overlapped in time and frequency
%as much as feasible in order to conserve bandwidth.
%This makes the baseband signal processing in the receiver far and away more
%complex, because it has to sort out these overlapping repetitions even after
%they are distorted in an unknown way in the medium.
%The resulting processing also magnifies or ''enhances'' the noise, resulting
%in a penalty in power efficiency.
%In interstellar communication, assuming that spectral efficiency is a secondary
%consideration neither this added complexity and processing overhead,
% nor this noise penalty, is necessary.

To come up with the channel model appropriate for studying fundamental
limits, the input-output model of Figure \ref{fig:ICHidea} must be generalized.
That model is linear in $\sqrt{\energy_{h}}$, so that the sequence of
root-energies can be replaced by a general discrete-time complex-valued input signal $X_{k}$.
The resulting model is essentially a discrete-time version of \eqref{eq:scintillationchannel},
\begin{equation}
\label{eq:discretechannelmodel}
Z_{k} = S_{k} \cdot X_{k} + M_{k} \,.
\end{equation}
Both the random phase and magnitude of the scintillation have been included for generality.
As before the power constraint (as a discrete-time channel) is $F \cdot \expec{|X_{k}|^{2}} \le \power$,
where $F$ is the average rate at which the energy bundles are transmitted.
An interesting feature of this channel relates to $F$. 
In the power-efficient regime, the bandwidth of the signal is unconstrained, or equivalently
there is no constraint on $F$.
It is perfectly acceptable to let $F \to \infty$, as long as
$\expec{|X_{k}|^{2}} \le \power /F$ approaches zero.
This will prove to be significant.

The question to be answered is whether the power efficiency of this discrete-time
channel that is constrained to base its signals on the ICH is any less than that of \eqref{eq:scintillationchannel}.
The answer will be a qualified ''no''.

%The presence of scintillation puts severe restrictions on the choice of $A$.
%In fact, examination of the distribution of $Z$ in \eqref{eq:singleIU} reveals that
%any phase component in $A$ is obscured by the random phase
%introduced by scintillation (Appendix \ref{sec:withmod}).
%Thus there is no possible way for the
%receiver to extract useful information about the phase of $A$ from $Z$.
%The data constellation underlying $A$ must take this into account by not
%embedding any information in the phase of $A$, or equivalently
%$A$ must be chosen to be real-valued and $A \ge 0$.

%\section{Amplitude modulation}
%\label{sec:am}
%
%A waveform $h(t)$ can be used as a ''carrier''
%for information by exploiting the linearity of the channel model and employing amplitude modulation.
%In this approach the transmitted signal is proportional to $A \cdot h(t)$, rather
%than just $h(t)$, where
%$A$ is a complex-valued \emph{data symbol} drawn from a finite alphabet $\Omega$.
%
%In summary, the random and changing phase introduced by scintillation
%precludes using any form of phase modulation.\footnote{
%When there is expected to be a relatively small difference between $\Phi_{k}$
%and $\Phi_{k+1}$ in \eqref{eq:sequenceIU},
%then differential phase-shift keying (DPSK) is a possibility.
%Similarly, when there are two or more IU's per ICH, there will be
%phase coherence in the scintillation that can be exploited.
%}
%The simplest such constellation is \emph{on-off keying} or OOK,
%where $\Omega = \{ 0, 1 \}$ and thus $A = 0$ or $A = 1$
%depending upon a single information bit.
%Conceptually the number of alternatives for $A$ can be increased to
%$N >2$, thereby conveying $\log_{\,2} N >1$ bits of information.
%
%We call the association of data symbol $A$ with waveform $h(t)$
%an \emph{information unit} (IU).
%For \eqref{eq:singleIU} to be valid,
%the waveform $h(t)$ associated with a single IU must fall within a single ICH.
%This technique is called a \emph{single-use} ICH, because there is
%a one-to-one association between IU's and ICH's.
%It is possible to define a \emph{multi-use} ICH, in which
%two or more IU's are associated with a single ICH.
%This possibility is explored (for the special case of two IU's per ICH)
%in Appendix \ref{sec:multiuse}.
%One reason for undertaking this complexity is improved spectral efficiency,
%but this may be unimportant for interstellar communication.
%There are, however, other advantages that make this option worth considering.
%In the remainder of this paper, a single-use ICH will be assumed, and in particular
%it is shown that this simple approach can achieve the maximum possible power efficiency.
%
%\section{Single-carrier vs. multicarrier modulation}
%\label{sec:SCandMCM}
%
%An arbitrary number of single-use ICH's can be transmitted.
%As long as they are non-overlapping in both time and frequency,
%a filter matched to any one of them will not respond to any of the others.
%If a sequence of transmitted ICH's is labeled by an index $k$, the result is a discrete-time
%channel as illustrated in Figure \ref{fig:ICHsequence},
%and written mathematically as
%\begin{equation}
%\label{eq:sequenceIU}
%Z_k = \sqrt{\recenergy} \, \sqrt{\flux_{k}} \, e^{\,i\,\Phi_{k}} \, A_k + M_k \,.
%\end{equation}
%
%\incxy
%	[@C=1cm] 
%	{ICHsequence}
%	{
%	Extending the model for a single ICH in Figure \ref{fig:ICHidea},
%	a sequence of data symbols $\{ A_k \}$ can be communicated
%	by a one-to-one association of the data symbols $A_k$ with a
%	a sequence of ICH's.
%	If those ICH's are non-overlapping in time and frequency,
%	then this discrete-time model has statistically
%	independent noise samples $\{ M_k \}$.
%	The  phases $\Phi_{k}$ will generally change much faster
%	than the magnitudes $\sqrt{\flux_{k}}$.
%	}
%	{
%	\sqrt{\recenergy} \, A_{k} \ar@{=>}[r] 
%	&
%	*{\bigotimes} \ar@{=>}[r] 
%	&
%	*{\bigoplus} \ar@{=>}[r] 
%	&
%	Z_{k}
%	\\
%	&
%	\sqrt{\flux_{k}} e^{\,i\,\Phi_{k}} \ar@{->}[u] 
%	& 
%	M_{k} \ar@{=>}[u]
%	}
%	
%%One striking feature of the ICH model of Figure \ref{fig:ICHsequence}
%%is that the statistics of the $Z_{k}$ are Gaussian for both $\recenergy >0$
%%and $\recenergy = 0$.
%%The only effect of $\recenergy>0$ is to increase the energy in $Z_{k}$,
%%and due to the circular symmetry in the distribution of $Z_{k}$ there is
%%no information in the phase.
%%Thus, the discovery of a signal must of necessity be based on an estimate of
%%the energy, or equivalently the magnitude of the MF output $|Z|$.
%%
%%A basis $g_{k} (t), \, 1 \le k \le B_{c} T_{c}$
%%
%%$N_{0}$ is unknown
%
%%Two other important parameters that affect the reliability
%%of decision making are $\recenergy$, the received energy per IU,
%%and $I_{U}$, the number of information bits per IU.
%%The resulting model for the reception is
%%shown on the right side of Figure \ref{fig:ICHsequence}.
%%The noise samples $M_{k}$ are independent from one ICH to another,
%%and we cannot depend on any relationship between scintillation
%%values $S_{k}$ either.
%%An exception to this rule is that
%%there may be some correlation in $|S_{k}|$ from one $k$ to another
%%if the scintillation coherence time is greater than the ICH coherence time
%%(the latter may be dominated by acceleration rather than scintillation).
%
%Some specific and sensible options for how these ICH's can be separated
%in time and frequency are
%illustrated in Figure \ref{fig:IUstructure}.
%As shown in Figure \ref{fig:IUstructure}(a)  all IU's
%are assumed to have the same time duration $T_0 \le T_c$ and
%bandwidth $B_0 \le B_c$, all are presumed to use the same
%baseband waveform $h(t)$.
%One option shown in Figure \ref{fig:IUstructure}(b)
%uses the same $f_{c}$ for all the IU's, so they overlap in frequency but not in time.
%This is called \emph{single-carrier modulation}.
%Another option shown in Figure \ref{fig:IUstructure}(d) is to transmit
%two or more such streams on different carriers with sufficient spacing that
%their spectra do not overlap.
%This is called \emph{multicarrier modulation} (MCM).
%Both approaches have the feature that the IU's are transmitted
%at a constant rate.
%If that rate is called $F$, then the information rate $\rate$ is
%$\rate = N \, F$, where $N$ is the number of information bits 
%mapped into each IU.
%For the example of OOK, the value of $N$ is $N=1$.
%
%\incfig
%	{IUstructure}
%	{.8}
%	{The structure of a transmitted signal utilizing a single carrier
%	or multiple carriers.
%	In (a) the chosen parameters $\{ T_{0}, B_{0}, f_{c} \}$ of a single 
%	information unit (IU) are labeled.
%	In (b) a stream of IU's are transmitted at rate $1/T_{0}$.
%	If either a lower or higher information rate is desired,
%	then the remaining options are available.
%	In (c) the rate of IU's is lowered to less than $1/T_0$
%	by spacing the IU's out in time, and in
%	(d) the rate of IU's is increased by transmitting $M$ streams
%	of IU's (shown is $M=2$) with different values of $f_{c}$ chosen so that
%	their spectra are non-overlapping.
%	}

%It is attractive in this case to space these IU's by $T_{0}$ so as to minimize
%the peak transmitted power.
%If in addition,
%the energy of $h(t)$ is spread uniformly over time $T_{0}$ then
%the peak transmitted power is minimized because it is equal to the average transmitted power.
%For example, $h(t)$ can be a sinusoid, or alternatively a spread spectrum signal chosen to maximize the
%RFI immunity in the receiver \citeref{211}.


%In fact, this power corresponds to the minimum power that is useful for an
%interstellar beacon that is designed to attract attention without embedding information.
%
%Second, if the bandwidth of each IU is $B_{0}$, then that bandwidth must conform to $B_{0} \le B_{c}$.
%Due to the constraint that $B_{0} T_{0} \ge 1$,
%it follows that $T_{0}$ is also lower bounded by $T_{0} \ge 1/B_{c}$.
%Thus in the approach of Figure \ref{fig:IUstructure}(b) there is also an
%\emph{upper} limit on the rate $\rate \le I_{U} B_{c}$ that can be achieved.
%This upper bound is more severe if there is a desire to increase the signal
%degrees of freedom by choosing $K_{0} = B_{0} T_{0} \gg 1$, for example
%in the interest of greater RFI immunity at the receiver \citeref{211}.
%In that case the maximum rate for a single stream of IU's is reduced to $\rate \le I_{U} B_{c}/K_{0}$.
%
%Suppose the transmitter has more power available and wishes to leverage that power
%to increase the information rate.
%There is a simple way to do this, as illustrated in Figure \ref{fig:IUstructure}(c).
%The transmitter can simply transmit $M$ streams of ICH's concurrently using
%different carrier frequencies chosen so that the frequency spectra do not overlap.
%If bandwidth is unconstrained, there is no limit on $M$, but of course at some point
%the available transmit power is exhausted.
%The total information rate is then $\rate = M\, I_{U} / T_{0}$ bits per second
%and the total average power is $\power = M \, \recenergy / T_{0}$,
%so the tradeoff $\rate \propto \power$ is preserved, the power efficiency is
%not altered, and the peak transmitted power remains equal to the average transmitted power.
%If bandwidth is considered to be unconstrained, the total information capacity of the ISM
%is also unconstrained, even under the condition that the structure of the signal conforms to
%the ICH so that there is no transmit or receive processing associated with ISM impairments.

\section{Fundamental limits on interstellar communication}

Generalizing the capacity formula of \eqref{eq:capacity} to
a channel model including scintillation is dependent in part of the assumptions
about knowledge of the current conditions on scintillation on the part of
transmitter and receiver \citeref{632}.
For a simple intuitive explanation of these options, \citerefWloc{574}{Sec. 5.4} is recommended.
In interstellar communication, it is apparent that the transmitter has no knowledge of the
current state of the scintillation.
The receiver, on the other hand, has the ability to estimate the current scintillation flux
$\flux$ by observing the fluctuations in received power.
By observing these fluctuations over a period of time, it should be possible to
distinguish the effects of scintillation from the uncertainty in transmitted power,
since the latter, although unknown, should at least not vary with time. 

%The impairments introduced by the ISM are familiar, replicating similar impairments
%in terrestrial systems with a different parameterization.
%
%This section addresses fundamental limits in communication, and 
%Chapter \ref{sec:discovery} considers fundamental limits in discovery.
%
%Our approach to fundamental limits follows that of the ICH,
%and uses only power efficiency as the metric of performance.
%We first derive limits on power efficiency in the presence of Category II impairments that characterize the ICH;
%namely, AWGN with power spectral density $N_{0}$ watts per Hz (or equivalently Joules)
%and scintillation with variance $\vs$.
%This neglects all the other Category I impairments due to the ISM and source/observer motion.
%Obviously those other impairments, if considered,
%would not increase the achievable power efficiency.
%However, we then demonstrate that a communication design structured around the ICH
%and ignoring spectral efficiency can approach those very same fundamental limits.
%This demonstrates that in fact for unconstrained bandwidth
%the neglected impairments do not have to reduce the power efficiency.
%This result also strongly suggests that structuring the signal around the ICH,
%in spite of its simplicity, is a meritorious design approach
%that both transmitter and receiver designers would be well advised to employ.
%
%\section{Tradeoff between power efficiency and spectral efficiency}
%\label{sec:tradeoff}
%
%Consider first the effect of additive noise alone, neglecting scintillation.
%In particular, the design approach described in 
%Chapter \ref{sec:channelmodelstructure} is moderately
%to highly inefficient in its use of bandwidth (depending on the choice of $K$)
%because it does not attempt to overlap IU's in time or frequency,
%and this is one reason it is able to achieve the proportionality $\rate \propto \power$
%that characterizes the fundamental limit.
%The constant of proportionality is a different matter, as explored in the context of
%a concrete design in Chapter \ref{sec:infosignals}.
%

\subsection{Channel coding}
\label{sec:channelcoding}

The right-hand side of limit \eqref{eq:capacity} is the \emph{channel capacity} $\capacity$.
To fully understand capacity, it is helpful to appreciate that
achieving reliability for $\rate \le \capacity$ requires \emph{channel coding}.
The basic idea behind channel coding is illustrated in
Figure \ref{fig:blockcoding}.
In a \emph{block} code at information rate $\rate$ bits per sec,
a block of $\rate \cdot T_{b}$ bits is translated into one of $2^{\rate \cdot T_{b}}$ codewords
of length $T_{b}$ seconds and that codeword is transmitted through the noisy channel.
At the receiver, the codeword most representative of the reception is chosen and converted
back to  $\rate \cdot T_{b}$ bits.
Essentially this scheme spreads
each and every bit over the entire codeword of $T_{b}$ seconds,
so the effects of noise are averaged out in the detection of that bit.
Shannon's remarkable insight was that there exists a codebook
(mapping from $\rate \cdot T_{b}$ bits into $2^{\rate \cdot T_{b}}$ codewords)
such that the error probability approaches zero as $T_{b} \to \infty$,
if (but only if) $\rate \le \capacity$.

\textbox
	{Channel coding is a big subject}
	{
Shannon's clever proof that communication is subject to fundamental
limits introduced the idea of channel coding.
However, he only proved the conditions under which a good channel
code is possible (the rate is below capacity), but the proof did not
construct any actual channel codes.
In the spectrally efficient domain finding actual codes that
are practical is very difficult, as the complexity of a channel code grows
exponentially with the memory of the code.
Thus, researchers were forced to search for codes that had an
algorithmic structure to deal with this complexity, and after decades of incremental
improvement the problem was essentially solved by 1993, based on part on
the declining cost of memory and processing.
Fortunately, however, in the power-efficient domain where bandwidth is unconstrained,
finding channel codes that approach capacity proved relatively easy, and this
problem was essentially solved by 1960 for the AWGN channel and by 1969 for
the AWGN channel with scintillation.
In fact, the capacity of the scintillation channel was established by a very
different approach from that originally proposed by Shannon.
It was observed that scintillation can only reduce the capacity, so the
best possible circumstance is if scintillation does not affect the capacity.
Concrete channel codes were then demonstrated that achieved the AWGN capacity
on the scintillation channel.
Remarkably, this achievement did not depend on any knowledge of the
state of the scintillation at either the transmitter or receiver.
This work is thus directly applicable to interstellar communication.
%It was five decades from Shannon's original paper until practical \emph{turbo} codes that
%could approach his bounds for the general
%Gaussian noise channel were invented \citereftwo{618}{167}.
%However, for the unconstrained bandwidth case appropriate for interstellar
%communication, it has long been known that a simpler class of 
%\emph{orthogonal} codes can approach capacity \citeref{633},
%and this class of codes has been proposed for interstellar communication
%(although omitting consideration of the ISM impairments)  \citeref{196}.
%The use of channel coding in interstellar communication
%creates an additional layer of obfuscation that makes extraction of information more difficult
%(although it should not interfere with discovery).
%Thus, we would question the applicability of channel coding to interstellar communication,
%and our concrete design of Chapter \ref{sec:infosignals} omits channel coding.
	}

\incxy
	[@C=.7cm] 
	{blockcoding}
	{
	The basic idea behind channel coding is to divide the raw data
	into blocks, and for each block translate the block of data into
	a codeword which is corrupted by noise.
	At the receiver, the codeword most representative of the reception is chosen
	and converted back to data.
	On a fading channel, this structure is likely to be combined with interleaving \citeref{574}.
	}
	{
	*+{\begin{matrix}
			\text{Input} \\
			\text{data}
		\end{matrix}
		}
	\ar@{->}[r] &
		*+<1pc>[F-,]{
			\begin{matrix}
			\text{Channel} \\
			\text{coding}
			\end{matrix}
			}
		\ar@{->}[r] &
		*{\bigoplus}
		\ar@{->}[r] &
		 *+<1pc>[F-,]{
			\begin{matrix}
			\text{Channel} \\
			\text{decoding}
			\end{matrix}
			}
		\ar@{->}[r] &
		*+{\begin{matrix}
			\text{Output} \\
			\text{data}
		\end{matrix}
		}
		\\
		&& \text{Noise} \ar@{->}[u] 
		        }




\subsection{Ergotic capacity}
\label{sec:ergotic}

When the assumption is made that the receiver (but not transmitter)
has knowledge of the current state of scintillation $S(t)$ at all times,
the capacity is relatively simple to determine.
This is called the \emph{ergotic capacity}, the formula for which is a
simple adaptation of \eqref{eq:capacity},
\begin{equation}
\label{eq:ergoticcapacity}
\capacity = \expec{B \cdot \log_{2} \left( 1 + \frac{\power \, \flux}{N_{0} B} \right)} \,.
\end{equation}
The expectation $\expec{\cdot}$ is with respect to the random ensemble for $\flux$.
This applies to the general case where both power $\power$ and bandwidth $B$ are constrained.

The assumptions behind the ergotic capacity
 can be summarized as follows  \citerefWloc{574}{Sec. 5.4.5}.
For any fixed value $\flux_{t} = \flux$, the received power is scaled by $\flux$
and thus \eqref{eq:capacity} applies with total power $\power \flux$.
This ''instantaneous'' capacity is increased relative to the noise-only case if $\flux >1$
or decreased if $\flux < 1$.
As the actual flux $\flux_{t}$ changes with time, this ''instantaneous'' capacity also changes,
and \eqref{eq:ergoticcapacity} is the average of these instantaneous capacities.\footnote{
The term ''ergotic'' refers to an equality between a time average
and ensemble average.
This definition of capacity assumes that the time-average capacity is equal to the
ensemble-average capacity, which will be valid for a wide range of conditions.}

The definition of ergotic capacity assumes
that the transmitter has no knowledge of the value of $\flux$ at any given time.
This is clearly a necessary assumption for interstellar communication, 
since the propagation delay is very large relative to any
time scale over which $\flux$ changes appreciably.
It assumes that the transmitter does know the statistics of $\flux$.
This is a valid assumption because the transmitter presumably is 
aware of the strength of the scattering to expect on a given line of sight.
The transmitter cannot tailor the channel code at different times according to the
instantaneous conditions.
The transmitter can, however, use a channel code with a block length that is very large
relative to the known time scale of the fluctuations in $\flux$,
and also tailor the code to the known distribution of the scintillation.
In this case each code word statistically experiences the full range of $\flux$ for which it is designed.\footnote{
In practice the transmitter is likely to employ interleaving together with a shorter block length
to achieve a reliable information rate approaching \eqref{eq:ergoticcapacity}.}
This approach does introduce a very large delay in the reception and decoding of each
code word, but that should not be an issue for interstellar communication,
where the propagation delay is already very large relative to the typical
timescale of scintillation.

While \eqref{eq:ergoticcapacity} cannot be reduced to a closed-form expression in general,
as always the power-efficient domain is easier.
Substituting the approximation of \eqref{eq:capproxBlarge},
which assumes unconstrained bandwidth $B$,
into \eqref{eq:ergoticcapacity},
\begin{equation}
\label{eq:scincapacity}
\capacity
\underset{B \to \infty}{\longrightarrow} 
\expec{ \frac{\power \, \flux \, \log_{2} e}{N_{0}} }
= \frac{\power \, \vs \, \log_{2} e}{N_{0}}
\end{equation}
Thus, the global maximum ergotic power efficiency becomes
\begin{equation}
\label{eq:powerescin}
\powere \le \powerescin = \frac{\vs \, \log_{2} e}{N_{0}} \,.
\end{equation}
The \emph{energy contrast ratio per bit} is defined as
\begin{equation}
\label{eq:ecrb}
\ecrb = \frac{\energybit \, \vs}{N_{0}} \,.
\end{equation}
Note the similarity to definition \eqref{eq:ecrs}, simply replacing $\energy_{h}$
by a normalized energy per bit $\energybit$.
Expressed in terms of \eqref{eq:ecrb}, the bound on power efficiency of \eqref{eq:powerescin} becomes
\begin{equation}
\ecrb \ge \log_{e} 2
\end{equation}
This is equivalent to the earlier bound for the AWGN channel \eqref{eq:ecrawgn},
with the addition of $\vs$ reflecting the fact that scintillation has been added to the model.

This same bandwidth-unconstrained ergotic capacity 
applies to both strong and weak scattering, and further in both cases
 $\vs = 1$ from \eqref{eq:sigmasone}.
Comparison of \eqref{eq:powerescin} and \eqref{eq:poweremaxAWGN} thus
reveals the startling conclusion that scintillation due to scattering
has no effect on the fundamental limit for ergotic power efficiency.

\subsection{Capacity of the unconstrained-bandwidth Rayleigh fading channel}

As we have seen, ergotic capacity is simple to calculate but makes the strong
assumption that the receiver has knowledge of the current state of scintillation.
A stronger result due to R.S. Kennedy in 1969 \citeref{637} is that the bandwidth-unconstrained limit on power efficiency of \eqref{eq:powerescin}
is unchanged when the receiver has no knowledge of the scintillation. 
In other words, the presence or absence of
knowledge of the current state of scintillation in the receiver
does not affect the achievable power efficiency.
More surprising than this conclusion is the way in which it was derived,
by actually demonstrating a channel code that achieves the fundamental limit asymptotically.
Building on the known capacity of the AWGN channel without scintillation,
Kennedy noted that scintillation could not increase the capacity, 
and then demonstr a channel code
that achieves the AWGN capacity in the presence of scintillation.
For a more modern and concise exposition of this result, \citerefWloc{638}{Section II} is recommended.

Kennedy's construction of a channel code builds on the five principles of
power-efficient design in Section \ref{sec:principles}.
In fact, that is where we got these five principles.
These principles used in combination suffice
to approach the fundamental limit on power efficiency.
However, this result applies to the channel model of \eqref{eq:scintillationchannel},
which is not directly applicable to interstellar communication because it
ignores all the additional impairments discussed in Chapter \ref{sec:incoherence}.
Thus, our final step in deriving a fundamental limit that applies to
interstellar communication is to show that the $B$-unconstrained power efficiency of \eqref{eq:powerescin}
equals the $F$-unconstrained capacity of the discrete-time model of \eqref{eq:discretechannelmodel}.

\subsection{Communication structured on the ICH}

Consider a communication system based on the discrete-time
model in \eqref{eq:discretechannelmodel}, or in other words
a design making use of energy bundles that fall within the ICH and thereby render
negligible all impairments other than noise and scintillation.
The ergotic capacity for finite $F$ is easily calculated,
and as $F \to \infty$ the resulting limit on power efficiency is precisely \eqref{eq:powerescin}.
See Appendix \ref{sec:capacity} for a derivation of this result.
This establishes that the fundamental limit on power efficiency of \eqref{eq:powerescin}
applies to interstellar communication, even taking into account all impairments.
Because it is based on ergotic capacity, it does
assume that the receiver has knowledge of the state of the scintillation.
It also presumes, of course, that the ICH exists as a viable basis for design, or $K_{c} \gg 1$.

%It is also demonstrated in Appendix \ref{sec:capacity} that the fundamental
%limit on power efficiency for a discrete-time communication system
%based on a sequence of ICH's
%(as represented by the model in Figure \ref{fig:ICHsequence}) is also \eqref{eq:powereffscintillation}.
%A lower limit on
%the energy associated with each IU conveying $I_{U}$ information bits follows,
%\begin{equation}
%\recenergy \ge \frac{I_{U} \, N_{0} \, \log_{\,e} 2}{\vs}\,.
%\end{equation}

This is a deceptively simple result, but one with profound implications.
Building on the ICH structure does not reduce the
achievable power efficiency under the assumption that the receiver is able
to accurately estimate the current state of the scintillation.
There is no danger that an advanced civilization can achieve a power
efficiency higher than what is achievable by structuring the
transmit signal on energy bundles, which are in turn structured around the ICH.
In fact, this result is stronger that it appears because any transmitter design that
violates ICH integrity introduces additional ISM and motion impairments into the
received signal, and we would expect that dealing with these would reduce the power efficiency.
A reasonable hypothesis is that a design based on the ICH structure can achieve greater power efficiency
than any design that deliberately violates the integrity of the ICH.

It is important, and perhaps somewhat surprising, that the fundamental limit on power efficiency
is \emph{not} affected by the size of the ICH represented by parameters $\{ B_{c}, \, T_{c}, \, K_{c} \}$,
assuming of course that $K_{c} \gg 1$.
Intuitively this is because the only impact of the ICH size is
the rate at which IU's can be transmitted for a single carrier and the bandwidth of
that single carrier.
If it is necessary to increase $\rate$ by going to MCM, that further increases
the total bandwidth, but does not affect the power efficiency.
Another practical impact of ICH size is the achievable RFI immunity, but that measure is not incorporated
into the power efficiency measure and thus does not affect it.

Can knowledge of the state of
the scintillation in the receiver can be relaxed, as on the continuous-time
channel?
Probably not, since the channel code defined by Kennedy \citeref{637}
has one design feature that violates the conditions for an ICH.
This is a duty cycle $\delta \to 0$, which under the constraint $B T \gg 1$
implies a growing bandwidth that
eventually exceeds the coherence bandwidth.
This suggests (although does not prove) that the power efficiency
is slightly poorer for interstellar communication when no side
information about the scintillation is available to the receiver.

\chapter{Power-efficient information-bearing signals}
\label{sec:infosignals}

Having established the fundamental limit on power efficiency
in Chapter \ref{sec:fundamental},
the question is how close this limit can be approached
with a relatively simple concrete design of an information-bearing signal.
A concrete design is now undertaken as an illustration of
 an end-to-end interstellar communication system based on
 energy bundles, as illustrated earlier in Chaper \ref{sec:powerefficient},
 those energy bundles avoiding most impairments by restricting the
 waveform $h(t)$ to fall in the interstellar coherence hole (ICH)
 described in Chapter \ref{sec:channelmodel}.
According to the classification of Figure \ref{fig:threelayers} 
proposed in \citeref{583}, this design
only addresses the signal layer, omitting the reliability and message layers.
The signal layer is intrinsically unreliable,
due to noise and scintillation, and thus the
design of the reliability and message layers will be strongly affected by the
results described here.


%In Chapter \ref{sec:discovery}, the design of power-efficient beacons
%was undertaken, and it was found that they are intrinsically information-bearing.
%The question is, is a beacon designed in part for its information-bearing
%properties also power efficient?
%For that purpose, power efficiency $\powere$ is defined in the information sense
%(information rate divided by average received power),
%and that $\powere$ can be compared to the fundamental bounds
%developed in Chapter \ref{sec:fundamental}.
%
%The design of power-efficient information-bearing signals is
%very much easier than spectrally-efficient signals.
%One manifestation of that is the low-complexity
%channel codes that can achieve channel capacity for an AWGN 
%channel if bandwidth is unconstrained.
%This is in sharp
%contrast to the bandwidth-constrained case, where many decades
%of intensive research was needed to find capacity-achieving codes.
%The resulting codes were also very complex, making them
%problematic for interstellar communication where end-to-end
%coordination is not feasible.
%
%In this Chapter we make use of that past work to find
%a power-efficient design of an information-bearing signal.
%The resulting signal has similar characteristics to the power-efficient beacons
%that were designed in Chapter \ref{sec:discovery}.
%The reason is that trying to convey as much information as possible
%using a signal that is intermittent with as little transmission time as possible
%is the standard approach to achieving power efficiency.
%In fact, we will find signal designs that are simultaneously power-efficient
%as beacons and as information bearers.
%Putting the two requirements together beneficially constrains the
%signal structure and parameterization, providing yet another form of
%implicit coordination between transmitter and receiver.
%This implies that a separate beacon is unnecessary, and
%highly power-inefficient as well.

\incxy
	{threelayers}
	{
	Three distinct layers of functionality
	in the interstellar communication of messages \citeref{583}.
	These are the signal layer (including generation and detection),
	the reliability layer (including redundancy and assertion),
	and the message layer (including creation and interpretation).
	Our concrete design considers only the signal layer,
	but demonstrates that the reliability layer
	must deal with not only random dispersed errors but also
	substantial periods with no recovered data due to scintillation.
	}
	{
		*+<1pc>[F-,]{
			\begin{matrix}
			\text{Message} \\
			\text{creation}
			\end{matrix}
			}
		\ar@{=>}[r] &
		*+<1pc>[F-,]{
			\begin{matrix}
			\text{Reliability} \\
			\text{redundancy}
			\end{matrix}
			}
		 \ar@{=>}[r] &
		 *+<1pc>[F-,]{
		 	\begin{matrix}
			\text{Signal} \\
			\text{generation}
			\end{matrix}
			}
		  \ar@{=>}[r] &
		  	{
		  	\begin{matrix}
			\text{Radio} \\
			\text{channel}
			\end{matrix}
			}
		  \\
			{
			\begin{matrix}
			\text{Radio} \\
			\text{channel}
			\end{matrix}
			}
		 \ar@{=>}[r] &
		*+<1pc>[F-,]{
			\begin{matrix}
			\text{Signal} \\
			\text{detection}
			\end{matrix}
			}
		\ar@{=>}[r] &
		*+<1pc>[F-,]{
			\begin{matrix}
			\text{Reliability} \\
			\text{assertion}
			\end{matrix}
			}
		 \ar@{=>}[r] &
		 *+<1pc>[F-,]{
			 \begin{matrix}
			\text{Message} \\
			\text{interpretation}
			\end{matrix}
		 } & \\
      }

%A structure within the signal generation and detection layer that can approach the
%global maximum power efficiency $\powerescin$ of \eqref{eq:powerescin}
%is shown in Figure \ref{fig:channelcoding}.
%This recognizably requires complex channel coding, as described in Section \ref{sec:channelcoding}.
%This channel coding is omitted here, and as a result a gap between the power efficiency and the
%fundamental bound of \eqref{eq:powerescin} is opened up.
%The size of that gap is quantified.
%Also, only the strong scattering case is considered because the resulting
%Rayleigh fading statistics give simple analytical results.
%Weak scattering, which can only be dealt with numerically, will generally
%give more favorable results.
%
%\incxy
%	[@C=.7cm] 
%	{channelcoding}
%	{
%	The major functions in the signal generation and detection
%	layer, assuming the ICH structure so that there is no ISM-specific
%	signal processing in the transmitter or receiver.
%	In the design undertaken here channel coding is not included, which
%	contributes to a gap between the achieved power efficiency and the
%	fundamental limit.
%	}
%	{
%	\text{Data} \ar@{=>}[r] &
%		*+<1pc>[F-,]{
%			\begin{matrix}
%			\text{Channel} \\
%			\text{coding}
%			\end{matrix}
%			}
%		\ar@{=>}[r] &
%		*+<1pc>[F-,]{
%			\begin{matrix}
%			\text{Amplitude} \\
%			\text{modulation}
%			\end{matrix}
%			}
%		 \ar@{=>}[r] &
%		 \text{ISM}
%		  \ar@{=>}[r] &
%		  *+<1pc>[F-,]{
%		 	\begin{matrix}
%			\text{Matched} \\
%			\text{filtering}
%			\end{matrix}
%			}
%		 \ar@{=>}[r] &
%		 *+<1pc>[F-,]{
%			\begin{matrix}
%			\text{Channel} \\
%			\text{decoding}
%			\end{matrix}
%			}
%			\ar@{=>}[r] &
%			\text{Data}
%		        }

%\section{Discrete-time channel model}
%
%The basis for our design is the discrete-time channel model 
%of Figure \ref{fig:ICHsequence} and \eqref{eq:sequenceIU}.
%All signal terms in this baseband model are complex-valued.
%Absent channel coding, the mapping from information bits to data symbols
%$\{ A_{k} \}$ is memoryless.
%The information can be extracted by processing the received $\{ Z_{k} \}$.
%The  $\{ M_{k} \}$ is a sequence of additive noise samples
%and the  $\{ \sqrt{\flux_{k}} \, e^{\,i\,\Psi_{k}} \}$ is a sequence of scintillation amplitudes
%(both magnitude and phase).
%For the assumed strong scattering case, $\sqrt{\flux_{k}} \, e^{\,i\,\Psi_{k}} = S_{k}$
%where $S_{k}$ is a zero-mean complex-valued Gaussian random variable.
%The $\{ M_{k} \}$ in \eqref{eq:sequenceIU} are statistically independent.
%The $\{\flux_{k} \}$ are normally not statistically independent,
%and may vary slowly when the magnitude of the time coherence scintillation is on a longer time-scale
%than other forms of incoherence that dominate $T_{c}$.

\section{Dealing with scintillation}

Scintillation is manifested by a variation in received signal flux
as described in Section \ref{sec:scintillation}.
This impacts discovery, requiring multiple observations
to have a good chance of observations occurring during 
periods of relatively high flux as discussed in Chapter \ref{sec:discovery}.
Following discovery, the receiver moves into communication mode,
where the information is extracted from the signal.
The question is how to deal with scintillation during communication,
since the location of the signal is known and thus multiple observations
are not helpful.
Two strategies will be analyzed and compared: Outages and diversity.

\subsection{Outage strategy}

The approach in using an outage strategy is to suspend operations
during periods of low received signal flux.
As assumed in the calculation of ergotic capacity in
Section \ref{sec:ergotic}, it is assumed that the receiver can
estimate the received signal flux.
Time can then be divided into two situations:
outage time, when the received flux is too small to reliably extract
information, and non-outage time, when the received flux is larger. 
During non-outages information is
recovered with some error probability $\pe \approx 0$,
and during outages the information embedded in the signal is
simply discarded.

Define $\po$ as the probability of an outage, or equivalently the fraction of
time spent in outages.
Then the power efficiency can be defined as
\begin{equation}
\label{eq:powereoutage}
\powere = \frac{(1 - \po) \cdot \rate }{\power} = \frac{1 - \po}{\energybit} \,.
\end{equation}
The $(1-\po)$ factor takes into account the reduction in actual recovered
information rate due to the loss of all information during outages.
$\rate$ is the information rate embedded in the information-bearing signal,
and $\power$ is the average received power with or without scintillation
(which are the same since $\vs = 1$).

One outcome of discovery is not only a declaration of signal presence,
but also estimates of signal level (represented by scintillation flux
$\flux$) and noise power density (represented by $N_0$).
During communication these variables can be tracked, and
thus we assume that the current received signal flux $\flux$ and noise power density $N_0$ are known
quantities to the receiver during communication.
The receiver can thus declare an outage when $\flux < \oot$,
where $\oot$ is the \emph{outage threshold}.
For a chosen $\oot$, the outage probability is
\begin{equation}
\label{eq:poutage}
\po = \prob{ \flux < \oot } = 1 - \exp \left\{ - \frac{\oot}{\vs} \right\} \,.
\end{equation}
During non-outages, the reliability of information recovery still varies
widely depending on the actual flux $\flux$.
Our criterion for setting $\oot$ is to insure that $\pe \approx 0$
in the worst case, which is $\flux = \oot$.
At all other times during non-outages the reliability is even better, and usually \emph{much} better.
It is useful to remember that when $\pe$ is calculated for $\flux = \oot$,
this is not representative of the overall average error probability during non-outages,
which is much smaller.
All subsequent calculations of $\pe$ assume that $\flux = \oot$.
The received energy per bit at the threshold of outage is not $\energybit$,
but rather $\energybit \oot$.

Two definitions of the energy contrast ratio at the MF output have been displayed,
$\ecrs$ in \eqref{eq:ecrs} and $\ecrb$ in \eqref{eq:ecrb}.
In the context of outages, it is appropriate to display a third definition,
\begin{equation}
\label{eq:ecro}
\ecro = \frac{\energybit \, \oot}{N_{0}} \,.
\end{equation}
This is equivalent to the definition of $\ecrb$, except that the
average flux $\vs$ has been replaced by the flux at the threshold of outage $\oot$.

What is the appropriate choice of threshold $\oot$?
A principled way to choose $\oot$ (and hence $\po$) is to maximize the
power efficiency $\powere$, or in other words maximize the average rate at which
information is extracted from the signal taking into account the loss of information during outages.
This choice can only be considered in the context of a specific channel code,
and will be repeated below for OOK and M-ary FSK.

\subsection{Diversity strategy}

Diversity combining is one of the
principles of power-efficient design of Section \ref{sec:principles},
and a technique that has been shown to contribute to
approaching the fundamental limit on power efficiency \citereftwo{637}{638}.
It is more complicated than the outage strategy, but also much more
sophisticated since it can approach $\pe \approx 0$ without
loss of data due to periods of low signal flux.
The idea behind time diversity is to transmit each
information symbol multiple times with a time spacing large
relative to the coherence time of the channel, or a frequency spacing
large relative to the coherence bandwidth of the channel.
At the receiver, diversity combining averages the signal energy
from these redundant versions of the symbol to form an
estimate that asymptotically averages out the received flux
and thus allows reliable extraction of the information in spite of scintillation.

Replacing an outage strategy with time diversity combining increases the
power efficiency, but also
benefits the reliability and message layers of Figure \ref{fig:threelayers},
since the 37\% outage loss of information places a large burden on these
layers.
Time diversity can eliminate this loss of information, and replace it with a more or
less uniform probability of error $\pe$ on all the information, not just the information
that happens to arrive during periods of relatively high received signal flux.
On the other hand, time diversity adds another complication to the signaling
scheme which must be reverse engineered by the receiver, whereas
an outage strategy has no impact on the transmitted signal at the signal processing
layer in Figure \ref{fig:threelayers}.

Time diversity combining will be analyzed in a future version of this report.

\section{Channel codes}

In our concrete design of an interstellar communication system,
two specific channel codes will be analyzed: OOK and M-ary FSK.
These were described in Chapter \ref{sec:powerefficient}.
OOK is a baseline choice that does not attempt to maximize power efficiency,
while M-ary FSK is one element of the channel code that asymptotically
achieves the fundamental limit on power efficiency in the AWGN plus scintillation channel \citereftwo{638}{639}.
(Other elements are time diversity combining and low duty cycle.)
In both cases there is a gap to the fundamental limit, and comparing them gives a sense
of the improvement in power efficiency that is feasible using relatively simple channel codes.

A two-dimensional representation of the pattern of energy bundles
in OOK and in M-ary FSK is shown in Figure \ref{fig:OOKvsFSKtwoD}.
This illustrates how energy bundles are arranged in time and frequency
to convey a stream of information.

\incfig
	{OOKvsFSKtwoD}
	{.8}
	{
	OOK and M-ary FSK (for $M=8$) are illustrated in a two dimensional diagram of
	time vs. frequency.
	Each bundle of energy (and the time duration and bandwidth of the waveform $h(t)$
	representing that bundle) is shown as rectangle.
	The absence of an energy bundle in a location it might potentially occur is represented by a dashed outline.
	For M-ary FSK each column of frequencies harbors exactly one energy bundle,
	and $\log_{2} 8 = 3$ bits of information are conveyed with roughly the same energy
	that it takes to convey one bit of information in OOK
	(the exact energy required depends on a detailed analysis of reliability).
	}

\subsection{On-off keying}

In on-off keying (OOK),
an energy bundle with received energy $\energy_{h}$ is transmitted
to convey a ''one'' bit, and no signal energy is transmitted to convey a ''zero'' bit.
The transmit signal is thus of the form
\begin{equation}
X(t) = \sum_{k} A_{k} \cdot  \sqrt{\energy_{h}} \, h(t - kT)
\end{equation}
where information is conveyed by setting $A = 0$ or $A = 1$.
When waveform $h(t)$ is chosen to fall within the ICH,
a MF at the receiver can recover a noisy version of $A$ without need for
any processing related to the impairments introduced in the ISM.
The signal at the output of the MF corresponding to one symbol at time $k$ is then
\begin{equation}
\label{eq:ookmf}
Z = \sqrt{\, \energy_{h} \, \flux \,} \cdot A + M =  \sqrt{\, 2 \, \energybit \, \flux \,} \cdot A + M
\end{equation}
where $\energybit$ is the average received energy per bit in the absence of
scintillation, $M$ is additive Gaussian noise with variance $N_{0}$,
and $\flux$ is the current scintillation flux. 
The phase of the scintillation is not included in the model because we plan to use phase-incoherent detection.
The association $\energybit = \energy_{h}/2$ assumes that the two values of $A$ occur
with equal probability.

Our interest is in calculating the
error probability $\pe$ at the threshold of outage, 
which corresponds to $\flux = \oot$.
Substituting this value, and also normalizing
the MF output of \eqref{eq:ookmf},
\begin{equation}
\label{eq:normalMFook}
\sqrt{\frac{2}{N_{0}}} \cdot Z = \sqrt{4 \, \ecro} \cdot A + V
\end{equation}
where $V$ is a normalized (unit variance real and imaginary parts) Gaussian random variable.
The decision on $A = 0$ and $A = 1$ is made by applying $|Z|^{2}$
(or its normalized version) to an appropriate threshold.
Thus the reliability of information extraction (represented by $\pe$)
is completely controlled by $\ecro$.

Combining \eqref{eq:powereoutage}, \eqref{eq:poutage}, and \eqref{eq:ecro},
the power efficiency of OOK is
\begin{equation}
\powere = \frac{1}{N_{0} \, \ecro} \cdot \oot \, \exp \left\{ - \frac{\oot}{\vs} \right\} \,.
\end{equation}
This gives us an objective way to choose the outage threshold $\oot$, since $\powere$
is maximized at $\oot = \vs$.
Recalling that $\vs = \expec{\flux}$,this choice of outage threshold equals the average flux.
Any received flux below average is declared to be an outage.
and information is extracted from
the received signal whenever the flux equals its average or higher.
Also, at the threshold of outage $\ecro = \ecrb$.
This results in an outage probability from  \eqref{eq:poutage} equal to
\begin{equation}
\po = 1 - \frac{1}{e} = 0.368 \,.
\end{equation}
Increasing the outage probability directly reduces the information rate but also reduces the
energy per bit required to achieve the reliability objective at the threshold of outage,
since the flux at that threshold is increased.
The optimum tradeoff falls at 37\% outage time.
The reduction in power efficiency $\powere$ attributable to outages is a factor of $e^{-1}$ ($4.3$ dB).

With the power efficiency-maximizing choice of $\oot$,
\begin{equation}
\label{eq:gapOOK}
\powere 
\le \powerescin \cdot \frac{e^{-1} \, \log_{e} 2}{\ecro} =  \powerescin \cdot \frac{0.255}{\ecro} \,.
\end{equation}
The gap between the global maximum $\powere = \powerescin$ and OOK is the factor $0.255/\ecro$.
The size of this gap depends on the size of $\ecro$,
which depends in turn on our objective for $\pe$.
This is calculated in Appendix \ref{sec:peook} and plotted 
in Figure \ref{fig:gapFundamental} (for AWGN alone) and again 
in Figure \ref{fig:peOOKvsFSK} (at the threshold of outage) as a function of $\ecro$.
If we demand that $\pe = 10^{-4}$ at the threshold of outage, then
the $\ecro \approx 16$ dB.
This implies that the gap between the power efficiency achieved by OOK and the
fundamental limit is, from \eqref{eq:gapOOK}, about 22 dB.
Thus, there is an opportunity to reduce the received average power
relative to OOK by up to 22 dB, or a linear factor of $156$, without violating the fundamental limit.
A substantial portion of this gap will now be closed by using M-ary FSK.

\incfig
	{peOOKvsFSK}
	{.8}
	{A log plot of the biterror probability $\pe$
	for both on-off keying (OOK, dashed curve) and M-ary frequency-shift keying (FSK).
	The horizontal axis is the energy contrast ratio at the threshold of outage
	$\ecro$ in dB (defined in \eqref{eq:ecrb}).
	For M-ary FSK the plot is the upper bound on $\pe$ given by \eqref{eq:peFSKbound},
	for $M = 2^{n}$ and $1 \le n \le 12$.}

\subsection{Orthogonal coding: M-ary FSK}
\label{sec:channelcoding}
	
A substantial portion of the $\approx 22$ dB reduction in received power
can be obtained by very simple channel coding.
As early as 1960 it was found
that  M-ary FSK (illustrated in Figure \ref{fig:fskIllustrate})
can achieve capacity on the AWGN channel asymptotically as $M \to \infty$.
The simplicity of this result is a testament to the relative ease of
power efficient design in comparison to spectrally efficient design.
Further, it was shown in the 1960's that the capacity of the Rayleigh fading channel
(which applies to interstellar communication in the strong scattering regime)
for the bandwidth-unconstrained case
is the same as the capacity of the AWGN \citeref{637}.
The proof of this result was constructive, by demonstrating a channel coding
technique that achieves AWGN capacity.
Although based in part on M-ary FSK,
temporal diversity combining (to offset the variation in signal flux due to scintillation) and
low duty-cycle (to offset the variation in phase due to scintillation) are included.
For those interested,
a simpler modern derivation can be found in \citeref{638}.

Here the coding gain achievable by simple M-ary FSK in conjunction with
our outage strategy is determined.
This will not approach the fundamental limit, but it
will demonstrate that
large reductions in received power relative to OOK can be achieved by M-ary FSK
in conjunction with the outage strategy.
Following that, outages will be replaced by time-diversity to demonstrate a
further improvement in power efficiency.
In Chapter \ref{sec:discovery} the discoverability of this signal will be considered,
and in particular it will be shown that with a particular choice of parameters
the M-ary FSK signal becomes a power-optimized beacon as well.

The transmit signal for M-ary FSK is of the form
\begin{equation}
X(t) = \sum_{k} \sqrt{\energy_{h}} \, h(t-kT) \, \exp \left\{ \, i \, 2 \pi A_{k} \, B_{s} \, t \right\}
\end{equation}
where $A_{k}$ is chosen from the alphabet $\{ 0, \, 1, \, \dots \,, M-1 \}$
and $B_{s}$ is the spacing of carrier frequencies, where $B_{s} \ge B$
(so that the spectra do not overlap\footnote{
In spectrally efficient design,
it is possible to strengthen this condition and overlap spectra while maintaining
the orthogonality of the waveforms at different frequencies.}).
As in OOK, $h(t)$ is chosen to fall in an ICH so that receiver processing
related to impairments in the ISM are not required.
Each symbol time of length $T$ is used to represent one of $M$ alternative frequencies,
conveying $\log_{2} M$ bits of information.
Besides simplicity, M-ary FSK has other desirable properties for interstellar communication.
One is that a peak signal power which equals the average signal power
when the duty cycle is $\delta = 1$, the case of maximum information rate $\rate$
on a single carrier.
Another is compatibility with phase-incoherent detection.
It is necessary to estimate the received signal flux with time
in order to apply the outage strategy as defined earlier, it is not necessary to estimate the
phase of the scintillation nor the carrier phase
to decode M-ary FSK.
Rather, the decoding of the information can rely on simple estimates of the
energy for the candidate locations for energy bundles.


The receiver realizes $M$ MF's, one for each frequency $\{ m B_{s} , \ 0 \le m < M \}$.
Let those outputs at time $k$ be denoted by $\{ Z_{k,m} , \ 1 \le m \le M \}$.
Non-frequency overlap implies only one of the $M$
MF outputs contains a signal term; the others are noise-only.
In that case, the outputs can be written, for $A_{k} = n$,
\begin{equation}
\label{eq:MFoutputOrthog}
Z_{k,m} = \begin{cases}
\sqrt{\, \log_{2} M \,\, \energybit \, \flux \,} + M_n \,, & m = n \\
M_m \,, & 1 \le m \le M-1 \,, \ m \ne n \,.
\end{cases} \,.
\end{equation}
The signal level reflects the fact that the energy of the pulse $\energy_{h}$
represents $\log_{2} M$ bits of information, and thus $\energybit = \energy_{h} / \log_{2} M$.
Because of the $\log_{2} M$ factor, $\energybit$ for FSK can be smaller than for OOK, 
and this is the source
of a gain in power efficiency (recall that $\energybit$ is the reciprocal of $\powere$).

As we saw with OOK, in conjunction with the outage strategy the error probability $\pe$ at the
threshold of outage is calculated for a received flux at the threshold of outage $\flux = \oot$,
with the assurance that $\pe$ will be consistently lower during periods of larger flux.
A normalized version of the MF outputs is
\begin{equation}
\label{eq:mfoutfsk}
\sqrt{\frac{2}{N_{0}}} \, Z_{k,m} = \begin{cases}
\sqrt{\, 2 \, \log_{2} M \,\, \ecro \,} + V_n \,, & m = n \\
V_m \,, & 1 \le m \le M-1 \,, \ m \ne n \,,
\end{cases}
\end{equation}
where $\ecro$ is defined by \eqref{eq:ecro}.
Clearly the error probability $\pe$ depends on both $M$ and $\ecro$,
so that as $M$ is increased $\ecro$ can be decreased, and this
in turn decreases $\energybit$ and increases $\powere$.

If it is assumed that all $M$ possibilities are equally likely, then the
optimum phase-incoherent detector chooses as the signal location the $m$ that satisfies
\begin{equation}
\max_{1 \le m \le M} | Z_{k,m} |^2 \,.
\end{equation}
An advantage of FSK over OOK is that this detection algorithm does not
depend on knowledge of either the noise $N_{0}$ nor the signal level (e.g. flux $\flux$);
rather, it simply works more reliably when $N_{0}$ decreases or $\flux$ increases.
A tight upper bound on the bit error probability $\pe$ is determined in Appendix \ref{sec:peppm},
\begin{equation}
\label{eq:peFSKbound}
\pe \le \frac{1}{4} \, M^{1 - \frac{\ecro}{2 \, \log_{e} 2}} \,.
\end{equation}
$\pe$ is compared to OOK in Figure \ref{fig:peOOKvsFSK} for different $M$.
This shows that for the same reliability $\pe$
M-ary FSK can achieve a substantial reduction in 
$\ecrb$ relative to OOK.

A striking property of \eqref{eq:peFSKbound} is that when
\begin{equation}
\label{eq:ecrbbound}
\ecro > 2 \, \log_{e} 2 \,,
\end{equation}
then $\pe \to 0 \ \ \ \text{as} \ \ \  M \to \infty$.
This simple coding can achieve arbitrarily high reliability as $M \to \infty$
as long as \eqref{eq:ecrbbound} is satisfied.
This lower bound on $\ecro$ is a factor of two larger than the fundamental limit on the AWGN channel,
reflecting the loss in sensitivity due to using phase-incoherent detection.
Otherwise, this is a re-verification that M-ary FSK can approach the
fundamental limit on power efficiency as $M \to \infty$ on the AWGN channel,
although not when scintillation is added to AWGN (due to the loss of information
during outages). 

Also \eqref{eq:peFSKbound} can be solved for $\ecro$ to
quantify the tradeoff between $\ecro$ and $M$ at fixed $\pe$,
\begin{equation}
\label{eq:ecrbVsPe}
\ecro = 2 \, \log_{e} 2 \cdot \left( 1 - \frac{2 + \log_{2} \pe}{\log_{2} M} \right) \,.
\end{equation}
Note that the first term equals \eqref{eq:ecrbbound},
and the second term is the gap between that limit and the effect of using
a finite $M$, as a function of $\{ \pe, \, M \}$.
This is plotted in Figure \ref{fig:ecrbVsM} and compared to the asymptote of \eqref{eq:ecrbbound}.
This illustrates that there is a diminishing return as $M$ increases.
At what might be considered a practical value of $M=2^{8}$, the
gap is 3.8 dB.

\incfig
	{ecrbVsM}
	{.7}
	{A plot of the energy contrast ratio per bit $\ecro$ in dB
	required to achieve a reliability $\pe = 10^{-4}$
	vs the number of bits
	per symbol $\log_{2} M$ for M-ary FSK.
	As $M$ increases the required $\ecro$ decreases,
	approaching the asymptote $2 \, \log_{e} 2$, shown as a dashed line.}

\subsection{Orthogonal coding: M-ary PPM}

An alternative to M-ary FSK is M-ary pulse-position modulation (PPM), which
is illustrated in Figure \ref{fig:FSKvsPPM}.
PPM conveys information by situating an energy bundle in time rather
than frequency.
The identically same model for the MF output of \eqref{eq:MFoutputOrthog}
applies to both FSK and PPM, and thus $\pe$ is identical.
There are however two substantive practical differences between the FSK and PPM:
\begin{description}
\item[Peak vs average power.] 
FSK is a constant envelope modulation scheme,
in which the transmitted power does not vary with time,
when $\rate$ is maximized for a single carrier.
However, will be illustrated later, when the $\rate$
and power is reduced by lowering the duty cycle $\delta$,
FSK is no longer constant-envelope.
On the other hand, PPM is \emph{never} constant envelope,
as the essence of the scheme is to vary the signal power vs time.
\item[Discovery efficiency.]
It will be shown in Chapter \ref{sec:discovery} that PPM can be discovered
with slightly greater efficiency.
This is because all the signal power is concentrated at a single frequency,
which means there are fewer places to look.
However, in practical terms this is not likely to be an issue, since
discovery searches will typically  perform a multichannel spectral analysis
that will naturally capture the different FSK frequencies.
\end{description}
The choice between FSK and PPM should largely be driven by technology,
and in particular the extent to which constant-envelope modulation is
advantageous in the implementation of a high-power transmitter or not.

\incfig
	{FSKvsPPM}
	{.8}
	{
	An illustration of M-ary frequency-shift keying (FSK) and M-ary pulse-position modulation (PPM)
	for the same value of $M=8$, implying that both convey the same $\log_{2} 8 = 3$
	information bits per simply.
	FSK transmits an energy bundle at one of eight frequencies, and PPM transmits an energy
	bundle (with eight times shorter duration) at one of eight locations in time.
	Assuming the bundles contain the same energy in each case, these options operate at the
	same power efficiency for the same error probability $\pe$.
	Since that same energy is packed into one-eighth the time duration for PPM, its peak power is
	eight times higher, as illustrated by the different saturation.
	}

\subsection{Power efficiency of orthogonal coding with outages}

Our outage strategy works exactly the same way for M-ary FSK and PPM as for OOK,
and the resulting power efficiency has to be adjusted for the information lost during outages,
\begin{equation}
\powere = \frac{1 - \po}{\energybit} = 
\frac{\oot \, \exp \left\{ - \frac{\oot}{\vs} \right\}}{N_{0} \, \ecro} \,.
\end{equation}
As with OOK the power efficiency-maximizing outage threshold is 
$\oot = \vs$, and substituting from \eqref{eq:ecrbVsPe} and \eqref{eq:powerescin},
\begin{equation}
\label{eq:powereFSKrealistic}
\powere = \frac{\vs \, \log_{2} e}{\displaystyle 2 \, e \, N_{0} \,  \left( 1 - \frac{2 + \log_{2} \pe}{\log_{2} M} \right)}
= \powerescin \cdot \frac{1}{\displaystyle 2 \, e \, \left( 1 - \frac{2 + \log_{2} \pe}{\log_{2} M} \right)}
\,.
\end{equation}
The gap to the fundamental limit $\powere/\powerescin$ 
is plotted in Figure \ref{fig:gapFSKscin} for $\pe = 10^{-4}$.
The asymptote as $M \to \infty$ is a gap of 7.4 dB, which is
composed of 3 dB because of the phase-incoherent detection
and 4.4 dB due to the outage strategy.
There is an additional contribution to the gap as a penalty for using finite $M$.
For example, at $M = 2^8$, the total gap is 11.1 dB
(linear factor of 12.9).
This compares to 22 dB for OOK at the same $\pe$
(linear factor of 159).
Thus, the improvement in power efficiency relative to OOK is 10.9 dB
(linear factor of 12.3).
At the same information rate $\rate$, M-ary FSK with $M=2^{8}$ requires
a factor of 12.3 (91.8\%)  less average power $\power$

\incfig
	{gapFSKscin}
	{.7}
	{For M-ary FSK with $\pe = 10^{-4}$, the power efficiency $\powere$ 
	relative to the fundamental limit $\powerescin$ in dB vs.
	the number of bits per symbol $\log_{2} M$
	The limit $\powerescin$ is for the channel with AWGN and scintillation. 
	The dashed line is the $1/2 e$ asymptote as $M \to \infty$.}

The power efficiency can be further improved, capturing more of the remaining 
11.8 dB gap to the fundamental limit by using a combination of time diversity combining
and low duty cycle.
The question is whether these techniques are practical
in the uncoordinated environment of interstellar communication, whether the benefit in power
efficiency is worth the additional complexity, and whether
these signals can be as readily discovered.
Another issue is whether there may be other techniques to reduce this
gap that would be friendlier to interstellar communication.
All these issues are certainly worthy of further investigation.

\subsection{Power efficiency of orthogonal coding with time diversity}

The loss in power efficiency due to outages can be reduced by replacing
the outage strategy with a time diversity strategy.
This strategy will be analyzed in a later version of this report.


%\comment{Left over.}
%
%There are two simple codes known to be power efficient.
%Both use simple on-off data symbols, but each codeword bases a
%set of $M \ge 2$ symbols on $\log_2 M$ bits of information.
%They have identical reliability, and both achieve capacity
%asymptotically as $M \to \infty$ on the phase-coherent AWGN channel.
%
%$\{ g_m (t) \,, \ 1 \le m \le M \,, \ 0 \le t \le T \}$
%\begin{equation}
%g_m (t) =
%\begin{cases}
%h(t) \, \exp \left\{\displaystyle \, i \, 2 \pi m B t \right\}  \,, & \text{M-ary FSK} \\
%\sqrt{M} \cdot h \left( \displaystyle \frac{t - (m - 1) \, T}{M} \right) \,, & \text{M-ary PPM}
%\end{cases}
%\end{equation}
%In both cases, the $\{ g_m (t) \}$ have unit energy and are mutually
%orthogonal because they do not overlap one another in frequency (FSK) or
%do not overlap one another in time (PPM).
%Both of these codes communicate one of $M$ alternatives
%($\log_2 M$ bits of information) through the \emph{location}
%of one signal.
%\begin{equation}
%\label{eq:mfoutputFSK}
%y(t) = \sqrt{\energy_h} \, g_m (t) + M(t)
%\end{equation}
%\begin{equation}
%Z_m = 
%\int_{}^{} y(t) \, \cc g_m (t) \, dt
%= \begin{cases}
%\sqrt{\energy_h} + M_m \,, & m = M \\
%M_m \,, & 1 \le m \le M-1 \,.
%\end{cases}
%\end{equation}
%
%
%\begin{description}
%\item[Pulse-position modulation]
%(PPM) is similar to OOK except it incorporates memory.
%Instead of one bit influencing one and only one data symbol,
%a block of bits determines a block of data symbols.
%In particular, there are $M \ge 2$ data symbols in one block,
%where exactly one of those symbols is $A = 1$ and exactly $(M-1)$ of those
%symbols are $A = 0$.
%Thus, there are exactly $M$ distinct code words, which conveys $\log_{2} M$
%bits of information to the receiver.
%If $M = 2^{N}$ is chosen to be a power of two, then
%PPM maps a block of $N \ge 1$ input bits into $M = 2^N$ OOK-encoded symbols.
%This coding is illustrated in Table \ref{tbl:ppm} for the special case $M = 2^{4}$ or $N = 4$.
%PPM is the most power-efficient block code known,
%and in fact it was observed some decades ago that it can achieve
%channel capacity as $M \to \infty$ on the AWGN channel with unconstrained bandwidth.
%PPM is deliberately spectrally inefficient because it conveys only $\log_{2} M / M \le 1/2$
%information bits per symbol, as compared to one bit per symbol for OOK.
%It is deliberately power efficient, however, because it requires only one
%non-zero symbol per $\log_{2} M$ bits.
%As $M$ increases, PPM becomes more spectrally inefficient even as it becomes
%more power efficient, displaying a tradeoff between the two forms of efficiency that mirrors
%the fundamental limits in Section \ref{sec:tradeoff}.
%\item[Frequency-shift keying]
%(FSK) is the same idea as PPM, but based on the time-frequency duality.
%In FSK
%\end{description}
%
%\doctable
%	{\small}
%	{ppm}
%	{
%	Example of pulse-position modulation with $M = 2^{4} = 16$ and a duty cycle
%	of $\delta= 1/M = 1/16$.
%	Four information bits are coded as the position of a single
%	one bit in one of $2^{4} = M$ positions.
%	There is a bandwidth expansion of $16/4 = 4$, as well as
%	a substantial reduction in transmit power because four input
%	bits are represented by transmitting a single one-bit.
%	}
%	{| cc | cc |}
%	{
%\toprule
%\textbf{Information} &   &
%\textbf{Information} &  \\
%\textbf{bits} & \textbf{Codeword}  &
%\textbf{bits (con't)} & \textbf{Codeword} \\
%\toprule
%0000	&	0000000000000001	&	1000	&	0000000100000000	\\
%0001	&	0000000000000010	&	1001	&	0000001000000000	\\
%0010	&	0000000000000100	&	1010	&	0000010000000000	\\
%0011	&	0000000000001000	&	1011	&	0000100000000000	\\
%0100	&	0000000000010000	&	1100	&	0001000000000000	\\
%0101	&	0000000000100000	&	1101	&	0010000000000000	\\
%0110	&	0000000001000000	&	1110	&	0100000000000000	\\
%0111	&	0000000010000000	&	1111	&	1000000000000000	\\
% \bottomrule
%	}
%
%The basic parameters of PPM are compared with OOK
%in Table \ref{tbl:OOKvsPPM}.
%For a fixed symbol time duration $T$, both the rate $R$ and power $P$
%are smaller for PPM by a factor of $\log_{2} M / M \le 1$.
%To maintain the same $\rate$ for OOK and PPM,
%either $T$ could be decreased for PPM
%(never reducing it so far that $B T < 1$),
%or $T$ can be kept fixed and additional carrier signals added.
%In either case, the signal bandwidth will be greater, and the spectral
%efficiency lower.
%This shows that as $M$ is changed PPM trades off reduced spectral efficiency
%for greater power efficiency, following the $\rate \propto \power$
%characteristic of the fundamental limit.
%
%Table \ref{tbl:OOKvsPPM} does not consider the reliability of OOK and PPM.
%However, the reason that PPM can achieve considerably greater reliability
%for the same $\powere$, or greater $\powere$ for the same reliability,
%is evident upon examination of the Table.
%The reliability in detecting whether or not a signal is
%present is dependent on the size of the signal in the MF output,
%which is proportional to $\energy_h$.
%To compare OOK and PPM on a fair basis, keep $\powere$
%(or equivalently the energy per bit $\energybit$) fixed at the same
%value for all cases, and compare the value of $\energy_h$,
%\begin{equation}
%\label{eq:constpowere}
%\frac{\energy_h}{\energybit} = \begin{cases}
%2  \,, &  \text{OOK} \\
%\log_2 M  \,, & \text{PPM}
%\end{cases}
%\end{equation}
%Although this is not the full story, it indicates that the reliability of PPM improves as $M$ increases,
%while it remains fixed for OOK.
%
%
%%It was shown in the 1960's that PPM can achieve the fundamental limit of
%%channel capacity on the AWGN channel \citerefWloc{}{}.
%%However, our channel model includes not only AWGN, but also scintillation.
%%There are two reasons that PPM as defined in our design does not reach the fundamental limit.
%%First, due to our outage strategy there are periods when no information is received.
%%Approaching capacity would require some exploitation of the outage periods.
%%Second, because of scintillation we do not know the phase $\Psi$, and our way of dealing with this is to
%%use phase-incoherent detection which results in a 3 dB penalty.
%
%\doctable
%	{\small}
%	{OOKvsPPM}
%	{
%	A list of the performance characteristics of OOK and PPM in terms of
%	the energy $\energy_{h}$ and the symbol time duration $T$. 
%	For OOK it is assumed that $\prob{A =0} = \prob{A=1} = 1/2$.
%	}
%	{llllll}
%	{
%	\textbf{Characteristic} & \textbf{Variable} && \textbf{OOK} && \textbf{PPM} \\
%	\toprule
%	\addlinespace[3pt]
%	Average received power & $\power$ 
%		&& $\displaystyle \frac{\energy_{h}}{2 \, T} = \frac{\energybit}{T}$  
%		&& $\displaystyle \frac{\energy_{h}}{M \, T} = \frac{\log_{2} M}{M} \cdot \frac{\energybit}{T}$
%	\\
%	\addlinespace[5pt]
%	Information rate & $\rate$ 
%		&& $\displaystyle \frac{1}{T}$ && $\displaystyle \frac{\log_{2} M}{M} \cdot \frac{1}{T}$
%	\\
%	\addlinespace[5pt]
%	Power efficiency & $\powere$ 
%		&& $\displaystyle \frac{2}{\energy_{h}}$ && $\displaystyle \frac{\log_{2} M}{\energy_{h}}$
%	\\
%	\addlinespace[5pt]
%	Energy per bit & $\displaystyle \energybit = \frac{1}{\powere}$ 
%		&& $\displaystyle \frac{\energy_{h}}{2}$ && $\displaystyle \frac{\energy_{h}}{\log_{2} M}$
%	\\
%	\addlinespace[1pt]
%	\bottomrule
%	}
%
%\subsection{Probability of error}
%
%OOK
%
%PPM
%
%
%%\incfig
%%	{peOOKvsPPM}
%%	{1}
%%	{ A log plot of the error probability $\pe$, holding power efficiency $\powere$ constant,
%%	against $\snr_{b}$.
%%	The dashed curve is for OOK, while the solid curves are for PPM
%%	with $M = 2^{\,2}$, $2^{\,4}$ and $2^{\,8}$.
%%	}
%%	
%
%\subsection{PPM and capacity}
%
%Figure \ref{} is a good testament to power-efficient design,
%but we can make an even stronger statement.
%Examining \eqref{eq:peppmfinal}, $\ecrb = 2 \log_{e} 2$ is a very special demarkation,
%as can be verified by examining the limit
%as $M \to \infty$,
%\begin{equation}
%\label{eq:ppmpelimit}
%\pe \to
%\begin{cases}
%0 \,, & \snr_{b} > 2 \log_{e} 2 \\
%1 - \frac{1}{\sqrt{e}} \,, & \snr_{b} = 2 \log_{e} 2 \\
%1 \,, & 0 < \snr_{b} < 2 \log_{e} 2
%\end{cases}
%\end{equation}
%Thus, for any $\ecrb$ in Figure \ref{fig:peOOKvsPPM} larger than
%1.4 dB, as $M$ gets larger the error probability will approach zero.
%Recall the fundamental limit on reliable communication over
%an AWGN channel of \eqref{eq:ebn0}, 
%which is that $ \snr_{b} > \log_{e} 2$ is required for reliable communication.
%Eq. \eqref{eq:ppmpelimit} establishes that 
%asymptotically as $M \to \infty$, PPM with phase-incoherent
%detection comes within a factor of two (3 dB) of the fundamental limit.
%That 3 dB penalty is due to our phase-incoherent detection scheme.
%However, this analysis does not take account of scintillation, which will be
%addressed shortly.
%
%\section{Dealing with scintillation}
%
%\subsection{Discovery}
%
%
%
%Replace $\energy_h$ by $\energy_h \oot$.
%The $\pe$ is determined by
%\begin{equation}
%\snro = \frac{\energy_h \, \oot}{N_0}
%\end{equation}
%
%The resulting power efficiency is
%\begin{equation}
%\powere = \frac{(1 - \po) \, \log_2 M}{\energy_h}
%\end{equation}
%
%\begin{equation}
%\frac{\energybit}{N_0} = \frac{\energy_h}{N_0 \, \log_2 M}
%\end{equation}
%\begin{equation}
%\rate = (1 - \po) \cdot \frac{\log_2 M}{M \, T}
%\end{equation}
%
%\begin{align}
%&\po = 1 - \exp \left\{ - \frac{\snro}{\ecrs} \right\} \\
%&\frac{\oot}{\vs} =  \frac{\snro}{\ecrs} \\
%&\powere = \frac{\log_2 M}{\energy_h} \cdot \exp \left\{ - \frac{\snro}{\ecrs} \right\} \\
%&\powere =  \frac{\log_2 M \, \vs}{N_0 \, \ecrs} 
%\cdot \exp \left\{ - \frac{\snro}{\ecrs} \right\} \\
%&\powere = \powerescin \cdot \frac{\log_e M}{\ecrs}
%\exp \left\{ - \frac{\snro}{\ecrs} \right\}
%\le \powerescin \cdot \frac{( \log_e M )/ e}{\snro}
%\end{align}
%
%$\powere$ is maximized for $\ecrs = \snro$.
%
%%\subsection{Probability of error}
%%
%%It is known that on the simple AWGN channel, PPM
%%can achieve capacity in the sense that $\pe \to 0$
%%as $N \to \infty$ when $\rate \le \capacity$.
%%However, this result does not apply in the current
%%circumstance for a couple of reasons.
%%First, the AWGN does not suffer from outages,
%%and these will clearly reduce the rate at which bits are
%%communicated reliably.
%%Second, the reception is incoherent, in the sense that
%%the scintillation phase $\Psi$ is unknown.
%%Fortunately PPM is compatible with incoherent detection,
%%but we do not expect the technique to approach capacity.
%%
%%During periods of non-outage, the decision variable $Q = |Z|^2$
%%can be used to recover data symbols, since it is assumed that
%%accurate estimates of $\{ \recenergy , \vs , N_0 \}$ are available.
%%However, the reliability with which data symbols can be detected
%%depends on the current scintillation flux $\flux$.
%%During non-outages,
%%most of the time the error probability $\pe$ will be negligible,
%%but the concern is for those marginal times when $\flux$ is near or at the
%%threshold of outage.
%%Thus, our design approach is to focus on the worst-case situation
%%at the threshold of outage, or $\flux = \oot$.
%%The decision variable in this marginal case is
%%\begin{equation}
%%\label{eq:Qdec}
%%Q = \left| \, \sqrt{\recenergy \, \oot}  \, A + M \, \right|^{2} \,.
%%\end{equation}
%%In this case, the decision
%%$A = 0$ is made if $Q < \ddt$ for a chosen threshold $\ddt$.
%%It is shown in Appendix \ref{sec:performancecalc} 
%%that the error probability $\pe$ at the threshold of outage is
%%determined by the signal-to-noise ratio at the threshold of outage,
%%\begin{equation}
%%\label{eq:snro}
%%\snro =\frac{\recenergy \, \oot}{N_{0}} 
%%%= \ecrs \cdot \log_e \frac{1}{1-\po}
%%\,.
%%\end{equation}
%%%from \eqref{eq:poutage}.
%%%It follows that $\oot \ge \vs$. 
%%$\pe$ is specified by the receiver designer,
%%and this determines the required $\snro$.
%%Although no closed-form expression for $\pe$ is available, it is plotted in Figure \ref{fig:peOutage}.
%%$\pe$ is monotonically decreasing with $\snro$, and
%%values on the order of $\snro \approx 15$ dB are required to achieve
%%small $\pe$.
%%
%%\incfig
%%	{peOutage}
%%	{.8}
%%	{
%%	A plot of the relationship between the SNR (in dB) at the threshold of outage
%%	$\snro$ and the probability of error $\pe$ at the threshold of outage.
%%	Outside of outage, scintillation usually gives a higher signal power 
%%	and thus a smaller $\pe$.
%%	}
%
%%The parameters of the design and performance metrics, listed in Table \ref{tbl:designParameters},
%%are defined in the context of the following specific detection and decision strategy.
%%Most of the time the receiver is operating in \emph{discovery mode},
%%in which the receiver is searching for an information-bearing signal of extraterrestrial origin.
%%In this mode, the following steps will be involved:
%%\doctable
%%	{\small}
%%	{designParameters}
%%	{
%%	 A list of the design parameters for the signal processing algorithms
%%	 described in the text. $Q = |Z|$ is the magnitude of the MF output
%%	 sampled at time $t=0$ for one carrier frequency, and $R = |S|$
%%	 is an estimate of the current scintillation magnitude.
%%	 During discovery,
%%	 the processing is repeated for different times and carrier frequencies,
%%	 and during communication it may be repeated for different carrier frequencies.
%%	}
%%	{c c p{9cm}}
%%	{
%%	\textbf{Mode} & \textbf{Parameter} & \textbf{Description} \\
%%	\toprule
%%	\textbf{Discovery} & $\hht$ &  
%%	$Q> \hht$ is defined as a hit, suggesting the location
%%	is a candidate for one IU.
%%	\\
%%	\cmidrule{2-3}
%%	& $\pfa$ &
%%	Probability of false alarm, or the probability that a
%%	hit occurs as a result of noise alone.
%%	Depends on $\hht$ and $N_0$.
%%	\\
%%	\cmidrule{2-3}
%%	& $\oot$ &
%%	An outage is defined as $R < \oot$.
%%	This is the scintillation magnitude for which a snapshot of both
%%	$\pd$ and $\pe$ are determined.
%%	\\
%%	\cmidrule{2-3}
%%	& $\pd$ &
%%	The probability of detection,
%%	or the presence of a signal will result in a hit.
%%	A snapshot is taken
%%	at the threshold of outage, so $\pd$ applies to 
%%	scintillation magnitude $R = \oot$.
%%	\\
%%	\cmidrule{1-3}
%%	\textbf{Communication} & $\oot$ &
%%	 During an outage ($R < \oot$),
%%	 no attempt is made to extract information.
%%	\\
%%	\cmidrule{2-3}
%%	& $\po$ &
%%	Probability that an outage occurs at any given time.
%%	The threshold $\oot$ is chosen to achieve the desired $\po$.
%%	\\
%%	\cmidrule{2-3}
%%	& $\ddt$ &
%%	When $Q > \ddt$, $A = 1$ is decided, otherwise $A = 0$.
%%	\\
%%	\cmidrule{2-3}
%%	& $\pe$ &
%%	Probability of error in the $A$ decision.
%%	A snapshot is taken at the threshold of outage $R = \oot$.
%%	\\
%%	\bottomrule
%%	}
%%\begin{description}
%%\item[Initial hit.] 
%%When the receiver has not yet established that a signal is present,
%%it systematically searches over different starting times and carrier frequencies by
%%applying a bank of MF's to the signal, each assuming a different carrier frequency.
%%The decision variable $Q$ from \eqref{eq:normdv} is used for initial
%%screening as to the likely presence of signal $h(t)$ because of its
%%robust adaptation to unknown signal and noise power.
%%The criterion for a hit is when $Q > \hht$ where $\hht$ is the hit threshold.
%%The measure of performance is false alarm probability $\pfa$, or the probability
%%of a hit in the presence of noise alone.
%%The value of $\hht$ is chosen to achieve the desired $\pfa$.
%%Since $N_{0}$ depends on the line of sight (due to astronomical objects near
%%that line of sight that may be emitting noise-like energy), the receiver should
%%estimate $N_{0}$ for each new line of sight and adjust $\hht$ accordingly
%%with the objective of keeping $\pfa$ fixed.
%%\item[Post-hit processing.]
%%Most of the time a hit represents a false alarm.
%%%To be relatively sensitive to low-power signals, $\pfa$ should be designed to
%%%be reasonably large, and the resulting hits further investigated by other criteria.
%%For a hit to occur in response to an actual signal, then 
%%(a) that signal must use the waveform $h(t)$ that is matched by the MF,
%%(b) the starting time and carrier frequency of the MF must be
%%accurately aligned with that signal, and
%%(c) $A = 1$.
%%For any $\{ \hht,\pfa \}$ the detection probability $\pd$ is
%%a function of unknown parameters $\{ \recenergy , \vs \}$.
%%This establishes the sensitivity of signal discovery when the latter is
%%based on a single IU.
%%
%%The detection sensitivity can be improved by taking advantage of 
%%other expected signal characteristics.
%%In particular,  the receiver expects to see a sequence of IU's corresponding
%%to a single carrier frequency, potentially repeated as well at other carrier frequencies.
%%Having seen one such event, the receiver can revert to a single MF at the
%%detected carrier frequency and look for a repeated sequence of such events,
%%and estimate the period of such repetition.
%%This phase of discovery is very similar to pulsar detection, and similar algorithms can be used
%%(of course absent the ''de-dispersion'' processing that is necessary for pulsars).
%%Depending on whether the transmitter and/or receiver have compensated for
%%their own acceleration component in the line of sight,
%%both the carrier frequency and repetition period may wander, and in this case there
%%is also a tracking issue.
%%\item[Outage and repeated observations.]
%%Another defining characteristic of a signal of interstellar origin  is
%%scintillation, which is manifested by a variation in received signal power.
%%Thus define an \emph{outage} as any time interval during which the signal power
%%is too low for reliable discovery, and following discovery is too low for
%%reliable extraction of the embedded information.
%%Our greatest concern is in detecting a signal that will be in non-outage
%%during the communication phase, and thus $\pd$ is calculated
%%at the threshold of non-outage, or $R = \oot$.
%%Most of the time during a non-outage the actual detection probability
%%will be much higher than $\pd$, and conversely detection is still possible
%%during an outage but with actual detection probability lower than $\pd$.
%%
%%Another consequence of outages is that observations at a single carrier frequency should be
%%repeated with a time spacing larger than the scintillation coherence time.
%%This insures that outages cannot be a cause of discovery failure.
%%\end{description}
%%
%%Most of the time the receiver is operating in this discovery mode.
%%When discovery is successful and the presence of a signal has been reasonably established,
%%the receiver can move on to the \emph{communication mode},
%%in which the signal is observed continuously and information is extracted from it.
%%In this mode, the following steps will be involved:
%%\begin{description}
%%\item[Estimation of signal parameters.]
%%During discovery it is likely that the period of repetition of IU's $T_{0}$ has been determined.
%%With the luxury of long-term observation, the other signal parameters
%%$\{ \recenergy, \vs, N_{0} \}$ can be estimated.
%%In particular $\{ \recenergy, \vs \}$ requires an observation of the scintillation
%%magnitude over a period long relative to the scintillation coherence time,
%%since in the short-term only their product $ \recenergy \, \vs$ can be observed.
%%By matching the variations in $ \recenergy \, \vs$ to the Rayleigh distribution,
%%the variation due to $\vs$ can be separated out 
%%from the non-variable effect of $\recenergy$.
%%\item[Outages.]
%%Armed with an estimate of $\{ \recenergy, \vs \}$ the receiver can track
%%the scintillation magnitude $R$ as it varies with time, and thereby also
%%determine outages, which are defined by $R < \oot$.
%%The value of $\oot$ is chosen according to the desired outage
%%probability $\po$, and also with an eye to the probability of error $\pe$
%%at the threshold of outage.
%%The minimum acceptable probability of error $\pe$
%%is calculated at the threshold of outage.
%%\item[Non-outages.]
%%During periods of non-outage, the detection of $A=0$ vs $A=1$ is
%%achieved by observing whether $Q > \ddt$ for a decision threshold $\ddt$.
%%During the non-outage time, not only is the probability of error
%%less than $\pe$, but it is usually much less than $\pe$.
%%Thus, non-outage communication is typically (but not always) very reliable.
%%\end{description}
%%
%%What is notably missing from this description is any signal processing related to
%%propagation impairments (other than noise and scintillation) like Doppler,
%%plasma dispersion, and multipath distortion.
%%The reason for this is that the ICH structure avoids these impairments entirely
%%at the expense of lower spectral efficiency.
%%For this reason, an interstellar communication transmitter and receiver
%%signal processing as described above is much simpler than the norm in terrestrial communication.
%%On the other hand, discovery is considerably more difficult due to the lack of coordination
%%between transmitter and receiver
%%and lack of prior knowledge of where to look for a signal.
%
%
%\subsection{Outage probability}
%
%The received energy $\recenergy$ and noise power density $N_{0}$
%are not under the control of the receiver designer, but based on
%\eqref{eq:snro} $\oot$ can be determined from the required $\snro$
%and this in turn determines the probability of an outage probability $\po$.
%\begin{equation}
%\po = \prob{\flux < \oot} = 
%\prob{ \left| \, \sqrt{\gamma} \, \sigma_{s} + \sqrt{1 - \gamma} \, S \, \right|^{2} < \oot} \,.
%\end{equation}
%Once again this can be expressed in closed form for the strong scattering case ($\gamma = 0$),
%\begin{equation}
%\label{eq:poutage}
%\po =  1 - \exp \left\{ - \frac{\oot}{\vs} \right\}
%= 1 - \exp \left\{ - \frac{N_{0} \, \snro}{\recenergy \, \vs} \right\}
%= 1 - \exp \left\{ - \frac{\snro}{\ecrs} \right\}
%\,.
%\end{equation}
%This is the worst-case in the sense that outages will be less prominent for weak scattering.
%This relationship is plotted in Figure \ref{fig:pOvsSNR},
%where the horizontal axis is $\ecrs / \snro$ in dB.
%Recall that $\ecrs$, which was defined in \eqref{eq:ecrs},
% is the signal-to-noise ratio at the output of the MF averaged over
% all scintillation outcomes,
%including outages and non-outages.
%The receiver designer has no control over $\ecrs$,
%but Figure \ref{fig:pOvsSNR} shows how $\po$ is affected by $\ecrs$.
%From Figure \ref{fig:pOvsSNR},
%$\ecrs \gg \snro$ is needed to achieve a very small $\po$,
%which implies that $\flux > \oot$ almost all the time.
%
%The condition $\ecrs \gg \snro$ is too stringent for most practical purposes,
%and a significant $\po \gg 0$ must be accepted.
%In fact, as will now be shown the power efficiency is maximized when 
%$\ecrs = \snro$ and thus $\po = 63$\%.
%This means that outages are occurring most of the time.
%That is the bad news, but the good news is that useful information is still
%being extracted from the signal 37\% of the time,
%and that is the operating point that achieves maximum power efficiency.
%
%\incfig
%	{pOvsSNR}
%	{.8}
%	{A logarithmic plot of the outage probability $\po$ (expressed 
%	as a percentage of the time an outage occurs) as a function
%	of the input signal-to-noise ratio $\ecrs$ in relation to the
%	outage threshold signal-to-noise ratio $\snro$ as determined
%	from the desired probability of error $\pe$ in Figure \ref{fig:peOutage}.
%	}
%	
%\subsection{Power efficiency with outages}
%
%To review what we have developed thus far, there are only
%two parameters $\{ \vs , N_0 \}$ that together characterize the
%ISM for ICH-structured communication.
%One of them is known and constant, $\vs = 1$.
%While the transmitter may have some estimate of $N_{0}$,
%only the receiver has the ability to accurately
%observe and estimate $N_{0}$ during the course of communication.
%A third parameter $\{ \recenergy \}$ is determined by the transmitter's
%choice of transmitted power coupled to the spreading loss
%and antenna gains.
%The receiver chooses the performance parameter
%$\{ \snro \}$ that specifies the lowest signal-to-noise ratio
%(or highest $\pe$) that can be accepted during periods of non-outage.
%Most of the time during periods of non-outage, the signal-to-noise is higher
%and the error probability is lower.
%
%It is useful to calculate the power efficiency $\powere$
%of OOK, for two reasons.
%The first is that we need a principled way to target an
%appropriate outage probability $\po$, and
%choosing $\po$ to maximize $\powere$ accomplishes that.
%The second motivation is
%to compare $\powere$ to the fundamental limits $\powerescin$ calculated in
%Chapter \ref{sec:fundamental}.
%Of course it must be that $\powere < \powerescin$ to communicate reliably, but the
%size of the gap reveals valuable insights into the origins of the
%suboptimality and how OOK might be modified to reduce the gap.
%
%In calculating and interpreting $\powere$
%the context and purpose should be kept in mind.
%The reason $\powere$ is important to the transmitter
%designer is the desire to either minimize the transmitted power,
%or to maximize the distance over which
%communication can occur, or both.
%Meanwhile $\powere$ is of no consequence to the receiver designer,
%as the receiver must live with the received power no matter what it is.
%The only design freedom available to the receiver is to choose the acceptable
%$\pe$ (and hence $\snro$), which together with the received energy
%per symbol $\recenergy$ determines the outage probability $\po$.
%
%With these motivations in mind, 
%for purposes of calculating $\powere$ we define the received power
%as $F \, \recenergy \, \expec{ A^{2} } = F \, \recenergy /2$, leaving out the
%$\expec{\flux} = \vs = 1$ term.
%Also, since OOK communicates one bit of information per IU, but a fraction
%$\po$ of those bits are lost during outages so the net information rate
%is $\rate = F \cdot ( 1 - \po)$.
%Thus the overall power efficiency is
%\begin{equation}
%\displaystyle
%\powere =
%\frac{F \cdot (1 - \po )}{F \cdot \frac{1}{2} \, \recenergy } 
%=\powerescin \cdot \frac{2 \log_{e} 2}{\ecrs} \,  \exp \left\{ - \frac{\snro}{\ecrs} \right\} 
%\le \powerescin \cdot \frac{2 \log_{e} 2 / e}{\snro}
%\,.
%\end{equation}
%The global maximum $\powere$ is achieved when the transmitter adjusts transmit
%power so that the signal-to-noise at the MF output is $\ecrs = \snro$ as mentioned earlier.
%
%There are two limitations to the accuracy with which the transmitter can achieve
%this operating point in order to maximize $\powere$, and thus minimize
%its transmit power in relation to the effective information rate $\rate$ taking outages into account.
%For one thing, the transmitter must know $\ecrs$, which requires
%knowledge of $N_{0}$.
%For another, to achieve $\ecrs = \snro$ requires knowledge of $\snro$,
%which means knowledge of the highest $\pe$ that is acceptable to the receiver designer
%during periods of non-outage.
%To address this information paucity,
%the transmitter designer must make reasonable assumptions on both counts.
%As illustrated in Figure \ref{fig:powereVsSNRMF},
%$\powere$ decreases when either $\ecrs > \snro$ or $\ecrs < \snro$,
%and that penalty is particularly large when $\ecrs < \snro$.
%Thus, in making its assumptions, the transmitter designer should err on the size
%of transmitting too much power.
%Any technical or budgetary limitation on the maximum transmit power can be accommodated by
%adjusting $F$ (and hence $\rate$) downward.
%
%At the maximum $\powere$ the outage probability is $\po = 63$\%.
%This indicates that the transmitter designer should deliberately target
%a relatively high outage probability of 63\%, because it would be too expensive
%(in terms of the increased transmit power) to reduce that outage probability.
%If the transmitter has more power available, the most effective way to exploit that
%power to achieve a higher $\rate$ is to increase $F$ rather than try to reduce $\po$.
%
%\incfig
%	{powereVsSNRMF}
%	{.8}
%	{For on-off keying, a plot of the loss in power efficiency relative to the
%	fundamental limit $\powere / \powerescin$  (expressed in dB) vs. the
%	signal-to-noise ratio $\ecrs$ at the matched filter output for $\snro= 15$ dB.
%	The rate $\rate$ used to calculate $\powere$ reflects the loss of data during outages,
%	and the average power $\power$ takes into account spreading loss but not scintillation.
%	At low $\ecrs$ the efficiency falls off rapidly due to increasing outage time,
%	and at high $\ecrs$ the efficiency falls off because the 
%	benefit in reduced outage time is not justified by the increasing received power.
%	The minimum efficiency loss relative to fundamental limits
%	is 18 dB for this case, and occurs at $\ecrs = \snro = 15$ dB.}
%
%%The reason $\powere$ is important to the receiver designer
%%is as a principled way to choose $\po$.
%%In both cases, the question arises as to how much is known
%%at the transmitter or receiver about the scintillation variance $\vs$,
%%because this parameter (as well as transmit power and spreading loss)
%%affects the received power.
%%In the following, two diametrically opposite assumptions are made
%%in calculating $\powere$: Either (a) $\vs$ is accurately known,
%%or (b) $\vs$ is unknown, in which case we assume that $\vs = 1$.
%%Assumption (a) is most likely to apply to the receiver design,
%%since $\vs$ can be estimated during communication.
%%Assumption (b) is most likely to apply to transmitter design,
%%since the transmitter has limited ability to observe the propagation
%%impairments encountered by its radio signals.
%%Of course, it would be possible to develop intermediate models
%%that take advantage of partial information about the scintillation.
%%
%%The presence of outages makes this a little more tricky.
%%\begin{equation}
%%\powere = \powere_{\text{NO}} \cdot (1- \po ) + \powere_{\text{O}} \cdot \po
%%\end{equation}
%%where $\powere_{\text{NO}}$ is the power efficiency during periods of
%%non-outage, and $\powere_{\text{O}} = 0$ is the power efficiency during
%%periods of outage.
%%Focus, then on periods of non-outage.
%%If $F$ is the rate at which IU's are transmitted and received,
%%for OOK there is one bit per IU and therefore $\rate = F$.
%%
%%
%%\begin{equation}
%%\power =
%%\begin{cases}
%%F \cdot E \left[ \, \recenergy \, |S|^2 \, A^2 \left. \right| |S|^2 \ge \oot \, \right] 
%%& \text{(a)} \ \vs \ \text{known}
%%\\
%%F \cdot E \left[ \, \recenergy \, A^2  \right]
%%& \text{(b)} \ \vs \ \text{unknown}
%%\end{cases}
%%\end{equation}
%%Case (a) uses the actual received power, while (b) uses the
%%hypothetical received power in the absence of scintillation.
%%
%%The conditional expectation can be determined from the
%%Rayleigh distribution,
%%\begin{equation}
%%E[ |S|^2 \left. \right| |S|^2 \ge \oot ] = \oot + \vs \,,
%%\end{equation}
%%and for OOK $E[A^2] = 1/2$.
%%The energy $\recenergy$ can be eliminated by substituting
%%for $\recenergy$ in terms of $\snro$ from \eqref{eq:snro},
%%and $\oot$ can be eliminated by substituting for
%%$\oot$ in terms of $\po$ from \eqref{eq:poutage}.
%%The result is
%%\begin{equation}
%%\powere = \frac{F}{\power_{\text{NO}}} =
%%\begin{cases}
%%\displaystyle
%% \powerenoise \cdot f(\po) \cdot g (\pe) 
%% \\
%% \displaystyle
%%\powerescin \cdot f(\po) \cdot g (\pe)
%% \end{cases}
%%\end{equation}
%%where the first term is the maximum power efficiency
%%for noise ($\powerenoise$ from \eqref{eq:powerenoise})
%%and for noise plus scintillation ($\powerescin$ from \eqref{eq:powerescin}).
%%The other two factors $f(\po)$ and $g(\pe)$ reduce the
%%power efficiency relative to this theoretical maximum.
%%(taking into account multi-carriers if they are used).
%%Then $F$ is also the ''raw'' information rate since our choice was one bit per IU.
%%However, in practice the effective information rate $\rate$ must take account of
%%outages, where higher $\po$ rests in a lower effective information rate.
%%In choosing a larger outage probability $\po$, the receiver designer
%%is affecting $\powere$ not only directly through the information rate, but
%%also in allowing the received energy $\recenergy$ required to achieve
%%an objective on $\pe$ to be lower.
%%This implies a tradeoff, resulting in an optimum $\po$.
%%Given our single-minded focus on $\powere$, $\po$ should be chosen
%%to maximize $\powere$.
%%
%%Taking account $F$, 
%%Then the effective average information rate extracted reliably at the receiver,
%%taking account of the outage probability $\po$, is
%%\begin{equation}
%%\label{eq:p0rate}
%%\rate =(1 - \po) \, F \,.
%%\end{equation}
%%Define received power as that in the absence of scintillation.
%%Because $E[A^{2}] = 1/2$, the average power is
%%\begin{equation}
%%\label{eq:erpower}
%%\power = \frac{1}{2} \, \recenergy \, F \,.
%%\end{equation}
%%The achieved power efficiency thus depends on $\po$ and $\recenergy$,
%%which depend in turn on the criteria applied to the
%%reliability of a decision on $A=0$ vs $A=1$ 
%%(the the outage probability $\po$ and the error probability $\pe$).
%%As shown in Appendix \ref{sec:performancecalc}, the
%%$\pe$ is predicted by the SNR measure
%%\begin{equation}
%%\label{eq:snre}
%%\snre  = \left( \frac{\snro}{1 + \sqrt{1 + 2 \, \snro }} \right)^{2}
%% \,,
%%\end{equation}
%%where the outage-adjusted SNR is
%%\begin{equation}
%%\label{eq:snr0}
%%\displaystyle
%%\snro =  \ecrs \cdot \log_{e} \left( \frac{1}{1-\po} \right) \,.
%%\end{equation}
%%Thus, the tradeoff between parameters $\{ \recenergy, \po \}$ for
%%a given line of sight (which is characterized by $\{ N_{0} , \vs \}$) and
%%with the goal of achieving a given $\pe$ is defined
%%by setting $\ecrs$ such that the value of $\snre$ is appropriate.
%%Combining \eqref{eq:snr0} with \eqref{eq:p0rate} and \eqref{eq:erpower}, 
%%the resulting power efficiency can be written
%%\begin{equation}
%%\label{eq:powerefficbinary}
%%\powere = \powerescin \cdot f(\po) \cdot g (\pe)
%%\end{equation}
%%This is similar in form to the fundamental bound of \eqref{eq:ctchan},
%%except for two factors which reduce the power efficiency
%%relative to that bound:
%%\begin{description}
%%\item[Outage penalty.]
%%The $f(\po)$ factor
%%\begin{equation}
%%\label{eq:outageonpowere}
%%f(x) = 
%%\begin{cases}
%%\displaystyle
%%\frac{(1-x) \log_{e} (1/(1-x))}{1 + \log_{e} (1/(1-x))}
%%\\
%%\displaystyle
%%(1-x) \log_{e} (1/(1-x))
%%\end{cases}
%%\end{equation}
%%is plotted in Figure \ref{fig:outagePowerLoss}.
%%This is the penalty in power efficiency due to our strategy of defining outage
%%periods and not trying to extract information during those periods.
%%If all $\{ A_{k} \}$ were used as part of a coding strategy with memory large relative to
%%the scintillation coherence time, then this penalty could in principle be avoided.
%%For OOK
%%the adverse effect is minimized for $\po = 1-e^{\frac{1}{2} \left(1-\sqrt{5}\right)} = 0.46$, with result
%%that $f(\po)= 0.205$ (6.86 dB).
%%The conclusion is that an uncoded OOK system utilizing an outage strategy should, in the
%%interest of maximizing power efficiency, operate at very high (46\%) outage probability.
%%\item[Coding penalty.]
%%The penalty for not using channel
%%coding is $g(\pe)$, where
%%\begin{equation}
%%g(x) = \frac{2 \, \log_{e} 2}{\snro} = \frac{1.386}{\snro} \,.
%%\end{equation}
%%For example, a typical value is $\snro = 15$ dB, which results
%%in a penalty of 13.58 dB.
%%\end{description}
%
%The best power efficiency obtainable by OOK  without channel coding
%represents a loss relative to fundamental limits
%equal to $\snro$ plus $\approx 3$ dB.
%In the example of Figure \ref{fig:powereVsSNRMF} this is an 18 dB loss in efficiency,
%corresponding to an increase in transmit power (or transmit/receive antenna gains)
%by a linear factor of 62.
%This substantial gap between OOK and the fundamental limit
%could be a motivation for a transmitter designer to seek channel coding 
%strategies to reduce this gap.
%There are two sources of this gap, and hence two ways it could be reduced.
%The first is the absence of channel coding, suggesting some
%form of channel coding simple enough to permit
%reverse engineering by the receiver.
%The second related source is the outage strategy, which could be relaxed by
%conveying useful information during periods of low received power.
%It should be emphasized that this gap is unrelated to the use of
%the ICH in the structure of the transmitted signal, the design choice of binary IU's,
%and the design choice of a single-use ICH.

%\incfig
%	{outagePowerLoss}
%	{.8}
%	{A plot of the factor $f(\po)$ in \eqref{eq:outageonpowere}
%	representing the penalty in power efficiency for using an outage strategy.}


%\section{Discovery sensitivity}
%
%A legitimate concern is whether it is possible to discover a
%signal with sufficient power to reliably recover information.
%If this is not possible, then this would be a compelling argument
%for using an information-free beacon to attract attention, as
%has been the assumption of virtually all SETI searches to date.
%The essential question is whether an information-free signal
%can be discovered with greater sensitivity or more easily than
%an information-bearing signal such as OOK.
%The ''sensitivity'' question is easier (the answer is no)
%while answering the ''ease'' question is more nuanced and subjective.
%
%Suppose that discovery is attempted by detection of an isolated IU
%as described earlier (the MF output is applied to a ''hit'' threshold $\hht$).
%The detection probability $\pd$ then depends on the choice of $\hht$, which
%also determines the false alarm probability $\pfa$.
%For a given choice of $\hht$, $\pd$ (but not $\pfa$) also depends on
%nature's choice of scintillation amplitude $R$, as does $\pe$.
%Thus, we need to compare $\pe$ and $\pd$ for the same value of $R$
%to get a useful comparison.
%In particular, it makes sense to choose $R = \oot$, or the threshold
%of outage as the basis for comparison.
%It is shown in Appendix \ref{sec:performancecalc} that a snapshot of the
%detection probability $\pd$ at signal level $R = \oot$ is predicted by $\snrd$, where
%\begin{equation}
%\label{eq:snrd}
%\snrd = \frac
%{\left( 1 - \log_{e} \left( \frac{1}{\pfa} \right) + \ecrs \right)^{2}}
%{1 + 2 \, \ecrs}
%\ \ \ \ \text{for} \ \ \ \ 
%\log_{e} \left( \frac{1}{\pfa} \right) < \ecrs
% \,.
%\end{equation}
%Comparing to \eqref{eq:snre}, as expected the target $\pfa$ enters
%into the required $\snrd$ because of its influence on the choice of $\hht$.
%
%As a starting point, the relationship of $\pe$ and $\pd$ to (respectively)
%$\snre$ and $\snrd$ is shown in Figure \ref{fig:pEvsSNR}.
%Actually, $\pe$ and $(1-\pd)$ follow the same curve; that is,
%a $\snr$ that results in small $\pe$ also results in large $\pd$, both of which are desirable effects.
%Also note that this is a ''cliff'' effect at approximately $\snr = 10$ dB, where
%$\pe$ begins to fall rapidly as $SNR$ increases.
%Thus, $SNR = 10$ dB is a useful benchmark.
%
%\incfig
%	{pEvsSNR}
%	{.8}
%	{
%	A plot of the relationship between SNR value and probability of detection or error.
%	For equal values of SNR, $(1-\pd)$ and $\pe$ are equal.
%	}
%
%Now we are in a position to compare the sensitivity of the receiver during the
%discovery and communication phases.
%For $\ecrs \gg 1$, we see that $\snre \approx \snrd \approx \ecrs$,
%so there is about equal difficulty in discovering an OOK signal at high SNR
%as in reliably extracting useful information from it.
%However, when seeking a small $\pfa$ there is a range of $\snr$
%where discovery becomes compromised by the desire to maintain a small $\pfa$.
%This is illustrated in Figure \ref{fig:snr0vssnrD}, where the relationship between
%$\snre$ and $\ecrs$ is shown as the dashed line.
%Taking $\snre = 10$ dB as a benchmark, this requires that $\ecrs = 13.1$ dB.
%The larger $\ecrs$ required to achieve a given $\snrd $ are also plotted as
%the solid lines in Figure \ref{fig:snr0vssnrD} for different values of $\pfa$.
%For example, $\snrd = 10$ dB requires $\ecrs = 13.6$ dB for $\pfa = 10^{-1}$
%to  $\ecrs = 17.9$ dB for $\pfa = 10^{-12}$.
%
%\incfig
%	{snr0vssnrD}
%	{1}
%	{
%	The $\ecrs$ required to achieve a given $(1-\pd)$ or $\pe$
%	are compared for different values of $\pfa$.
%	The dashed line represents the $\ecrs$ to achieve a given $\snre$
%	(which reflects a target $\pe$).
%	The solid lines represent the $\ecrs$ to achieve a given $\snrd$
%	(which represents a target $\pd$) for different values of $\pfa$
%	from $10^{-1}$ to $10^{-12}$.
%	Generally discovery (represented by $\pd$) requires a higher SNR than
%	communication (represented by $\pe$), and the required discovery
%	SNR increases as the requirement on $\pfa$ is made more stringent.
%	The relationship between $\snre$ and $\pe$
%	(as well as $\snrd$ and $(1-\pd)$) can be found in Figure \ref{fig:pEvsSNR}.
%	}
%

\section{Adjusting information rate and average power}
\label{sec:adjrateandpower}

Consider M-ary FSK, and address the issue of how the
power and rate can be changed.
The previous development calculated the power efficiency for
a single symbol.
As multiple symbols are transmitted on a single carrier at a rate $F$,
the information rate is $\rate = F \cdot \log_{2} M$ and the
average power is $\power = F \cdot \energy_{h}$.
Thus, the power efficiency remains constant, independent of $F$.

If the transmitter wants to reduce $\power$ (at the expense of $\rate$),
it is advantageous to maintain $F = 1/T$, and increase $T$ as
$F$ is decreased.
This has the desirable effect of reducing the peak power as well as the
average power, by spreading the symbols out over a greater time.
However, there is a limit to how large $T$ can be increased while
maintaining the ICH constraint $T \le T_{c}$.
If further reductions in $\power$ are desired, then without affecting
$T$ a duty cycle $\delta < 1$ can be introduced, so that the
peak power becomes higher than the average power $\power$.
This is illustrated in Figure \ref{fig:FSKvsDelta}.

Similarly, an increase in $\rate$ is desired (at the expense of $\power$),
$T$ can be reduced while increasing $F$.
However, a different limit is reached when it is necessary to increase
bandwidth $B$, because eventually the ICH constraint $B \le B_{c}$ will be violated.
In that case,
multicarrier modulation can be used as illustrated in Figure \ref{fig:FSKvsCarriers}.
The desirable feature of equal peak and average powers is preserved by MCM.

 \incfig
 	{FSKvsDelta}
	{.7}
	{
	Illustration of the location of energy bundles for M-ary FSK
	(with $M=8$), and how the information $\rate$ can be
	reduced by reducing the duty cycle to $\delta = 0.2$ without changing $T$.
	The result is a reduction in both information rate $\rate$ and average power $\power$
	by a factor of five, while maintaining the same power efficiency.
	}

\incfig
	{FSKvsCarriers}
	{.7}
	{
	Illustration of the location of energy bundles for M-ary FSK
	(with $M=8$), and how the information $\rate$ can be
	doubled by adding a second carrier.
	The average power $\power$ is also doubled, so the
	power efficiency is the same.
	Note that this is different than doubling $M$ to $M = 16$
	(even though the diagram would look similar)
	which would increase $\rate$ by $4/3$ and $\power$ not at all.
	The difference in the two cases is two vs. one energy bundles per symbol time.
	}

\section{Spectral efficiency}
\label{sec:FSKspectralefficiency}

As $M$ increases in M-ary FSK and $\powere$ increases as a result, 
a decrease in spectral efficiency $\spectrale$ can be anticipated.
To characterize $\spectrale$,
assume that a single carrier is used with a rate of transmission of energy bundles equal to $F$.
Each symbol time (time duration of $h(t)$) is $T$, and the duty cycle is
\begin{equation}
\delta = T \cdot F \,.
\end{equation}
The bandwidth required for $h(t)$ is $B = K /T$, where $K$ is the degrees of freedom of the signal
defined in Section \ref{sec:channelmodeldof}.
To avoid overlap in the frequency domain, the minimum total bandwidth must be
\begin{equation}
B_{\text{FSK}} = M \cdot B \,.
\end{equation}
The information rate is
\begin{equation}
\label{eq:inforateR}
\rate = F \cdot \log_{2} M = \frac{\delta}{T} \cdot \log_{2} M
\end{equation}
and thus the spectral efficiency is
\begin{equation}
\spectrale = \frac{\rate}{B_{\text{FSK}}} = \frac{\delta}{K} \cdot \frac{\log_{2} M}{M} \,.
\end{equation}
Indeed $\spectrale \to 0$ as $M \to \infty$ as expected.
Improving power efficiency is associated with decreased spectral efficiency.

Another useful insight is that the spectral efficiency is proportional to $\delta$.
Thus, from a spectral efficiency standpoint it is desirable to run each carrier at the
highest $\rate$ possible; that is, $\delta = 1$.
If this $\rate$ is not large enough, multiple carriers (MCM) can be used.
On the other hand, if the transmit power is available to support $\delta = 1$ is not available,
$\power$ can be reduced by choosing a smaller $\delta$ at the expense of a smaller $\rate$.
Because of the fixed $\powere$, $\power \propto \delta$.
Finally, $\spectrale \propto 1/K$, 
so increasing the degrees of freedom reduces $\spectrale$.

\section{Choice of $h(t)$}

In the development of this chapter thus far, nothing has been said about $h(t)$
other than the assumption that it has finite bandwidth $B$ and time duration $T$ and unit energy.
It has not been necessary to say more, because from the perspective of
reliability (reflected in the bit error probability $\pe$) and power efficiency $\powere$
the choice of the waveform $h(t)$ does not matter.
Another useful (and perhaps surprising) insight is that the power efficiency $\powere$
is not dependent on the parameters $\{ B_{c} , \, T_{c} , \, K_{c} = B_{c} \, T_{c} \}$.
Whatever these parameters may be, the transmitter can work around them while
maintaining fixed power efficiency through a combination of duty cycle $\delta$
and number of carriers, and achieve any desired information rate $\rate$.

There are however a few practical considerations that weigh in on the
choice of $h(t)$, all of them related to the detection of energy bundles
during both discovery and communication.
This challenge is considered in Chapter \ref{sec:detection}, 
where considerations in the choice of $h(t)$ will be discussed.
These include the receiver designer's ability to guess $h(t)$ in order to
implement an MF,
the design of multi-channel spectral analyzers including the MF,
and most notably immunity to radio-frequency interference (RFI).

\chapter{Discovery}
\label{sec:discovery}

To state the obvious, interstellar communication cannot occur unless
a receiver can discover the presence of an information-bearing signal.
Discovery is the grand challenge of interstellar communication because
of the lack of explicit transmitter/receiver coordination and the ''needle
in a haystack'' problem of searching for a viable signal over a large
range of spacial, temporal, and frequency parameters.
Even in the absence of reliable recovery of embedded information,
discovery of a signal
established as having a technological (as opposed to natural) origin
is valuable to the receiver,
because it reveals the existence of extraterrestrial life and a present or past
intelligent civilization capable of creating technologies.

In this Chapter the challenge of discovery of signals designed for
power efficiency is analyzed.
We start with some background and a basic set of assumptions
that will form the basis of this analysis.

\section{Background}

Before attempting a serious attempt at discovery,
some basic questions must be cleared up.
What kind of signals are we trying to discover?
What distinguishes a ''better'' and ''worse'' design of a signal
from the perspective of discovery?
What are the tradeoffs that must be resolved in discovery?

\subsection{Categories of signals to be discovered}

Past and present SETI observation programs have
emphasized discovery of a beacon, rather than recovery of information.
What is a beacon?
Here we define a beacon as a signal that is intended to be
discovered, but not intended to convey information, such as the
signals described in Chapter \ref{sec:infosignals}.
Within this expanded context, and from the perspective of
discovery, three categories of signals can be identified:
\begin{description}
\item[Beacon.]
This signal does not embed information, but is intended to
be easily and efficiently discovered.
\item[Information-bearing signal.]
This signal is designed as the most efficient bearer of information,
without considering the challenges of discovery.
This was the perspective taken in Chapter \ref{sec:infosignals}.
\item[Discovery-optimized information-bearing signal.]
This signal is optimized for easy and efficient discovery,
but also embeds information in a way that does not compromise discovery.
The need for this category follows from the very different design
criteria that govern discovery and information extraction at low powers.
\end{description}
This chapter will analyze the discovery characteristics of all three
categories.
Our conclusion is that within the low-power regime, beacons and discovery-optimized
information-bearing signals are performance-equivalent.
That is, there is no advantage to transmitting a beacon, as it is neither
easier to discover nor does it offer any other advantage such as lower average power
at a given discovery reliability.
Any civilization going to the trouble to transmit a discovery-optimized signal
is well advised to embed information within it.
On the other hand, discovery-optimized information-bearing signals
are likely to have relatively low average power $\power$, and thus relatively low information rate $\rate$.
When the power resources are available to increase both $\power$ and $\rate$ then the resulting
information-bearing signal can be even more discoverable with less imperative to power-optimize for discovery.

\subsection{Signals structured around energy bundles}

This report in its totality addressed power-efficient and power-optimized design.
In this context, it can be assumed that all three signal categories are
 structured around time-frequency patterns of energy bundles.
 The energy bundle building block is a relatively short time-duration and
 relatively low bandwidth signal that bears some amount of energy.
 It is based on a waveform $h(t)$ that has a bandwidth $B$ and time duration $T$
 that falls in an interstellar coherence hole (ICH) as described further in Chapter \ref{sec:incoherence}.
 
 What is the justification for this assumption?
 In the case of information-bearing signals, this signal structure avoids most interstellar channel
 impairments and thus allows the design to approach the fundamental limit on power efficiency
 as described in Chapter \ref{sec:fundamental}.
 In the case of a beacon, energy bundles
confined to an interstellar coherence hole (ICH),
can be detected without any processing related to impairments in the interstellar channel
other than noise and scintillation.
This is significant since discovery is a processing-hungry process.
This also improves the discovery reliability because the processing that is avoided
will generally enhance the noise and worsen the noise immunity.
Finally,
basing all categories of signal on energy bundles allows the same front-end processing
(matched filtering combined with multi-channel spectral analysis)
to be employed in simultaneously seeking all three categories of signals.

Consistent with this assumption,
present and past SETI searches seek such energy bundles, typically
based on the assumption of a sinusoidal signal or pulse combined with 
phase-incoherent multichannel spectral analysis.
The two major differences between the present work and that past practice,
which is based on the prescription of the Cyclops study \citeref{142}
is twofold:
\begin{description}
\item[Expanding the signal waveforms.] 
Here $h(t)$ is allowed to be any waveform that conforms to the
ICH constraints for a given line of sight and carrier frequency.
Generally this class of waveform includes sinusoidal signals.
In practical terms this implies an enhanced multi-channel spectral analysis
that also incorporates filtering matched to non-sinusoidal signals,
although certainly as a starting point it is sufficient to begin with sinusoidal signals.
\item[Pattern recognition of intermittent signals.]
Power-efficient and power-optimized signals are consistently intermittent,
so short-term persistence of the signal cannot be counted on.
Thus, the pattern recognition algorithms following the detection of energy bundles
has to be more general, including not relying on persistence.
\end{description}

\subsection{Decomposition of the discovery process}

Discovery of a signal structured around energy bundles becomes a two-stage process:
\begin{description}
\item[Energy detection.]
The first stage is the detection of a single energy bundle.
In making a large number of observations in different locations
(with spatial, temporal, and frequency variables), a single positive detection then triggers the second stage.
With power-efficient and low-power signals a much larger number of observations with the same
spatial and frequency variables is necessary to have a reasonable chance to
successfully detect an energy bundle.
This is because (a) such signals are intermittent and hence many observations
will not coincide with an energy bundle
and (b) lower-power signals depend more strongly on periods of
high received signal flux due to scintillation, and these favorable periods are present only
a fraction of the time.
\item[Pattern recognition.]
The receiver develops more convincing statistical evidence of a discovery
by detection of more than a single energy bundle with the same spatial characteristic
but with different temporal and frequency coordinates consistent with a low-power signal.
Unlike power-inefficient and high-power signals, short-term persistence of the signal is not expected.
That is,
an energy bundle is unlikely to be followed immediately by another energy bundle,
so the pattern recognition has to take account longer periods of time
and different (although relatively nearby) frequencies.
The pattern recognition algorithms are not looking for any prescribed deterministic pattern,
since in fact the location of energy bundles is likely to vary randomly in
accordance with embedded information.
\end{description}
In the energy-detection stage we are seeking a
\emph{signal of interest} (SoI).
This SoI is distinguished by its non-natural origin,
and could be either information-bearing or
information-free (a beacon).
At the energy-detection stage these two cases
will not be distinguishable, but during the pattern
recognition phase the relevant characteristics of the
SoI will be estimated, including the presence or
absence of embedded information.

\subsection{Discovery reliability}
\label{sec:discoveryrel}

In evaluating any strategy for discovery, we
are primarily concerned with these probabilities,
\newcommand{\pa}{P_{\text{A}}}
\begin{align*}
&\pd = \prob{ \text{''SoI detected''} \left. \right| \text{''SoI is present''}} \\
&\pa= \prob{ \text{''SoI is present''} \left. \right| \text{''SoI detected''}} \,.
\end{align*}
The miss probability
$(1-\pd)$ tells us how frequently,
given that an SoI is present, the strategy fails to flag that signal location
as worthy of further examination.
Of course we want $\pd \approx 1$.
The accuracy probability $\pa$ recognizes that sometimes an SoI detection
is in error, by which we mean the discovery strategy
says an SoI is present when in fact the observations consist of noise alone.
Of course we want $\pa \approx 1$ as well.

In order to determine $\pa$, it is necessary to know two other
probabilities,
\begin{align*}
&\pfa = \prob{ \text{''SoI detected''} \left. \right| \text{''noise alone''} }\\
&\pb = \prob{ \text{''SoI is present''} }
\end{align*}
The false alarm probability $\pfa$ tells us how often the discovery strategy
incorrectly flags a SoI when the observations consist of noise alone.
Of course we desire $\pfa \approx 0$.
The SoI probability $\pb$ is the a priori probability that an SoI
is in fact present.
It is not a feature of the discovery strategy, but rather an assumption
about the frequency with which SoI can be expected will be present
in our observations.
These is no completely convincing way to choose
a specific value for $\pb$, but surely it is very small.
Based on these probabilities, $\pa$ becomes
\begin{equation}
\pa = 
\frac{\pd \cdot \pb}{\pd \cdot \pb + \pfa \cdot (1 - \pb )}
\approx \frac{1}{\displaystyle 1+\frac{\pfa}{\pb}}
\end{equation}
When $\pb \ll \pfa$,
most detections of an SoI are actually false alarms,
and thus most of the time a detected SoI is actually noise alone.
On the other hand, when $\pfa \ll \pb$
$\pa \approx 1$ and a detection is much more meaningful because
most of the time it flags that an SoI that is actually present.
The important conclusion is that
to avoid wasting a lot of effort further analyzing a signal location
(or to have the confidence to announce the discovery in a public press release)
$\pfa$ must be mighty small, in particular much smaller than $\pb$.

The two direct metrics of discovery strategy performance are
$\{ \pfa , \, \pd \}$.
The analysis of these probabilities can be applied at any stage of the discovery process. 
In the following analysis, this analysis will be applied to the initial 
energy bundle detection stage.
At this stage,
$\pfa$ is defined as the probability that one or more energy bundles are
declared present in the $L$ observations in the presence of noise alone.
$\pd$ is defined as the probability that one or more energy bundles are declared
present when in fact a SoI overlaps the observations.
In numerical examples the values $\pfa = 10^{-12}$ and $10^{-8}$ will be chosen
to get some idea of the sensitivity of the resulting $\{ \pd , \, L \}$ to the desired reliability.
These values of $\pfa$ are not nearly small enough to give us confidence in the discovery
of an SoI, but they are reasonable objectives for the
energy detection stage.
Dramatically further reducing $\pfa$ is the function of the subsequent pattern recognition stage, which
observes the location and nearby locations for each discovered energy bundle over a longer period of time,
looking for additional energy bundles and eventually identifying a recognizable pattern.
Eventually, after a much longer period of observation
we can hopefully develop sufficient confidence that an SoI is actually present
(low enough $\pfa$ to assert that $\pa \approx 1$)
to announce that conclusion to the world.

\subsection{What makes a design good for discovery}

In this report the focus is on design of a transmitted
signal with the goal of minimizing the average received power
that is necessary to discover that signal.
However, the ''minimize power'' criterion of design has
to be defined more carefully to distinguish discovery from communication.
During communication the
criterion of power efficiency was adopted in Chapter \ref{sec:fundamental}.
This criterion has no relevance to discovery,
so a different metric called \emph{power optimization} is needed.

Unless the received power is very large, in the energy-detection stage
to achieve simultaneously $\pfa \approx 0$ and $\pd \approx 1$
requires more than one independent observation by the receiver.
Therefore, assume there are $L>1$ observations.
An appropriate figure of merit for a signal design with respect to its
discoverability is the value of $L$ required to achieve a fixed $\pfa$ and $\pd$.
A design is said to be ''power-optmized for discovery''
when $L$ is minimized for a given average power $\power$
and a given reliability $\pfa$ and $\pd$.
This criterion attempts to satisfy both transmitter and receiver
by jointly minimizing transmit power and the
computational resources that the receiver must devote to discovery,
subject to a constraint on the reliability of discovery.

\subsection{Important role of duty cycle in discovery}

Our approach in comparing different signals from a discoverability
perspective is to (a) optimize the signal to minimize the required $L$
and (b) determine how the resulting $L$ varies with received
signal power $\power$.
One conclusion is that to achieve a low signal power
for either a beacon or an information-bearing signal,
the signal design much be intermittent
rather than continuously transmitted.
A continuously transmitted signal
as was assumed in the Cyclops study \citeref{142}
has been assumed in many current and past SETI searches,
but such a signal design must have a significantly larger $\power$
than is necessary.

For a fixed average power, as the duty cycle $\delta$ of the beacon is reduced
the peak power level is increased by a factor of $1/\delta$.
Such a beacon is illustrated in Figure \ref{fig:beaconDutyCycle},
and compared to a continuously transmitted beacon and a simple
information-bearing signal, also with low duty cycle.
With small $\delta$, many observations will not overlap energy bundles,
so this increases the necessary value of $L$.
On the other hand, for a given value of $\power$,
a small $\delta$ increases the amount of energy within each bundle
and thus increases the probability that a bundle that does overlap an
observation will be detected.
Given this tradeoff, a principled choice of $\delta$ 
follows the power-optimization criterion, which is to
choose $\delta$ so as to minimize $L$.
We will see that the resulting reduction in $L$ can be very large,
 in one case by about twelve orders of magnitude
(from $L \approx 10^{15}$ to $10^{3}$).
Thus, choosing a designed low-duty cycle is
generally very compelling in terms of its
reduction in the receiver's processing resources for a given received
average power $\power$, unless $\power$ is already so large
that $L \approx 1$.

\incfig
	{beaconDutyCycle}
	{.8}
	{
	An illustration of a beacon with duty cycle $\delta$ for $\delta = 1$ and $\delta = 1/8$.
	To keep the beacon average power constant, the energy per bundle
	is proportional to $1/\delta$, as illustrated by the saturation of color.
	With appropriate choice of $\delta$, this higher energy can very significantly reduce
	the number of observations $L$ by allowing the detection of an energy pulse to
	be more reliable for each observation that happens to overlap
	an energy pulse.
	Two examples of $\delta = 1/8$ are shown: uniform spacing
	(which tails to convey information)
	and pulse-position modulation (PPM) which is an information-bearing signsl
	rather than a beacon.
	Both signals have the same discovery properties.
	}

Depending on the category of signal, there are several
ways in which a low duty cycle can occur:
\begin{description}
\item[Reducing information rate by reducing duty cycle.]
An example of this is M-ary FSK when the information rate and power have been reduced
by slowing the rate at which symbols are transmitted, as illustrated in Figure \ref{fig:FSKvsDelta}.
The need to reduce $\power$ (with an attendant reduction in $\rate$)
is naturally accompanied by a reduction in duty cycle.
\item[Increasing peak power by reducing duty cycle.]
As illustrated by the beacon in Figure \ref{fig:beaconDutyCycle},
a beacon's average power can be held fixed as the duty cycle is reduced,
thereby increasing the power during the fraction of time $\delta$ that the signal is transmitted.
This beneficially increases $\pd$ for a fixed $L$ in cases where the greater chance of observing during
the duty-cycle ''off'' period is more than compensated by the higher probability of detecting
a signal for observations that occur during the ''on'' period.
\item[Channel codes with inherently low duty cycle.]
This is illustrated in Figure \ref{fig:beaconDutyCycle} by an M-ary PPM information-bearing signal.
PPM is a different type of example 
in which a power-efficient information-bearing signal for which $\delta < 1$
because information is conveyed by the location of energy bundles in time.
In Chapter \ref{sec:infosignals}  this property was cited as a possible disadvantage
of PPM relative to FSK.
However, from the perspective of discoverability that intermittent character becomes
an advantage at low average powers.
\end{description}

\subsection{Antenna-processing tradeoffs in discovery}

It will be demonstrated that information-bearing signals can be discovered
at considerably lower average power levels than is required to reliably extract information.
This is achieved by increasing the number of observations $L$ in conjunction with
 the property of scintillation that it sometimes behaves like an ''amplifier''
of signal flux rather than just an ''attenuator''.
What is the point of discovering an information-bearing signal at a lower power
than information can be extracted from it?
One answer is that the signal has beneficially attracted the attention of the receiver,
and established the existence of a technologically advanced civilization in a given
location.
This alone is of considerable value to the receiver.

But there is an even better answer.
The received signal power at baseband is proportional to the
antenna collection area.
When a receiver discovers an SoI, 
if the average power $\power$ proves to be insufficient to reliably
extract information from that SoI
(or even reliably ascertain whether the SoI embeds information),
the receiver designer has the option of increasing
the collection area of its receive antenna as one measure in
studying that SoI further.
This points to an important tradeoff for the receiver designer between
antenna collection area and the processing resources associated with multiple observations.
A cost-effective approach during the discovery stage is to 
trade off the cost of processing against antenna collection area,
and choose a minimum-cost point based on the characteristics of the available technology.
Then when an SoI is discovered, the collection area can be increased to explore
more fully its characteristics, including uncovering and extracting embedded information,
which is something that no amount of processing can accomplish.
This incremental investment strategy, which permits the expenditure of resources
only when justified by experimental outcomes, is an attractive option for receiver designer.

%Actually, the Shannon limit does apply indirect.
%The Shannon limit teaches us that the received energy per bit $\energybit$
%is the important signal parameter, with a lower bound on that quantity
%proportional to the noise power spectral density $N_{0}$ if the goal is
%reliable extraction of information.
%But a beacon is intended to carry one bit of information; namely,
%''we are here'' or ''we are not here''.
%The transmitter of a beacon does not know when the receiver might be
%looking in the right location, so it must transmit a beacon indefinitely.
%The receiver has no bound on the time it can take deciding on the
%presence or absence of a beacon.
%Thus, the energy available to the receiver to make its decision is
%effectively unlimited, regardless of how low the received power may be.
%This suggests that a beacon can be detected at very low powers,
%much lower than necessary to convey information, and perhaps
%even at arbitrarily low powers.
%In fact that is the case, but there is a practical limit based on how
%long the receiver is willing to look.
%
%Actually pretty much the same is true of information-bearing signals.
%The signal must be transmitted indefinitely, and for purposes of
%discovery the receiver can look for as long as it chooses.
%Thus, because the receiver is not attempting to extract information,
%the energy available to it for purposes of discovery is effectively
%unlimited.
%Furthermore, we have shown that the power efficiency of
%an information-bearing signal is constant, both at fundamental
%limits and in concrete designs.
%This implies that $\power \propto \rate$, and an information
%bearing signal can be transmitted at arbitrarily low $\rate$,
%necessitating correspondingly low $\power$.
%Thus, one way to think of a beacon is as an information-bearing
%signal in the limit of $\rate \to 0$.
%Thus, there is little motivation to transmit a beacon, since one
%might as well transmit an information-bearing signal with a
%small $\rate$.
%
%There is really not a very big difference between the two
%types of signal for purposes of discovery.
%Both types of signals can be discovered for arbitrarily low
%received powers if the receiver is patient enough.
%The beacon does have a practical advantage, however,
%in that not attempting to convey an ongoing information stream
%allows it to be designed with only discovery in mind.
%We show that for a given receiver observation time,
%the beacon can as a result be recovered at lower received powers.
%The reason is that by locating energy bundles according to the information it is conveying,
%the information-bearing signal increases the opportunities for false alarms during discovery.

%Our philosophy of beacon design follows that of Chapter \ref{sec:fundamental}
%in our focus on power efficiency.
%The meaning of power efficiency is somewhat different, however.
%The power efficiency is defined as the lowest power than can achieve
%a given objective on $\pfa$ and $\pd$.
%As in Chapter \ref{sec:fundamental}, the design of a power-efficient
%beacon does not constrain bandwidth, but strictly focuses on minimizing
%receive (and hence transmit) power.
%Scintillation does not affect average received power
%(see \eqref{eq:sigmasone}), 
%and hence a transmitter designer knowing the distance to the target star
%(at least to some accuracy) and knowing the characteristics of its transmit
%antenna can predict the received power flux.
%The remaining uncertainty is primarily the characteristics of the receive
%antenna.
%A beacon can be designed assuming a minimum receive antenna
%collecting area, for example an area typical of radio astronomy.
%Subject to this uncertainty, it is a reasonable objective for the transmitter
%to consciously design the most power efficient beacon possible,
%because that will pay dividends in the energy cost of transmission.
%
%A fundamental property of power-efficient beacons is uncovered.
%They are intrinsically information-bearing!
%This is because power-efficient beacons do not transmit continuously,
%but rather intermittently in order to conserve average transmit power.
%Making that intermittency random is beneficial to the discovery function.
%Once we stipulate that the beacon transmission is randomly intermittent,
%it is a small step to couple that intermittency to information, with
%no penalty in power efficiency.
%In Chapter \ref{sec:infosignals} the design of power-efficient
%information-bearing signals is considered.
%It is shown there that such signals can also, without penalty in power efficiency,
%serve as power-efficient beacons.
%Thus, in power-efficient design there is a complete convergence of
%beacons and information-bearing signals: they are, in fact, one and the same!
%This beneficially provides another source of implicit transmitter/receiver
%coordination.
%The design of a signal that serves both purposes well further constrains that
%signal, both in terms of structure and parameterization, reducing the
%complexity of discovery searches.


\section{Beacons power-optimized for discovery}

Beacons structured around transmitting a pattern of energy bundles
made a good starting point for addressing 
the issues surrounding power-optimization for discovery.
We make the reasonable assumption that a beacon consists of
a \emph{periodic} sequence of energy bundles as was illustrated in Figure \ref{fig:beaconDutyCycle}.
These results are relatively easily extended to information-bearing signals,
which we note are as discoverable as beacons.

\subsection{Beacon structure and parameters}

The three parameters of a periodic beacon and its
discovery are illustrated in Figure \ref{fig:beaconParam}.
Each energy bundle is assumed to have duration $T$,
and bundles are spaced $T_{p}$ apart, implying a duty cycle
\begin{equation}
\delta_{p} = \frac{T}{T_{p}} \,,
\end{equation}
where $0 < \delta_{p} < 1$.
One observation interval, which begins at a random time,
is assumed to have duration $T_{o}$.
An individual energy bundle is said to fall in an observation if the
observation interval completely overlaps the time duration of the bundle,
so that an MF captures its full energy.
Assume that a single observation occurs at a random time relative to the
periodicity of the beacon.
Then the average number of energy bundles in that observation is
$(T_o - T) / T_p$.
%\begin{equation}
%\label{eq:avgbundles}
%\frac{T_{o} - T}{T_{p}} = n_{o} + \delta_{o}
%\end{equation}
%where $n_{0} \ge 0$ is an integer and $0 \le \delta_{o} <1$.
For example, there is always exactly one energy bundle in each 
observation when $T_{o} = T_{p} + T$.
%in which case $n_{o} = 1$ and $\delta_{o} = 0$.
%When $\delta_p$ is small, the interval between energy bundles is large
%and it is far more likely that $T_o \ll T_p$.
Another example is $T_o = 2 T$,
%In that case $n_o = 0$ and $\delta_o = \delta_p$.
in which case there is always either zero
(probability $(1-\delta_p)$) or one (probability $\delta_p$)  
energy bundle overlapping a given
observation.

\incfig
	{beaconParam}
	{1}
	{
	An illustration of the three parameters of a periodic beacon and its observation.
	The parameters are the duration of an energy bundle $T$,
	the time interval between energy bundles $T_{p}$, 
	and the duration of one observation $T_{o}$.
	}

Finally, there are assumed to be $L$ observations, spaced far enough apart in time
that they are statistically independent.
This implies that the spacing between observations is large relative to
the coherence time of the channel as described in Chapter \ref{sec:incoherence}.
Each observation is assumed to begin at a random
time relative to one period of the beacon.

\subsection{Tradeoffs in detection reliability}

Short of doing a full analysis of the beacon reliability,
some simple calculations reveal much about the tradeoffs in
power-optimized beacon design.

\subsubsection{Observations overlapping energy bundles}

There are two ways in which a failed detection (miss) can occur.
First, when $T_{o} < T_{p}+T$ it can happen
that no energy bundles fully overlap an observation,
and this occurs in a single observation with probability $(T_{o} - T)/T_{p}$.
Second, even if one or more energy bundles overlaps an observation,
noise may prevent it from being detected.
The first effect can be isolated by an upper bound
that results from ignoring the second possibility,
\begin{equation}
\label{eq:Llowerbd}
\pd \le 1 - \left(1-\frac{T_{o}-T}{T_{p}} \right)^{L} 
\ \ \ \ \text{or} \ \ \ \ 
L \ge \frac{\log \left( \frac{1}{1 - \pd} \right)}{\log \left(\frac{T_{p}}{T_{p}-T_{o}+T} \right)} \,,
\end{equation}
This relation reveals how large $L$ must be chosen to overcome
the duty cycle effect, and we will find it to be accurate
for very small duty cycles.

\subsubsection{Total energy principle}

We now state two easy-to-apply criteria that
turn out to accurately predict the reliability with which a beacon
can be detected in $L$ observations.
The first is the  \emph{total energy} principle, which predicts that
a certain fixed total signal energy in the 
collective $L$ observations is required for detection at a fixed
level of reliability as measured by $\{ \pd , \, \pfa \}$.

In the case of information-bearing signals,
the reliability of information extraction
is determined by $\energybit$, the received energy per bit.
A beacon is designed to convey a single bit of information,
namely whether ''beacon is present'' or ''beacon is not present''.
Thus, it is a reasonable to assume that the total received energy
available for observation is germane to the reliability with which
that one bit of information can be extracted.
%To apply this principle, we must recognized that,
%for intermittent signals some observations may not overlap energy packets..

%To illustrate this principle,
%consider the special case $T_o = 2 T$, for which $\delta_o = \delta_p$.
To apply this principle,
the average power of the beacon is
$\power = \energy_h / T_p$,
%\begin{equation}
%\label{eq:powervsdeltap}
%\power = \frac{\energy_h}{T_p} = \frac{\delta_p \, \energy_h}{T}
%\end{equation}
where each bundle has energy $\energy_h$.
The average total energy available for observation is
%\begin{equation}
%\label{eq:totalenergy}
%\expec{\energy_{\text{total}}} =
%L \, \delta_{p} \, \energy_h =
%L \, \power \, T \,.
%\end{equation}
\begin{equation}
\label{eq:totalenergy}
\expec{\energy_{\text{total}}} =
L \cdot \left( \frac{T_o - T}{T_p} \right)  \cdot \energy_h =
L \, \power \, ( T_o - T ) \,.
\end{equation}
The first term is the number of observations, the
second is the average number of energy bundles per observation,
and the third term is the amount of energy in each bundle.
There are several interesting conclusions that follow from \eqref{eq:totalenergy}.
First, for fixed $\{ \power, \, T,  \, T_o \}$ the total observed energy does
not depend on $T_p$ and hence the duty cycle $\delta_p$.
Second, under the same conditions
the average total energy increases with $L$ without bound,
so the total energy hypothesis would suggest that 
for any $\power$ no matter how small a beacon can
be detected with any given reliability by choosing $L$ sufficiently large.

The third observation is more subtle.
As expected, the value of $L$ decreases as $T_o$ increases,
so there is a tradeoff between the number of observations and the
time duration of each observation.
However, this can be misleading 
since statistically independent observations make a larger
contribution to reliability than observations that are closely
spaced and hence more likely to experience similar received scintillation flux.
Thus, increasing $T_o$ up to a value $T_o = T_p + T$ will
reduce $L$ in direct proportion, but beyond that
there can be more than one energy bundle per observation,
and this is not as effective as increasing $L$.

\subsubsection{Bundle energy principle}

The total energy principle offers no insight into the appropriate
duty cycle $\delta_p$.
A second principle, the \emph{bundle energy} principle states that as the average power $\power$
is changed, the energy in each individual bundle should remain fixed,
and this can be accomplished by manipulating the duty cycle $\delta_{p}$.

%Although the total energy does not depend on $\delta_p$,
%\eqref{eq:powervsdeltap} indicates that the $\power$ is proportional
%to the product of $\delta_p$ and $\energy_h$.
The reliability of detection at the level of a single energy bundle
will depend on $\energy_h$.
As $\power$ is varied, this principle states that
$\energy_h$ should be kept constant in order to maintain a fixed
reliability in the detection of an individual energy bundle.
From this, $\delta_p = T / T_p$ becomes
%\begin{equation}
%\label{eq:deltapvspower}
%\delta_p = \frac{\power \, T}{\energy_h} \,.
%\end{equation}
\begin{equation}
\label{eq:deltapvspower}
\energy_h = \power \, T_p
\ \ \ \ \text{or} \ \ \ \ 
\delta_p = \frac{\power \, T}{\energy_h}
\le  \frac{\power \, T_c}{\energy_h} \,.
\end{equation}
As $\power$ is decreased,
reducing the duty cycle $\delta_p$ can
be avoided by increasing $T$,
but the time coherence of the channel limits this to $T \le T_c$.
Beyond this, maintaining high reliability in the detection of individual energy bundles
as $\power$ is reduced
requires also reducing the duty cycle $\delta_p$ so that $\energy_{h}$ can be kept fixed.

\subsubsection{How to reduce average beacon power}

The two principles guide the reduction in beacon average
power without affecting detection reliability, namely by choosing
$L \propto 1/\power$ and $\delta_p \propto \power$.
There are two effects that must be overcome in choosing a value for $L$.
The first is the \emph{duty cycle effect}, which is the presence
of an energy bundle in only a fraction of the observations
due to intermittent transmission.
The second is the \emph{scintillation effect}, which is 
a received signal flux sufficiently large to permit reliable
detection of an individual energy bundle in only a fraction of the observations.

%The average received power $\power$ can be decreased
%as much as we like, at the expense of a growing
%number of observations $L$.
%To maintain fixed detection reliability as $\power$ decreases,
%the duty cycle $\delta_p$ should also decrease.
%By reducing $\delta_p$, the energy per bundle $\energy_h$ can
%be kept fixed even as $\power$ decreases.
Achieving very low $\power$ requires action on the part of
both the transmitter and receiver designers.
The transmitter has to reduce the duty cycle, and the
receiver has to increase the number of observations it makes
in each location.
Fortunately, these actions need not be coordinated.
The transmitter can reduce its average transmit power
as long as it also reduces $\delta_p$ in proportion,
keeping $\energy_h$ fixed.
This gives the receiver an equal chance at detecting the
beacon, although only those receivers that choose a
sufficiently large $L$ or sufficiently large observation time $T_o$
to account for the lower duty cycle.
From the receiver perspective, increasing antenna collection area
or observation time $T_o$ (up to a limit) or number of observations $L$ will
allow lower received average power beacons to be detected, regardless
of the duty cycle chosen by the transmitter.

\subsection{Detection reliability for a periodic beacon}

The intuitive logic of the last section is very helpful to build intuition,
but fails to take account of (a) the statistical variation in the
number of energy bundles that overlap observations and (b)
the relationship between $\energy_h$ and detection reliability.
Thus, the conclusions there are only approximate.
Exact results are derived in Appendix \ref{sec:Lobs},
making use results from Chapter \ref{sec:detection}.

The detection reliability is characterized by $\{ \pfa , \, \pd \}$,
where $\pfa$ is the probability of one or more detected energy bundles
out of $L$ observations in the presence of noise alone,
and $\pd$ is the same probability in the presence of a bean.
In general only numerical results are available, but
for the special case $T_{0} = 2 T$ there is a simple analytical relationship
between $\pfa$ and $\pd$,
\begin{equation}
\label{eq:discoveryequation}
\pd [\, \pfa, \, \ecrs, \,  \delta_{p}, \, L \, ]
\approx 1 - \left[ 1-\delta_{p}  \, \left( \frac{\pfa}{2 \, L} \right)^{ \, \frac{1}{1+ \ecrs}} \right]^{\, L}
 \,.
\end{equation}
As a reminder, $\ecrs$ is the energy contrast ratio given by \eqref{eq:ecrs},
$L$ is the number of statistically independent observations,
and $\delta_p = T/T_{p}$ is the duty cycle of the beacon or equivalently the
average fraction of the observations that completely overlap an energy bundle.

%To understand these effects quantitatively,
%the relationship among the parameters $\{\ecrs, \, \delta , \, \pfa , \, \pd , \, L \}$
%can be characterized, and then applied to the different circumstances described above.
%For this purpose, assume that there are $L$ statistically independent
%observations, implying that they are spaced at time intervals larger
%than the coherence time of the channel.
%A detection (with probability $\pd$) is said to occur when one or more energy bundles
%is detected in these $L$ observations, where an energy bundle is present in
%a specific observation with probability $0<\delta \le 1$.
%A false alarm occurs (with probability $\pfa$) under identical circumstances
%except that $\delta = 0$.
%The energy contrast ratio in a specific observation, conditioned on an energy
%bundle present, is $\ecrs$, and it is assumed that the noise power $N_{0}$ is known
%as in \eqref{eq:asympPfaVsPd}.
%Under these conditions,
%it is shown in Appendix \ref{sec:Lobs}
%that \eqref{eq:asympPfaVsPd} is replaced by
%the $L$-observation \emph{discovery relation}
%\begin{equation}
%\label{eq:discoveryequation}
%\pd \left[ \pfa, \, \ecrs, \, \delta, \, L \right] \approx 1 -
%\left(1 - \delta  \left(\frac{\pfa}{L}\right)^{\frac{1}{1+\ecrs}} \right)^L \,
%\end{equation}
%Although an exact relation is easy to derive, this approximation
%is accurate when $\pfa \approx 0$.
%As expected, $\pd [ \pfa, \, \ecrs, \, 1, \, 1]$ reduces to \eqref{eq:asympPfaVsPd}.

%A major factor that is not taken into account in \eqref{eq:discoveryequation} is the search.
%The tradeoff in \eqref{eq:discoveryequation} is conditioned on the matched filter being
%applied in the correct location with respect to spatial and frequency variables,
%and then repeating observations over time.
%In a realistic operational scenario, the receiver is also performing a discovery
%search over these other parameters.
%To a large extent this larger reality can be accounted for by the choice of $\pfa$,
%but a separate analysis of any given search strategy should be undertaken
%to get more accurate results.

$\pd$ is monotonically increasing with $L$, and thus
the receiver always improves reliability by implementing a larger $L$.
For any $\pfa > 0$, $\ecrs > 0$ and $0 < \delta_{p} \le 1$,
\begin{equation}
\pd \underset{L \to \infty}{\longrightarrow} 1 \,.
\end{equation}
Thus, it doesn't matter how small is $\pfa$, $\delta_{p}$, or $\ecrs$,
$\pd \approx 1$ can always be
achieved if $L$ is sufficiently large.
This nice property is a happy outcome of scintillation, since periods
of large flux reliably coincide with an energy bundle in at least one observation if $L$ is sufficiently large.
In this sense, scintillation is the savior of discovery, since
it permits discovery under the most adverse conditions.
However, in practical terms the size of $L$ could easily be too large.
For example, if $L$ is so large that it requires observations over a period of time large relative to the
existence (or for that matter patience) of a civilization, 
in practical terms the beacon is non-discoverable.
The transmitter designer must be aware of this and insure that the received signal flux
at the destination is sufficient for discovery with parameters that it considers feasible and practical.

\subsection{Optimization of duty cycle}

The bundle energy principle suggests that the duty cycle $\delta_p$
should be chosen to keep $\ecrs$ fixed as $\power$ is changed.
The question of choosing $\delta_p$ to minimize $L$ can be
studied more precisely using \eqref{eq:discoveryequation}.
From \eqref{eq:deltapvspower} the energy per
bundle $\energy_h$ and the energy contrast ratio $\ecrs$
are related to the beacon average power $\power$ through
\begin{equation}
\label{eq:xivspower}
\energy_h = \frac{\power \, T}{\delta_p}
\ \ \ \text{or} \ \ \ \ 
\ecrs = \frac{\power \, T \, \vs}{N_0 \, \delta_p} 
= \frac{\xi_0}{\delta_p} 
\end{equation}
where $\xi_{0}$ is a fixed parameter related to $\power$.
For convenience, the following numerical results will be expressed in terms
of the energy contrast ratio $\xi_{0}$ rather than the power.
%Regarding observation time, it is natural to set
%$T_{o} = (n+1) \, T$ in \eqref{eq:avgbundles}, so there is an
%integral number of energy bundle durations in each observation.
%In that case,
%\begin{align}
%&n_{o}+\delta_{o} = n \cdot \delta_{p} \\
%&\pfaa = \frac{\pfa}{ (n+1) \cdot L }
%\end{align}
%and hence $n_{0} = \lfloor n \cdot \delta_{p} \rfloor$.
%where $\lfloor \cdot \rfloor$ is the floor function.
%The total number of potential locations for energy bundles is $(n+1) \cdot L$,
%and $\pfaa$ is the false alarm probability in the detection of an individual
%energy bundle.
%Hence $\pfaa$ has to be a factor of $(n+1) \cdot L$ smaller than $\pfa$
%to account for the multiple observations in the absence of a beacon.
%The baseline case is $n=1$, and lengthening the observation interval by choosing $n >1$
%will, all else being equal, reduce $\pd$.
Then \eqref{eq:discoveryequation} applies to a constant-average-power beacon
with the choice of parameters
\begin{equation}
\pd [ \pfa, \, \xi_{0}/\delta_{p}, \, \delta_{p} , \, L] \,,
\end{equation}
where the beacon power is related to $\xi_0$ through \eqref{eq:xivspower}.
For an average beacon power represented by $\xi_0$
and a target reliability represented by $\{ \pfa , \, \pd \}$, this
equality can be solved numerically to find the tradeoff between
$\delta_p$ and $L$.
The result shown in Figure \ref{fig:Lvsp1} illustrates that at lower
beacon powers there is an optimum value of $\delta_p$
that is a compromise between two competing factors,
the probability that an energy bundle overlaps an observation 
(which dominates $L$ for smaller values of $\delta_{p}$) and
the energy of that bundle (which dominates for larger $\delta_{p}$).
In the high-power regime (in this case corresponding to $\xi_{0} = 15$ and $20$ dB),
$L$ is monotonically decreasing with $\delta_{p}$ and thus $\delta_{p} = 1$ is the best choice
for a beacon power-optimized for discovery.
However, to achieve detection of a low-power regime ($\xi_{0} = 10$,
$5$ and $0$ dB),
there is an optimum value of $\delta_{p} <1$ that minimizes $L$.

\incfig
	{Lvsp1}
	{.8}
	{
	A log plot of the number of observations $L$ vs the transmit duty cycle $\delta_{p}$.
	For each curve, the average beacon power is kept fixed as $\delta_{p}$ is varied.
	For all the plots $\pfa = 10^{-12}$ and $\pd = 0.9999$ are kept fixed.
	The different curves correspond to different
	beacon average powers
	(represented by energy contrast ratio
	$\xi_0$ in dB at $\delta_{p} = 1$).
	The dashed curve is the lower bound on $L$ from \eqref{eq:Llowerbd}
	that captures only misses attributable to $\delta_{p} < 1$.
	This lower bound is accurate for small $\delta_{p}$, where misses
	attributable to the duty cycle dominate.
	}

The bundle energy principle predicts that $\delta_p \propto \xi_0$,
of course with the constraint that $\delta_p \le 1$.
The optimum value of $\delta_{p}$ 
(the minimum of the curves in Figure \ref{fig:Lvsp1})
as a function of $\xi_{0}$ is shown in Figure \ref{fig:optP1vsSNR},
where we see that it closely adheres to this principle.
As one anchor,
the optimum duty cycle is 3.0\% at $\ecrs = 0$ dB,
and this duty cycle works well for $L < 1000$.
This value will be used in subsequent numerical results.

\incfig
	{optP1vsSNR}
	{.6}
	{A log plot of the optimum duty cycle $\delta_{p}$ as a function of
	the beacon average power (represented by
	$\xi_{0}$ in dB) for the same conditions as in Figure \ref{fig:Lvsp1}.
	At $\xi_{0} = 0$ dB, the optimum value is $\delta_{p} = 0.030$ (3\%).
	The value of $\delta_p$ predicted by the
	bundle energy principle ($\delta_p \propto \xi_0$)
	is shown as the dashed line.}

The effect of reducing the duty cycle on
the number of observations $L$ is illustrated in Figure \ref{fig:optLvsSNR}.
In the low-power regime, the effect of using a low transmit duty cycle
is quite dramatic.
For example, at $\xi_{0} = 0$ dB, the value of $L$ is reduced by about
12 orders of magnitude (to $L=848$) by reducing the duty cycle from $\delta_p = 1$
to $\delta_p = 0.03$ (3\%).
Clearly it is not practical to discover a continuous beacon at this low power,
but reducing the duty cycle to 3\% saves the day as long as the receiver is
willing to implement hundreds of independent observations.
An alternative way to quantify the effect of duty cycle is to measure horizontally
rather than vertically.
The reduction in signal
power that is possible for a fixed $L = 848$ observations attributable to reducing the
duty cycle, which is $8.3$ dB, or an 85\% reduction in average beacon power.

\incfig
	{optLvsSNR}
	{.8}
	{A log plot of the number of observations $L$ required to achieve the same
	performance parameters as Figure \ref{fig:Lvsp1} vs
	the average beacon power (represented by $\xi_{0}$).
	This is shown for both a 100\% duty-cycle ($\delta_{p} = 1$)
	and for the optimum duty cycle $\delta_{p}$.}

The level of reliability that is demanded in the detection of a beacon has an
impact on the required $L$ as illustrated in Figure \ref{fig:optLvsSNRlowDuty}.
If lower reliability is demanded, of course this reduces the required $L$.
The prediction of the total energy principle that $L \propto 1/\xi_0$
(modified slightly so that $L \to 1$ as $\xi_0 \to \infty$)
is shown by the dashed line.
This prediction is fairly accurate, but notably only if $\delta_p$
is chosen optimally
(or equivalently the bundle energy principle is applied simultaneously).

\incfig
	{optLvsSNRlowDuty}
	{.8}
	{Figure \ref{fig:optLvsSNR} is repeated showng only the
	number of observations required when the transmit duty
	cycle $\delta_{p}$ is optimized to minimize $L$. Two levels of reliability are shown:
	''More reliable'' is  $\pfa = 10^{-12}$ and $\pd = 0.9999$
	(the same as in Figure \ref{fig:Lvsp1})
	and ''Less reliable'' is $\pfa = 10^{-8}$ and $\pd = .99$.
	Smaller $L$ results in reduced reliability.
	The dashed lines illustrate the prediction of the
	total energy principle that $L \propto 1/\xi_0$.
	}

The overall conclusion is that imposing a multiple-observation requirement
on the receiver can have a dramatic impact in reducing the required transmit power.
For the detection reliability parameters $\{ \pfa, \, \pd \}$ chosen in Figure \ref{fig:Lvsp1},
increasing the number of observations from $L = 10$ to $L = 831$
reduced the required average transmit power by $17$ dB, or a linear
factor of about $50$.
The transmitter designer may view this imposition on the receiver
as relatively modest in light of its 98\% reduction in average transmitted power,
especially since it is the receiver that derives all the value from successful 
beacon discovery.
A second conclusion is that a low duty cycle $\delta_{p}$ is required in the transmitter
if $L$ is to be kept to a reasonable level in the low-power regime.
Of course small $\delta_p$ in itself implies a relatively large $L$, so there
is no avoiding a relatively large $L$ for low-power beacons.
Indeed, past and present SETI searches would have a negligible hope of success
in discovering a beacon power-optimized for discovery in the low-power regime.
	
%This is illustrated in Figure \ref{fig:discoveryReliability}, where
%$P_{\text{D},L}$ is plotted against both $L$ and $P_{\text{FA},L}$.
%For any $\ecrs$, the detection probability increases markedly as $L$ is increased.
%However, at the lower values of $\ecrs$ the number of observations has to be very large to
%achieve $\pd \approx 1$.
%At $L = 50$ the achievable pairing of $\{ P_{\text{FA},L} , P_{\text{D},L} \}$ is reasonable when
%$\ecrs \ge 15$ dB.
%It will be shown in Chapter \ref{sec:infosignals} that $\ecrs \approx 15$ dB is a reasonable
%target for reliable communication in the absence of channel coding
%(with channel coding, lower values of $\ecrs$ become feasible).
%This typical case requires $L \approx 50$ independent observations to achieve
%simultaneously high detection probability and low false alarm probability.
%
%\incfig
%	{discoveryReliability}
%	{.7}
%	{For the same four values of $\ecrs =$ 5, 10, 15, and 20 as in Figure \ref{fig:detectionProbability}, 
%	a log-log plot of the detection probability $P_{\text{D},L}$ for $L$ statistically
%	independent observations.
%	On the top the horizontal axis is $L$ for $P_{\text{FA},L} = 10^{-12}$,
%	and on the bottom the horizontal axis is $P_{\text{FA},L}$ for $L = 50$.
%	 }
%
%As others have previously noted \citeref{121}, scintillation is of major importance to discovery.
%Most of the time it reduces the possibility of discovery by adding excess attenuation
%to the received power, but fortunately it also sometimes creates periods of higher power.
%If we are patent enough (revisit the same carrier frequency enough times for
%a given line of sight) then arbitrarily high detection probability can be achieved
%for any $\pfa > 0$ and for any $\ecrs >0$.
%Because of scintillation, in a fundamental sense discovery of information-bearing
%signals is not a limiting factor.
%
%In the presence of data modulation (Section \ref{sec:datamoddisc}), 
%multiple observations are also important
%since detection may missed simply because $A = 0$.
%Observations spaced out more than the coherence time of scintillation
%are equally helpful, but more closely spaced observations are also useful
%in countering the effects of data modulation.

\subsection{Consequences of non-coordination}

In practice, the responsibility for choice of parameters is distributed between transmitter
and receiver, and without the possibility of coordination.
It is the transmitter that determines the parameters $\{ T, \, T_{p} \}$,
and it is the receiver that chooses the parameters $\{ \pfa , \, T_{o},  \, L \}$.
Both the transmitter and receiver designers have influence over $\ecrs$,
the transmitter through choosing the transmit power and transmit antenna gain
and the receiver through choosing the receive antenna gain.
Thus, $\pd$ is not entirely under the individual
control of either transmitter or the receiver designers.
The receiver designer will presumably choose values 
for $\{ \pfa , \, T_{o}, \, L \}$ based on
operational objectives, capital budget, and speed of a search.
These choices divide parameters $\{ \ecrs , T, \, T_{p} \}$ 
into two regions, one for which $\pd$ is acceptable, and the
other for which it is not.

This was illustrated in Figure \ref{fig:beaconCompare}
for a choice $\delta = 0.03$ (3\%) and $L = 1000$.
Even though the parameters were optimized for a very low average power
corresponding to $\xi_{0}$ dB, the figure illustrates how results vary for a range
of larger $\xi_0$.
In particular, larger beacon power is always preferable
in terms of achieving a higher $\pd$ (smaller miss probability).
There is a 28.5 dB gap in achievable $\xi_{0}$ required to realize $\pd = 0.9999$
due to the choice of a 3\%  duty cycle rather than 100\%.
This corresponds to a linear factor of 708 reduction  (99.86\%) in average
beacon power.
However, this does assume that the receiver makes a large number of observations
($L = 1000$).

More cases that illustrate the
results of not explicitly coordinating $\delta_p$ and $L$ are illustrated in
Figures \ref{fig:beaconVsL} and  \ref{fig:beaconVsDelta}.
Generally $\delta_p$ is chosen by the transmitter
according to an objective for the lowest power
at which the beacon can be reliably detected.
In Figure \ref{fig:beaconVsL} it is assumed that the 
transmitter chooses $\delta_p = 0.03$, corresponding to $\xi_0 = 0$ dB.
With that assumption,
the consequences of the receiver making different choices for $L$ are shown.
As expected, larger $L$ results in significant improvements in detection reliability.
However, to be fully effective a value $L \gg 1/\delta_p$ must be chosen
to account for the fact that only a fraction $\delta_p$ of the observations
overlap energy bundles.
Too small a $L$ results in a saturation effect, where even a large $\xi_0$
(which helps to overcomes noise and scintillation) cannot compensate for
the duty cycle effect.

\incfig
	{beaconVsL}
	{.8}
	{
	A log plot of the miss probability $(1-\pd)$ vs the average beacon power
	(represented by $\xi_{0}$).
	Each curve represents a different choice for $L$ made by the receiver,
	but for all curves the transmitter has chosen $\delta = 0.03$ (3\%),
	which is optimized for $\xi_{0} \approx 0$ dB.
	This is why all the miss probability begins dropping in the region of
	$\xi_{0} \approx 0$ dB for all the cases.
	}
	
Figure \ref{fig:beaconVsDelta} illustrates the consequences of the transmitter
choosing different values for $\delta$ as the receiver uses a fixed $L = 500$ 
observations.
In this case, to be fully effective $\delta_p \gg 1/L$ must be chosen,
again to overcome the duty cycle effect.
This constraint shows up in the saturation effect for $\delta_p = 0.001$.
As expected, the most reliable detection at a
signal power corresponding to $\xi_0 = 0$ dB occurs at $\delta_p = 0.03$.
At larger values of $\xi_0$ the reliability can be improved by choosing
$\delta_p > 0.03$, although $\delta_p = 0.03$ gives consistently good
results because it is large enough that $L = 500$ can overcome the
duty cycle effect.

\incfig
	{beaconVsDelta}
	{.8}
	{
	A log plot of the miss probability $(1-\pd)$ vs the average beacon power
	(represented by $\xi_{0}$).
	Each curve represents a different choice for $\delta_p$ made by the transmitter,
	but for all curves the receiver has chosen $L = 500$.
	}

Overall the conclusion is that the transmitter can reduce its average transmit power
very significantly if it also significantly reduces the duty cycle $\delta_p$ at the same time.
Meantime, the receiver gets what is pays for.
The larger the number of independent observations the receiver performs, the
lower the average received power it can accommodate while still reliably detecting the beacon.
However, the receiver must choose $L \gg 1/\delta_p$ in order to overcome
the duty cycle effect.

\subsection{Increasing the duration of each observation}

One way the receiver can overcome the duty cycle effect is to
increase the number of independent observations.
Another way to overcome the duty cycle effect is to increase the
duration $T_o$ of each observation.
This will be beneficial up until $T_o = T_p + T$, at which point each
observation is guaranteed to completely overlap precisely one energy bundle.
Increasing $T_o$ further can result in two or more energy bundles
completely overlapping one observation, but the benefits 
are not as great since the received flux for those bundles will be correlated.
The receiver designer does not know the value of $T_p$ precisely,
so an observation interval must be chosen based on an assumption as to the
smallest duty cycle that might be used.
Fortunately the results are not very sensitive to the choice.
The $L$ observations, each with duration $T_o$,
should be statistically independent to help overcome the scintillation effect.
However, in response to increasing $T_o$ the value of $L$ can
be reduced accordingly.

Numerical results will be given in a future version of this report.

\section{Discovery of information-bearing signals}
\label{sec:discoveryoptimized}

The previous section simplified the problem of discovery by
specializing to a beacon consisting of a periodic sequence of energy bundles,
and then power-optimizing that beacon by adjustment of the duty cycle
and energy per bundle.
This does not address directly the question of discovery of
information-bearing signals.
However, information-bearing signals of the type considered in
Chapter \ref{sec:infosignals} have a remarkably similar structure.
They consist of a sequence of data symbols, each of which
conveys $\log_2 M$ bits of information by transmitting an energy bundle in
one of $M$ locations in time or frequency.
By adjusting the rate at which these symbols are transmitted,
the total information rate $\rate$ and average power $\power$
can be adjusted, in direct proportion to one another.

Note the parallel to adjusting the duty cycle
of a beacon.
Each data symbol consumes the same energy
(adhering to a bundle energy principle), but the power is
adjusted by choosing a rate at which to transmit a data symbol
(equivalent to an adjustment in duty cycle)
as described in Section \ref{sec:adjrateandpower}.
Thus, it is no surprise that discovery of power-efficient information-bearing signals
of the type considered in Chapter \ref{sec:infosignals}
is essentially the same challenge as the discovery of beacons that are
power-optimized for discovery.
The details are slightly different for M-ary pulse-position modulation (PPM)
and M-ary frequency-shift keying (FSK), so these are addressed separately.

One issue to address is the number of observations $L$ required to
reliably detect the presence of an information-bearing signal.
If the information-bearing signal has sufficiently high average power
to reliably extract information during periods of non-outage,
then $L$ will be relatively small.
If the information-bearing signal has lower average power than that,
then it can still be discovered, albeit with a larger $L$. 
This is not necessarily a problem for two reasons.
First, the discovery of this non-natural signal can have considerable value.
Second, as discussed in Section \ref{sec:discantennaobs} the received signal
power can always be increased by investing in a receive antenna
with a larger collection area.

\subsection{Discovery of M-ary FSK signals}

An M-ary FSK signal is essentially identical to a periodic beacon
with the same duty cycle, the one difference being that
energy bundles will be positioned at one of $M$ frequencies,
and that position will vary randomly (in accordance with the
embedded information) from one energy bundle to the next.
A discovery search algorithm that examines only one carrier frequency
at a time will thus see energy bundles that are not uniformly spaced,
but rather occur randomly at those uniformly spaced positions
but with a density that is a factor of $M$ lower.
This would have a substantial effect on detection, according to the
total energy principle increasing the number of observations $L$
by a factor of $M$ to maintain the same detection reliability
(since the energy per bundle does not change with $M$).
However, in practice a search will typically be conducted by a multi-channel
spectral analysis combined with matched filtering to $h(t)$, and in that
common case the observations that are candidates for detection
are those that overlap one data symbol in the M-ary FSK signal
in both time and frequency.

For purposes of discovery, a power-efficient information-bearing 
M-ary FSK or PPM signal possesses
three parameters $\{ \ecrb, \, M, \, \delta \}$ that together determine the tradeoff between discovery
reliability $\pd$ and the number of observations $L$.
The power efficiency is determined by $\ecrb$.
The size of the signal code set $M$ also determines the number of locations
that a discovery algorithm has to look (it is larger than $L$ for FSK).
The duty cycle $\delta$ is chosen by the transmitter based on the
information rate $\rate$ as described in Section \ref{sec:FSKspectralefficiency}.
In terms of the discovery relation $\pd [ \cdot ]$ of \eqref{eq:discoveryequation},
the detection probability is $\pd \left[ \pfa / M, \, \ecrb \cdot \log_{2} M, \, \delta , \, L \right]$.
%\begin{equation}
%\pd = \begin{cases}
%\displaystyle
%\pd \left[ \frac{\pfa}{M}, \, \ecrb \cdot \log_{2} M, \, \delta , \, L \right] , & \text{M-ary FSK} \\
%\displaystyle
%\pd \left[ \frac{\pfa}{M}, \, \ecrb \cdot \log_{2} M, \, \delta , \, L \right], & \text{M-ary PPM} \\
%\end{cases}
%\end{equation}
To relate this to the reliability of information recovery, it is expressed in terms of
the $\energybit$, or equivalently the bit energy contrast ratio $\ecrb = \ecrs / \log_{2} M$.
Then $\ecrb$ can be replaced by \eqref{eq:ecrbVsPe}, which then
relates $\pd$ to $\pe$, the reliability of later information extraction in the communication phase.
For FSK, the false alarm probability is forced to be a factor of $M$ smaller
to account for the $M$ frequencies, only one of which harbors an energy bundle.
The same is true of $PPM$ because of the $M$ time slots, only one of which contains an energy bundle.
Thus in both cases it is assumed that each of the $L$ observations actually
looks in $M$ locations (frequencies for FSK and time slots for PPM),
so in effect there are $L \, M$ observations in total.)

The discovery probability can be examined in several ways.
The first question is how many observations are required to reliably detect the
information-bearing signal with average power $\power$ sufficiently high to reliably extract
information from that signal once it is discovered.
That average power is proportional to rate $\rate$, and thus generally speaking
signals with a larger $\rate$ are easier to discover.
Figure \ref{fig:discoveryDataVsL} shows how $L$ is related to the miss probability $(1-\pd)$
for a single-carrier signal with the highest possible $\rate$ ($\delta = 1$).
On the order of $L = 20$ to $40$ suffices.
This is a much smaller $L$ than required to discover a power-optimized beacon
in general (see Figure \ref{fig:optLvsSNRlowDuty}),
the reason being the constraint that it be possible
to recover information with high reliability puts a higher floor on the average signal power $\power$.

\incfig
	{discoveryDataVsL}
	{.8}
	{
For an information-bearing M-ary FSK or PPM signal, 
a log plot of the discovery miss probability $(1 - \pd)$ vs the
number of observations $L$ for $M = 2$, $2^{8}$, and $2^{12}$.
The assumed conditions include a false alarm probability of $\pfa = 10^{-12}$,
a sufficiently high average power $\power$ to extract information at the threshold of outage
with error probability $\pe = 10^{-4}$, and $\delta = 1$, which corresponds
to the highest information rate $\rate$ that can be supported on a single carrier.
	}

Another insight from Figure \ref{fig:discoveryDataVsL} is that
increasing $M$ reduces the $L$ needed to achieve the same $\pd$.
Although increasing $M$ makes the energy bundles more sparse, which tends to increase $L$,
increasing $M$ also increases the power of each energy bundle that is present.
This is because $\energybit = \energy_{h} / \log_{2} M$, and thus larger $M$ requires
a larger $\energy_{h}$ to maintain the same $\energybit$.
This is explored in more detail in Figure \ref{fig:discoveryDataVsM}.
Increasing $M$ can decrease the miss probability
over a range of one to two orders of magnitude.
The net effect of increasing $M$ is favorable for discovery as well as for power efficiency.

\incfig
	{discoveryDataVsM}
	{.8}
	{
A log plot of the miss probability $(1 - \pd)$ vs the
number of bits per symbol $\log_{2} M$ for different values of $L$.
The other conditions are the same as in Figure \ref{fig:discoveryDataVsL}.
	}

The preceding applies to an information rate $\rate$ that is the
highest possible for a single carrier.
The impact of reducing $\rate$
is shown in Figure \ref{fig:discoveryDataVsDelta}.
Reducing the rate makes discovery less reliable, which is not surprising
since the average signal power $\power$ is being reduced in proportion to 
$\rate$ and $\delta$.
(This is in contrast to the comparison we made for an intermittent beacon, where 
we held $\power$ fixed as $\delta$ was decreased, and thus saw
a reduction in the number of observations up to a point.)
Figure \ref{fig:discoveryDataVsDelta} assumes that
the number of observations remains fixed at $L= 80$ as $\delta$
is reduced, but clearly
it is necessary to increase the number of observations to compensate for lower 
$\rate$ and $\delta$.
This effect is illustrated in Figure \ref{fig:discoveryDataVsLdelta},
where $L$ increases substantially as $\delta$ is reduced.
Thus the discovery of low-rate information-bearing signals
at the minimum power required for reliable communication
requires a number of observations $L$ more comparable to the discovery of a
power-optimized beacon at low power.
This may put a floor on $\rate$, or require a larger antenna collection area.

\incfig
	{discoveryDataVsDelta}
	{.8}
	{
A log plot of the miss probability $(1 - \pd)$ vs the duty cycle $\delta$
for several values of $M = 2$, $2^{8}$, and $2^{12}$ and assuming $L = 80$.
Smaller $\delta$ corresponds to smaller average signal power $\power$
and lower information rate $\rate$.
The the conditions are the same as in Figure \ref{fig:discoveryDataVsL}.
	}

\incfig
	{discoveryDataVsLdelta}
	{.8}
	{
A repeat of Figure \ref{fig:discoveryDataVsL} for different values of 
duty cycle $\delta$ and $M = 2^{8}$.
	}

Thus far we have assumed an information-bearing signal with sufficient average power $\power$
to reliably extract the information from the signal, but no more.
Discovering such a signal requires on the order of tens of independent observations.
If the number of observations $L$ is increased, we can anticipate that such a signal
can be discovered at lower average powers, in fact in principle approaching arbitrarily low power as $L \to \infty$.
However, it will not be possible to extract information from the signal reliably.
If on the other hand $L$ is decreased, the average power of the signal must be larger than necessary
for reliable extraction of information.

These conclusions suggest a tradeoff between the antenna collection area and processing resources
as was discussed in Sect \ref{sec:discantennaobs}.
An interesting option is to conduct a discovery search using a relatively small antenna
coupled to the increased processing power necessary to achieve a larger $L$.
When a signal is discovered, a larger antenna can be deployed in order to extract its information.
Alternatively, if only a small $L$ can be implemented economically,
it is possible to make up for that by increasing the antenna collection area,
using an antenna larger than necessary to extract information reliably from the signal following discovery.

\subsection{Discovery of M-ary PPM signals}

A PPM divides each symbol of duration $T$ into $M$ equal-duration segments,
each with duration $T/M$.
If these symbols are transmitted at rate $F$, then the duty cycle
defined in Section \ref{sec:adjrateandpower} was $\delta = F T$.
This is the duty cycle defined as the ratio of symbol interval to
symbol period.
However, for purposes of discovery, we need to define duty cycle $\delta_p$
differently, as the ratio of energy packet duration $T/M$ to symbol period, or
\begin{equation}
\delta_p = F \cdot \frac{T}{M} \,.
\end{equation}
Since $F T \le 1$, it follows that $\delta_p \le 1/M$, with equality
if and only if $\delta=1$ (symbols are immediately adjacent).
Thus the major difference between FSK and PPM is that the
duty cycle of PPM is a factor of $M$ smaller.

If the observation time $T_{o}$ is coupled to the duration of an energy bundle in both cases,
then PPM will require a substantially larger $L$ because of this lower duty cycle.
However, a more reasonable discovery algorithm will couple $T_{o}$ to
the symbol time, which is the same in both cases for equivalent $\rate$ and $\power$.
For PPM this implies a $T_{o}$ that is $M$ times the duration $T$ of a single energy bundle.
However, according to the total energy principle the number of observations
required is the same for PPM and FSK with this choice of $T_{o}$.
With this adjustment to the discovery algorithm, FSK and PPM are
essentially equivalent from a discovery perspective, as they are from
a power-efficiency standpoint.

\section{Power-optimizing information-bearing signals for discovery}
\label{sec:discoveryoptimized}

The discovery of periodic beacons and information-bearing signals have been considered
separately, but with different emphasis.
Beacons were examined from the perspective of achieving the lowest receive power $\power$
consistent with a fixed number of observations $L$,
while information-bearing signals were assumed to have sufficiently large $\power$
to reliably extract information from them.
Not surprisingly this led to the conclusion that $L$ is typically much smaller in
discovering an information-bearing signal than a beacon, mainly due to a larger $\power$.
However, this conclusion is suspicious because
we know that an information-bearing signal can have arbitrarily small $\power$
as long as it also has a commensurately small information rate $\rate$.
For fixed power efficiency $\powere$, we know that $\power \propto \rate$ and there
is no lower limit on either $\power$ or $\rate$.
In fact, a beacon can be considered to be the limiting case of an 
information-bearing signal as $\rate \to 0$.
Thus, an information bearing-signal can match the power of a beacon power-optimized
for discovery,
and still have sufficient power to reliably detect its embedded information.
We just have to be willing to accept a commensurately low information rate.

The question to be answered is whether or not a low-information-rate signal
is less discoverable than a beacon that matches it in received power.
That is, does the mere act of embedding information in the signal with a given $\power$
intrinsically increase the number of observations $L$ required to discover it, or not?
We now show that it does not.
That is, a low-rate information-bearing signal can match a periodic beacon
in both average power $\power$ and in the number of observations $L$.
This is not too surprising because starting with a periodic beacon,
turning it into an information-bearing signal requires the fairly small step
of randomizing somewhat the location of energy bundles in either time or frequency.
That randomization is keyed to the information being conveyed.
This randomization need not affect the discovery of the signal much, since
that discovery focuses on detecting energy bundles at random observation times,
so some randomness in the time or frequency of the bundles
added to the randomness of the observation times has little added impact.

In conclusion, in the power-efficient design regime there is really no reason to consider
transmitting a beacon, since an information-bearing signal at the same power can be discovered
just as effectively at the receiver.
However, if we want to match the low power that we might seek in a beacon, that information-bearing
signal will have a low information rate commensurate with that low power.
Addressing this issue requires us to merge the results of this
chapter and Chapter \ref{sec:infosignals}, because we are seeking
signals that are meritorious in both conveying information and in discovery.
We start by reviewing those earlier results.

\subsection{Differences between discovery and extracting information}

Merging the perspectives of discovery of a signal (beacon or information-bearing signal) vs. 
the extraction of information from the signal
(information-bearing signal only)
can be a little confusing because very different metrics of what measures success are used.
It is worthwhile to summarize and put perspective on what we have learned:
\begin{description}
\item[During discovery.] 
The goal is to minimize the number of observations $L$ necessary
for a given average power $\power$, or equivalently to minimize the $\power$
required for a given $L$.
At the stage of the detection of energy bundles,
beacons and information-bearing signals are essentially equivalent.
Periodic beacons and M-ary FSK and PPM signals all start by 
making some number $L$  independent observations spaced
at intervals larger than the coherence time of the scintillation,
typically combined with multi-channel spectral analysis.
The differences arise in the post-detection pattern recognition,
looking for multiple energy bundles arriving from the same direction
and at (or in the vicinity of) the same carrier frequency.

Our analysis of discovery has shown the duty cycle $\delta$ of the signal
(a measure of the density of energy bundles in time and frequency) and
the energy per bundle $\energy_{h}$ are important to discovery,
$\delta$ because it governs the fraction of observations that will overlap an energy bundle
and $\energy_{h}$ because it determines the reliability with which a
bundle that overlaps an observation is detected.
As $L \to \infty$ a beacon and an information-bearing signal can be
discovered reliability at any $\power$ no matter how small.
\item[During communication.]
The goal is to minimize the average
power $\power$ required to achieve a given information rate $\rate$, or equivalently
to maximize the $\rate$ achievable for a given $\power$.
During communication the duty cycle $\delta$ has no significance to reliability
because the receiver knows where to look for energy bundles,
and has sufficient prior knowledge to avoid observing in the ''blank intervals''
represented by the off-time in the duty cycle.
The receiver intrinsically makes only a single observation per candidate location for an energy bundle,
because it is making a determination of the presence or absence of each bundle, and
not the presence of absence of a signal overall.
The energy per bundle $\energy_{h}$ remains a significant characteristic of the signal,
because it largely determines the reliability with which information is extracted.
There is a fundamental lower bound on the power efficiency $\powere$.
However, this is \emph{not} a fundamental limit
on $\power$, because even in compliance with the fundamental limit
$\power \to 0$ as $\rate \to 0$.
\end{description}

\subsection{Turning a beacon design into an information-bearing signal}

The question we would now like to address is to whether removing the requirement of embedded information
renders a beacon somehow more effective at the discovery stage.
The answer is ''no'', as can be seen from the following argument.
Start by designing a periodic beacon at a given average power $\power$,
and for simplicity assume the observation interval is $T_{o} = 2 T$
so that the fraction of observations that completely overlap an energy bundle is
$\delta_{p} = T/T_{p}$.
The energy per bundle $\energy_{h}$ can be inferred from the
relation $\energy_{h} = \power \, T_{p} = \power \, T / \delta_{p}$.
We have seen that at this $\power$ there is an optimal duty cycle $\delta_{p}$,
the choice of which minimizes the number of observations $L$ required to achieve
a given set of probabilities $\{ \pd , \, \pfa \}$.
This optimum trades off the chance that there may be none or a small number of energy packets overlapping
the collective observations when $\delta_{p}$ is small
against the increased $\energy_{h}$ that results from choosing a small $\delta_{p}$.
The result is a beacon power-optimized for discovery for an average received power $\power$
coupled with a specific assumption on the value of $T_{o}$ chosen by the receiver.
Generally this power-optimized design will take advantage of any larger average received
power and/or longer observation interval to yield even more reliable discovery.

A key characteristic of the beacon that was not addressed earlier is the energy per bundle $\energy_{h}$ or the
the energy contrast ratio $\ecrs$ for the individual energy bundles in a power-optimized beacon.
The bundle energy principle predicts that $\energy_{h}$ (and hence $\ecrs$)
will remain fixed as the duty cycle $\delta_{p}$ is decreased, so that the reduction in $\power$
is entirely due to the reduction in duty cycle  (achieving by increasing the spacing $T_{p}$)
and not due to any reduction in energy per bundle.
This is confirmed in Figure \ref{fig:beaconECRoneBundle}, where we see that
$\ecrs = \xi_{o}/\delta_{p}$ does not vary much in the low-power region where $\delta_{p}<1$.
The small variation that does exist is in the opposite direction than we might expect, 
toward higher $\ecrs$ as $\delta_{p}$ (and hence $\power$) decreases.
Of course $\ecrs \propto \xi_{0}$ in the high-power region since $\delta_{p} = 1$ is fixed.
The other insight from Figure \ref{fig:beaconECRoneBundle}
 is relatively large (at about 14 to 15 dB) value for $\ecrs$.
This insures that those energy bundles that overlap an observation can
be detected fairly reliably, with misses occurring only 57\% of the time at $\ecrs = 15$ dB.
The benefit in $L$ due to decreasing this miss probability would be more than
offset by the penalty due to the reduced duty cycle that would be required to keep $\power$ fixed.

\incfig
	{beaconECRoneBundle}
	{1.0}
	{On the left, the energy contrast ratios $\ecrs = \xi/\delta$ in dB for a power-optimized beacon
	is plotted against $\xi_{0}$ in dB (which represents the beacon average power $\power$).
	This is a repeat of Figure \ref{fig:optP1vsSNR}, except it plots $\ecrs$ rather than $\delta_{p}$.
	At lower powers, where $\delta_{p} < 1$, $\ecrs$ is approximately constant as predicted by the
	bundle energy principle.
	The log plot on the right explains why the value $\ecrs \approx 15$ dB is optimum.
	It plots the miss probability $(1-\pd)$ \emph{for a single energy bundle} against the energy
	contrast ratio $\ecrs$ for that bundle in dB.
	That miss probability is $0.57$ at $\ecrs = 15$ dB.
	}

Having determined the parameters of a beacon power-optimized for discovery,
this can be turned into an information-bearing signal with the same $\power$
and essentially the same reliability in discovery.
For example, substitute an M-ary FSK signal with the same duty cycle $\delta=\delta_{p}$
and the same energy per bundle $\energy_{h}$.
This signal will be similar to the beacon, with the same on-off duty cycle,
the only difference being that each energy bundle will fall randomly at one of $M$ different frequencies,
thereby conveying $\log_{2} M$ bits of information per symbol.
This information-bearing signal has essentially the same discovery properties
as the periodic beacon.
We say ''essentially'' because there is an increase in the false alarm probability $\pfa$
due to the $(M-1)$ frequencies where there are no energy packets.
However, a multi-channel spectral analyzer typically employed during discovery
of the single-frequency beacon will also be examining these $M$ frequencies,
and will therefore have the same opportunities for false alarms.
We say that this M-ary FSK information-bearing signal is power-optimized for
discovery at average received power $\power$ and observation interval $T_{o} = 2 T$.
Although this information-bearing signal is optimized for discovery with the smallest
number of observations $L$, the remaining question addressed next is the properties
of this signal in terms of its information-bearing function.

\subsection{Reliability in extraction of information}

What are the special properties of an information-bearing signal that
is power-optimized for discovery?
The two aspects of this question are first the reliability with which its embedded
information can be extracted, and second its information rate.
Addressing the first question requires a change in mindset from our
discovery-dominated mentality, since discovery takes place in an
environment of scintillation, and in fact exploits that scintillation to its benefit.
Once we switch to the communication phase, the goal is to circumvent
rather than exploit scintillation.
The approach taken in Chapter \ref{sec:infosignals} was to estimate the
received scintillation flux and declare outage periods where reliable
extraction of information is ruled out.
The probability of error $\pe$ in the recovery of individual bits
was calculated at the threshold of outage, with the knowledge that
most of the time during periods of non-outage $\pe$ will be much smaller.
We also found that the optimum definition of outage is when the
received signal flux $\flux < \vs$, where $\vs = \expec{\flux}$ is the average flux.
At the threshold of outage, since $\vs = 1$, the received flux and average received
power and energy per bundle are all the same as if there were no scintillation at all.
Thus, we can use an energy contrast ratio $\ecrs$ that ignores scintillation to
determine the reliability of information extraction, reiterating that this applies
only at the threshold of outage.

\textbox
	{Some lessons for SETI programs}
	{
A question faced by SETI observation programs is whether to search for
beacons, which are information-free but serve to attract attention to the transmitting civilization,
or an information bearing signal.
Existing SETI programs have been influenced by terrestrial communications,
where power efficiency is sacrificed in favor of spectral efficiency.
In that domain, the classic argument that a beacon is worthwhile because it is
''obvious'' or ''easier to discover'' has some merit, because generally achieving
spectral efficiency requires complicated techniques that may generally interfere
with discovery and are likely to be very difficult to reverse engineer after discovery.
\newline
\newline
However, the power-efficient regime has several conditions
favorable to interstellar communication.
One is that power efficient signals are structured around on-off
signals, where detecting the presence of absence of an energy bundle is the
underlying receiver functionality.
This functionality is extremely simple, and the same signal processing
techniques apply to beacons and information-bearing signals.
As a result, it is simple to seek both types of signals simultaneously.
There is no ''simplicity'' argument in favor of a beacon.
At the same time, we have shown that a beacon has no advantage
over a low information rate signal in terms of the receiver resources
required to discover a signal at a given average receive power.
Thus, while there is no additional cost of complexity associated with
searching for a beacon simultaneously with an information-bearing signal,
it seems obvious that if we were to transmit a signal we would want to
embed information in that signal because there is no extra cost to us or the receiver designer in doing so.
Our main issue would be whether to choose a very low information rate necessary to
achieve the lowest receive power, or a higher information rate associated with a higher power.
\newline
\newline
In searching for more complex and wider bandwidth signals, a big concern
expressed by many others has been the interstellar impairments and the receiver processing
required to deal with those impairments.
In the power efficient regime this is not a concern, because
a basic principle of power efficient design is to choose a transmit signal
that avoids these impairments.
During discovery, no processing associated with interstellar impairments is required.
On the other hand, in the power-efficient regime the receiver does have to
deploy the processing necessary to perform multiple independent observations at the
same location and at or near the same carrier frequency,
as well as pattern recognition algorithms to interpret the results.
A receiver performing one or a few observations will discover
only signals at considerably higher power levels than is necessary for either discovery
or reliable recovery of information, as we have shown.
}


For M-ary FSK the energy contrast ratio $\ecro$ required
to achieve reliable information extraction is given by \eqref{eq:ecrbVsPe}
and plotted in Figure \ref{fig:ecrbVsM}.
However, $\ecro = \ecrs / \log_{2} M$ is expressed in terms of the bundle energy per bit
in an $M$-bit symbol.
Performing this normalization on the upper bound on error probability $\pe$ from
\eqref{eq:peFSKbound},
\begin{equation}
\log_{2} \pe \le \log_{2} M - \frac{\ecrs}{2 \, \log_{e} 2 } - 2 \,.
\end{equation}
Thus $\log \pe$ is a linear function of $\log_{2} M$, the number of bits per symbol.\footnote{
Note that $\pe > 1$ for sufficiently large $M$.
This is possible because this is merely an upper bound on $\pe$,
and the bound is tight only when $\pe \ll 1$.}
The error probability is plotted in Figure \ref{fig:peVsMpowopt}.
The error probability increases as $M$ increases because the energy contrast ratio
per bit $\ecro$ grows smaller.
A physical explanation for this behavior is that as $M$ increases there are more opportunities for noise in
one or more of the $(M-1)$ locations that lack energy bundles to mimic an energy bundle.

\incfig
	{peVsMpowopt}
	{.8}
	{A log plot of the probability of bit error $\pe$ vs the number of bits per symbol $\log_{2} M$
	between one and 20 for an energy contrast ratio $\ecrs = 15$ dB.
	This applies to
	an M-ary FSK information-bearing signal that has been power-optimized for discovery
	for low-power case where the duty cycle $\delta <1$.
	The assumption $\ecrs = 15$ dB applies
	approximately independently of the average power $\power$.
	At higher powers, $\pe$ will decrease rapidly with average power $\power$ for any value of $M$.}

The primary conclusion from Figure \ref{fig:peVsMpowopt} is that information can be extracted with high reliability.
This is especially true in the regime $M \le 10$, which may also be considered the most practical case.
Due to the bundle energy principle, this conclusion applies regardless of how low the
average power $\power$.

Although reliability does not change, the information rate $\rate$ does change
in proportion to average power $\power$.
The rate is
\begin{equation}
\rate = \frac{ \log_{2} M}{T_{p}} = \delta_{p} \cdot \frac{ \log_{2} M}{T} \,,
\end{equation}
which (along with $\power$) decreases in proportion to $\delta_{p}$
in the low-power regime where $\delta_{p} < 1$.
The case $\delta_{p} = 1$ is the maximum rate that can be supported
on a single carrier with energy bundle duration $T$.
For example, we saw that the optimum is $\delta_{p} = 0.03$
in the region of $L = 848$, at which point both the average power and
the information rate are a factor of 33 smaller than could be supported
by a single carrier.

The overall conclusion is that an M-ary FSK information bearing signal
can be just as effective as a beacon in achieving the lowest average received
power for a given number of observations, or equivalently the smallest
number of observations for a given average received power.
It is simply a matter of choosing a low information rate, which achieves a correspondingly low power.
At low power levels, a relatively large number of independent observations is
required, on the order of hundreds or thousands.
Information-bearing signals with information rates
closer to the maximum that can be supported by a single carrier
will require a higher average power but only tens of observations.
Current SETI programs are using only one or at most a few observations.
Such a small number of observations will succeed in discovering signals which have considerably
higher average power than is necessary to support reliable extraction of information from the signal.
This situation can occur if the transmitter designer has presumed a smaller antenna collection
than the observer has actually deployed, if the transmitter designer has targeted reception
at some point further away along or close to the same line of sight,
or has deliberately chosen to transmit a higher power than necessary to make the
signal easier to discover.


%The idea of replacing an intermittent beacon with an
%information-bearing signal with equivalent discoverability
%is a general one.
%Suppose a specific $\delta$ is desired.
%Then a PPM signal with the largest $M$ that satisfies
%$\delta < 2^{-M}$ can be used, and  the duty cycle can
%be further reduced to exactly $\delta$ by adjusting the symbol rate downward
%as illustrated in Figure \ref{fig:FSKvsDelta} applied to PPM rather than FSK.
%This does constrain the maximum value of $M$, and thus limits the maximum
%power efficiency in the subsequent communication mode.
%The process of discovery optimization has impacted the design of the
%information-bearing signal.
%
%Although a discovery-optimized information-bearing signal
%is specifically designed to be discoverable at a relatively low
%average power level, this does not imply that information can be
%reliably extracted from it at this power level.
%For discovery, the relevant parameter is the energy contrast ratio $\ecrs$,
%but for reliability of information extraction the equivalent parameter
%is $\ecrb$.
%For a PPM signal, the relationship between these parameters is
%$\ecrs = \ecrb \cdot \log_2 M$.
%If the average power is such that $\ecrs$ is very small, then
%$\ecrb$ is even smaller, and thus information cannot be reliably
%extracted.
%So what is the point of an information-bearing signal that
%can be discovered but whose
%average power is so low that information cannot be
%reliably extracted from it?
%
%As an example, suppose that the receiver is searching for
%an intermittent beacon with $\delta = 1/32$ at an $\ecrs = 0$ dB
%by making $L = 831$ observations at each location.
%If this beacon is actually a discovery-optimized PPM signal,
%it may be using $M = 32$ or $\log_2 32 = 5$ bits per symbol
%to achieve $\delta = 1/32$.
%If it is discovered at $\ecrs = 0$ dB this corresponds to
%$\ecrb = 0 - 10 \times \log_{10} 5 = - 7$ dB.
%However, from Figure \ref{fig:peOOKvsFSK} the required
%$\ecrb$ to reliably extract information is about
%$\ecrb = + 7$ dB, or 14 dB higher (a linear factor of about 25).
%This higher energy per bit can be achieved by increasing the
%received antenna collection area by a factor of 25.
%
%\section{Discovery of information-bearing signals}
%\label{sec:discoveryinfosignals}
%
%In considering a beacon, as well as a discovery-optimized information-bearing signal,
%the basis of comparison was to keep the average signal power fixed as the
%duty cycle $\delta$ is varied.
%The result is a peak power that increases proportionally to $1/\delta$
%without consideration of the reliability of information extraction from the signal.
%Now consider an information-bearing signal possessing 
%an average power chosen for
%reliable information extraction at the threshold of outage.
%This signal may or may not have been optimized for discovery as
%described in Section \ref{sec:discoveryoptimized}.
%The question is what $L$ is required for reliable discovery of this signal.
%Of course we know that such an $L < \infty$ exists, the only question is how large it is.
%Even if the communication stage uses an outage strategy,
%in the discovery stage there is no knowledge of the scintillation flux, so
%the outage threshold is not relevant and observations are completely blind to the
%current state of scintillation flux.
%The only influence of an outage strategy is in determining the average signal power;
%otherwise, an outage strategy is not relevant to the discovery stage.


%During discovery there is no extraction of information, so an M-ary PPM signal
%simply appears like a beacon with duty cycle $\delta = 1/M$.
%Thus, for PPM the discovery probability is
%$\pd [ \pfa, \, \ecrb \cdot \log_{2} M, \, 1/M , \, L]$.
%We are interested in the detection reliability (reflected by $\pd$)
%for an information bearing signal at a power level where its embedded
%information can be reliably extracted,
%and this is reflected in the value of $\pe$ at the threshold of outage.
%The resulting $\ecrb$ is given by \eqref{eq:ecrbVsPe}, and substituting this value
%gives a relation for $\pd$ vs the parameters $\{ \pfa, \, \pe, \, M. \, L \}$.
%The resulting miss probability $(1-\pd)$ is
%plotted in Figure \ref{fig:discoveryPPMvsEcrb}.

%\incfig
%	{discoveryPPMvsEcrb}
%	{.8}
%	{
%	A log plot of the miss probability $(1 - \pd)$ vs the
%	number of bits per symbol $\log_{2} M$ in the detection of M-ary PSK
%	at the maximum information rate possible for a single carrier.
%	It is assumed that the power level is set so the information-extraction
%	probability is $\pe = 10^{-4}$, and three values for the number
%	of observations $L = 10$, $100$, and $1000$ are shown.
%	The miss probability increases as $M$ increases.
%	}
%
%Increasing $M$ improves the power efficiency
%(as was shown in Figure \ref{}).
%Equivalently, increasing $M$ reduces the average power $\power$
%of the PPM signal, and also reduces the duty cycle $\delta$.
%Both these characteristics are harmful to discovery,
%and the result is that  
%
%
%FSK
%
%is the SNR at the MF output
%for the special case that $\delta = 1$, or the transmitter is always transmitting.
%If the average transmit power is kept constant while $\delta < 1$,
%then the transmitter can devote more power 
%for the fraction of the time that it is transmitting.
%Thus, conditioned on a signal present during a single observation,
%the MF output SNR is actually $\ecrs / \delta$.
%This is where the advantage of an intermittent transmission comes in.
%During one observation by the receiver, a signal is only present
%with probability $\delta$.
%However, when it is present it is more likely to be detected because
%its SNR is higher.
%
%The results of Section \ref{sec:FSKspectralefficiency} are useful in modeling the discovery of an M-ary FSK
%signal of the type considered in Chapter \ref{sec:infosignals}.

%Information can be recovered from an M-ary FSK signal only after it is
%discovered.
%As was described for a beacon in Chapter \ref{sec:discovery},
%such a signal can be discovered with $\pd \to 1$ if the number of
%independent observations $L$ using a filter matched to $h(t)$ is sufficiently large.
%The method of discovery is not fundamentally different, but only the signal
%parameterization is different.
%In fact, the same receiver can be used to discover either one,
%although some difference in post-analysis pattern analysis may be warranted.
%A beacon designed for discovery at low received power levels will use
%a single carrier frequency and use a low duty cycle $\delta$.
%In contrast, an information-bearing signal designed for high power efficiency
%may use M-ary FSK, in which case the energy bundles will appear at $M$
%different frequencies.
%Two perspective on the FSK signal are both correct.
%It is an intermittent signal at a single frequency with duty cycle $\delta = 1/M$,
%or it is a continuous signal appearing at one of $M$ frequencies with 
%duty cycle $\delta = 1$.
%
%There are thus two methods of discovery for the FSK signal.
%The first is to make multiple independent observations at a single frequency, looking for a signal with
%low duty cycle $\delta = 1/M$.
%The second and more likely approach is
%to monitor a whole range of
%frequencies concurrently using a multi-channel spectral analyzer
%combined with an MF to $h(t)$.
%Since the carrier frequency is unknown, and there are advantageous
%algorithms for multi-channel spectral analysis based on the FFT,
%assume the second approach.
%In this case, it can be assumed that the receiver, when tuned to the
%appropriate range of frequencies, will observe the signal if the
%scintillation flux is sufficiently large.
%
%In this case the discovery relation \eqref{eq:discoveryequation} applies with $\delta = 1$.
%However, to capture this FSK discovery situation, two modifications have to
%be made to \eqref{eq:discoveryequation}.
%First, in determining the false-alarm probability, $L$ should be replaced by $L M$
%because each observation (among the $L$) is actually an observation at
%$M$ frequencies, increasing the possibility of false alarms.
%Second, the appropriate measure of signal power is $\ecrb$ rather than $\ecrs$
%for an information-bearing signal.
%With these two modifications, the discovery relation \eqref{eq:discoveryequation} becomes
%\begin{equation}
%\pd \approx 1 -
%\left(1 -
%   \delta  \left(\frac{\pfa}{L \, M}\right)^{
%   \frac{1}{1+ \log_{2} M \,\ecrb}} \right)^L \,
%\end{equation}
%The resulting $L$ required to achieve two levels of
%discovery reliability is plotted in Figure \ref{fig:discoveryFSK}
%for the particular case of $M = 256$, chosen because it looks like an
%attractive option.
%The most interesting value of $\ecrb$ is $\ecrb = 6$ dB, 
%because we saw in Figure \ref{} that this is the lowest $\ecrb$
%for which reliable discovery is possible with $M = 256$.
%The number of observations required to discover this 256-ary FSK signal is 
%$L = 23$ for the more reliable case and $L = 8$ for the less reliable case.
%
%\incfig
%	{discoveryFSK}
%	{.8}
%	{A log plot of the number of observations needed to achieve two
%	reliability objectives in discovery of an M-ary FSK information-bearing
%	signal with $M = 256$.
%	The objectives are the same as Figure \ref{fig:optLvsSNRlowDuty}.
%	The more reliable case is $\pfa = 10^{-12}$ and $\pd = 0.9999$,
%	and the less reliable case is $\pfa = 10^{-8}$ and $\pd = 0.99$.
%	}
%
%Figure \ref{fig:discoveryFSKdelta}
%
%Model $L \power$ constant, or
%\begin{equation}
%\label{eq:Lmodel}
%L = \frac{L_0}{\delta}
%\end{equation}
%
%\incfig
%	{discoveryFSKdelta}
%	{.8}
%	{A log plot of the number of observations $L$
%	as the power $\power$ and information rate $\rate$
%	of an information-bearing M-ary FSK signal is reduced
%	by decreasing the duty cycle $\delta$.
%	The same two levels of reliability as in
%	Figure \ref{fig:discoveryFSK} are shown.
%	The dashed line is the simple model of \eqref{eq:Lmodel}.}
	
%\comment{Make a constant power efficiency assumption
%in \eqref{eq:discoveryequation} and redo the number of observations.}
%
%The number of observations is predicted by \eqref{eq:discoveryequation}, except
%for an information bearing signal it is appropriate to keep the
%power efficiency $\powere$ (or equivalently energy per bit $\energybit$)
%constant.
%This implies that 
%\begin{equation}
%\ecrs = \snr_{2} \cdot \log_{2} M
%\ \ \ \text{and} \ \ \ 
%p_{1} = \frac{1}{M} \,,
%\end{equation}
%where $\snr_{2}$ is the value of $\ecrs$ at the minimum value of $M=2$.
%This case is plotted in Figure \ref{fig:LvsM},
%where a similar behavior is observed to the constant average power
%case plotted in Figure \ref{fig:Lvsp1}.
%
%\incfig
%	{LvsM}
%	{.8}
%	{A repeat of Figure \ref{fig:Lvsp1} for an information-bearing PPM signal,
%	where the horizontal axis is the number of positions of a pulse $M$.
%	Rather than keep average power $\power$ constant as $p_{1}$ is varied,
%	here we keep power efficiency $\powere$ constant as $M$ is varied.}
%
%The number of observations required to achieve the performance parameters of
%Figure \ref{fig:Lvsp1} are plotted in Figure \ref{fig:optLvsSNRm}.
%In the high-power regime, on the order of $L = 10$ to $20$ suffixes,
%but in the low-power regime $L$ must be on the order of $10^{2}$ to $10^{4}$.
%The number of bits per PPM codeword is plotted in Figure \ref{optMvsSNR}.
%Over a range of $\ecrs$ down to 2 dB, never more than six bits per
%codeword is required.
%
%\incfig
%	{optLvsSNRm}
%	{.8}
%	{A log plot of the minimum number of observations required to achieve the
%	performance parameters of Figure \ref{fig:Lvsp1} is plotted against $\snr_{2}$ in dB.
%	At each value of $\snr_{2}$ the value of $M$ that minimizes $L$ is chosen.
%	}
%
%\incfig
%	{optMvsSNR}
%	{.8}
%	{For the same conditions as Figure \ref{fig:optLvsSNRm}, the number of bits
%	per PPM codeword $\log_{2} M$ is plotted against $\snr_{2}$.}
%
%The other consideration is the merit of
%OOK and PPM as power-efficient beacons.
%Although they both transmit intermittently as a power-efficient beacon
%that minimizes the number of receiver observations must,
%PPM offers much greater flexibility because
%\begin{equation}
%\delta = \prob{A = 1} = \frac{1}{M}
%\end{equation}
%allows flexible choice of $p_{1}$ by choosing $M$.
%OOK, on the other hand, offers only the choice
%$\delta = 2^{-1}$.
%
%The treatment of discovery in Chapter \ref{sec:discovery} applies
%directly to OOK.
%As described in Section \ref{sec:datamoddisc}, the presence
%of the data symbol $A$ implies that multiple short-term observations
%at a single carrier frequency can insure statistically that $A = 1$ is encountered.
%It should be emphasized that discovery of a signal in the presence of channel
%coding would not be significantly more challenging because the OOK
%data symbol $A$ would merely be replaced by something possessing multiple levels.



%For OOK we know that $\ecrs = \snro$ is the most power-efficient choice,
%and at this power level the relationship between $\pfa$ and $\pd$ of \eqref{eq:asympPfaVsPd}
%becomes
%\begin{equation}
%\label{eq:pdVspfaSNRo}
%\pd = \pfa^{\,\frac{1}{1+\snro}} \,.
%\end{equation}
%This is plotted in Figure \ref{fig:pdVsPfaSNRo} for a typical value of $\snro$.
%As described in Section \ref{sec:beacondiscovery}, multiple independent observations
%are required to achieve $\pd \approx 1$.
%By ''independent'' we mean sampling of independent observations of the scintillation.
%This can be achieved by spacing these observations at frequencies
%large relative to the scintillation coherence bandwidth, or large relative to the scintillation coherence time.
%
%\incfig
%	{pdVsPfaSNRo}
%	{.8}
%	{A log-log plot of the relationship between false alarm probability $\pfa$
%	and the detection probability $\pd$ of \eqref{eq:pdVspfaSNRo}
%	for OOK with $\snro = 15$ dB.
%	This shows that for a single observation, $\pfa \approx 0$ and
%	$\pd \approx 1$ is unattainable; multiple independent observations are required.}
%
%The information rate that can be supported by a single carrier is limited by the
%coherence bandwidth $B_{c}$ as described in Section \ref{sec:SCandMCM}.
%In our design, the available transmit power may exceed the maximum necessary to support
%the highest information rate on a single carrier, particularly for targets at relatively short distances.
%As illustrated in Figure \ref{fig:IUstructure}, this additional power can be used to increase the
%information rate by transmitting multiple carriers.
%Two strategies can be employed in choosing the spacing of those carriers.
%One would be to locate them as closely as permitted by the single-carrier bandwidth $B$,
%which is to say a carrier spacing equal to $B$ with some guard interval.
%The second would be to choose a large enough carrier spacing that the scintillation effects
%for the carriers are statistically independent,
%as has been suggested \citeref{140}.
%This would improve the prospects for discovery by a receiver that had the computational
%resources to concurrently process a wide bandwidth, and reduce the necessity for
%multiple observations at widely separated times.
%
%
%%Figure \ref{fig:snr0vssnrD} suggests that discovery requires a higher SNR
%%than communication.
%%However, a couple of considerations undercut this conclusion.
%%First, the effect of errors (reflected in $\pe$) is much different from the
%%effect of missed opportunities for discovery (represented by $(1-\pd)$).
%%An $\snre = 10$ dB corresponds to $\pe = 0.00078$ in Figure \ref{fig:pEvsSNR},
%%and the same value for $\snrd$ results in $\pd = 1 - 0.00078 = 0.9992$.
%%In fact, much larger values for $(1-\pd)$ should be permissible.
%%This is particularly compelling when the effect of scintillation is taken into account
%%as discussed in Section \ref{sec:discovery}.
%%Scintillation demands multiple observations for the same $f_{c}$
%%if outages are not to adversely affect discovery, and those multiple observations
%%can also increase $\pd$ to any extent necessary to allow a signal with
%%sufficient power for reliable communication to be discovered.
%%
%%There are several types of multiple observation, and this is related to
%%the signal structure illustrated in Figure \ref{fig:IUstructure}.
%%A specific example of such a signal is shown in Figure \ref{fig:subcarrierOutputs}.
%%\begin{description}
%%\item[Successive symbol intervals in a single carrier.]
%%At a single carrier frequency, the signal $h(t)$ repeated with different data symbols $A_{k}$
%%would be expected.
%%This can be exploited by repeated successive observations at the same $f_{c}$,
%%primarily as a strategy to counter the short-term variation in magnitude due to the
%%data symbols.
%%(A relatively rapid variation in phase is to be expected due to time-incoherence, but this
%%is countered by energy detection that is insensitive to phase.)
%%Incoherent addition of energy in successive observations could also be used to improve discovery sensitivity.
%%A drift in carrier frequency would be expected due to the relative velocity of transmitter and receiver
%%as discussed in Section \ref{sec:doppler}.
%%\item[Different carrier frequencies.]
%%One feature of MCM is that the total received power across all parallel carriers is greater
%%than that required for reliable reception of a single carrier data stream.
%%Multiple observations performed concurrently at different carrier frequencies would
%%accomplish much the same as described for a single carrier.
%%This could counter the magnitude variation due to data symbols, and also
%%permit the incoherent addition of energy across carriers.
%%\item[Relatively infrequent revisits.]
%%Short term observations across time or frequency will always suffer the vagaries of
%%relatively long-term magnitude variations due to scintillation.
%%The resulting outage periods will affect both discovery and reliable communication.
%%The only way to counter this is to repeat observations at the same carrier frequencies
%%at intervals long relative to the time coherence of scintillation.
%%\end{description}
%
%Figure \ref{fig:subcarrierMagnitudes} illustrates the noise-free output magnitudes for a bank
%of MF filters.
%Different opportunities for multiple-observation discovery can be identified,
%including multiple observations in time at a single carrier frequency (countering the random data symbols)
%and multiple observations in frequency at a single time.
%Superficially this bank of outputs resembles that encountered with pulsars,
%and similar approaches can be used to detect the presence of a signal
%and estimate its parameters.
%Significant differences with pulsar discovery are the effects of random on-off keying
%(the pulsar signal is consistently ''on''), 
%the precise carrier-frequency alignment required for OOK
%(pulsar filter banks do a crude spectral analysis),
%and the
%very different front-end MF processing
%(pulsar discovery requires a costly de-dispersion algorithm).
%
%\incfig
%	{subcarrierMagnitudes}
%	{1}
%	{The noise-free continuous-time output of  a set of 10
%	 subcarrier incoherent matched filters is plotted as a function of time.
%	 This is an artificial example intended to illustrate the several effects, rather
%	 than indicative of any particular line of sight.
%	Uniformly spaced symbols
%	are modulated at $A = 0$ or $A = 1$ generated by independent
%	fair coin tosses.
%	The case shown is
%	$K = 10$, which results in an approximate 10\% on-off duty cycle.
%	Across subcarriers the plasma dispersion group delay is sufficient to
%	offset the subcarrier outputs in time, even though they were generated synchronously
%	at the transmitter.
%	}
%
%\section{Mulitple-bit communication}
%
%As long as they are non-overlapping, multiple bits
%can be conveyed using ICH's non-overlappng
%in time and frequency.
%
%The power efficiency remains constant, since both the information rate $\rate$
%and the average power $\power$ are proportional to the rate at which ICH's are transmitted
%and received.
%Thus, the comparison between \eqref{eq:fundamentallimit} and \eqref{eq:actual}
%remains in tact.
%The important observation is that both $\rate$ and $\capacityinf$ are proportional to
%$\power$, and there remains a fixed gap between them at all rates and average powers.
%
%
%
%\comment{Following is left over and needs to be updated.}
%
%Objective (A) in Section \ref{sec:introduction} is the maximization of power efficiency,
%defined as $\rate/\power$.
%This will now be addressed for the conditions
%listed in Table \ref{tbl:conditions}.
%The overall conclusion is that the maximum power efficiency is given by
%\begin{equation}
%\label{eq:overallpe}
%\frac{\rate}{\capacityinf} = 
%\frac{\log_{\,e} 2}{\ecrs}
%\ \ \text{with} \ \ 
%B = 
%\frac{K \, \capacityinf \, \log_{\,e} 2}{ \ecrs} \\
%\,,
%\end{equation}
%where $\capacityinf$ is the fundamental limit on information rate
%for a AWGN channel with bandwidth $B \to \infty$.
%$\capacityinf$ is proportional to the available receive power $\power$,
%and thus $\rate / \capacityinf$ is proportional to power efficiency.
%As illustrated in Figure \ref{fig:ultimateRate}, the power efficiency
%is fixed at all power levels, but is reduced if we wish greater
%reliability (larger $\ecrs$).
%The gap between $\rate$ and $\capacityinf$ is substantial;
%for example,
%$\rate$ is a factor of $14.4$ smaller than $\capacityinf$ at $\ecrs = 10$ dB. 
%Also, from \eqref{eq:overallpe} as RFI immunity is increased (larger $K$)
%a larger $B$ is consumed, but $\rate$ is not affected. 
%The most striking conclusion is that the power efficiency and $\rate$
%are not reduced by dispersion.
%
%The maximum efficiency of \eqref{eq:overallpe} is a meaningful
%principle to guide the transmitter and designers.
%It provides very specific and credible insight into the type of modulation
%that should be used.
%To demonstrate this,
%it is shown in Section \ref{sec:dispersionfree} that \eqref{eq:overallpe}
%is the maximum power efficiency that can be achieved by QAM in the absence of dispersion.
%Subsequently it is shown in Sections \ref{sec:dispersionconstrained} and \ref{sec:multicarrier}
%that \eqref{eq:overallpe} can be achieved in the presence
%of dispersion by using MCM in conjunction with a subcarrier bandwidth limited
%by the coherence bandwidth $B \le B_{c}$.
%Finally the minimum rate and power case is addressed in Section \ref{sec:minimumrate}.
%
%\comment{Following is wrong and needs reworking because larger $N$ requires large $\recenergy$.}
%
%Comparing $\rate$ and $\capacityinf$ is apples and oranges.
%Since $P = f_{i} \, \recenergy$, for $N$ bits per ICH it follows that
%\begin{equation}
%\frac{\rate}{\capacityinf} = \frac{N \, \log_{\,e} 2}{\ecrs} \,.
%\end{equation}
%There is a fixed gap for a given $\ecrs$, which depends on the
%details of modulation and detection and reliability objectives.
%
%\doctable
%	{\footnotesize}
%	{conditions}
%	{
%	A list of the conditions under which the total information rate
%	$\rate$ during communication
%	is calculated in Section \ref{sec:inforate}.
%	Issues of discovery are deferred to Section \ref{sec:discovery}.
%	}
%	{p{2cm} p{12cm}}
%	{
%	\textbf{Condition} & \textbf{Description} \\
%	\toprule
%	Modulation &  
%	Use QAM as in \eqref{eq:modulation} without channel coding
%	\\
%	\cmidrule{1-2}
%	RFI &
%	Choose $h(t)$ to have DOF $K$ as described in \citeref{211}, with $K$ as large as
%	necessary for the RFI environment
%	(non-spread-spectrum QAM is the $K=1$ special case)
%	 \\
%	 \cmidrule{1-2}
%	Noise &
%	Operate at or near the fundamental power limit for QAM dictated by additive AWGN
%	due to natural sources (such as background radiation or sky noise)
%	 \\
%	 \cmidrule{1-2}
%	 Dispersion &
%	 Design requirement that dispersion does not affect $\rate$ 
%	 \\
%	\cmidrule{2-2}
%	 & As a side benefit, the receiver processing operates as if
%	 there were no dispersion, and in particular 
%	 de-dispersion
%	(used in pulsar astronomy \citeref{212} or in 
%	some  SETI pulse-detection techniques \citeref{605})
%	is avoided
%	  \\
%	 \cmidrule{1-2}
%	 Scattering &
%	 Scattering \citeref{582} is not considered here
%	  \\
%	 \cmidrule{1-2}
%	 Doppler &
%	 Doppler is not considered here
%	  \\
%	 \cmidrule{1-2}
%	 Carrier \newline frequency &
%	 There are \emph{no} restrictions on $f_{c}$, permitting lower 
%	 frequencies with larger dispersion, in part because these are
%	favorable to atmospheric noise and attenuation
%	\\
%	\bottomrule
%	}
%
%\incfig
%	{ultimateRate}
%	{.8}
%	{
%	The rate that can be achieved with maximum power efficiency, with or
%	without dispersion, is compared with the
%	the theoretical limit $\capacityinf$ (dashed curve)
%	for medium ($\snr_0 = 10$) and very high ($\ecrs = 20$ dB) reliability.
%	Achieving this requires a combination of biphase and MCM.
%	The horizontal axis is $\log_{10} \capacityinf$, which equals
%	$\log_{10} \power$ within an additive constant.
%	The gap between $\capacityinf$ and $\rate$ increases
%	with increasing reliability (smaller $\pe$).
%	}
%	
%\section{Dispersion-free case}
%\label{sec:dispersionfree}
%
%Building on the same linear modulation of QAM, but generating the
%symbols $A_{k}$ in a redundant and more complex way,
%it is possible to achieve $\rate \to \capacity$ corresponding to $B$.
%This is done by generating the $\{ A_{k} \}$ to multiple dimensions
%(data is mapped jointly onto a block of $\{ A_{k} \}$ rather than individual symbols).
%In our judgement, this \emph{channel coding}, at least in forms
%sophisticated enough to achieve $\rate \approx \capacity$,
%is not feasible for interstellar communications
%because it would be too difficult for the receiver to reverse engineer
%and recover the embedded information\footnote{
%The proof of \eqref{capacity} gives no hint as to how to achieve
%$\rate \to \capacity$, and thus we lack fundamental principles
%that guide channel code design.
%Five decades of intensive research identified a variety of incremental
%improvements on channel coding, culminating with turbo codes \citeref{618}
%which do achieve $\rate \approx \capacity$.
%Not only are turbo codes extremely complex, but
%there is undoubtably an infinite variety of channel codes achieving $\rate \approx \capacity$.}
%Once two civilizations have established  two-way communication 
%and are subsequently able to coordinate transmitter and receiver designs,
%$\rate \approx \capacityinf$ may be achievable.
%
%Consider a single-carrier QAM without channel coding as in \eqref{eq:modulation}.
%The parameters governing this signal and its successful reception of
% Table \ref{tbl:parameters}
%are organized differently in Table \ref{tbl:control}.
%The primary parameters $\{ f_c, \recenergy, K, N \}$
%control performance characteristics
%such as $\{ \pfa, \pd \}$ in discovery,
%the $\pe$ in communication, and the degree of RFI immunity.
%The secondary parameters $\{ B , \power, \rate \}$
%are determined by the primary parameters and measure quantities of concern to 
%system designers and users.
%Both $B$ and $T$ are temporarily considered to be unconstrained.
%
%\doctable
%	{\footnotesize}
%	{control}
%	{
%	A list of the primary parameters controlling the performance of the
%	QAM modulation of \eqref{eq:modulation} and secondary parameters
%	determined by the primary parameters.
%	}
%	{l c p{10cm}}
%	{
%	\textbf{Category} 
%	& \textbf{Parameter} 
%	& \textbf{Description} \\
%	\toprule
%	Primary & $f_{c}$ & Affects $B_{c} \propto f_{c}$ in \eqref{eq:coherencebandwidth},
%	which may affect $B$ \\
%	\cmidrule{2-3}
%	& $\recenergy$ & Controls $\ecrs = \recenergy/N_{0}$ and hence $\pfa$, $\pd$, and $\pe$;
%	\newline
%	Affects required received power through $\power = \recenergy/T$\\
%	\cmidrule{2-3}
%	& $K$ & Immunity to RFI increases with $K$ \citeref{211};
%	\newline
%	For fixed $B$, increases symbol time through $T = K/B$;
%	\newline
%	For fixed $B$, affects information rate through $\rate = N B/K$ \\
%	\cmidrule{2-3}
%	& $N$ & Minimal effect on discovery;
%	\newline
%	Affects $\rate$ through $\rate =  N/T$;
%	\newline
%	For a given $\snrnorm$, affects required $\recenergy$
%	through \eqref{eq:snrpamcommunication} \\
%	\cmidrule{1-3}
%	Secondary & $B$ & May be limited by $B_c$ 
%	for a given $f_{c}$ and $DM$ through \eqref{eq:coherencebandwidth} \\
%	\cmidrule{2-3}
%	& $T$ & Determined by the choice of $B$ and $K$ through $T = K/B$ \\
%	\cmidrule{2-3}
%	& $\power$ & Determined by $\recenergy$ and 
%	$T$ through $\power = \recenergy /T$;
%	\newline
%	After propagation loss, also determines transmit power \\
%	\cmidrule{2-3}
%	& $\pfa$,$\pd$ & Measures detection reliability during discovery \\
%	\cmidrule{2-3}
%	& $\pe$ & Measures reliability during communication \\
%	\cmidrule{2-3}
%	& $\rate$ & Determined by $N$ and $T$ through $\rate=N/T$ \\
%	\bottomrule
%	}
%
%The design constraints for QAM are
%\begin{subequations}
%\begin{align}
%\label{eq:rate1}
%&\rate = \frac{N}{T} = \frac{N \, B}{K} \\
%\label{eq:snrnorm}
%&\snrnorm = \frac{2 \pi}{2^{N}} \cdot \ecrs 
%= \frac{2 \pi \, \power \, K}{2^{N}\, N_{0} \, B}
%= \frac{2 \pi}{2^{N}} \cdot \frac{K}{B} \cdot ( \capacityinf \, \log_{\,e} 2 )
%\,.
%\end{align}
%\end{subequations}
%During communication $\pe$ is approximately fixed if $\snrnorm$ is fixed, and from this observation
%the appropriate choice of $B$ can be determined for a given $\power$,
%\begin{subequations}
%\begin{align}
%\label{eq:bandw}
%&B = \frac{2 \pi \, K \, \capacityinf \, \log_{\,e} 2}{2^{N} \cdot \snrnorm} \\
%\label{eq:powereffic}
%&\frac{\rate}{\capacityinf} = \frac{2 \pi \, N \log_{\,e} 2}{2^{N} \, \snrnorm}
%\,.
%\end{align}
%\end{subequations}
%From \eqref{eq:powereffic}, the power efficiency is maximized by biphase ($N=1$),
%and this is the special case\footnote{
%For $N=1$ the exact value $\snrnorm = 4 \cdot \ecrs$ has been substituted (Appendix \ref{sec:qam}).}
%given in \eqref{eq:overallpe} and illustrated in
%Figure \ref{fig:ultimateRate}.
%
%\section{Dispersion-constrained case}
%\label{sec:dispersionconstrained}
%
%In Section \ref{sec:discovery} it will be argued that
%the constraint $B \le B_{c}$ should be introduced to avoid
%a decrease in discovery sensitivity
%(the constraint $T \le T_{c}$ is deferred to Section \ref{sec:minimumrate}).
%This changes the single-carrier tradeoffs considerably.
%As $\power$ is increased, the power efficiency is maximized by $N =1$ 
%until $B = B_{c}$, after which the only way to increase $\rate$ further is by the less
%efficient vehicle of increasing $N$.
%From \eqref{eq:powereffic}, power efficiency is maximized by choosing the smallest $N$ satisfying $B \le B_{c}$.
%The resulting values of $\{ N, \, B \}$ are illustrated in Figure \ref{fig:NandBvsC}.
%
%\incfig
%	{NandBvsC}
%	{1}
%	{$N$ and $B$ for single-carrier QAM signal for $f_c=1$ GHz,
%	  $\deltadm = 100$, $\snrnorm = 10$, $B \le B_{c}$,
%	  and three values of $K$.
%	The horizonal axis is $\log_{10} \capacityinf$, but
%	since $\capacityinf \propto \power$ it also equals $\log_{10} \power$ 
%	within an additive constant.
%	The coherence bandwidth (dashed line) is $B_c = 34.7$ kHz.
%	Note that $N=1$ for $B < B_c$ (lower $\power$) but once the bandwidth saturates at
%	$B = B_c$ further increases in $\power$ require increasing $N > 1$ rather than $B$.
%	$B \propto \power$ for smaller $\power$ but $B \approx B_c$ for
%	larger $\power$
%	(the wiggles around $B \approx B_c$ are due to the quantization of $N$).
%	Larger $K$ saturates the bandwidth at lower $\power$.}
%
%The resulting $\rate$ is illustrated in Figure \ref{fig:powerLimitedRate}
%and compared with the
%fundamental limits $\capacityinf$ (for $B \to \infty$) and $\capacity$ 
%(for $B \le B_{c}$).
%As $\power$ and $\rate$ are increased to the point where $B=B_c$ and beyond,
%there develops an increasing gap between $\rate$ and $\capacityinf$ due to 
%abandoning biphase ($N > 1$).
%The power efficiency $\rate/\power$ shows a growing penalty 
%for $N > 1$ (for instance to 66.7\% of the $N=1$ value for $N=2$ and 3.1\% for $N=8$).
%
%\incfig
%	{powerLimitedRate}
%	{1}
%	{The solid curves are $\log_{10} \rate$ for the same
%	conditions as Figure \ref{fig:NandBvsC}.
%	The dashed curve is the fundamental rate limit $\log_{10} \capacityinf$
%	and the dotted curve is $\log_{10} \capacity$ for $B=B_{c}$.}
%
%For any given $K$, the operating point at $B = B_{c}$ and $N=1$
%is the maximum $\rate$ that can be supported by a single carrier without
%sacrificing power efficiency.
%From \eqref{eq:rate1} and \eqref{eq:snrnorm}, the design equations for this 
%desirable operating point are
%\begin{subequations}
%\begin{align}
%\label{eq:rateN1}
%&\rate = \frac{B_{c}}{K} \\
%\label{eq:snrN1}
%&\ecrs = K \cdot \snrin
%\ \ \ \text{for} \ \ \ 
%\snrin = \frac{\power}{B_{c} \, N_{0}} 
%= \frac{\capacityinf \, \log_{\,e} 2}{B_{c}} \,.
%\end{align}
%\end{subequations}
%$\snrin$ is the SNR at the input to the receiver, since
%$B_{c} N_{0}$ is the total noise power in bandwidth $B_{c}$.
%From \eqref{eq:snrN1}, the beneficial effect of the MF is to increase the SNR
%by a factor of $K$, since it extracts the noise in a single DOF
%from the total noise which is spread uniformly over $K$ DOF's.
%For a given requirement on $\ecrs$ (which determines $\pe$),
%this determines the needed $\power$.
%The dependence of $\rate$ on
%$f_c$ and $K$ is illustrated in Figure \ref{fig:rateVsFc}.
%Both $\power \propto B_{c}$ and $\rate \propto B_{c}$,
%so a greater $\rate$ (as long as $\power$ is commensurately larger) is possible
%at higher carrier frequencies $f_{c}$ (since $B_{c} \propto f_{c}^{\,3/2}$).
%
%\incfig
%	{rateVsFc}
%	{.8}
%	{A plot of the information rate $\log_{10} \rate$ that can be 
%	achieved with single-carrier biphase modulation ($N=1$)
%	in the presence of dispersion (for $\deltadm = 100$)
%	vs. $f_c$ for different values of $K$.
%	$\rate$ increases with $f_{c}$ because the milder dispersion 
%	allows a larger $B$.
%	Three values of $K$ are shown, where larger $K$ 
%	reduces $\rate$ due to the
%	bandwidth expansion.
%	Note the wide variation in $\rate$ 
%	(from $\approx 10^{-2}$ to $\approx 10^{7}$) depending on
%	the RFI immunity and carrier frequency.
%	Larger $\rate$ than shown here can be achieved by choosing $N>1$ as shown in 
%	Figure \ref{fig:powerLimitedRate} or by using multiple
%	carriers.
%	}
%
%Biphase is desirable for several reasons besides maximizing the power efficiency.
%It has the smallest and simplest constellation, and this is helpful
%for transmitter-receiver coordination and simple implementation.
%The energy per symbol, proportional to $| A_k |^2$ is always the same,
%making discovery easier and more consistent.
%A multi-symbol discovery algorithm that avoids precise knowledge of $h(t)$
%has been proposed for biphase \citeref{577}.
%
%Does the transmitter have any incentive to choose $B < B_{c}$?
%Even when the transmitter power budget is insufficient to support
%the received power $\power$ needed to achieve the
%maximum possible rate $\rate=B_c$ in \eqref{eq:rateN1},
%it is more logical to reduce $\rate$ by increasing $K$ 
%and the symbol time $T=K/B_{c}$ rather than by reducing $B$.
%This is because increasing $K$ increases RFI immunity at no cost,
%and conversely reducing $B$ reduces RFI immunity with no compensating gain.
%Since $\rate \propto 1/K$, there is an undesirable dependency between
%larger RFI immunity (large $K$) and larger $\rate$ (small $K$), but
%this is readily circumvented with MCM.

%\section{Multicarrier modulation}
%\label{sec:multicarrier}
%
%Our design when a single carrier is used is constrained by
%\eqref{eq:constantpowerbounds},
%which places an upper limit on the information rate per carrier of $B_c$
%bits per second when $K =1$, and a correspondingly lower limit
%when $K >1$ in the interest of RFI immunity.
%Without MCM, spread spectrum \citeref{211} would be considerably less
%attractive in the presence of dispersion, but the reduction in $\rate \propto 1/K$
%can be made up by choosing larger $M \propto K$.
%Higher bit rates can be obtained by expanding the number of carriers.
%These choices has no impact on power efficiency, as \eqref{eq:powerefficbinary}
%applies in all cases.
%Thus, there is a tradeoff between spectral efficiency and RFI immunity,
%with no impact on power efficiency.

%Comparing $\capacityinf$ and $\capacity$ for $B = B_{c}$ in Figure \ref{fig:powerLimitedRate}, at larger $\power$ the penalty in power 
%efficiency due to the dispersion constraint $B \le B_{c}$ is fundamental and not specific to QAM. This is a good reason to consider multicarrier modulation (MCM), a way to bypass this penalty and achieve the biphase power efficiency for arbitrarily large $\rate$ 
%as illustrated in Figure \ref{fig:ultimateRate}, and to do so
%simultaneously with a $B \le B_{c}$ constraint for each individual carrier. This strategy was previously advocated by S. Shostak in 1995 \citeref{127}. 
%
%The idea of MCM  is  simple. Consider the familiar AM/FM radio bands, where more stations are broadcast (at the expense of greater bandwidth) by separating them using different carrier frequencies (this is called frequency-division multiplexing). In the early days of digital communication this approach was eschewed in favor of using a single carrier bearing the total information rate, interleaving different information sources within that single stream (this is called time-division multiplexing). However, once highly dispersive and time-varying media were encountered in wireless channels, numerous advantages to transmitting multiple carriers became evident. Today MCM is widely used.
%
%Assume that $M$ subcarrier signals, each with bandwidth $B_{c}$, are transmitted with uniformly-spaced carrier frequencies such that their spectra are nonoverlapping.
%If $f_{0}$ is the spacing between carriers, then $f_{0} \ge B_{c}$, where $B_{c}$ is the coherence bandwidth corresponding to the
%lowest carrier frequency.\footnote{
%Two refinements would be to overlap the spectra, as is conventional in terrestrial MCM, or to decrease $f_{0}$
%with frequency taking advantage of the weakening dispersion.
%While these measures conserve bandwidth, 
%in interstellar communication there is little incentive to conserve bandwidth.
%In fact, Section \ref{sec:discovery} concludes that there are 
%advantages to $f_{0} > B_{c}$, such as $f_{0} = 2 \, f_{c}$.}
%If each subcarrier has rate $\rate$ and requires received power $\power$, 
%then the aggregate MCM rate becomes $M \rate$ and the total MCM power becomes $M \power$.
%Thus, the power efficiency is unchanged, and an arbitrarily large $\rate$ can be
%achieved without compromise and with the simplicity of biphase modulation.
%
%There are a number of advantages of MCM in interstellar communication.
%Without MCM, spread spectrum \citeref{211} would be considerably less
%attractive in the presence of dispersion, but the reduction in $\rate \propto 1/K$
%can be made up by choosing larger $M \propto K$.
%The relative powers allocated to different carriers can be adjusted
%to accommodate frequency-dependent phenomena such as a planet's
%larger atmospheric noise due to water vapor (concentrated at $f_c \gg 15$ GHz).
%The power allocated to one (and only one) subcarrier can be artificially increased
%to make discovery easier with only a small power penalty overall.
%MCM lends itself to parallelism in transmitter implementation.
%For example, any collection of subcarrier signals can be transmitted independently
%of the others using separate
%RF electronics and antennas, each optimized for its own carrier frequency.
%A transmitter designer on a limited budget can 
%expand total information rate over time by increasing $M$, 
%with a capital cost that scales no faster than $\rate$.
%As discussed in Section \ref{sec:discovery}, MCM can also improve
%the discovery sensitivity.
%Both transmit and receive implementations lend themselves to
%joint subcarrier manipulation at baseband using discrete Fourier
%transform techniques \citeref{612}.

%\section{Minimum-rate and minimum-power design}
%\label{sec:minimumrate}
%
%While the emphasis in MCM is on achieving a large $\rate$,
%a transmitter designer with limited transmit power resources
%may choose instead to transmit a signal with the lowest power that can be reliably discovered.
%Low $\power$ generally means a single-carrier modulation with low $\rate$.
%However, the time coherence constraint $T \le T_{c}$ puts a lower limit
%on single-carrier $\rate$, namely $\rate \ge 1/T_{c}$.
%At the lower limit, there remains freedom in the choice of $B$ within the constraint $B \ge K/T_{c}$.
%At no cost to $\power$, the RFI immunity can be maximized by choosing the
%maximum $K$, which corresponds to $B = B_{c}$ and $K = B_{c} \, T_{c}$.
%These design choices are attractive to the receiver 
%because both $B=B_{c}$ and $T= T_{c}$ are constrained by observable physical parameters
%and thus the discovery search space is relatively limited.
%Spread spectrum ($K > 1$) is what allows $B$ and $T$
%to be chosen independently to arrive at this desirable operating point.
%
%Consider the information-free ''beacon'' signal such as sought by
%current narrowband SETI searches \citeref{142}.
%Presumably the designer of such a signal would choose maximum time duration $T_{c}$
%because this minimizes the received power required for reliable detection with a MF.
%If the receiver knows or can guess the beacon waveform (such as a pure sinusoid),
%and a MF filter is used to detect this waveform, then for a given detection reliability the received
%power requirement is identical to the minimum-rate information-bearing signal with $\rate = 1/T_{c}$.
%It seems unlikely that a transmitter designer will chose to transmit such a beacon
%when an information-bearing signal requires the same receive power,
%can embed information (albeit at a relatively low rate), and has superior RFI immunity.
%Neither narrowband nor pulse searches is capable of discovering the minimum-rate signal.
%
%In the case of MCM, there is ambiguity in the $\rate$ per subcarrier 
%within the constraints $B \le B_{c}$ and $T \le T_{c}$.
%Whatever choice is made does not constrain the aggregate rate $M \rate$. 
%Recognizing the receiver's challenge in searching over $B$ and $T$, an attractive choice is $B=B_{c}$ and $T = T_{c}$. Each subcarrier then becomes a minimum rate information-bearing signal (with $\rate = 1/T_{c}$) and the RFI immunity assumes the largest feasible value based on physical constraints (corresponding to $K = B_{c} T_{c}$). In any search for information-bearing signals, search for a minimum-rate subcarrier is an attractive starting point.

%\section{Discovery}
%
%During discovery, the MF output $Q = |Z|$ can be applied to a threshold $\hht$
%to detect the presence of a signal or not, where $Z$ is Gaussian with statistics
%given by \eqref{eq:Zstats}.
%In this case, $Q$ is has $\chi$ and it is easy to determine the false alarm
%probability $\pfa$ and detection probabiity $\pd$,
%\begin{align}
%\pfa &= \prob{Q > \hht \left. \right| A = 0} = 1 - e^{- \hht^{\,2}/ N_{0}} \\
%\pd &=  \prob{Q > \hht \left. \right| A = 1} = 1 - e^{- \hht^{\,2}/ ( \recenergy \vs + N_{0})}
%\end{align}
%
%
%During communication, ISM impairments are less significant, especially
%relatively time-invariant phenomena such as plasma dispersion.
%This is because to some extent these can be estimated and equalized.
%
%During discovery, ISM impairments cause a disconnect between the
%power required for reliable communication and the power required for reliable
%discovery.
%This is the primary argument for confining a signal to the ICH.
%
%The argument in favor of choosing $B = B_c$ is based on
%objective (B) in Section \ref{sec:introduction}.
%It will now be shown that discovery operates at reduced sensitivity
%for $B > B_c$.
%Discovery is considered at the scales of an isolated pulse,
%a subcarrier, and multiple subcarriers.
%
%\section{Detection of an isolated-pulse}
%\label{sec:isolatedpulse}
%
%The simplest discovery detects the presence of a single symbol with a single carrier
%frequency, which we call \emph{isolated pulse} detection.
%The key observation in Figure \ref{fig:IRvsB} is no
%appreciable diminution in isolated pulse magnitude at the MF output as long
%as $B \le B_{c}$.
%In that case, the MF output in \eqref{eq:mfoutput} can be sampled
%as if there were no dispersion, and an estimate of the
%pulse energy is
%\begin{equation}
%\label{eq:ipdnod}
%Q = | Z(0) |^{2} \approx
%\left| \,
%e^{\, i \, \Theta} \, \sqrt{\recenergy} \, A_0
%+ \sqrt{N_0} \, M(0)
%\, \right|^{2} \,.
%\end{equation}
%If this $Q$ is applied to a threshold,
%$\pfa$ and $\pd$ are predicted (Appendix \ref{sec:qam})
%by the SNR measure
%\begin{equation}
%\label{eq:snrpamdiscovery}
%\snr_{Q} = \frac{\ecrs^{\,2}}{1 + 2 \cdot \ecrs} \,.
%\end{equation}
%For an $\ecrs$ large enough to support reliable communication, 
%$\snr_{Q} \approx \ecrs/2$, the 
%factor of two attributable to the inclusion of both
%in-phase and quadrature noise in the estimate.
%Discovery suffers an intrinsic 3 dB disadvantage
%relative to communication due to lack of knowledge and inability to
%estimate $\Theta$.
% 
%What happens to discovery when $B > B_{c}$?
%As illustrated in Figure \ref{fig:IRvsB}, \eqref{eq:ipdnod}
%will suffer a reduced sensitivity due to the decreased
%pulse amplitude appearing in $|Z(0)|$,
%violating objective (B).
%There are two paths to rescuing the situation 
%while sticking with the simplicity of isolated pulse detection.
%The first is to design a discovery algorithm that takes advantage of
%knowledge of $\max \tau_s$ corresponding to $\dm = \dm_{U}$ or $\deltadm$.
%The second searches over a range of actual values of $\dm_{L} \le \dm \le \dm_{U}$
%or $0 \le \dm \le \deltadm$.
%Here we take the first path and relegate
%the second path (which is considerably more complicated) to another paper \citeref{619}.
%Our assessment of both approaches is that a reduction in
%detection sensitivity is inevitable.
%
%Although $f(t)$ is not precisely known during discovery, it has two properties
%useful in choosing a replacement for $Q$ in \eqref{eq:ipdnod}.
%First, $f(t)$ is allpass ($|F(f)| = 1$)
%and thus the total energy in $f(t) \convolve R_h (t)$ equals the energy in $R_h (t)$.
%Second,
%the energy of $f(t)$ falls in the interval $t \in [0,\tau_{s}]$,
%where the worst-case value $\max \tau_{s}$ corresponding to the
%largest $\dm$ can be assumed.
%If $B \, T \gg 1$ then $R_h (t)$ is a narrow pulse relative to
%symbol interval $T$,
%and thus the energy in $f(t) \convolve R_h (t)$ is also concentrated
%in time interval $t \in [t_1,t_2]$,
%where $\tmax = (t_2 - t_1)$ is the sum of the intrinsic time duration of $R_h (t)$
%and the smearing of $R_h (t)$ by $\tau_s$.
%
%The incoherent MF of \eqref{eq:ipdnod} can be generalized by making $Q$
%an estimate of the energy in the interval where signal energy is known to reside,
%\begin{equation}
%\label{eq:Q}
%Q = \int_{t_1}^{t_2} \left| \, Z(t) \, \right|^{2} \, dt \,.
%\end{equation}
%This energy estimate works equally well regardless of
%the actual value of $\dm$ since \eqref{eq:Q} encompasses all the signal energy
%even if the actual $\tau_{s} < \max \tau_s$.
%Beneficially \eqref{eq:Q} excludes all noise and RFI not overlapping
%the worst-case pulse duration.
%It is significant that $\tmax \ll T$ because that makes the
%noise component in $Q$ smaller.
%Although $Q$ is non-Gaussian,  by Central Limit Theorem
%arguments it is well approximated as Gaussian and SNR
%measures at the threshold are a good predictor of $\pfa$ and $\pd$.
%The $\snr_{Q}$ at the threshold input is (Appendix \ref{sec:ipd})
%\begin{equation}
%\label{eq:snrQ}
%\snr_{Q} \approx 
%\frac{\left( \ecrs \right)^{2}}{2\,\alpha+ ( B / B_c )^2 + 2 \cdot \ecrs} \\
%\end{equation}
%The new parameter $\alpha$ determines the fraction of captured
%energy in $R_h (t)$
%(some energy is lost since $R_h (t)$ is not strictly time-limited).
%The choice $\alpha = 1$ is large enough to
%reduce the signal energy penalty to a fraction of a dB.
%Figure \ref{fig:snrVsB} illustrates $\snr_Q$ for different values
%of $B$, demonstrating the substantial penalty for $B > B_c$.
%
%Comparing \eqref{eq:snrpamdiscovery} and \eqref{eq:snrQ},
%there are two distinct regimes.
%For larger $\snr_0$, there is a minimal dispersion penalty in $\snr_Q$, but at
%lower $\snr_Q$ the penalty is more severe.
%The transition between these regimes can be defined as
%the bandwidth for which there is a 3 dB penalty due to dispersion,
%or $\snr_Q = \snr_0/4$ and hence $B = B_c \cdot \sqrt{2\, ( \snr_0 - \alpha )}$.
%For example, at $\snr_0 = 10$, $B \approx \sqrt{18} \, B_c$
%is the 3 dB penalty point, and
%$B \approx B_c$ results in a small penalty in $\snr_Q$.
%
%\incfig
%	{snrVsB}
%	{.8}
%	{
%	The penalty in $\snr_Q$ (the dashed line is
%	the dispersion-free case) during discovery of a subcarrier isolated pulse using a matched
%	filter followed by energy estimate \eqref{eq:Q} with $\alpha=1$
%	for different values of $( B/B_c )$.
%	 Typically $\snr_0 \approx 10$ is required for $\pe \approx 0$ in communication.
%	 Larger $B$ results in a greater reduction in SNR because $\tau_s$ and
%	 $\tmax$ become larger, admitting more noise into $Q$.
%	 }
%
%\section{Effect of bandwidth and symbol time offset}
%
%Since the receiver has no a priori knowledge of $f_c$ and $T$ (or equivalently $K$)
%and incomplete knowledge of $B_c$,
%a discovery search requires trying different values for these parameters,
%and this creates multiple opportunities for a false alarm and thus increases $\pfa$.
%Specifically consider the parameterization of $h(t)$ for a known spreading sequence,
%which can be summarized as
%$\{ B_{c} , K_t \}$ at the transmitter and $\{ B_{c} \, (1+\delta) , K_r \}$ at the receiver,
%where $\delta$ is a fractional offset in bandwidth.
%As noted in \citeref{211}, when the spreading sequence is chosen to be
%one-sided, $K_r \ne K_t$ is acceptable since the only effect is
%missing some signal energy or adding some noise energy.
%Thus a search over values of $K_r$ can be coarse-grained,
%say proceeding by powers of two.
%
%A search over $B_{c}$ must have finer granularity.
%The question is the size of $\delta$ that reduces signal level materially
%at the output of the incoherent MF.
%The rate at which the spreading sequence is generated is $B_{c}$ at the transmitter
%and $B_{c} \cdot (1+\delta)$ at the receiver.
%A material falloff in cross-correlation will occur when
%the $K_{r}$ value at the receiver is aligned with the $(K_{r}-1)$ or $(K_{r}+1)$ value from
%the transmitter.
%To avoid this,
%\begin{equation}
%\frac{K_r -1}{B_{c}} \lessapprox \frac{K_r}{B_{c} \, (1+\delta)} \lessapprox \frac{K_r +1}{B_{c}}
%\ \ \ \text{or} \ \ \ 
%\frac{1}{K_{r}+1} \lessapprox \delta \lessapprox \frac{1}{K_{r}-1} \,.
%\end{equation}
%In other words, the search granularity over $B_{c}$ must be on the order of $B_{c}/K_{r}$,
%and likewise the granularity in a search over $f_{c}$.
%Adopting a relatively smaller $K_{r}$ admits a relatively larger $\delta$, 
%as well as reduces the computational load for the MF.

%\section{Detection of a subcarrier}
%\label{sec:subcarrier}
%
%The continuous-time noise-free output 
%$| Z(t) |^2$ of $M$ incoherent MF's
%is shown in Figure \ref{fig:subcarrierOutputs}.
%For a given assumed $B_{c}$ and $f_{0}$,
%this filterbank can be implemented by
%a single demodulation with carrier $f_c$ followed by discrete Fourier
%transform techniques.
%Each subcarrier consists of a periodic sequence of pulses with duty cycle approximately equal to $1/K_{t}$
%and period equal to $K_{t}/B_{c}$, where there is uncertainty in $B_{c}$
%and $K_{t}$ is unknown.
%Uncovering periodicity in a noisy signal is a well-studied problem in signal processing.
%A representative algorithm forms the discrete Fourier transform and looks
%for peaks in the resulting spectrum.

%A challenge not directly addressed by the isolated pulse-detection
%of Section \ref{sec:isolatedpulse} is
%variation in background noise $N_{0}$ due to astronomical
%sources, the same natural noise-like signals essential to radio astronomy.
%A reliable discovery algorithm should therefore look for signal characteristics
%that strongly distinguish a signal of interest from natural sources of noise \citeref{581},
%and in particular rely on more than excess power for a given direction of arrival.
%Spread spectrum meets this requirement because it results in 
%an unnatural periodic train of narrow pulses at the incoherent MF output.
%This is a characteristic shared with pulsars.
%The de-dispersion algorithm in pulsar astronomy is replaced
%by the incoherent MF in QAM and MCM, so
%there is no danger of confusing a pulsar for spread-spectrum QAM or vice versa.
%
%\section{Detection of multiple subcarriers}
%\label{sec:MCMdetection}
%
%With additional computational burden, a joint search
%for multiple carriers can yield greater sensitivity than 
%an isolated-pulse or subcarrier search.
%Like extraction of the information symbols,
%discovery of a subcarrier is based on received power $\power$,
%but the aggregate received power is $M$ times larger.
%Multicarrier detection can take advantage of this larger power and
%thereby has the potential to discover 
%signals too weak to support reliable communication.
%
%Looking across subcarriers in Figure \ref{fig:subcarrierOutputs}, 
%the periodic pulses of each subcarrier are offset by
%a relative group delay that is linear in filter index.
%A filter bank approach is also used in discovering pulsars \citeref{212},
%and the filterbank outputs appear strikingly similar to Figure \ref{fig:subcarrierOutputs}.
%Pulsar discovery algorithms (with de-dispersion replaced by the
%much simpler incoherent MF) can thus be repurposed for MCM discovery.
%This two-dimensional signal has several distinguishing characteristics.
%In addition to the period pulse property of each subcarrier,
%repeated exactly across subcarriers,
%the linear variation in group delay vs. filter index
%is the signature of a signal influenced by plasma dispersion.
%An MCM signal can be explicitly designed to differ even more 
%powerfully from natural sources of energy.
%For example, an obvious opportunity is to choose $f_{0} = 2 B_{c}$
%so that filter outputs alternate between periodic pulses 
%plus noise and noise only.
%All these unique signatures also help to distinguish MCM from most sources of RFI.
%
%The expected bandwidth of
%each subcarrier and the spacing of subcarriers is related to $B_{c}$
%and thus $\dm_{U}$ or $\deltadm$.
%The relative group delay across subcarriers, on the other hand,
%is determined by the actual value of $\dm$, requiring a search over that
%unknown parameter with range equal to $\deltadm$
%and a granularity on the order of $1/B_c$.
%Consider the case where, in the course of a search, the correct
%parameters $\{ f_{0}, \, T, \, \dm \}$ are used and
%the incoherent MF outputs are accumulated
%from $L>1$ pulses either over time or over frequency.
%By the law of large numbers (Appendix \ref{sec:qam}),
%the resulting SNR at an energy threshold input is increased by $L$
%because the signal energy adds coherently but the noise energy adds incoherently.
%This concretely demonstrates the improved sensitivity obtainable
%from exploiting the entire power $M \power$.
%
%A discovery technique for biphase based on the autocorrelation
%of successive data symbols has also been proposed \citeref{577}.
%At the expense of lower sensitivity, this approach has the advantage
%that $h(t)$ need not be known or guessed as assumed here.
%This approach would apply as well to correlation across subcarriers.

%For both a beacon and OOK,
%$P_{\text{D},L} \to 1$ as $L \to \infty$, and thus $\pd \approx 1$
%can always be achieved by making $L$ sufficiently large.
%This is true for any $\ecrs >0$ and any $\pfa >0$,
%so virtually any signal level can be discovered with probability approaching unity,
%for a small false alarm probability.
%Intuitively this is a result of the benefits of scintillation in sometimes \emph{increasing}
%the signal flux, thus making up for a small $\ecrs$.
%As long as $L$ is sufficiently large, at least one of the observations is
%sure to occur during this period of received flux magnification.


%\section{Comparison of beacons and information-bearing signals}
%
%The question arises as to how this compares to the intermittent
%beacon that was studied in Section \ref{sec:beacondiscovery}.
%For the same case of $M = 256$, the relationship between
%symbol and bit energy contrast ratios is $\ecrs = \log_{2} \ecrb$.
%At the same operating point of $\ecrb = 6$ dB, it follows that
%$\ecrs = 15$ dB.
%From Figure \ref{fig:optP1vsSNR},
%this value of $\ecrs$ is right at the transition where 
%a duty cycle $\delta < 1$ makes sense, and therefore at this
%power level there is no opportunity to reduce the number of
%observations $L$ by reducing the duty cycle.
%Thus, we are not tempted to modify the FSK signal to make it more ''discoverable''.
%
%However, it is possible to discover an M-ary FSK signal
%at much lower power levels than required for reliable information
%recovery, at the expense of increasing $L$.
%In Figure \ref{fig:discoveryFSK} if up to $L = 1000$ observations
%are acceptable, the input power level can be reduced by about 6-8 dB
%or so, depending on the discovery reliability that is demanded.
%This could prove useful in a couple of circumstances.
%One is where the transmitter designer has higher expectations
%for receive antenna gain than is actually implemented by the receiver.
%Another is where the signal is actually intended for a different
%star but is intercepted at lower power because the receiver is
%in a side lobe or is at a greater distance.
%In either case, a receiver can successful discover
%an M-ary FSK signal at lower powers than necessary for
%the recover of information from that signal.

\section{Pattern recognition in discovery}

The previous analysis has presumed that detection of a beacon
or an information-bearing signal requires only the presence of a
single energy bundle in $L$ observations of duration $T_{o}$.
In the numerical examples the false alarm probability was set
fairly low, at $\pfa = 10^{-12}$ or $10^{-8}$.
Nevertheless, this form of detection will never suffice to declare
the discovery of a signal.
As discussed in Section \ref{sec:discoveryrel}, these values of
$\pfa$ are presumably still much larger than the a priori probability
of a signal being present, and thus false alarms will dominate
these detections rather than a high-confidence discovery.
Once an energy bundle is discovered, it is appropriate to
continue observing in that same location (line of sight and frequency)
to see if other energy bundles are detected.
In essence, conditional on a successful detection, either the
observation time $T_{o}$ (up to the estimated coherence time)
or the number of observations $L$ can be increased (keeping them separated in time
by more than the coherence time), or both.
In view of the possibility of a time-varying frequency shift due to
uncompensated acceleration and due to information-bearing signals
that utilize more than one frequency (such as the M-ary FSK used
in our examples), these observations should be conducted
over a range of frequencies near to the observed energy bundles.

Should these continued observations detect more energy bundles,
the receiver can extend the observations at that location,
and switch to a pattern recognition mode in which discernible
patterns of energy are sought.
A recognizable and repeatable pattern presents even more significant
evidence of the presence of a signal.
This requires statistical (rather than deterministic) pattern recognition, since at low average power
levels the probability of detection of an individual energy bundle
is expected to be small ($\pd \ll 1$), and also because the
location of bundles may be coupled to a random stream of information bits.
The literature and algorithms for statistical pattern recognition
appropriate for discovery of power-efficient signals is an
interesting topic for future research.

If it is assumed that the transmitter designer is motivated to minimize
transmitted average power, or if the receiver designer economizes on
antenna collection area,
then existing SETI searches are unlikely to discover the signals.
These existing searches do not realize the tens, hundreds, or thousands
of independent observations necessary to achieve a reasonable detection
probability for a power efficient signal or power-optimized beacon.
In addition, these existing searches typically assume short-term persistence of
the signal in an attempt to rule out false alarms, which is ineffective
for intermittent signals of the type we have considered here.
It is possible that past SETI searches have detected legitimate beacons
but incorrectly categorized them as false alarms because
they did not take account of the relatively low probability of detection
of a single energy bundle nor the possible intermittent nature of the signal.


%\section{Power-efficient beacons inherently bear information}
%
%\comment{Will be unable to reliably detect information at low power levels.}
%
%By definition,
%a power-efficient beacon operates in the low-power regime.
%Thus it uses a duty cycle less than 100\% in order to conserve power
%while simultaneously minimizing the number of observations at the
%receiver.
%An underlying assumption behind Figure \ref{fig:optLvsSNRlowDuty}
%is statistical independence of the receiver's observations.
%I significant point is that while the receiver needs to space out its
%observations in time to insure that the scintillation is independent,
%it is not necessary or appropriate for the transmitter to do the same.
%In our numerical examples, the observation-minimizing duty cycle is on the
%order of 2\% or higher, which is incompatible with the large spacing
%that would be necessary to achieve independent scintillation events.
%Rather, the transmitter can assure independence in the observations
%by randomizing the transmit times.
%
%The randomization of transmit times at the source can actually be
%coupled to information that it wishes to convey to the receiver.
%Thus, a power-efficient beacon is naturally information-bearing.
%To explore this further, during periods of relatively high received
%scintillation flux, in any given observation the receiver observes a signal
%with probability $\delta$ and no signal with probability $(1 - \delta)$.
%By choosing or not choosing to transmit at this time, the transmitter
%is conveying information to the receiver.
%How much information?
%As Shannon observed,
%the information in one observation equals
%the information entropy
%\begin{equation}
%H( \delta ) = - \delta \, \log_2 \delta - (1 - \delta) \, \log_2 \, (1 - \delta) \ \ \text{bits} \,.
%\end{equation}
%The entropy is plotted in Figure \ref{fig:beaconInformation}, and is maximum
%at $\delta = 1/2$, when the information conveyed in one observation is one bit.
%
%\incfig
%	{beaconInformation}
%	{.8}
%	{A plot of the information entropy  per observation $H( \delta )$ and power efficiency
%	$H( \delta )/\delta$ for a power-efficient beacon as a function of the duty cycle $\delta$. 		The power efficiency increases at lower duty cycles.}
%
%For the small $\delta$ appropriate at low powers, the amount of information
%conveyed is significantly smaller than one bit.
%Although $H(\delta) \to 0$ as $\delta \to 0$, the transmit power also
%approaches zero, and the power efficiency is proportional to the ratio,
%\begin{equation}
%\label{eq:powerebeacon}
%\powere \propto \frac{H(\delta)}{\delta} \,.
%\end{equation}
%As shown in Figure \ref{fig:beaconInformation}, the power decreases more
%rapidly than the entropy, so $\powere \to \infty$ as $\delta \to 0$.
%This is somewhat misleading, since this simplistic metric does not take into account
%reliability, and as indicated by \eqref{eq:powerescin} there is actually an upper bound on
%the $\powere$ that can be obtained with reliability.
%Nevertheless, \eqref{eq:powerebeacon} is encouraging, because it
%indicates that a power-efficient beacon is intrinsically a power efficient
%information-bearing signal.
%
%In Chapter \ref{sec:infosignals} the design of information-bearing signals is considered.
%This exercise confirms that a power-efficient information-bearing signal
%can serve as a power-efficient beacon.
%This provides a ready answer to one long-standing question regarding beacons.
%Is it advantageous to transmit a beacon separate from an information-bearing signal,
%that beacon being somehow easier to discover?
%The answer is a definitive negative for power-efficient design.
%Information-free beacons are only an interesting option when the transmitter
%is willing to devote considerably more transmit power than is necessary.
%
%A beacon can be effective at arbitrarily low SNRs, at the expense
%of increasing the number of observations $L$ expected of the receiver.
%This can be driven to arbitrary low powers, so the question arises
%as to how far should we take this?
%The answer is that there is a lower bound on the SNR
%(and hence the average transmitted power) for which
%the beacon in its dual role as an information-bearing signal can
%convey information reliably.
%We know this from the fundamental limits of Chapter \ref{sec:fundamental}.
%A natural objective for the beacon is to be discoverable at this SNR.
%This places a natural expectation on the $L$ that the
%receiver should implement.
%Of course, if the receiver chooses to implement a larger $L$,
%it can detect a beacon at a lower SNR without expecting
%reliable recovery of information from the beacon.


%\section{The impact of search on discovery}
%
%The false alarm probability $\pfa$ associated with a single IU will generally
%have to be very small in part because in the course of discovery the algorithm also
%has to search over multiple possible locations.
%Consider for example a single fixed ICH.
%There will generally be multiple possibilities in terms of IU's that overlap this ICH
%in some way, including those that start a different times and different carrier frequencies.
%The granularity of such a search is explored in Appendix \ref{}, where it is shown
%that in seeking a signal with bandwidth $B$ and time duration $T$ a search has to use a granularity
%on the order of $1/T$ in carrier frequency (for a total of $K = BT$ possibilities)
%and a granularity on the order of $1/B$ in starting time (for a total of $K$ possibilities).
%Thus, the total number of possibilities is on the order of $L = K^{2}$.
%A compound discovery of all the possibilities even overlapping a single ICH
%is composed of many individual opportunities for false alarms.
%
%The joint statistics of false alarms depends on the properties of $h(t)$,
%and in particular its autocorrelation function and Fourier transform.
%For the case of an $h(t)$ that is noise-like, as advocated in Section \ref{},
%the false alarms will be essentially statistically independent, so let's
%consider that case.
%Similar to \eqref{}, the $P_{\text{FA},L}$ for $L$ independent trials is
%\begin{equation}
%P_{\text{FA},L} = 1 - (1 - \pfa)^{L} \approx L \cdot \pfa \,.
%\end{equation}
%To compensate for this, all else being equal
%we have to reduce $\pfa$ by a factor of $L$, which implies
%from \eqref{eq:PfaVsPd} that the detection probability is also smaller,
%\begin{equation}
%P_{\text{D},L} \approx \left( \frac{\pfa}{L} \right)^{1/(1 + \ecrs)} \,.
%\end{equation}
%As we have seen, thanks to scintillation this can be compensated by increasing the
%number of observations.

\chapter{Detection of energy bundles}
\label{sec:detection}

The first stage of discovery is the detection of a single energy bundle.
This stage is characterized by the three parameters
$\{ \pfa , \, \pd , \, L \}$, and
understanding and quantifying the tradeoff among them is of interest.
If the designer demands either smaller $\pfa$ or larger $\pd$,
this requires that $L$ be increased.
This tradeoff is affected by
 impairments in the channel
(due to the ISM and motion) and radio-frequency interference (RFI).
Unlike during communication, during discovery there is no opportunity to
observe and estimate any of these impairments save noise and
motion due to the observer's local planetary system.
Especially there is no opportunity to observe the current state of scintillation,
so an outage strategy (which was helpful to our communication design) cannot be employed during discovery.
The impairment issues will be discussed first, followed by a discussion of
the matched filter, which is key to countering the effects of noise,
followed by a characterization of $\{ \pfa , \, \pd , \, L \}$.
All three categories of signals will be considered.

\section{Coherence hole}

In Chapter \ref{sec:fundamental} 
it was established that structuring the transmit signal around the
ICH is necessary to approach fundamental limits on power efficiency.
The ICH is even more important to discovery.
There are several reasons for this.
Eliminating most ISM and motion impairments as
a consideration removes whole dimensions of search during discovery.
For example, the computationally intensive de-dispersion algorithms
of pulsar astronomy are avoided, because unlike pulsars
interstellar communication signals can be rendered
impervious to dispersion by design.
Eliminating whole dimensions of search in turn reduces the false alarm
rate, and thus allows discovery to operate at higher sensitivity.
Finally, the ICH size can be estimated based on the observation of physical quantities,
and thus it serves as a source of implicit coordination between transmitter
and receiver that constrains parameters of search, 
principally signal bandwidth and time duration.
Thus, the detection algorithms considered in this chapter assume
that the transmit waveform $h(t)$ has been chosen to render
impairments from the ISM and motion insignificant.

In contrast, following discovery the ongoing observation
of an interstellar communication signal makes it feasible to
estimate and correct for some ISM and motion impairments.
An example is dispersion, because as a phase-only phenomenon it
can be corrected (or ''equalized'') without enhancement of the noise.
This renders some of these impairments potentially less significant during
communication.
It remains beneficial to structure around the ICH, because there
is no power-efficiency penalty in doing so and whole categories of
receiver processing are eliminated.

\section{Scintillation}

During communication, the strategy of Chapter \ref{sec:infosignals}
was to track the variation in received signal flux due to scintillation,
and to attempt to extract information only during periods when that
flux exceeds a threshold, declaring other periods to be outages.
This is not a viable strategy for discovery, since there is no known signal to track.
The implication of scintillation is that there are periods during which the
received signal flux is below the average, and other periods when it is
above the average.
The latter periods are actually quite helpful for discovery,
since a patient receiver will discover signals that would not be
visible in the absence of scintillation.

Given that an outage strategy does not work, the appropriate
model for a single energy bundle is,
from \eqref{eq:interstellarmodel},
\begin{equation}
Z =
\begin{cases}
 \sqrt{\energy_{h}} \, S + M \,, & \text{signal energy present} \\
 M  \,, & \text{noise only}
 \end{cases}
 \,.
\end{equation} 
The MF output is zero-mean Gaussian under both conditions, the only
difference being a larger variance when signal is present,
\begin{equation}
\text{Var} [ Z ] = \expec{|Z|^{2}}
\begin{cases}
 \energy_{h} \, \vs + N_0 \,, & \text{signal energy present} \\
 N_0  \,, & \text{noise only}
 \end{cases}
 \,.
\end{equation}
The energy contrast ratio $\ecrs$ of \eqref{eq:ecrs}
is a measure of the fractional increase in variance due to
a scintillated signal.

In the presence of scintillation a single observation cannot achieve reliable detection,
since that observation stands a good change of occurring during
a period of below-average received flux.
Thus, to take advantage of the periods of enhanced flux,
it is necessary to make multiple observations in the same
location.
By ''location'', we mean the same spatial and frequency parameters.
In the following, it is assumed that the receiver makes $L$ independent
observations.
By independent, we mean that the observations are separated by a
time interval large relative to the scintillation coherence time,
so that the observations can be considered to be statistically independent.
This has been pointed out previously and it was found that
$L \approx 3$ suffices for high-power signals \citereftwo{122}{121}.
Here we show that a much larger $L$ is needed to
reliably discover power-efficient signals of either the information-bearing or
beacon variety.
This is due to the intermittent nature of the signal itself,
which reinforces the intermittent nature of the scintillation.

\section{Radio-frequency interference}

Affects choice of $h(t)$

\section{Noise and the matched filter}
\label{sec:matchedfilter}

The foundation of discovery is the detection of a single
isolated bundle of energy.
This stage is the same for an information-bearing signal
and for a beacon.
The energy of the signal that is proportional to $h(t)$
is most efficiently captured by a filter matched to $h(t)$.
The sensitivity of this detector in the presence of scintillation
is now determined.
This sensitivity is quantified
by the relationship between the probability of false alarm $\pfa$ 
and the probability of detection $\pd$ as a function of $\ecrs$.

The basic building block for discovery is the filter matched (MF) to
waveform $h(t)$ defined in \eqref{eq:simplemf}.
To achieve high discovery sensitivity,
the receiver must guess the waveform $h(t)$ in use, 
or it may be able to search for a set of possible $h(t)$ waveforms
as long as the number of distinct possibilities is relatively small.
However, even making this guess successfully,
there are several degrees of uncertainty.
The actual waveform as observed at the receiver will be of the form
$h( \beta ( t - \tau) ) e^{\,i\,2 \pi f_1 t}$,
where the three uncertain parameters are $\{ \beta , \tau , f_1 \}$.
The receiver must search over some range of these parameters,
because there is no possible way to infer them precisely.
The time dilation parameter $\beta$ reflects uncertainty in the
time scaling of the signal.
Aligning the signal with an ICH can
reduce (although not eliminate) this uncertainty as discussed later.
The other unknowns are the starting time $\tau$ and frequency offset $f_{1}$.
For a reception $r(t)$, during discovery \eqref{eq:simplemf} is replaced by
\begin{equation}
\label{eq:searchMF}
z(\tau, \beta , f_{1}) = \int r(t) \, \cc h ( \beta ( t - \tau ) )  e^{-\,i\,2 \pi f_1 t} \,,
\end{equation}
which calculates the MF for different values of $\tau$.
During the search the integral representing the MF must be repeated for different values of 
$\beta$ and $f_{1}$.
The baseband processing will typically operate with a signal of bandwidth
$N B$ for some large value of $N$, and use the fast Fourier transform
to simultaneously calculate a bank of MF outputs (for different $f_{1}$) over time (for different $\tau$).

One question is what granularity is necessary in searching these
three parameters, this relating directly to the computational burden.
The granularity of $\tau$ is, by the sampling theorem, $1/B$.
As discussed in Appendix \ref{sec:searchgranulatiry},
the required granularity of $\beta$ is on the order of one part in $1/K$, and the
granularity of $f_{1}$ is on the order of $1/T$.
In the following, fixed values for $\{ \beta , f_1 \}$ are used,
as if the receiver knew precisely what values to use.
Without loss of generality, \eqref{eq:searchMF} is specialized to $f_{1} = 0$ and $\beta = 1$.

\subsection{The matched filter as a least-squares solution}
\label{sec:LSsolution}

Several different optimization criteria lead to the MF, but
our favorite is the least-squares (LS) criterion because it uses an intuitively
pleasing approach that makes no assumptions whatsoever about the
nature of the impairments.
This illustrates that the MF is a reasonable detection technique even when
the AWGN assumption is not valid
(for example in the presence of
radio-frequency interference (RFI))
or that assumption is valid but the noise power density is uncertain.

Suppose the received signal with a known waveform $\{ h(t ) , \, 0 \le t \le T \}$ is expected 
but in the reception $r(t)$ it is delayed by some unknown $\tau$,
multiplied by some unknown complex-valued factor $z$
representing an unknown magnitude and phase, and
corrupted by noise, interference, etc,
\begin{equation}
\label{eq:receptionGeneral}
r(t) = z \cdot h(t - \tau) + \text{noise} + \text{interference} + \dots \,.
\end{equation}
Recall from \eqref{eq:unitenergy} that $h(t)$ has unit energy,
so the unknown amplitude (and signal energy) is incorporated into the value of $z$.
The LS solution seeks to produce an estimate $\hat z$ of
the complex-vaued amplitude and of $\hat \tau$ the real-valued time offset.
%For any $\tau$ for which the estimated amplitude $| \hat z |$ is below
%some threshold $\hht$, it is decided that in fact the signal $h(t)$ is not present.

The LS criterion to estimating the unknowns is to define a quality metric
that, for any parameters $\{ z , \tau \}$ measures the energy in the error between
reception $r(t)$ and $z \cdot h(t - \tau)$,
\begin{equation}
\label{eq:LS}
\varepsilon (z,\tau ) =
 \int_{\tau} ^{\tau  + T} {\left| \, r(t) - z \cdot h(t - \tau) \, \right|^2 } \, dt \,.
\end{equation}
Our strategy is to determine, for each $\tau$, the value $z = \hat z$ that minimizes
$\varepsilon (z,\tau )$.
This eliminates one of the unknowns, leaving a resulting LS error 
$\varepsilon_{\min} (\tau ) = \varepsilon (\hat z,\tau )$
that depends only on $\tau$.
It is shown in Appendix \ref{sec:lscriterion} that the resulting estimate and residual error are
\begin{align}
\label{eq:LSsolnZ}
&\hat z (\tau) =  \int_{\tau} ^{\tau  + T} \, r(t) \, \cc h (t - \tau) \, dt = r(\tau) \convolve \cc h (\tau)
 \\
\label{eq:LSsolnE}
&\varepsilon_{\min} (\tau ) =   \varepsilon (0,\tau ) - | \hat z (\tau) |^{2} 
\ge 0
\end{align}
where $\convolve$ is the convolution operator.
The estimate $\hat z (\tau)$ as a function of time can be generated by
a filter with impulse response $\cc h(-t)$, which is a filter
 matched to $h(t)$.
The size of $0 \le \varepsilon_{\min} (\tau ) \le  \varepsilon (0,\tau )$
is a direct indication of the goodness of the fit between $h(t)$ and $r(t)$.
For example, if $\varepsilon_{\min} (\tau ) \approx 0$, or equivalently
$| \hat z (\tau) |^{2} \approx \varepsilon (0,\tau )$, it follows that $r(t) \approx \hat z \, h(t - \tau)$.
The MF output as a function of $\tau$ checks that fit for different
values of $\tau$.

A convenient way to measure the goodness of the fit is to calculate the decision variable
\begin{equation}
\label{eq:normdv}
Q =  \frac{\ | \hat z (\tau) |^{2}}{ \varepsilon (0,\tau )} \,.
\end{equation}
Then $Q$ is normalized to range $0 \le Q \le 1$, where the
value $Q=1$ indicates that $r(t)$ is totally aligned with $h(t)$
and $Q = 0$ indicates that $r(t)$ is orthogonal to $h(t)$.
$Q$ can serve as the basis of a decision as to whether $h(t)$ is present or
absent by comparing it to a threshold $\lambda$,
where $Q > \lambda$ results in the decision that a signal is present.

%\begin{equation}
%0 \le Q = \frac{\varepsilon_{min} (\tau ) }{ \varepsilon (0,\tau )} \le 1 \,.
%\end{equation}
%$Q$ is a measure of how well $r(t)$ is faithful to $h(t)$
%modified by an appropriate phase and magnitude,
%ranging from $V = 0$ ($r(t)$ is orthogonal to $h(t)$) to $V = 1$
%($r(t)$ is totally aligned with $h(t)$).

\subsection{White Gaussian noise and scintillation}

Corrupted by this additive noise and the multiplicative noise of scintillation, 
and assuming without loss of generality that $\tau = 0$,
as discussed in Section \ref{sec:noiseICH} within a single ICH the reception can
be modeled as a random process $R(t)$, where
\begin{equation}
\label{eq:receptionNoise}
R(t) = \sqrt{\recenergy} \, \sqrt{\flux} \, e^{\,i\, \Phi} \, h(t) + M(t) \,,
\end{equation}
where $\recenergy$ is the unknown energy in the received signal
and $\flux$ is a random scintillation flux with variance $\vs$
(thus $z =  \sqrt{\recenergy} \,  \sqrt{\flux}$
in the LS formulation of Section \ref{sec:LSsolution}).
If $N(t)$ has power spectral density $N_{0}$, then it is shown in Section \ref{sec:noiseICH}
that the complex-valued $M(t)$ is also AWGN with power spectral density $N_{0}$,
with real and imaginary parts that are statistically independent
AWGN processes each with power spectral density $N_{0}/2$.

If the detection algorithm must
make a decision as to whether $R(t)$ is noise alone ($\recenergy = 0$) or signal plus noise ($\recenergy = 0$),
by any reasonable criterion
(such as an optimum tradeoff between $\pfa$ and $\pd$) the MF followed by
a sampler is the best front-end processing \citeref{43}.
This is consistent with the LS solution of Section \ref{sec:LSsolution}.
If $N_{0}$ is known,
the threshold $\lambda$ can be chosen to control the tradeoff between $\pfa$ and $\pd$.
However, a special challenge of interstellar communication is that it operates
in an astronomical environment where there are numerous source of noise
with a thermal character, including those that are known or controlled
(the cosmic background radiation and thermal noise in the receiver)
and those which are uncontrolled (stars and galaxies) \citeref{581}.
Of course there would be ways to estimate the value of $N_{0}$
for a given line of sight based on many observations at different times and frequencies.
However, to illustrate the power of detection based on the MF,
make the worst-case assumption that there is no a priori knowledge of $N_{0}$.

Not only is the noise power spectral density unknown, but also the signal
strength is unknown, both because $\recenergy$ is unknown and because of the
randomness of scintillation (represented by $S$).
As the LS solution makes clear, the MF is well able to deal with this circumstance,
but it does require a decision strategy tailored to this assumption.
For example, the decision variable \eqref{eq:normdv} simply captures how
large the estimated signal component is in relation to the noise, without
making any prior assumptions about the size of the noise.
If the noise happens to be larger, then the decision is automatically adjusted
to require a correspondingly larger signal to register in decision variable $Q$.

The properties of decision variable $Q$ in the presence of AWGN
as in \eqref{eq:receptionNoise} provides additional insight into the role of
$\recenergy$ and $N_{0}$, even where both parameters are unknown.
If $h(t)$ has bandwidth $B$ and time duration $T$, then as discussed
in Section \ref{sec:channelmodeldof} it has degrees of freedom $K$.
To study the properties of the MF in the presence of AWGN,
it is useful to expand $h(t)$ in terms of a set of $K$ orthonormal basis functions
$\{ g_{k} (t) , 1 \le k \le K \}$, where
\begin{equation}
\int_{0}^{T} g_{m} (t) \, \cc g_{n} (t) \, dt = \delta_{m-n} \,.
\end{equation}
It doesn't matter what $\{ g_{k} (t) , 1 \le k \le K \}$ are chosen, so for
convenience choose as the first basis function $g_{1} (t) = h(t)$,
and the remaining basis functions arbitrarily to fill out a complete orthonormal basis.
Then the reception $R(t)$ (restricted to bandwidth $B$ and time duration $T$)
 can be represented by a set of $K$ coefficients w.r.t. this basis,
\begin{equation}
\label{eq:receptionexpansion}
R_{k} = \int_{0}^{T} R (t) \, \cc g_{m} (t) \, dt
= \begin{cases}
\sqrt{\, \recenergy \, \flux \, } \, e^{\,i\,\Phi}  + M_{1} , & k=1 \\
M_{k} , & 2 \le k \le K \,.
\end{cases}
\end{equation}
The first coordinate $R_{1}$ is precisely the output of a filter matched to $h(t)$
sampled at time $t = 0$, and the remaining coordinates are noise-only.
The noise components $\{M_{k} , 1 \le k \le K \}$ are readily shown to
be statistically independent, and thus only $R_{1}$
(and not $\{R_{k} , \, 2 \le k \le K \}$) offers any information to inform
the decision as to whether $\recenergy = 0$ or $\recenergy > 0$.
This is the ''sufficient statistic'' observation behind the optimality of the MF.

What is notable about \eqref{eq:receptionexpansion} is the 
 concentration of signal energy in only one out of the total of $K$ coordinates.
This concentration is the signature of the presence of signal $h(t)$ within the
bandwidth $B$ and time duration $T$, and will be evident as long as
$\recenergy \gg N_{0}$, no matter what the specific values of
$\recenergy$, $\vs$, and $N_{0}$, during the periods when $\flux$ is relatively large.

The decision variable \eqref{eq:normdv}
was chosen specifically to account for the case where little is known about the
signal and noise strength.
So let's see what happens should \eqref{eq:normdv} be adopted for 
the received signal model of \eqref{eq:receptionNoise}.
$Q$ in \eqref{eq:normdv} can be written in terms of expansion \eqref{eq:receptionexpansion} as\footnote{
It is not necessary to compute the $\{R_{k} , 2 \le k \le K \}$)
in order to generate $Q$; rather, the denominator equals the total
energy in $R(t)$ which can be determined directly.}
\begin{equation}
\label{eq:QR1K}
Q = \frac{|R_{1} |^{2}}{\sum_{k=1}^{K} |R_{k} |^{2}} \,.
\end{equation}
If signal is declared for $Q > \lambda$ for some threshold $0 < \lambda < 1$,
then $\pfa$ and $\pd$ can be determined as a function of $\lambda$, and
then $\lambda$ eliminated to find the relationship between $\pfa$ and $\pd$.
The performance of this criterion is studied in Appendix \ref{sec:discprob}.
Closed-form results for $\pd$ and $\pd$ can be obtained for
strong scattering (see Appendix \ref{sec:discoveryrayleigh}), giving the relationship between them as
\begin{equation}
\label{eq:pdvspfa}
\displaystyle
\pd = \left( 
\frac{\ecrs + 1}{\ecrs+ \pfa^{\, \frac{1}{ 1-K}}} \,
\right)^{K-1}
\end{equation}
where $\ecrs$, the symbol energy contrast ratio, was defined in \eqref{eq:ecrs}.
Note that $\recenergy \, \vs$ and $N_{0}$ enter only through their
ratio in $\ecrs$, so the detection algorithm automatically adjusts to
 unknown values for $\recenergy$ and $N_{0}$.
It does this by implicitly estimating $N_{0}$ by examining the noise
within the ICH that fall in the $K-1$ coordinates that are absent signal,
and comparing the estimated noise energy to the total reception energy.
Decision variable \eqref{eq:normdv} thus proves effective in automatically adjusting
to the relative signal and noise strength without knowing either in advance.
For weak scattering such simple results as \eqref{eq:pdvspfa} are unattainable,
but it can be confirmed that discovery becomes easier (see Appendix \ref{sec:discoveryrician})
due to the presence of the deterministic specular component of flux.

The detection probability is plotted for a fixed $\pfa$ in Figure \ref{fig:detectionProbability},
as a function of $K$ and $\ecrs$.
The increasing $\pd$ with $K$ is because the estimate of $N_{0}$ built into \eqref{eq:normdv}
has increasing accuracy in estimating $N_{0}$ as there are more coordinates available to form the estimate.
While $\pd$ does increase monotonically with $K$, significantly it approaches
an asymptote of
\begin{equation}
\label{eq:asympPfaVsPd}
\pd \overset{K \to \infty}{\longrightarrow} \pfa^{\frac{1}{ 1+\ecrs}} <1 \,.
\end{equation}
Even $K \to \infty$ cannot achieve $\pd \approx 1$, except in the case where
$\ecrs \to \infty$.
$\pd$ is monotonically increasing with $\pfa$ as also shown in Figure \ref{fig:detectionProbability}.
The overall impression from Figure \ref{fig:detectionProbability} is that
the detection reliability is rather poor in spite of using the optimum MF.
This can be blamed on scintillation, which sometimes results in periods with a low signal strength,
and during such ''outage'' periods the detector invariably declares ''noise'',
thereby failing to declare ''signal''.
The way around this challenge is to make multiple observations,
which as shown in Section \ref{sec:beacondiscovery} can achieve $\pd \to 1$.

\incfig
	{detectionProbability}
	{.7}
	{A log-log plot of detection probability for different values of $\ecrs =$ 5, 10, 15, and 20 dB.
	Larger $\ecrs$ corresponds to larger $\pd$.
	On the top the horizontal axis is the degrees of freedom $K$ with a fixed
	$\pfa = 10^{-12}$, and on the bottom the horizontal axis is $\pfa$ asymptotically as
	$K \to \infty$.}

\subsection{Improved detectabiliy if the noise power is known}

If the noise power spectral density $N_{0}$ is known, then decision variable
\eqref{eq:QR1K} can be replaced by $Q = |R_{1}|^{2}$.
Because $N_{0}$ is known, the threshold $\lambda$ can be chosen
to control $\pfa$ without ambiguity.
Not surprisingly, the relationship for $\pd$ vs $\pfa$ becomes  (Appendix \ref{sec:discprob})
the same as the asymptotic result of \eqref{eq:asympPfaVsPd}.
This is because as $K \to \infty$ the implicit
estimate of $N_{0}$ built into \eqref{eq:QR1K} becomes perfectly accurate
(by the law of large numbers)
as $K$ increases.

\textbox
	{Do sinusoidal signals get too much respect?}
	{
In the presence of AWGN, it has been shown that the
tradeoff between $\pfa$ and $\pd$ does not depend on the
waveform of $h(t)$, nor on any of its parameters like $B$ and $T$.
This includes a continuous-wave signal like $h(t) = \sqrt{2/T} \cdot \sin ( 2 \pi f t )$,
which has a small $B T \approx 1$,
or a spread-spectrum signal with a large $B T$.
It is often said in the physics community that sinusoidal waveforms are special
in that they cannot be generated by natural processes, and thus are
in some sense easier to distinguish from natural sources of noise.
If the noise in question is of thermal origin,
\emph{any} deterministic waveform $h(t)$ with unit energy is distinguishable
from AWGN to the same degree.
This is even true of an $h(t)$ that is noise-like, as in spread spectrum.
The noise-like character is not relevant to discovery, as the receiver
is applying a filter matched to a very specific waveform $h(t)$,
and not estimating the statistics of $h(t)$.
As an aid to intuition on this significant point,
Appendix \ref{sec:cointossing} describes an analogy to noise generated by random coin tosses,
which is easier to understand but displays the same characteristics.

The sinusoidal signal and its close cousin the high-bandwidth pulse has one advantage,
which is that signals with $B T \approx 1$ require one fewer dimension of search.
When $B T \gg 1$ a discovery search is forced to search over different values of $B$
or different values of $T$ (fortunately not both) with a fine granularity.
Our suggestion here is to narrow the range of that search substantially based
on a physical parameter observable by both transmitter and receiver, 
either the coherence bandwidth 
or the coherence time for the given line of sight and carrier frequency.
	}

\section{Choice of $h(t)$}

The receiver is presumed to use a MF for detection, and thus it is important to
choose an $h(t)$ that is relatively easy for the receiver to guess.
Our design is tailored to a specific line of sight and $f_{c}$, which in turn influences the size of the ICH.
This places a restriction on 
$B \le B_{c}$ and $T \le T_{c}$, and $K = B T$
for the chosen waveform $h(t)$,
but within these constraints any $B$ and $T$ can be chosen.
In terms of noise and scintillation, $h(t)$ does not matter,
but larger $K$ results in larger immunity to RFI sources in the vicinity of the receiver \citeref{211}.
For this reason, and also because a larger $T$ results in smaller peak transmitted power,
it is favorable to choose $B = B_{c}$ and $T = T_{c}$.
Given the inevitable uncertainty, the smallest credible values of $B_{c}$ and $T_{c}$ should be used.
To yield a peak power equal to the average power (its lowest possible value), 
the rate at which IU's are transmitted for a single
carrier is chosen to be $1 / T_{c}$, with MCM used if the $\power$
necessary to support higher information rates is available.
The choice of $B = B_{c}$ also constrains the minimum distance between carriers in a multicarrier signal.
In this fashion, the basic parameters of the IU structure of the signal are predetermined,
thereby restricting the receiver's search space during discovery to the range of its uncertainty
as to the size of an ICH.

The actual waveform used for $h(t)$ does not affect the power efficiency, so
as discussed in Section \ref{sec:rfi} the choice of $h(t)$ is strictly
an issue of RFI immunity and using a waveform that can be guessed at the receiver.
As argued in Section  \ref{sec:rfi} and in \citeref{211}, a readily guessable choice is based on a pseudorandom
sequence generated by the binary expansion of $\pi$.
As described in \citeref{211},  $h(t)$ is generated as a quadrature phase-shift keying (QPSK) signal 
(the lowest complexity meeting the requirement for statistical independence of the
real- and imaginary parts), two successive bits from $\pi$ can be mapped
onto a complex amplitude chosen from four QPSK points at rate $B_{c}$.
The resulting waveform $h(t)$ takes the concrete form
\begin{equation}
h(t) = \frac{1}{\sqrt{K}} \, \sum_{k=0}^{K_{c}-1} c_{k} \, g(t - k / B_{c}) \,,
\end{equation}
where each $c_{k} = (2 b_{k} -1) + i \, (2 b_{k+1} - 1)$ is chosen using two successive bits $\{ b_{k}, b_{k+1} \}$
from the binary expansion of $\pi$.
For example, the first 30 digits of $\pi$ equal
\begin{equation}
\{ b_{k} , \, 1 \le k \le 30 \} =
\{1,1,0,0,1,0,0,1,0,0,0,0,1,1,1,1,1,1,0,1,1,0,1,0,1,0,1,0,0,0\}\,,
\end{equation}
resulting in
\begin{equation}
\{ c_{k} , \, 1 \le k \le 15 \} =
\{1+i,0,1,i,0,0,1+i,1+i,1+i,i,1,1,1,1,0\} \,.
\end{equation}
The \emph{chip waveform} $g(t)$ is a sampling interpolation function
(and thus $g(0)=1$) for sampling rate $B_{c}$,
and the match between transmitter and receiver is non-critical.
Due to the embedded properties of the $\{ b_{k} \}$ sequence, the receiver is permitted to use
a different $K= K_{r}$ from the transmitter with some loss of signal energy if $K_{r} < K_{c}$,
or some unnecessary noise if $K_{r} > K_{c}$.

As an alternative, the simple sine wave or pulse could be used.
A sinusoid is especially attractive if the receiver designers are expected to
be astronomers or experimental physicists rather than communication engineers,
as spectral analysis is a familiar form of scientific inquiry
in many sub-disciplines of astronomy, physics, and chemistry.
The use of a short pulse as described in \citeref{578} is not attractive in our
transmitter design because it results in a high peak-to-average power ratio,
and this is hard to achieve at radio frequencies without an
increase in the capital cost of building the transmitter.

\section{Radio-frequency interference}
\label{sec:rfi}

\comment{Section needs some rework. The problem is that
a single above threshold-event may be caused by a transient
RFI signal. RFI is more difficult to deal with for 
low-duty cycle beacons. Spread spectrum can help rule this out.}

The specific waveform $h(t)$ has no effect on $\pfa$ and $\pd$
(as long as $h(t)$ is assumed to have unit energy).
However, the shape of $h(t)$ 
is a significant factor in the immunity to radio-frequency interference (RFI) that may be present
in the vicinity of the receiver \citeref{211}.
This is because RFI too is processed by the MF, and thus
is affected by the MF impulse response $\cc h (-t)$.
This is fortunate, since it provides a point of implicit coordination
between the designers of transmitter and receiver \citeref{583}.
The proper choice of $h(t)$ for RFI immunity meets statistical tests for a burst of
 AWGN limited to time $t \in [0,T]$ and with a power spectral density
 that is constant over frequencies $f \in [0,B]$.
 This results in an energy for $h(t)$ that is spread uniformly over  $t \in [0,T]$  and  $f \in [0,B]$.
 Intuitively it is this uniform spreading that contributes to the robustness of RFI immunity,
 since there is no identifiable place where the energy in $h(t)$ is concentrated;
 any such concentration would make $h(t)$ more
 susceptible to RFI concentrated in that same region.
  This technique, called spread-spectrum, is a common element of most terrestrial wireless standards.
 As an aid to intuition,
 in Appendix \ref{sec:cointossing} the analogy to a discrete-time version of $h(t)$ generated by a pseudo-random coin toss generator is discussed.
 
 The least-desirable choices of $h(t)$ from a RFI immunity perspective are
 highly concentrated in time (a broadband pulse) or in frequency (a sinusoid),
 since those choices for $h(t)$ are highly susceptible to RFI having similar concentration.
 These happen to be the $h(t)$ choices 
 of past SETI searches \citereftwo{142}{605}.
 As already discussed, those searches typically rely on a repeated-observation
 strategy to minimize the effects of RFI.
 Since that strategy relies on continuous transmission, it will not be effective
 in the low-power regime where the transmitter is 
 transmitting with a low duty cycle.
 Thus, the benefits of spread spectrum are considerably magnified in
 the low-power regime.
 
 Further information about appropriate choices of $h(t)$ follow from
 practical considerations  \citeref{211} like the feasibility of guessing $h(t)$ at the receiver
 (dictating algorithmically-generated pseudo-random waveforms),
 and Occam's razor (a four-level QPSK signal is the minimum-complexity signal that
 meets the randomness requirements).
 In the current context, a critical requirement is embedding, in which a shorter-length
 pseudo-random sequence must be the precursor to a longer sequence,
 eliminating one entire dimension of discovery search for the receiver.
 Either a search over $B$ is required (using a fixed $K$ and hence a variable $T = K/B$),
 or a search over $T$ is required (using a fixed $K$ and hence a variable $B = K/T$).
 In both cases, detection sensitivity is improved if some different values of $K$ are
 tried, but a relatively coarse granularity is sufficient.
 The choice between these two options might be governed by the estimated
 uncertainty in $B_{c}$ vs that in $T_{c}$.
 
 From a communication engineering perspective,
 where RFI would be taken seriously,
 these collective requirements
 on $h(t)$ leave very little ambiguity in the choice of $h(t)$.
 The embedding property is particularly powerful in reducing the
 number of options.
 Fortunately, a pseudo-random generator based on a binary expansion of
 an irrational number like $\pi$, $\sqrt{2}$, or $e$ meets all the requirements,
 and it is difficult to conceive of other choices that might be as readily guessed
 by a receiver designer.
 
Another relevant result \citeref{211} is that interference immunity increases with $K$.
There are two motivations, therefore, for using an $h(t)$ that distributes its energy
uniformly over an entire ICH, or $K = K_{c}$.
This maximizes interference immunity, or the attenuation of
interference by the MF.
This also ties all the parameters $\{ B, T, K \}$ to physical quantities that can be
observed by both transmitter and receiver designers, considerably reducing the search space
in a discovery search.
Reducing the search space reduces computational burden, but more importantly
reduces the potential for false alarms.


\chapter{Sources of time and frequency incoherence}
\label{sec:incoherence}

In Chapter \ref{sec:channelmodel} the impairments introduced in the ISM
and due to source/observer motion were divided into Category I and II,
and Category II impairments which are fundamental to interstellar
communication were modeled.
Now it is appropriate to address those Category I impairments.
The objective is not to model them in detail as is often the goal
in the physics literature, but rather to convince ourselves that they
are mitigated by limiting the bandwidth $B$ or time duration $T$
of an elemental signal $h(t)$ after propagation and matched filtering,
and to quantify the approximate coherence bandwidth $B_{c}$ and coherence time $T_{c}$.
One objective is to establish that interstellar communication carried
out in the manner of earlier sections is feasible, which requires that $K_{c} = B_{c} T_{c} \gg 1$.

When the impairments are considered individually, two distinctive forms of incoherence are encountered:
\begin{description}
\item[Frequency incoherence.]
In the presence of the impairment, the overall effect is linear and time-invariant,
and thus can be equivalently modeled in the frequency domain.
However, there is a frequency-dependent change in amplitude or phase
that causes a distortion of the signal.
This effect can be mitigated by reducing the bandwidth of the signal
until the distortion becomes insignificant.
\item[Time incoherence.]
In the presence of the impairment, the effect varies with time, and thus
frequency-domain modeling is not useful.
However, the effect can be mitigated by reducing the time duration of the signal
until the distortion becomes insignificant.
\end{description}
The impairments encountered here cause either a frequency-dependent
or time-dependent phase shift.
Our criterion for coherence is when the magnitude of the phase change is
less than $\alpha \, \pi$ for a parameter $0 \le \alpha \le 1$.
Choosing $\alpha$ smaller makes the criterion more strict.
At the limits of incoherence, there is generally both time and
frequency incoherence with additive phases, so the maximum
value $\alpha = 0.5$ insures that the total phase shift is
at most $\pi$.
The appropriate value of $\alpha$ depends on the
use to which the ICH is put, and the impact of incoherence on that use.
in all numerical examples, the conservative choice of $\alpha = 0.1$ is assumed.
The coherence bandwidth $B_c$ and coherence time $T_c$
are defined by the most stringent of the conditions that arise across all impairments.

\section{Plasma dispersion}
\label{sec:dispersion}

Although it approaches an ideal vacuum, the ISM contains an extremely low-density 
plasma consisting of hydrogen ions and free electrons 
arising from the presence of hydrogen gas and ionizing radiation from the stars \citeref{213}.
The charged particles create a conductive medium that influences radio waves 
propagating over long distances.
This results in plasma dispersion, a frequency-dependent
group delay due to the free electons' lossless absorption and wavelength-dependent delayed emission of photons.

A model for dispersion used in pulsar astronomy \citeref{212}
is a frequency-dependent group delay $\tau (f)$.
Let the transfer function at passband be
\begin{equation}
\label{eq:passbanddispersiontf}
G(f) = e^{\,i\, 2 \pi \, \phi (f)}
\end{equation}
so that there is a phase shift $\phi (f)$ with no effect on signal magnitude.
The group delay $\tau(f)$ and $\phi(f)$ are related by
\begin{equation}
\label{eq:delayFromPhase}
\tau (f) = - \frac{1}{2 \pi} \cdot  \frac{\partial \phi (f)}{\partial f} \,.
\end{equation}
The standard model used in pulsar astronomy is \citeref{212}
\begin{equation}
\tau(f) = \frac{\dc \, \dm}{f^{2}}
\end{equation}
As illustrated in Figure \ref{fig:delayAndPhase},
$\tau(f)$ decreases monotonically (and approximately linearly) with $f$.
While \emph{dispersion constant}
$\dc \approx 4.15 \times 10^{15}$ 
depends only on known physical constants
(and has units of $\text{Hz}^2 \ \text{pc}^{-1} \ \text{cm}^{3} \ \text{s}$),
the \emph{dispersion measure} $\dm$
summarizes all that needs to be known about
the current interstellar ''weather'' in order to predict the group delay profile for a given
direction of arrival (and has units of $\text{cm}^{-3} \ \text{pc}$).
Typically $\dm$ ranges over about two orders of magnitude, from about 10 to about 1000,
depending on the average electron density along the line of sight.

\incfig
	{delayAndPhase}
	{1}
	{
	The dispersive group delay $ \tau(f)$ in msec
	(with $\tau_0$ chosen so that $\tau(B)=0$)  and resulting unwrapped phase
	$\phi(f)/2 \pi$ (with $\phi(f)$ in radians and $\phi_0=0$) 
	plotted against baseband frequency $f$ for
	$f_{c} = 1$ GHz, $B = 1$ MHz,
	and $\dm = 100$ $\text{cm}^{-3} \ \text{pc}$.
	The phase experiences more than 400 rotations across the bandwidth, and this
	phase variation will increase with 
	$\dm\uparrow$, $B\uparrow$, or $f_{c}\downarrow$.
	}

The ICH test is shown in Figure \ref{fig:dispersion}.
Over the frequency range $f \in [f_{c}, f_{c} + B]$, if $B$ is kept small
enough $\phi (f)$ can be modeled by a linear dependence on $f$,
\begin{equation}
\label{eq:appxphase}
\phi (f) \approx \phi (f_{c}) - \tau (f_{c}) \cdot f
\end{equation}
which corresponds to an unknown phase $\phi (f_{c})$ plus a
fixed (not frequency-dependent) group delay $\tau (f_{c})$.
If the deviation of the actual $\phi (f)$ from \eqref{eq:appxphase}
is less than $\alpha \, \pi$ radians over the entire range $f \in [f_{c}, f_{c} + B]$
then the distortion of $h(t)$ due to nonlinear phase can be neglected.

It is shown in Appendix \ref{sec:plasmaappx} that 
approximation \eqref{eq:appxphase} is accurate within $\alpha \, \pi$ radians when
\begin{equation}
\label{eq:dispersioncoherencebandwidth}
B <  B_{0} = \rho \, f_{c}^{\, 3/2}
\ \ \ \text{for} \ \ \ \ 
\rho
= \sqrt{\frac{\alpha}{2 \, \dc \, \dm}} \,.
\end{equation}
As illustrated in Figure \ref{fig:noDispersion}, $B_{0}$
decreases (dispersion becomes more severe) as $\dm$ increases
or $f_c$ decreases.
The value of $B_{0}$ varies over about four orders of magnitude for the parameters shown.
The line of sight ''weather conditions'' also influence $B_{0}$ through the $\sqrt{\dm}$ term in $\rho$.

\incxy
	[@C=10pt] % Change default spacing
	{dispersion}
	{
	A model for plasma dispersion within an ICH.
	At passband (top diagram) the effect is a frequency-dependent group delay
	$\tau (f)$.
	The bottom baseband model results when approximation \eqref{eq:appxphase} is applied,
	 the resulting passband filter is referred to baseband,
	 and then the order of the dispersion and matched filters is reversed.
	}
	{
 	h(t) \ar@{=>}[r] &
	*{\bigotimes} \ar@{=>}[r]^<<<<<{\displaystyle x(t)} &
	*+<1pc>[F-,]{
	\begin{matrix}
	\text{Group delay} \\
	\displaystyle \tau(f)
	\end{matrix}
	} \ar@{=>}[r]^>>>>>{\displaystyle y(t)} &
	*{\bigotimes} \ar@{=>}[r] &
	*+<1pc>[F-,]{\cc h(-  t)} \ar@{=>}[r] & 
	z(t)
	\\
	& \displaystyle e^{\, i \, ( 2 \pi \, f_{c} \, t + \theta)} \ar@{=>}[u] &&
	\displaystyle e^{ - \, i \, 2 \pi \, f_{c} \, t } \ar@{=>}[u] \\
	R_{h} (t) \ar@{=>}[rr] &&
	*+<1pc>[F-,]{
	\begin{matrix}
	\text{Phase} \\
	\displaystyle \theta + \phi(f_{c})
	\end{matrix}
	} \ar@{=>}[r]&
	*+<1pc>[F-,]{
	\begin{matrix}
	\text{Delay} \\
	\displaystyle \tau(f_{c})
	\end{matrix}
	} \ar@{=>}[rr]&&
	z(t)
	}

\incfig
	{noDispersion}
	{1}
	{
	A log-log plot of the coherence bandwidth
	$B_{0}$ of \eqref{eq:dispersioncoherencebandwidth} in kHz 
	vs carrier frequency $f_c$ in GHz for low,
	moderate, and severe dispersion.
	A stricter ($\alpha = 1/10$) criterion for coherence is used.
	}

The baseband model for dispersion when \eqref{eq:dispersioncoherencebandwidth} is satisfied
is illustrated in Figure \ref{fig:dispersion}.
The result is the phase shift $\phi (f_{0})$ which is unknown and
added to unknown carrier phase $\theta$ together with a
baseband delay equal to the plasma dispersion delay at the carrier frequency
$\tau (f_{c})$.
In the time domain, this model becomes
\begin{equation}
|z(t)| \approx  \left| R_{h} ( t - \tau (f_{c}) ) \right| \,.
\end{equation}
The phase shift does not affect $|z(t)|$, and 
flat delay $\tau (f_{c})$ can be neglected since it is added to an already-large
and unknown propagation delay.
When $B > B_{0}$, however,
 the MF output becomes smeared over time and, as a result reduced in amplitude.
This is illustrated in Figure \ref{fig:IRvsB}, where the effect of dispersion on
$R_{h} (t)$ as in Figure \ref{fig:dispersion} is illustrated for different values of $B$.
Violating  \eqref{eq:dispersioncoherencebandwidth}
reduces the sensitivity of a detector that depends on the statistic $|z(0)|$.

\incfig
 	{IRvsB}
	{.8}
	{The response $z(t)$ to input $R_{h} (t)$ in Figure \ref{fig:dispersion}
	shown for difference values of $B$.
	The parameters are the same as Figure \ref{fig:delayAndPhase}
	except the bandwidth is much smaller ($B$
	satisfying  \eqref{eq:dispersioncoherencebandwidth} is 34.7 kHz).
	Plotted is magnitude $| f(t) \convolve R_h (t) |$ (but not phase) for different
	values of $B$ ranging from $B = 0.3 \, B_0$ to $B = 10 \, B_0$.
	For $B < B_0$ the pulse broadens due to reduced bandwidth
	rather than dispersion.
	For $B > B_0$ the pulse is smeared out in time
	and reduced in magnitude.
	The effect of dispersion at $B = B_0$ in terms of smearing
	and magnitude reduction is visible but 
	has no material effect on $|z(0)|$.}


There is an alternative interpretation of \eqref{eq:dispersioncoherencebandwidth}
that  lends additional insight,
and follows the convention in wireless communications \citeref{574}
of focusing on group delay rather than phase.
The effect of
$B \gg B_0$ can be observed in the impulse response of the dispersion,
which is illustrated in Figure \ref{fig:impulseResponse} for the same
parameters as Figure \ref{fig:delayAndPhase}.
After removing the smallest fixed band-edge group delay $\tau (f_{c}+B)$,
the remaining group delay is approximately distributed
uniformly through $[ 0, \tau_s]$.
Thus the magnitude of the impulse response is approximately spread uniformly
over time $[ 0, \tau_s]$, where $\tau_{s}$ is called the \emph{delay spread},
defined as the range of group delays across the bandwidth
\begin{equation}
\label{eq:delayspread}
\tau_{s} = \tau (f_{c}) - \tau(f_{c} + B)
 \,.
\end{equation}
The phase, however, is chaotic and very sensitive to $\dm$.
Delay spread $\tau_{s}$ is a measure of how much the dispersion increases the time duration of a signal.
It is easily shown that
\begin{equation}
B \, \tau_s = \left( \frac{B}{B_0} \right)^2
\ \ \ \text{for} \ \ \ \
\alpha = 1
 \,.
\end{equation}
This is strikingly similar to \eqref{eq:delaycbw} because
$B_{0} \tau_{s} = 1$.
A coherence bandwidth defined as the inverse of the delay spread
is a fundamental characteristic of wireless propagation \citeref{574}.
	
\incfig
	{impulseResponse}
	{1}
	{
	The magnitude and phase of the dispersive impulse response $f(t)$ for the
	 $F(f)$ illustrated in Figure \ref{fig:delayAndPhase}
	 after bandlimiting to $f \in [0,B]$.
	The magnitude is roughly uniformly spread between 0 and $0.83$ msec,
	corresponding to a delay spread $\tau_s =0.83$ from \eqref{eq:delayspread}.
	The oscillations and non-causality in $| f(t) |$ are caused by 
	ideal band limiting of the impulse response rather than dispersion,
	whereas the rapidly varying phase 
	(reflecting the 1 MHz bandwidth) is due primarily to dispersion.
	}

There are two related issues related to transmitter/receiver coordination
that are addressed in Appendix \ref{sec:equalization}.
First, based on pulsar observations both the transmitter and receiver can estimate $\dm$ along the line-of-sight.
However, both estimates have some uncertainty, both individually and jointly.
Second, it is possible for either the transmitter or the receiver to equalize
the dispersion, presumably for the lowest $\dm$ estimate.
Either may do this because they motivated to increase the worst-case
coherence bandwidth $B_{0}$, which is dominated by the highest $\dm$ estimate
(possibly reduced by the equalization of the lowest $\dm$ estimate).
This has implications for the receiver strategy in estimating a value for $B_{0}$ to inform
its search strategy.

\section{Source/observer motion}
\label{sec:doppler}

Source-observer motion is potentially an important source
of impairment in the form of Doppler shifts in frequency,
time dilation, and fading.
Although elementary physics texts describe motion effects in terms of
a shift in frequency, this is a monochromatic approximation and the
effect on finite-bandwidth signals is more complicated.
This is now modeled, making the simplification that the
velocities are low relative to the speed of light so that
relativistic effects can be neglected.

\subsection{Effect of time-varying distance and passband signals}

Assume that the distance between source and observer
parallel the line of sight is a function of time $d_{\parallel} (t)$.
This time-varying distance results in a time-varying group
delay $d_{\parallel} (t) / c$, where $c$ is the free-space speed of light.
The effect of this delay on a passband signal of the form of \eqref{sec:passbandsignal} is
\begin{equation}
y(t) = 
\Re \left\{
\exp \left\{ \,i\, 2 \pi \, f_{c} \left( t - \frac{d_{\parallel} (t)}{c} \right)  \right\}
\cdot h \left( t - \frac{d_{\parallel} (t)}{c} \right)
\right\}
\end{equation}
Thus, the equivalent complex-valued baseband signal is
\begin{equation}
\label{eq:dopplerbaseband}
\exp \left( - \,i\, 2 \pi \, \frac{d_{\parallel} (t)}{\lambda_{c}} \right)
\cdot h \left( t - \frac{d_{\parallel} (t)}{c} \right) \,.
\end{equation}
There are two effects.
\begin{description}
\item[Time incoherence.] 
A time-varying phase shift due to the effect of velocity on the carrier
is negligible if $T$ is sufficiently small.
The total change in phase will be less than $\alpha \pi$ if $T$ satisfies
\begin{equation}
\label{eq:tccarrier}
\frac{d_{\parallel} (t+T) - d_{\parallel} (t) }{\lambda_{c}} \ll \frac{\alpha}{2} \,.
\end{equation}
\item[Frequency incoherence.]
There is a time-varying group delay experienced by the baseband waveform $h(t)$,
which is potentially a source of frequency incoherence.
However, when $T$ satisfies \eqref{eq:tccarrier},
this effect is negligible because
the corresponding delay spread affecting $h(t)$ is
\begin{equation}
\tau_{s} =
\frac{d_{\parallel} (t+T) - d_{\parallel} (tT) }{c} \ll \frac{\alpha}{2 \, f_{c}} \,.
\end{equation}
Since it will always be true that $B \ll f_{c}$,
it follows that $2 B \tau_{s} \ll \alpha \, B / f_{c} \ll 1$ and thus by the criterion of \eqref{eq:delaycbw}
the delay spread can be neglected.
\end{description}
The condition on coherence time \eqref{eq:tccarrier} will now be investigated
for typical motion scenarios.

\subsection{Constant velocity}

Any constant delay term in $d_{\parallel} (t)$ can be ignored
as a fixed phase shift.
It is also possible to neglect any constant velocity term in $d_{\parallel} (t)$
within a given ICH, but not necessarily for different ICH's.
To see why, assume that $d_{\parallel} (t)$ represents a fixed velocity, or
$d_{\parallel} (t) = v_{\parallel} t$, over the time interval $[0,T]$
corresponding to a single ICH.
Then the baseband signal over that interval is
\begin{equation}
\exp \left( - \,i\, 2 \pi \, \frac{v_{\parallel}}{\lambda_{c}} \, t \right)
\cdot h \left( t \left( 1 - \frac{v_{\parallel}}{c} \right) \right)
\end{equation}
The effect is a frequency shift of $v_{\parallel} / \lambda_{c}$ and
a time dilation of $h( \cdot )$.
Neither effect is significant because the receiver has no absolute reference
for either the carrier frequency or the time dilation, as both these parameters
are fixed by the transmitter.

On the other hand, suppose that two ICH's experience different
velocities, $v_1$ and $v_2$. Then the frequency offsets and time dilations
are different for the two ICH's.
Clearly this cannot be ignored when a receiver is, for example,
doing pattern matching on energy bundles across time.

The foregoing applies to the component of velocity parallel to the line of sight $v_{\parallel}$.
In contrast,
the velocity transverse to the line of sight $v_{\bot}$ is the direct cause
of fading, which is the time variation component of scintillation.
This material effect is considered in Section \ref{sec:fading}.

\subsection{Diurnal rotation and orbital motion}

While two solar systems may have a substantial relative velocity,
we have seen that this results in a carrier frequency offset and 
time dilation of $h(t)$ that cannot be distinguished from parameter choices
made by the transmitter.
Generally the only germaine origin of \emph{variation}
in velocity is the diurnal rotation of a planet about its axis
and its orbital motion about its host star.
Of course both the transmitter and receiver will typically contribute to
these effects, unless either locates its equipment on a spacecraft.

To qualitatively understand the effect this has on the baseband signal,
the effects due to rotation and orbital motion at transmitter and at receiver
will be considered separately.
Also make the simplification that the motion is circular and
the worst-case assumption that it falls in a plane containing the line of sight.
The time-variation of distance for a simple circular motion is
\begin{equation}
d_{\parallel} (t) = R \cdot \sin \left( 2 \pi \, \frac{t}{P} \right)
\end{equation}
where $R$ is the radius of the circular motion and $P$ is the period.
Approximate values for these parameters for Earth are give in Table \ref{tbl:ctaccel}.

Consider one ICH extending over time interval $t \in [ t_1, t_1 + T ]$.
Assuming the distance change is small over this interval,
a Taylor series expansion of the distance 
about $t = t_1$ yields
\begin{align}
d_{\parallel} (t) =&
R \,  \sin \left(\frac{2 \pi  t_1}{P}\right) +
\frac{2 \pi \, R \, (t-t_1) \, \cos \left(\frac{2 \pi t_1}{P}\right)}{P} -
\frac{2 \pi ^2 \, R \,  (t-t_1)^2 \, \sin \left(\frac{2 \pi t_1}{P}\right)}{P^{\,2}} \\
&-
\frac{4 \pi ^3 \, R (t-t_1)^3 \, \cos \left(\frac{2 \pi t_1}{P}\right)}{3 \, P^{\,3}} +
\, \dots \, + \,.
\end{align}
The first term can be neglected since there are
other sources of unknown fixed phase, including carrier phase and scintillation.
The next term is a constant velocity, which can be neglected within
a single ICH.
However, it will cause a differential shift in frequency across different ICH's,
with a frequency shift as large as
\begin{equation}
 | \Delta f | \le \frac{4 \pi \, R}{\lambda_c \, P} \,.
\end{equation}
From Table \ref{tbl:ctaccel}, $ | \Delta f | $ is larger for orbital motion,
and increases in proportion to $f_{c}$.
However, the frequency shift will be much smaller over time scales short
relative to $P$ (one day or one year).

Within an ICH, the most significant source of impairment is the acceleration term $(t-t_0)^{2}$.
This is potentially a significant source of time incoherence, but one that
can be rendered negligible by choosing
$T$ sufficiently small.
A maximum phase shift less than $\alpha \pi$ determines
\begin{equation}
\label{eq:dopplercoherence}
\frac{2 \pi^{2} \, R \, T^{2}}{\lambda_{c} \, P^{2}} \ll \frac{\alpha}{2}
\ \ \ \text{or} \ \ \ \ 
T \ll \frac{P}{2 \pi} \cdot \sqrt{\, \frac{\alpha \, \lambda_{c}}{R} \, }
\end{equation}
From Table \ref{tbl:ctaccel},
the coherence time $T$ of the ICH decreases as $f_{c}^{\,-1/2}$, and acceleration becomes
an increasingly significant phenomenon for larger $f_{c}$.
The resulting coherence times are plotted as a function of $f_{c}$ in Figure \ref{fig:coherenceTimeAccel}.

\doctable
	{\small}
	{ctaccel}
	{The approximate radius $R$ and period $P$ for Earth
	and the resulting coherence time $T_{c}$ and frequency shift $\Delta f_{c}$, where
	$f_{\text{GHz}}$ is the carrier frequency in GHz.
	Since many planets or moons may have a smaller radius or shorter period,
	a safety factor of $\alpha = 1/100$ on the maximum phase shift is assumed
	in calculating $T$.
	}
	{l c c c}
	{
	\textbf{Case} & \textbf{Parameter} & \textbf{Coherence time} & \textbf{Frequency shift} \\
	\toprule
	\addlinespace[3pt]
	Diurnal rotation & $R = 6.39 \times 10^{6}$ m \\
	& $P = 8.6 \times 10^{4}$ sec & $T \ \text{sec} = 3 \, f_{\text{GHz}}^{\,- 1/2}$
	& $| \Delta f | \ \text{kHz} = 3 \, f_{\text{GHz}} $
	\\
	\cmidrule{1-4}
	Orbital motion & $R = 1.5 \times 10^{11}$ m \\
	& $P = 3.15 \times 10^{7}$ sec & $T \ \text{sec} = 7 \, f_{\text{GHz}}^{\,- 1/2}$
	& $| \Delta f |  \ \text{kHz}  = 200 \,f_{\text{GHz}}$
	\\
	\addlinespace[3pt]
	\bottomrule
	}
	
\incfig
	{coherenceTimeAccel}
	{.8}
	{The coherence time $T$ corresponding to
	the dynamics of Earth with an additional safety factor of $\alpha = 1/100$
	using the formulas from Table \ref{tbl:ctaccel}.}

%\comment{Left over}
%To address the effects of motion, the ICH test of
%Figure \ref{fig:ICHidea} can be relaxed
%as shown in Figure \ref{fig:coherenceholetest}
%to allow static carrier frequency offset $\ecrb$ frequency offset and time dilation $\beta$.
%Permitting both these effects
%is benign since there is no absolute frequency reference and signal time scale.
%
%\incxy
%	[@C=.4cm] 
%	{coherenceholetest}
%	{
%	To account for some benign effects due to Doppler,
%	the test for a coherence hole of Figure \ref{ICHidea} needs to be modified.
%	The receiver demodulation is allowed to use a frequency offset $\ecrb \ne 0$
%	in the demodulation and to use a time dilation $\delta$ in
%	is matched filter.
%	In practice, during discovery the receiver must
%	search over different carrier frequencies and time dilations so
%	this happens naturally.
%	The accuracy required for these parameters is an issue in receiver design
%	rather than ICH modeling, and is considered in Section \ref{sec:searchgranulatiry}.
%	}
%	{
% 	h(t) \ar@{=>}[r] 
%	&
%	*{\bigotimes} \ar@{=>}[r]^<<<<<{\displaystyle x(t)} 
%	&
%	*+<1pc>[F-,]{
%	\begin{matrix}
%	\text{ISM} \\
%	\text{model}
%	\end{matrix}
%	} \ar@{=>}[r]^>>>>>{\displaystyle y(t)} 
%	&
%	*{\bigotimes} \ar@{=>}[r] 
%	&
%	*+<1pc>[F-,]{\begin{matrix}\text{LPF} \\ f \in [0,B] \end{matrix}} \ar@{=>}[r] 
%	&
%	*+<1pc>[F-,]{\begin{matrix}\text{MF} \\ \cc h ( -(1 + \delta) \, t) \end{matrix}} \ar@{=>}[r] 
%	&
%	z(t)
%	\\
%	& 
%	\displaystyle e^{\, i \, ( 2 \pi \, f_{c} t + \theta)} \ar@{=>}[u] 
%	&&
%	\displaystyle e^{ - \, i \, 2 \pi \, (1 + \ecrb) \, f_{c} \, t } \ar@{=>}[u]
%	}
%
%Doppler due to the relative motion of transmitter and receiver
%compromises time coherence if $T$ is too large, but has an insignificant
%effect on frequency coherence.
%When there is relative motion,
% the distance from the source to receiver $d(t)$ is a function of time.
%Neglecting relativistic effects,
%the propagation delay is $\tau (t) = d(t)/c$ where $c$ is the speed of light.
%Since a large fixed delay is not a concern,
%for convenience choose $d(0) = 0$
%and ask how $\tau (t)$ affects the received signal over $t \in [0,T]$.
%Also, we consider only the components of velocity $v_{\parallel}$
%and acceleration $a_{\parallel}$ that are parallel to the line of sight.
%The transverse component of velocity $v_{\bot}$ is also
%significant in the context of fading in Section \ref{sec:fading}.
%The distance can be approximated by the first two terms in a Taylor series,
%\begin{equation}
%d(t) = v_{\parallel} \, t + \frac{1}{2} \, a_{\parallel} \, t^{\,2} \,.
%\end{equation}
%The resulting passband model is shown in Figure \ref{fig:passbanddoppler}.
%
%As shown in Appendix \ref{sec:doppleranalysis},
%the $\delta$ and $\ecrb$ in Figure \ref{fig:coherenceholetest} represent more
%than a receiver ''mistuning'' in the case of Dopper.
%They are actually important corrections for Doppler effects, and they happen
%automatically in a search over carrier frequency and time dilation.
%When
%\begin{equation}
%\label{eq:judiciousparam}
%\delta = \ecrb = - \frac{v_{\parallel}}{c} \,,
%\end{equation}
%the simple baseband model shown in Figure \ref{fig:passbanddoppler} results.
%
%\incxy
%	{passbanddoppler}
%	{
%	A model for Doppler shift due to velocity $v_{\parallel}$ and acceleration $a_{\parallel}$ at passband (above)
%	and baseband (below).
%	The baseband model assumes that the receiver has made a judicious choice of
%	parameters $\delta$ and $\ecrb$.
%	By choosing $B$ and $T$ sufficiently small, the effects of delay and phase
%	in the baseband model can be rendered insignificant.
%	}
%	{
% 	h(t) \ar@{=>}[r] &
%	*{\bigotimes} \ar@{=>}[r]^<<<<<{\displaystyle x(t)} &
%	*+<1pc>[F-,]{
%	\begin{matrix}
%	\text{Delay} \\
%	\displaystyle \frac{v_{\parallel} \cdot t + a_{\parallel} \cdot t^{\,2}/2}{c}
%	\end{matrix}
%	} \ar@{=>}[r]^>>>>>{\displaystyle y(t)} &
%	*{\bigotimes} \ar@{=>}[r] &
%	*+<1pc>[F-,]{\cc h(- (1 + \ecrb )\, t)} \ar@{=>}[rr] && 
%	z(t)
%	\\
%	& \displaystyle e^{\, i \, ( 2 \pi \, f_{c} t + \theta)} \ar@{=>}[u] &&
%	\displaystyle e^{ - \, i \, 2 \pi \, (1+\delta ) \, f_{c} \, t } \ar@{=>}[u] 
%	\\
%	h(t) \ar@{=>}[rr] &&
%	*+<1pc>[F-,]{
%	\begin{matrix}
%	\ \ \text{Delay} \ \ \\
%	\displaystyle \frac{a_{\parallel} \cdot t^{\,2}}{2 c}
%	\end{matrix}
%	} \ar@{=>}[r] &
%	*+<1pc>[F-,]{
%	\begin{matrix}
%	\ \text{Phase}\  \\
%	\displaystyle - \,\frac{\pi \, a_{\parallel} \cdot t^{\,2}}{\lambda_{c}}
%	\end{matrix}
%	} \ar@{=>}[r] &
%	*+<1pc>[F-,]{\cc h(- t)} \ar@{=>}[r] &
%	z(t)
%	}
%
%The time-varying phase in Figure \ref{fig:passbanddoppler}
%due to acceleration is a source
%of time incoherence, but it can be rendered insignificant
%if the total range of phase shifts over $t \in [0,T]$ is smaller than $\alpha \pi$ radians,
%\begin{equation}
%\label{eq:cond1}
%\left|
%\frac{a_{\parallel} \, T^{\,2}}{\lambda_{c}}
%\right| < \alpha
%\ \ \ \text{or} \ \ \ 
%T <  \sqrt{ \frac{\alpha \, \lambda_{c}}{| a_{\parallel} |} } 
%= \sqrt{ \, \frac{\alpha \, c}{| a_{\parallel} | \, f_{c}}}
%\,.
%\end{equation}
%The coherence time $T$ shortens as either $|a_{\parallel}|$ or $f_{c}$ increases, and does not depend on $v_{\parallel}$.
%
%The other effect is a quadratic delay introduced at baseband due to acceleration $a_{\parallel}$.
%This is a source of frequency incoherence, since an $h(t)$ with a bandwidth too large will
%be noticeably affected.
%When  \eqref{eq:cond1} is satisfied, the delay spread is bounded by
%\begin{equation}
%\tau_{s} = \frac{|a_{\parallel}| \, T^{2}}{2 \, c} \ll \frac{\alpha}{2 \, f_{c}} \,.
%\end{equation}
%Thus, frequency coherence is never an issue because $B \ll f_{c} $ and thus $2 B \tau_{s} \ll 1$.
%
%In summary, considering the direct effects of Doppler,
% velocity $v_{\parallel}$ is never an issue, and frequency coherence is never an issue.
%The dominant effect is time incoherence claused by acceleration $a_{\parallel}$.
%In Section \ref{sec:fading} the interaction of the transverse velocity $v_{\bot}$
%with scattering will also be found to be a significant source of time incoherence.

\subsection{Motion compensation}

While the relative velocity of two stars may not be known accurately,
the dynamics of each solar system is well known to the local inhabitants.
For example, on Earth the HORIZONS System from the
Jet Propulsion Laboratory provides real-time data on
the current status of the solar system \citeref{636}.
There is an opportunity for the transmitter and the
receiver to compensate for this known dynamics.
The full correction within an ICH and among ICH's can be
performed at baseband by multiplying by the conjugate of the time-varying
phase factor of \eqref{eq:dopplerbaseband}
\begin{equation}
\exp \left( \,i\, 2 \pi \, \frac{d_{\parallel} (t)}{\lambda_{c}} \right) \,.
\end{equation}
If the transmitter and receiver both do this independently, it
will eliminate the component of motion 
aligned with the line of sight as a source of frequency incoherence.
A simpler compensation is to remove the 
frequency offset among different ICH's without compensating for the
time-varying phase shift within an ICH.
The resulting time incoherence can be rendered negligible
by choosing $T$ in accordance with \eqref{eq:dopplercoherence}. 


%One characteristic of acceleration is that it is an absolute
%rather than relative phenomenon.
%As illustrated in Figure \ref{fig:dopplercorrection},
%conceptually the transmitter can predict the component of its own acceleration
%in the direction of transmission and correct for that acceleration in its transmit signal,
%and similarly the receiver can correct for its own acceleration.
%For the most significant sources of acceleration (a planet's diurnal rotation
%and its orbital motion about its host star) it is straightforward to
%form an accurate estimate $\hat a_{\parallel}$ of the component of acceleration in the transmit or receive
%line of sight.
%Depending on the accuracy of the correction, the coherence time due to Doppler is increased.
%This compensation is only worthwhile up to the point where this incoherence
%becomes insignificant relative to other sources of time incoherence that cannot
%be compensated.
%
%\incxy
%	{dopplercorrection}
%	{
%	Baseband correction of Doppler in the transmitter based on an estimate $\hat a_{t}$ of the
%	transmitter's acceleration component in the line of sight,
%	and similarly baseband correction in the receiver based on an estimate $\hat a_{t}$ of the receiver's
%	acceleration component in the line of sight.
%	}
%	{
% 	h(t) \ar@{=>}[r] &
%	*{\bigotimes} \ar@{=>}[r] &
%	\dots \dots \ar@{=>}[r] &
%	*{\bigotimes} \ar@{=>}[r] &
%	*+<1pc>[F-,]{\cc h(- t)} \ar@{=>}[r] &
%	z(t)
%	\\
%	& e^{\,i\, \pi \, \hat a_{t} \, t^{\,2} / \lambda_{c} } \ar@{=>}[u] &&
%	e^{\,i\, \pi \, \hat a_{r} \, t^{\,2} / \lambda_{c} } \ar@{=>}[u] 
%	}

\section{Scattering}
\label{sec:scattering}

Interstellar scattering has been investigated by a variety of techniques,
including relatively simple geometric optics \citerefthree{628}{629}{630}
and numerical evaluation of turbulent gas models \citeref{627}, always evaluating the models
by comparison to empirical observations of pulsar signals.
Here we employ the simplest possible methodology, geometrical optics 
and ray tracing assuming a one-dimensional
scattering screen.
A recommended tutorial on scattering that assumes a two-dimensional screen is \citeref{598}.
Of course reality is much more complicated, as the scattering medium is dispersed
through three-dimensional space, but three-dimensional modeling is necessarily computational,
and while it can improve the accuracy of numerical results it does not introduce any major new
issues or insights.

Our motivation in using a deliberately simple model is threefold.
First, the goal is to convey the mechanisms of scattering in the simplest fashion,
to emphasize intuition over accuracy.
Second, the limited objective is to convince the reader of the existence of the ICH
and convey an appreciation of the physical mechanisms that determine its size.
Third, the needs of interstellar communication are much different from astrophysics.
Astrophysics must work backwards to estimate the characteristics of
a natural source after propagation through the interstellar medium,
whereas communication seeks to design an artificial signal that circumvents
the impairments introduced in that propagation.
If this design is successful, the detailed modeling of those impairments is unnecessary
because they can be neglected.
Having said this, a serious effort at quantifying the size of the ICH
in the context of an interstellar communication system design
will want to draw upon the full suite of modeling and observations represented in the astrophysics literature,
rather than relying on the simple model illustrated here, in order to obtain the
most numerically accurate result.

\subsection{Geometry of scattering}

For the interstellar medium, where scales are vastly larger than one wavelength,
scattering can be qualitatively explained in terms of the simple ray model of
Figure \ref{fig:scattering-geometry}, where a thin one-dimensional scattering screen
is assumed.
The actual ISM has variations in electron density, which manifest themselves as spatial
variations in the plasma dispersion effects.
In the thin screen model, these variations are represented by a variation in
group delay and phase shift with lateral distance $x$ \citeref{598}.
The variations in electron density are typically quite small, and thus have little effect on the
group delay of propagation through the screen, but do cause a substantial variation in phase shift.
Phase is very sensitive to small perturbations in electron density.

\incfig
	{scattering-geometry}
	{.8}
	{Illustration of the geometry of scattering using a simplified one-dimensional
	scattering screen. (a) Rays passing through the screen at different lateral distances $x$
	encounter different group delays and phase shifts due to small variations in electron density.
	The total distance from source to observer is $(D_{1}+D_{2})$, divided between
	$D_{1}$ from source to screen and $D_{2}$ from screen to observer.
	(b) An ideal slit is opaque to all rays except over the range $[x_{0}-\rdiff/2, x_{0}+\rdiff/2]$. 
	(c) Motion of the observer in the direction of the line of sight with acceleration $a$ 
	and transverse to the line of sight with velocity $v$.}

A slightly refined model to Figure \ref{fig:scattering-iD-illustration} is shown in
Figure \ref{fig:scattering-geometry}a.
It is still one dimensional and assumes a thin screen, but it captures
the distance from source to screen and
screen to observer.
Consider a single ray passing through point $x$ on the screen as shown in
Figure \ref{fig:scattering-geometry}a.
Define the excess distance travelled along the ray (relative to $x = 0$) as $d(x)$,
and that $|x| \ll D_{1}$ and $|x| \ll D_{2}$.
The Fresnel approximation assumes that third and higher powers of $x$ can be neglected,
\begin{equation}
d(x) = \sqrt{D_{1}^{\,2} + x^{2}} + \sqrt{D_{2}^{\,2} + x^{2}} - (D_{1} + D_{2})
\approx \frac{x^{2}}{2 D}
\ \ \ \text{for} \ \ \ \ 
|x| \ll D
\end{equation}
where $D$ is defined by
\begin{equation}
\label{eq:d12}
\frac{1}{D} = \frac{1}{D_{1}} + \frac{1}{D_2}
 \,.
\end{equation}
Thus, after the Fresnel approximation, the simpler model of Figure \ref{fig:scattering-iD-illustration}
still applies, with $D$ defined by \eqref{eq:d12}.

The excess propagation delay associated with a ray passing through
point $x$ on the screen is thus approximately $d(x)/c$.
This delay has frequency transfer function
\begin{equation}
\label{eq:delaytf}
\exp \left\{ - \,i\, 2 \pi \, f \, \frac{d(x)}{c} \right\} 
\approx
\exp \left\{ - \,i\, \pi \, \frac{f x^2}{c \, D} \,\right\}
=
\exp \left\{ - \,i\, \pi \, \frac{x^2}{\rf^{\,2}} \right\}
 \,.
\end{equation}
The Fresnel scale $\rf$ was defined in \eqref{eq:rf}.
It is interpreted as the scale $0 \le x \le \rf$ over which there
is a $\pi$ radian phase shift in the transfer function.
Notably $\rf (f)$ is a function of frequency $f$, but this dependency has
been suppressed in \eqref{eq:delaytf} because the variation is negligibly small
over the band $f \in [f_{c}, f_{c} + B ]$.
Expanding in a Taylor series,
\begin{equation}
\frac{\rf ( f_{c} + \Delta f)}{\rf ( f_{c})} = 1 - \frac{\Delta f}{2 \, f_{c}} - \dots \,,
\end{equation}
so that $\rf (  f_{c} + \Delta f ) \approx \rf (  f_{c} )$ for $\Delta f \le B \ll f_{c}$.

When the screen itself introduces an extra phase shift $\phi(f,x)$,
the transfer function of \eqref{eq:delaytf} should be multiplied by
$\exp \left\{ \,i\, 2 \pi \,\phi (f,x) \right\}$.
This phase can be a function of both $x$
(because of inhomogeneities in the turbulent clouds of ionized gasses)
and $f$ (because of plasma dispersion).

The idea behind ray tracing in geometric optics is that the total response at the observer is
the superposition of the responses due to individual rays 
corresponding to different values of $x$.
The total response is given by the Fresnel-Kirchoff integral,
which integrates the transfer function of screen plus delay over 
all values of $x$,
\begin{equation}
\label{eq:fresnelkirchoff}
\psi (f) = \frac{e^{- \, i \, \pi/4}}{\rf} \int_{-\infty}^{\infty} \exp \left\{ i \, \phi(x,f) - i \, \pi \, \frac{x^{2}}{\rf^{\,2}} \right\} \, dx \,.
\end{equation}
Due to the identity
\begin{equation}
 \int_{-\infty}^{\infty} \exp \left\{ - i \, \pi \, \frac{x^{2}}{\rf^{\,2}} \right\} \, dx = \rf \, e^{ \, i \, \pi/4} \,,
\end{equation}
the normalization constant in \eqref{eq:fresnelkirchoff}
results in $\psi (f) \equiv 1$ (no attenuation or phase shift)
for the special case $\phi (x,f) \equiv 0$
(no scattering).
In particular this normalization renders the attenuation to be frequency-independent,
 in agreement with the plane wave
solution of Maxwell's equations for freespace propagation.
It does, however,
ignore the spreading loss (which increases as the square of distance) .
Thus, \eqref{eq:fresnelkirchoff} isolates the effects of the scattering screen
while omitting spreading loss.

%It is actually remarkable that \eqref{eq:fresnelkirchoff} is able to
%model freespace propagation in the absence of scattering.
%There is a plethora of frequency-dependent interference occurring between
%different ray paths, and yet they add up to no interference overall.
%This rather magical net cancellation of terms is destroyed when
%the extra phase effects of $\phi(f,x) \ne 0$ are introduced,
%destroying this fragile equilibrium.

\subsection{Scattering within a coherence hole}

The scattering model of \eqref{eq:fresnelkirchoff} can be simplified
considerably within an ICH.
Although scattering may place more restrictive conditions,
the bandwidth $B$ of the signal at minimum satisfies
\eqref{eq:dispersioncoherencebandwidth}, 
and the resulting model for $\phi(f,x)$ simplifies to that
of Figure \ref{fig:dispersion}.
Namely, the phase through the scattering screen consists of a
fixed phase $\theta + \phi (f_c,x)$ together with a group delay $\tau(f_c,x)$
that depends on carrier frequency but is otherwise frequency-independent.
In addition, within the turbulent ionized gasses, the inhomogeneity
in electron density over the scales of interest is quite small, so that the group delay
$\tau (f_c,x)$ can be considered to be independent\footnote{
Even if there were a variation of $\tau (f_c,x)$ with $x$, the resulting
effect would be negligible within an ICH if $2 B \tau_{s} \ll 1$ for
a total delay spread $\tau_{s}$.}
of $x$,
and further can be neglected because it is added to the very large
propagation delay.
The net effect of these assumptions is that we substitute
a phase that that is frequency-independent, or $\phi (f,x) \approx \phi (x)$.
The fixed unknown carrier phase $\theta$ can also be neglected,
since $\phi (x)$ is also unknown.

In view of these simplifications, any waveform distortion of signal
$h(t) \, e^{ \, i \, 2 \pi \, f_c t }$ passing through the screen
on a ray through point $x$ can be
neglected, but rather $h(t)$ is merely delayed by $d(x)/c$ 
and shifted in phase by $\phi(x)$.
The resulting observed signal is
\begin{equation}
e^{\,i\,\phi (x)} \, 
h \left( t - d (x)/c \right) \,
\exp \{ \, i \, 2 \pi \, f_c \left( t - d (x)/c \right) \} \,,
\end{equation}
with corresponding baseband signal
(after substituting for $d(x)$)
\begin{equation}
\label{eq:htafterscreen}
h \left( t - d (x)/c \right) \cdot \exp \{  i \, \phi(x)  - \, i \, 2 \pi \, x^2 / \rf^{\,2} \} \,.
\end{equation}
Within an ICH, the bandwidth of $h(t)$ is small enough that the delay can be
neglected.
In that event, the total observation is the superposition of this signal over all $x$, or
$\sqrt{\flux} \cdot h(t)$ for scintillation flux
\begin{equation}
\label{eq:fresnelkirchoffs}
\flux =
\left| \,
\frac{1}{\rf} \int_{-\infty}^{\infty} \exp \left\{ i \, \phi(x) - i \, \pi \, \frac{x^{2}}{\rf^{\,2}} \right\} \, dx
\, \right|^{2}
 \,.
\end{equation}
Again, \eqref{eq:fresnelkirchoffs} has been normalized so that
$\flux = 1$ when $\phi(x) \equiv 0$.
Also note the parallel between this logic and the simplified modeling of Section \ref{eq:scinsum},
with the replacement of a sum by the Fresnel-Kirchoff integral.

%Generally speaking, for a $\phi(x)$ with any specific statistics,
%$S$ will be well-approximated as a zero-mean Gaussian random variable,
%but since the relationship between $\phi(x)$ and $S$
%is highly nonlinear, the variance $\vs$ has to be estimated by Monte Carlo simulation
%rather than analytically.
%While we expect that $\vs < 1$, if $S$ is Gaussian it is also statistically possible that $|S| >1$.
%Thus, it is statistically possible for the screen to actually amplify the signal relative to
%free-space propagation.
%The physical reasoning behind this behavior will now be examined,
%along with a modeling of the energy coming arriving as a function of $x$.

%\section{Dispersion in freespace propagation}
%
%Even in the case of a transparent screen a wideband signal experiences dispersion,
%by which we mean frequency-dependent effects.
%To visualize the source of this dispersion, rewrite the integral in \eqref{eq:freespace}
%in the form
%\begin{equation}
%\label{eq:shortlong}
%\psi = \left( \frac{e^{- \, i \, \pi/4}}{\rf} \int_{|x| \le R} \exp \left\{ i \, \pi \, \frac{x^{2}}{\rf^{\,2}} \right\} \, dx \right)
%+ \left(  \frac{e^{- \, i \, \pi/4}}{\rf} \int_{|x| \ge R} \exp \left\{ i \, \pi \, \frac{x^{2}}{\rf^{\,2}} \right\} \, dx \right) = 1 \,.
%\end{equation}
%The first term is the interference pattern due a hypothetical slit which allows only energy
%passing through for rays with $|x| \le R$, while the second term is the remaining 
%energy that passes through for rays with $|x| > R$.
%The former energy experiences less group delay than the second, since it
%travels along shorter paths.
%This difference is obscured in the monochromatic model, since in this case
%the different delays manifest themselves in different phase shifts,
%and sorting out a delay-induced phase shift from an interference-pattern phase shift is impossible.
%
%However, the proportion of the energy in the two terms in \eqref{eq:shortlong}
%is wavelength and frequency dependent.
%Hence, there is dispersion in the form of a frequency-dependent attenuation
%in freespace.
%This can be quantified by observing that the
%transfer function of a single path in Figure \ref{fig:scattering-geometry}a
%is $\exp \{ - \, i \, 2 \pi f d(x)/ c \}$ as a function of frequency $f$, and forming the superposition of paths
%the total freespace response is
%\begin{equation}
%\psi (f) =  \frac{e^{- \, i \, \pi/4}}{\rf} \int_{-\infty}^{\infty} \exp \left\{ -\, i \, \pi \, \frac{f x^{2}}{c D} \right\} \, dx
%= \sqrt{\frac{f_{c}}{f}} \,.
%\end{equation}
%Thus, there is an attenuation that grows with $f$.
%
%A reasonable definition of frequency coherence is a power loss at $f_{c}+B$
%that is less than two (3 dB), which occurs when
%\begin{equation}
%B \ll f_{c} \,.
%\end{equation}
%Thus, coherence is well maintained for all but very large $B$. 

%The basic idea of Hyguens was to 
%
%\begin{equation}
%\psi ( x_0, \Delta x ) =
%\frac{1}{\rf} \int_{x_0-\delta/2}^{x_0+\delta/2} 
%\exp \left\{ - i \, 2 \pi \frac{x_0 \, \Delta x}{\rf^{\,2}}  \right\} \, d \Delta x
%=
%\frac{\delta}{\rf} \, \text{sinc} 
%\left\{ 
%\pi \, \frac{x_0}{\rf} \, \frac{\delta}{\rf}
%\right\} \,.
%\end{equation}
%All the variables are normalized by $\rf$.
%The amplitude of the signal at $x_0$ is proportional to $\delta/\rf$,
%since the energy allowed through the slit it proportional to the size of the slit.
%However, the amplitude, while oscillating is also dropping off
%as $\pi x_0 / \rf$.
%
%Defining the distance from screen to receiver as $D$, and the wavelength as $\lambda_{c} = c/f_{c}$.
%the Fresnel scale is $r_{F} = \sqrt{\lambda_{c} D}$.
%Ignoring the receiver velocity and assuming that $|x| \ll D$,
%the propagation distance from screen to receiver\footnote{
%A more refined analysis must also take into account the dependence of the distance
%from transmitter to screen, which is another component of the total propagation distance.}
%for a ray passing through the screen at $x$ is
%\begin{equation}
%\label{eq:totaldistance}
%\sqrt{D^{2} + x^{2}} \approx D + \frac{x^{2}}{2 D} + \dots \ \,.
%\end{equation}
%Thus, for $|x| \le r_{F}$ (called the first Fresnel zone) the total variation in ray propagation distance
%is less than $\lambda_{c} /2$.
%Thus there is the potential for constructive interference of rays due to coherence patches with any scale
%that fall within the first Fresnel zone.. 
%
%Consider the region outside the first Fresnel zone, $|x| > r_{F}$, where
%\begin{equation}
%\sqrt{D^{2} + (x+\Delta x)^{2}} \approx D + \frac{x \, \Delta x}{D} + \dots \ \,.
%\end{equation}
%The total variation in distance is less than $\lambda_{c}/2$ on a scale
%$| \Delta x | \le r_{F}^{2}/2 x$.
%This scale is inversely proportional to $x$, and reaches the diffraction scale
%at $x = \rref = r_{F}^{\,2} / \rdiff$, where $\rref$ is called the \emph{refraction scale}.
%Within the refraction scale, the effect of coherent patches is undiminished,
%but for $|x| > \rref$ geometry takes over to prevent the full diffraction effects.
%Thus $|x| \le \rref$ defines the range of $|x|$ that contribute most of the
%energy arriving at the receiver. 
%
%With this background the influence of scattering on time and frequency coherence can be appreciated.
%There are three primary influences on the ICH that are now covered individually.
%A more complete analysis is relegated to another paper \citeref{624}.
%It should be emphasized that all these effects depend on $f_{c}$, because both the
%geometric scale $r_{F}$ and the scale of phase variations $\rdiff$ are wavelength-dependent. 

\subsection{Coherent patches on the scattering screen}
\label{sec:coherentpatch}

The size of integral \eqref{eq:fresnelkirchoffs} depends on the spatial coherency of the
phase.
In regions of $x$ for which that phase is changing rapidly, the contribution to the
integral will be small, while the most significant contributions to $\flux$ come from
areas of slow phase variation.
There are two contributors to phase variation, the random phase due to inhomogeneities
in electron density $\phi(x)$, and the geometric variation due to path length changes
that is proportional to $x^{2}$.
The latter increases in importance with large $x$, and its greater rate of variation with increasing $x$
effectively limits the scale over which a significant contribution to $\flux$ can occur.

Statistically $\phi (x)$ displays ''coherence patches''
over distances in $x$ over which the variation in $\phi(x)$ is small
roughly equal to its diffraction scale $\rdiff$ \citeref{598}.
It is these coherent patches that contribute most of the energy in $\flux$.
As illustrated in Figure \ref{fig:scattering-geometry}b,
the effect can be captured qualitatively by modeling a single coherent patch located
at $x = x_{0}$ as an ideal slit $[x_{0}-\rdiff/2,x+\rdiff/2]$, 
within which the phase shift introduced by the screen is a constant $\phi(f_{c},x) = \phi_{0}$.
The contribution of such a slit to $\flux$ is
\begin{equation}
\label{eq:fresnelkirchoffslit}
\flux =
\left| \,
\frac{1}{\rf} \int_{-\rdiff/2}^{\rdiff/2} \exp \left\{ - i \, \pi \, \frac{(x_{0}+u)^{2}}{\rf^{\,2}} \right\} \, du
\right|^{2}
\,.
\end{equation}
When modeling a small scale patch on the screen,
the Fraunhofer approximation can simplify the integration by eliminating the $x^{2}$ term.
This approximation notes that
\begin{equation}
(x_{0}+u)^{2} = x_{0}^{\,2} + 2 \, x_{0} \, u + u^{2}
\end{equation}
and the first term introduces a constant phase that can be neglected,
while the $u^{2}$ term can be neglected when $\rdiff \ll x_{0}$.
Thus, the Fraunhofer approximation to the magnitude of \eqref{eq:fresnelkirchoffslit}, is
\begin{equation}
\label{eq:fresnelkirchofffraun}
\flux \approx
\left| \,
\frac{1}{\rf} \int_{-\rdiff/2}^{\rdiff/2} \exp \left\{ - i \, 2 \pi \, x_{0}\,u/ \rf^{\,2} \right\} \, du
\, \right|^{2}
= \left| \,  \frac{\rdiff}{\rf} \cdot \text{sinc} \left( \frac{\pi \, \rdiff \, x_{0}}{\rf^{\,2}} \right) \, \right|^{2}
\,.
\end{equation}
This spells out how, as the location $x = x_{0}$  of an ideal slit (with scale $\rdiff$) is changed,
the magnitude of the contribution of that slit to $\flux$ changes.
This is a ''reverse'' diffraction pattern, capturing the effect of a variation in slit location
to the energy arriving at a single point of observation.
This pattern defines the new refraction scale $\rref = \rf^{\,2} / \rdiff$, and written in terms of $\rdiff$ \eqref{eq:fresnelkirchofffraun} becomes
\begin{equation}
\label{eq:fresnelkirchofffraunslit}
\flux \approx
\left| \frac{\rdiff}{\rf} \cdot  \text{sinc} \left( \frac{\pi \, x_{0}}{\rref} \right) \right|^{2}
\,.
\end{equation}
The scale $\rref$ equals
half the width of the main lobe in the pattern, and thus $|x| \le \rref$ is the
primary source of energy arriving at the observer
(that is why it is called the refraction scale).
Of course, some energy originates from outside the screen's refraction scale, but it is smaller.
%Scattering can be divided into strong and weak regimes \citeref{598}.
%Scattering in the interstellar medium is of the strong variety, where $\rdiff \ll \rf$.
%This means that within the Fresnel scale the scattering resolves into smaller
%coherent patches, and thus the dominant refractive effect is multipath distortion,
%where $S$ consists of the superposition of energy arriving from non-overlapping
%coherent patches.
%For this strong scattering case $\rref \gg \rf$, and
%thus the refraction scale is larger than the Fresnel scale.
The energy $\flux$ in \eqref{eq:fresnelkirchofffraunslit} is 
plotted in Figure \ref{fig:observationDiffraction} for two
 strong scattering scenarios.
From \eqref{eq:fresnelkirchofffraunslit} the energy arriving at the observer
for $x_{0} = 0$ is greater for a wider slit (larger $\rdiff$) because a wider slit allows more
total energy to pass the screen.
The nulls occur at multiples of $\rref$, so these nulls are closer together
for a wider slit (larger $\rdiff$).

\incfig
	{observationDiffraction}
	{.8}
	{A log plot of the energy $|S|^{2}$ arriving at the observer and emanating 
	from an ideal slit of width $\rdiff$ located at point $x_{0}$
	on the screen. 
	It is assumed that $\rf=1$, so in effect the abscissa has
	units of one Fresnel scale.
	Two values of $\rref$ are shown: $\rdiff=0.1$ (or $\rref=10$) has its first
	null at $x_{0}=10$, and $\rdiff=0.01$ (or $\rref=100$)  has its first
	null at $x_{0}=100$. The amplitude at $x_{0} = 0$ is higher for the
	wider slit ($\rdiff=0.1$) because more incident energy is able to pass through.}

\subsection{Focusing by the scattering screen}
\label{sec:lensing}

Coherent patches cannot explain the behavior $\flux > 1$, since in the limit
of dense coherent patches with the same constant phase,
$\flux \approx 1$ (this becomes equivalent to freespace propagation).
Focusing by the screen offers a physical explanation for $\flux >1$.
In \eqref{eq:fresnelkirchoffs} the contribution to $\flux$ from a given region can
 be large, even for very large $x_{0}$, if the screen-induced phase approximately cancels out the
pathlength-induced phase, or\footnote{
If \eqref{eq:lensphase} were valid for all $x$ then $\flux \to \infty$,
which indicates a problem with the model.
This non-physical behavior is because the Fresnel approximation
is not valid for large $|x|$.
This is not of concern because \eqref{eq:lensphase} is unlikely to be satisfied for any
range of $x$ much larger than $\rdiff$.}
\begin{equation}
\label{eq:lensphase}
\phi(f_c,x) \approx \pi \, \frac{x^{2}}{\rf^{\,2}} 
\ \ \ \text{or} \ \ \ \
\frac{\partial \phi(f_c,x) }{\partial x} \approx 2 \pi \frac{x}{\rf^{\,2}}
\,.
\end{equation}
This is, of course, the definition of a lens that focuses the energy on the
observer's reference point.
While \eqref{eq:lensphase} is unlikely to be satisfied over significantly large
scales, it is certainly possible within the diffraction scale $\rdiff$.
Note that over the range $[x_{0}-\rdiff/2,x+\rdiff/2]$,
$\phi(f_{c}, x)$ must vary over the range of $2 \pi x_{0} / \rref$
to satisfy \eqref{eq:lensphase}.
Outside the refraction scale $|x_{0}| > \rref$ this variation must be larger than $2 \pi$,
which makes it statistically unlikely.
When lensing does occur, it's contribution to $|S|$ is the same
as the ideal slit with the same aperture located at $x_{0} = 0$,
regardless of whether the lensing occurs inside or outside the refraction scale.

\subsection{Frequency coherence of scattering}
\label{sec:delayspread}

%Scattering can cause both bandwidth and time incoherence.
%The frequency incoherence is due to the energy arriving from different
%portions of the screen arriving with different delays.
%This results in a delay spread, much the same as the variation in group delay
%vs frequency in plasma dispersion, except in this case the delay spread is
%caused by a variation in group delay with screen position $x$.
%
%The physics literature typically applies a monochromatic model, which
%does not capture delay spread, and focuses on the detailed characteristics
%of the refraction patterns at the observer.
%This is because the intended application
%is in pulsar astronomy where the characteristics of the source cannot be controlled.
%For purposes of interstellar communication, the details of the refraction patterns are of little significance
%since the goal is to render the effects of scattering insignificant through the choice of 
%a sufficiently small ICH bandwidth $B$, or in other words insures frequency coherence.
%The definition of ''frequency coherence'' depends secondarily on the intended use of the ICH.
%For a single-use ICH, the objective is to insure that most of the received energy
%in $h(t)$ is preserved in the sampled output of an MF after it is subject to scattering.

Approximation \eqref{eq:fresnelkirchoffs} assumes that the effect of delay on $h(t)$
in \eqref{eq:htafterscreen} can be neglected, and this in turn limits the acceptable $B$.
The criterion for this is $2 \, B \tau_{s} < \alpha$, where $\tau_{s}$
is the delay spread or equivalently the excess delay of components for the largest
$|x|$ that contributes significant scattering energy.

Consider first the strong scattering case.
The main lobe of the interference pattern at the observer corresponds to $|x| \le \rref$.
If we include the energy from a scale $n$ times larger than this to be conservative,
the delay spread becomes
\begin{equation}
\tau_{s} = \frac{d( n \, \rdiff )}{c} \approx \frac{n^{2}}{2 \, f_{c}} \cdot
\left( \frac{\rf}{\rdiff} \right)^{\,2} \,.
\end{equation}
Thus frequency coherence is achieved when
\begin{equation}
\label{eq:scatterngcb}
B < \frac{ \alpha }{n^{2}} \cdot f_{c} \left( \frac{\rdiff}{\rf} \right)^{2} \,.
\end{equation}
Taking into account the frequency dependence of $\rdiff$ and $\rf$,
the $B$ in \eqref{eq:scatterngcb} increases as $f_{c}^{4.4}$, which is
much more rapidly
than the coherence bandwidth for plasma dispersion.
Thus,
the relative importance of plasma dispersion increases with $f_{c}$.

For weak scattering, most of the scattered energy arrives from the first Fresnel zone $|x| \le \rf$,
and again to be conservative by including $n$ times this scale,
\begin{equation}
\tau_{s} \le \tau_{s} = \frac{d( n \, \rf )}{c} \approx \frac{n^{2}}{2 \, f_{c}} \,.
\end{equation}
The criterion for frequency coherence is then
\begin{equation}
B < \frac{ \alpha }{n^{2}} \cdot f_{c} \,.
\end{equation}
Thus, once we move into the weak scattering regime, the coherence
bandwidth increases more slowly with $f_{c}$.
However, the coherence bandwidth is so large in this regime that it unlikely to be significant.

%As long as $B$ is small enough that \eqref{eq:delaycbw} is satisfied,
%the delayed energy will contribute fully to the sampled MF.
%We have seen that a coherent patch located at $x = x_{0}$ contributes smaller energy as $x_{0}$
%increases, while the delay with which that energy arrives also increases with $x_{0}$.
%This decay in energy with delay is the physical mechanism 
%by which frequency coherence can be preserved by choosing
%$B$ sufficiently small.
%One useful benchmark is the scale over which the energy that arrives is in the main lobe
%of the diffraction pattern, which is $|x| \le \rref$.
%The excess delay of energy arriving from the outer extent of this main lobe
%(relative to the direct path through $x = 0$) is
%\begin{equation}
%\tau = \frac{\rref^{2}}{2 \, c \, D} = \frac{1}{2 f_{c}} \left( \frac{\rf}{\rdiff} \right)^{2} \,.
%\end{equation}
%This energy will contribute fully to the MF sampled output as long as $B$ is chosen small enough,
%\begin{equation}
%\label{eq:scatterngcb}
%B \ll f_{c} \left( \frac{\rdiff}{\rf} \right)^{2} \,.
%\end{equation}

%This of course does not capture all the energy, since there are additional sidelobes
%in the diffraction pattern from each slit.
%Consider the $n$th sidelobe, where $n=0$ is the main lobe.
%The maximum is contribution to $|S|$ comes from a coherent patch that happens to fall
%at $x_{0} = (n +1/2) \pi$, which corresponds to energy and delay
%\begin{align}
%&|S|^{2} =  \left( \frac{\rf}{\rdiff} \right)^{2} \frac{1}{(\pi (n+1/2))^{2}} \\
%&\tau = (\pi (n+1/2))^{2} \, \frac{\rref^{2}}{2 \, c \, D} =  \frac{(\pi (n+1/2))^{2}}{2 \, f_c} \left( \frac{\rf}{\rdiff} \right)^{2} \,.
%\end{align}
%The energy due to these sidelobes drops as $n^{2}$, with the delay increasing as $n^{2}$.
%By choosing $n$ large enough, any fraction of the total energy arriving at the observer can be captured,
%with the consequence that the coherence bandwidth $B$ must be a factor of $n^{2}$ smaller.


%It is important to understand the consequences of using a smaller $n$ in determining
%coherence bandwidth $B$.
%When the output of the MF is sampled, any energy with delay $\tau > 1/2B$ is ''lost'',
%in the sense that it does not appear in a single sample at the MF output.
%There is no direct harm caused by this loss of energy, but only the opportunity cost of neglecting some energy
%that has been made available by the scattering.
%The consequence of choosing a larger $B$ is thus a reduction in the sensitivity with which
%the presence of the signal can be detected due to the loss of energy arriving from the far fringes
%of the screen.

Arriving at a more accurate estimate for the $B$ that guarantees
frequency coherence depends on the detailed statistics of $\phi(x)$
and the resulting distribution of the energy arriving as a function of delay.
For energy arriving within a scale $|x| \le r$,
the scattering amplitude seen at the MF output is given by
\eqref{eq:delayspread},
\begin{equation}
\label{eq:fresnelkirchoffsx}
\flux =
\left| \, \frac{1}{\rf}  \cdot \int_{-r}^{r} \exp \left\{ i \, \phi(x) - i \, \pi \, \frac{x^{2}}{\rf^{\,2}} \right\} \, dx \, \right|^{\,2} \,.
\end{equation}
This model is a considerable improvement to the ideal slit in that it 
captures the effects of coherent patches and lensing
as well as other detailed effects.
%For communication purposes all we need to know is $\vs$, the variance of $S$ given by
%\eqref{eq:fresnelkirchoffsx} when averaged over the ensemble of phases $\phi(f_{c},x)$.
%This can be determined by Monte Carlo simulation applied to \eqref{eq:fresnelkirchoffsx} or other means.

\section{Fading and the time coherence of scintillation}
\label{sec:fading}

In a static model of scattering of Section \ref{sec:scattering}, time coherence is not an issue because
the model for $S$ is not time-dependent.
In reality, there are two sources of nonstationarity.
One is changes in $\phi(x)$ with time due to the turbulence of the interstellar clouds.
This is a phenomenon that plays out over days or weeks, and thus is not a factor
in defining the size of an ICH.
Over shorter time scales, the dominant source of non-stationarity is
the interaction of source/observer motion with scattering.
As $T$ is decreased
the total degree of variation decreases and eventually becomes insignificant.

Within an ICH, fading is a velocity rather than acceleration phenomenon.
In Figure \ref{fig:scattering-geometry}c,
the velocity of the receiver causes a carrier frequency offset that was
neglected in Section \ref{sec:doppler}.
However, in the presence of scattering velocity cannot be neglected because
the component of receiver motion in the direction of each incoming ray
from the scattering screen varies slightly with $x$.
This results in a small relative frequency offset among the rays, and that in turn
causes the constructive interference mechanism of refraction
to vary with time and turn causes a variation in scintillation amplitude.
This effect cannot be compensated
at the receiver as argued in Section \ref{sec:doppler} by a simple carrier-frequency offset.
The superposition of the Doppler-shifted rays occurs
\emph{before} to the receiver's observation, and thus there is no single correction that can
simultaneously take care of all the Doppler frequency shifts for all the rays.

The effect of observer motion
can be modeled by assuming two components of velocity,
 $v_{\parallel}$ parallel to the line of sight and $v_{\bot}$ transverse to the line of sight.
 As pictured in Figure \ref{fig:scattering-geometry}c, only $v_{\bot}$
 is a significant source of fading.
 The variation in velocity
 for $t \in [0,T]$ due to acceleration is very small and can be neglected.
The total excess length of a ray through point $x$ on the screen then becomes, as a function of time,
\begin{equation}
\label{eq:dwv}
\sqrt{D_{1}^{\,2} + x^{2}}
+ \sqrt{(D_{2}+ v_{\parallel} t )^{2} + (x - v_{\bot} t)^{2}} 
- ( D_{1} + D_{2} )
\approx
d(x) + v(x) \cdot  t \,.
\end{equation}
In Appendix \ref{sec:fadinganalysis} a Fresnel approximation is applied to \eqref{eq:dwv},
and it is shown that the resulting effect at baseband is a time varying phase
that depends on $x$.
If $T$ is kept sufficiently small, the total phase change can be kept small.
This phase variation is less than $\alpha \,\pi$ radians when
\begin{equation}
\label{eq:tcf}
\left| \,
\frac{f_{c} \, v_{\bot} \, x \, T} {c \, D_{2}} 
\, \right| < \alpha \,
\end{equation}
 for all values of $x$.
 In particular \eqref{eq:tcf} must be satisfied for the largest $x$ that is a significant contributor
to energy arriving at the observer.

Consider first the strong scattering regime.
Following Section \ref{sec:delayspread},
suppose that only $|x| \le n \, \rref$ is is a significant source of energy,
in which case the most stringent condition on $T$ for \eqref{eq:tcf} becomes
\begin{equation}
\label{eq:tcfr}
T \ll \frac{\alpha \, c \,D_{2}}{f_{c} \, | v_{\bot} | \, n \, \rref} 
\,.
\end{equation}
Since $D \le D_{2}$, a slightly more stringent version of \eqref{eq:tcfr} is
\begin{equation}
\label{eq:sctsc}
T < \frac{\alpha \, c \, D}{f_{c} \, | v_{\bot} | \, n \, \rref} 
= \frac{\alpha \, \rdiff}{n \, | v_{\bot} |} \,.
\end{equation}
Thus, significant time variations in scintillation amplitude occur on spatial
scales of observer motion that are greater than a multiple of the diffraction scale $n \, \rdiff$.
Since whatever happens at the plane of motion of the observer is a mirror of the
scattering screen (with appropriate geometric corrections), this significant change
over a scale that mirrors significant phase change at the screen is not surprising.
Since $\rdiff \propto f_{c}^{\,6/5}$, this coherence time increases (albeit relatively slowly)
with $f_{c}$.

For the weak scattering regime, the significant range is  $|x| \le n \, \rf$.
The coherence time becomes \eqref{eq:sctsc} with $\rdiff$ replaced by $\rf$, or
\begin{equation}
T < \frac{\alpha \, \rf}{n \, | v_{\bot} |} \,.
\end{equation}
This case (which for a given $D$ corresponds to larger $f_{c}$) sees
a decreasing $T$ with increasing $f_{c}$.


\section{Numerical example}

While some impairments have been deemed to be insignificant,
the operative sources of incoherence are summarized in Table \ref{tbl:ICHsources}.
A safety factor of $\alpha \le 1$ permits an adjustment of the stringency of the criterion.
There are two primary contributions to frequency incoherence,
both resulting from a spreading of the arriving energy over time.
One is the frequency-dependence of group delay that is characteristic of
plasma dispersion, and the other is the spatial-dependence of group delay due to scattering.
Two primary contributors to time incoherence have been identified,
both due to time-varying phase shift caused by relative source/observer motion.
One is the component of acceleration of
source and observer along the line of sight, and the other is the interaction between the
velocity of the observer transverse to the line of sight and the spatial distribution of angle of arrival
due to scattering.
Rendering all these effects insignificant within an ICH determines the
coherence time $T_{c}$ and coherence bandwidth $B_{c}$
of the ICH, and thus the degrees of freedom $K_{c}$.
The most important physical determinants are the 
distribution of electron density in the ISM
along the line of sight and the relative motion of source and observer.
There is also a strong dependence on the carrier frequency $f_{c}$.

\doctable
	{\small}
	{ICHsources}
	{The significant sources of time and frequency incoherence in interstellar communication,
	distinguishing between the strong and weak scattering regimes.}
	{l l c c}
	{
	\textbf{Type} & \textbf{Source} & \textbf{Strong} & \textbf{Weak}\\
	\toprule
	\addlinespace[3pt]
	Frequency & Plasma dispersion 
	& $B <  \rho \, f_{c}^{\, 3/2}$ 
	& \text{Same}
	\\
	\addlinespace[3pt]
	\cmidrule{2-4}
	& Scattering delay spread 
	& $\displaystyle B < \frac{\alpha}{n^{2}} \cdot f_{c} \, \left( \frac{\rdiff}{\rf} \right)^{2}$
	& $\displaystyle B < \frac{\alpha}{n^{2}} \cdot f_{c} $
	\\
	\addlinespace[3pt]
	\cmidrule{1-4}
	Time & Acceleration 
	& $\displaystyle T < \frac{P}{2 \pi} \cdot \sqrt{\, \frac{\alpha \, \lambda_{c}}{R}}$
	& \text{Same}
	\\
	\addlinespace[3pt]
	\cmidrule{2-4}
	& Scintillation 
	& $\displaystyle T < \frac{\alpha \, \rdiff}{n \, | v_{\bot} |}$
	& $\displaystyle T < \frac{\alpha \, \rf}{n \, | v_{\bot} |}$
	\\
	\addlinespace[3pt]
	\bottomrule
	}

The coherence bandwidth and coherence time are plotted in
Figure \ref{fig:btCoherence} for the numerical values given
in Table \ref{tbl:assumptions}.
A value $\alpha = 0.1$ is used, except for acceleration
where a more conservative factor $\alpha = 0.01$ is used
to account for the strong possibility that another planet or moon
may experience a stronger acceleration than Earth, and also to
account for the possible accumulation of accelerations due to transmitter
and receiver.
Over the entire range of carrier frequencies, one impairment
is more constraining than the other.
In the case of frequency coherence, plasma dispersion
determines the ICH coherence bandwidth $B_c$.
For time coherence, acceleration dominates the coherence
time $T_c$.
The resulting $B_c$ increases with $f_c$, and $T_c$
decreases with $f_c$.
As shown in Figure \ref{fig:dofICH}, the net effect
is a $K_c = B_c T_c$ that starts at $K_{c} \gg 1$
and increases monotonically with $f_c$. 

\incfig
	{btCoherence}
	{.8}
	{Log-log plots of coherence bandwidth $B_c$ above and coherence
	time $T_c$ below, plotted against carrier frequency $f_{c}$
	for the assumed physical parameters of Table \ref{tbl:assumptions}.
	In all cases, it is assumed that $\alpha = 0.1$
	and $n = 2$.
	For scattering phenomena, the break in the slope corresponds to the
	transition from strong scattering (at lower $f_{c}$) to weak scattering (at higher $f_{c}$).
	In each case there are two impairments
	that limit the size of an ICH, but one always is dominant}
		
Any receiver designer should be cognizant of two possible corrections that may be performed in the transmitter.
In the interest of increasing the coherence bandwidth $B_{c}$, the transmitter may perform
partial equalization for the minimum dispersion.
In the interest of increasing the coherence time $T_{c}$, the transmitter may
correct for the component of acceleration along the line of sight.
Interestingly, these are the very same impairments that
dominate $B_c$ and $T_c$, and thus there is motivation to
make these corrections if there is a desire to increase $K_c$,
for example to obtain greater immunity to RFI.

	
%\section{Model for an ICH}
%
%As a starting point, the methodology of communications engineering is to identify the
%simplest model that accurately (or reasonably accurately)
%captures the channel.
%While the ICH by definition preserves waveform integrity by choosing$\{ B, T \}$ sufficiently small, 
%a model cannot hide three impairments that are inevitable regardless of $\{ B, T \}$.
%\begin{description}
%\item[Additive noise]
%\item[Random phase]
%\item[Fading]
%\end{description}
%
%
%The raw reception after band limited is given by
%\begin{equation}
%Y(t) = S \cdot X(t) + M(t)
%\ \ \ \ \text{where} \ \ \ \ 
%S = A \cdot e^{\,i\, \Theta}
%\end{equation}
%In this model,
%$M(t)$ is complex-valued stationary AWGN
%that is circularly symmetric ($E [ M(t) M(t+\tau) ] = 0$)
%and has autocorrelation function $R_{M} (\tau) = E [ M(t + \tau) \cc M (t)]$.
%The signal fading term $S$ is a complex-valued zero-mean Gaussian
%random variable that is also circularly symmetric ($E[ S^{2} ] = 0$)
%and with variance $E | S |^{2} = \vs$.
%In some cases it is convenient to write $S$ in polar coordinates,
%in which case random variable $\Theta$ is uniformly distributed on $[ - \pi , \pi ]$
%and random variable $A$ has a Rayleigh distribution.
%In this model the real- and imaginary parts of all random variables and processes
%are mutually statistically independent.



\chapter{Conclusions}

The conclusions of this study have implications to the
transmitter design should humanity decide to transmit attention-getting
or information-bearing signals to other stars.
In the near term, it also has implications to SETI observational programs.
It has been established that the interstellar medium combined with
motion impairments provide sufficient coherence
in radio propagation to support interstellar communication.
Assuming that power efficiency is the overriding consideration,
fundamental limits on such communication have been established,
and found to be limited by noise of thermal origin alone.
Communication structured around the interstellar coherence hole (ICH) can approach
the fundamental limit, without transmitter or receiver processing
related to any impairments other than noise and scintillation.
In terms of power efficiency,
a more advanced civilization could not improve on this approach.
This strongly suggest that our own transmissions as well as future
SETI observations should be based on the ICH.

The ICH has even stronger implications for the discovery
of information-bearing signals, because interstellar impairments
other than noise and scintillation are eliminated as considerations, from both 
a cost (processing overhead) and performance
(false alarm probability) perspective.
The parameters of the ICH, which are based on physical
quantities subject to observation, strongly limit the scope of a search
in the dimensions of bandwidth and time duration.
As others have previously observed, scintillation aids discovery
by providing periods of elevated signal level.
We have established that with multiple observations
reliable discovery becomes possible at any received signal level and for
any false alarm probability.
In practice these performance measures are limited by the number of
independent observations that the receiver is willing and able to make.

One implication of the ICH-structured signal is that
higher rate and power signals will necessarily employ multiple carriers.
Multicarrier modulation (MCM) has a number of other advantages, including that the
total received power is higher than required for reliable extraction of
information, thus providing an opportunity for multiple concurrent observations.
MCM also lends itself to implementation of a high-power transmitter based on
parallel lower-power transmitters.

A strawman design of an end-to-end interstellar communication system
at the signal layer reveals that scintillation is a major consideration in communication
as well as discovery.
Employing an outage strategy,
the maximum power efficiency is achieved at a high outage probability,
and this implies that most of the transmitted data is lost due to outages.
This places a burden on the reliability and message layers to achieve
message understanding and completeness in the face of substantial data losses.

This work suggests a number of related issues that deserve study.
Although the size of an ICH does not affect the achievable power efficiency,
it does serve as a point of transmitter/receiver coordination.
Thus, a more accurate modeling of the ISM impairments and
relative source/observer motion than undertaken here,
and taking into account future progress in astrophysics and astronomy, should be
a component of any future SETI observation program.
While approaching fundamental limits is predicated on matched
filtering, this places a burden on the receiver to guess the transmitted
waveform within an ICH.
Schemes that relax this requirement while minimizing the resulting reduction in
power efficiency deserve study.
Similarly, achieving fundamental limits requires channel coding,
which would place a large burden on the receiver to reverse engineer
the codebook.
Simple coding schemes that achieve an appreciable improvement in
power efficiency without compromising message understanding
would be of interest.
This work has emphasized power efficiency, but consideration
of techniques that exchange lower power efficiency for higher
spectral efficiency might be of interest under some circumstances,
particularly for designs operating at higher information rates.
Finally, the implementation of a discovery search strategy for ICH-structured
signals is needed, including algorithms, estimates of computational burden,
and the implications to false alarm probability.


%The two objectives (A) and (B) stated in Section \ref{sec:introduction} can be met.
%Each makes a strong statement about the design of a QAM signal, and each requires no compromise in the other. Objective (A) implies a specialization of QAM to biphase modulation, the simplest known data modulation scheme for passband channels. Objective (B) implies a subcarrier bandwidth equal to the coherence bandwidth corresponding to the worst-case variation in DM. The resulting limit on information rate is easily circumvented (with no penalty in objective (A)) by MCM \citeref{612}, in which multiple biphase signals at non-overlapping frequencies are transmitted. As demonstrated by the widely used OFDM \citeref{613}, greater bandwidth efficiency can be obtained, but there is seemingly no incentive to do so in interstellar communication. MCM has other advantages, such as the option to construct a high-power signal using a collection of lower-power transmitters and the ease with which the signal can be tailored to frequency-dependent characteristics like atmospheric noise.
%
%The resulting receiver (for both discovery and communication) is implemented as if there were no dispersion, and in particular does not require the computationally intensive de-dispersion algorithms used in pulsar astronomy. The receiver can operate at the fundamental limits of noise sensitivity, and the transmitter can build in any degree of RFI immunity by increasing the number of carrier signals while reducing the information rate per carrier. There is no constraint on carrier frequency (although lower frequencies require lower information rate per carrier, and more carriers to achieve the same rate) thereby permitting the use of frequencies most favorable for atmospheric attenuation and noise. The total maximum information rate is unaffected by dispersion, and is proportional to the minimum total received power (which in turn depends on transmit power, worst-case propagation loss, and antenna gains).
%
%A search for any information-bearing signal must deal with ambiguity in the bandwidth-time pair $\{ B, \, T \}$, where the transmitter can choose these parameters independently (by adjusting the degrees of freedom $K = B T$). Fortuitously $\{ B, \, T \}$ are constrained by observable physical quantities, greatly reducing the receiver's search space. Dispersion informs the transmitter's choice of bandwidth per subcarrier based on the worst-case variation in DM for the line of sight. The coherence time (period of time over which the propagation can be considered time-invariant) upper bounds the transmitter's choice of $T$.
%
%A single carrier signal can be discovered at power levels appropriate for reliable communication. Discovery based on detection of an isolated pulse requires a power about 3 dB higher, but this 3 dB deficit can be made up by searching over multiple pulses. More complex algorithms searching over multiple subcarriers can discover signals considerably too weak for reliable communication. In all cases, a fine-grain (but limited-range) search over bandwidth per carrier is required due to the receiver's uncertainty about the transmitter designer's perception of worst-case DM. For maximum sensitivity, a relatively coarse-grain and low-cost search over the symbol rate per carrier should be included. To discover a spread spectrum signal ($K > 1$), the receiver must guess the spreading sequence \citeref{211}, and will likely search for more than one possibility (including the case of no spread spectrum). Discovery is not compromised if (A) is relaxed to allow channel coding (thereby abandoning the simplicity of biphase), although extraction of useful information from the signal becomes extraordinarily difficult.
%
%The minimum-rate signal with symbol interval equal to coherence time is an attractive alternative to narrowband attention-attracting beacons because it can be discovered at the same received power level. By also setting the bandwidth equal to the coherence bandwidth, the maximum feasible RFI immunity can be achieved while reducing the search space to a minimum by constraining both bandwidth and symbol interval based on observable physical quantities. If higher information rates are desired, additional subcarriers can be added. This is an attractive starting point in any search for information-bearing signals.
%
%Detailed consideration of the effects of scattering (or multipath) and Doppler are deferred to future papers. These two impairments are the primary determinants of the coherence time, and it is also possible for scattering to reduce the coherence bandwidth below that of dispersion alone. Understanding these effects is thus an important precursor to both transmitter and receiver design. This paper has considered only linear modulation schemes in which information is embedded in the amplitude and phase of a subcarrier. The alternative is orthogonal modulation, in which the embedded information is signaled by the choice among a set of orthogonal waveforms. Forms of MCM (like OFDM) that overlap subcarrier spectra may also be worth considering. Here a particular approach to combining MCM with spread spectrum has been considered, but alternatives should be explored \citereftwo{615}{621}.

\chapter*{Acknowledgements}

This research was supported in part by a grant from the
National Aeronautics and Space Administration to the SETI Institute.
The author is indebted to the following individuals for
generously sharing their time for discussion and comments:
James Benford,
Samantha Blair, 
Gerry Harp,
Ian S. Morrison,
Andrew Siemion,
Jill Tarter,
and
Dan Werthimer.

% Switch to appendix-style numbering
\appendix
%\appendixpage
\addappheadtotoc

\chapter*{Appendicies}

\chapter{Matched filtering}

This appendix provides an analysis and justification of the matched filter
as the optimum receiver processing in the presence of AWGN alone.

\section{Modulation and demodulation}
\label{sec:moddemod}

To prepare this signal for radio transmission, it is multiplied by $\sqrt{\recenergy}$
to give it total energy $\recenergy$, and then modulated by
carrier frequency $f_{c}$ before taking twice the real part $\Re \{ \cdot \}$.
The modulating carrier has a phase $\theta$ that is unknown to the receiver.
The resulting real-valued signal
\begin{equation}
\label{sec:passbandsignal}
2 \, \Re \left\{ \sqrt{\recenergy} \, h(t) \, e^{\,i\,\theta} \, e^{\,i\, 2 \pi \, f_{c} t } \right\}
\end{equation}
is suitable for transmission by electromagnetic means through  the
interstellar medium (ISM), and is confined to frequency range $|f| \in [f_{c}, f_{c} + B ]$.

For purposes of defining the ICH,
the front-end of a receiver is optimized for AWGN
while pretending that there are no other ISM impairments.
The first step is to demodulate the received signal to baseband,
and in the absence of any impairments from the ISM this yields
\begin{equation}
r(t) =
\text{LPF} \left\{
2 \Re \left[ \sqrt{\recenergy} \, h(t) \, e^{\,i\,\theta} \, e^{\,i\, 2 \pi \, f_{c} t }  \right\}
\, e^{- \,i\, 2 \pi \, f_{c} t }
\right]
= \sqrt{\recenergy} \, h(t) \, e^{\,i\,\theta} \,,
\end{equation}
where the low pass filter (LPF) eliminates
frequency components in the vicinity of $2 f_{c}$ and
eliminates all noise outside the bandwidth of $h(t)$.

The optimum baseband receiver processing to counter AWGN is
the matched filter (see Section \ref{sec:matchedfilter} for a derivation of this).
As illustrated in Figure \ref{fig:ICHidea} a filter matched to $h(t)$ has
impulse response $\cc h( - t )$, yielding output signal $z(t)$, where
\begin{equation}
\label{eq:simplemf}
z(t) = \int_{- \infty}^{\infty} r(\tau) \, \cc h (\tau - t) \, d \tau \,.
\end{equation}
In particular 
\begin{equation}
z(0) =  \sqrt{\recenergy} \, e^{\, i \, \theta} + \text{noise} \,.
\end{equation}
Although $\theta$ is unknown to the receiver,
its effect can be eliminated by the energy estimate
\begin{equation}
\left| z(0) \right|^{2} = \recenergy + \text{noise} \,,
\end{equation}
yielding an estimate of the received energy $\recenergy$.

\section{The LS solution}
\label{sec:lscriterion}

Minimizing \eqref{eq:LS} can be accomplished by differentiation with respect to $z$.
However, \eqref{eq:LS} is not an analytic function of $z$ because it includes both $z$ and $z^*$. 
Written in the following form,
$\varepsilon$ is a real-valued analytic function of $z$  and $\cc z$  considered as independent variables.
\begin{equation}
\label{eq:LSerror}
\varepsilon (z, \cc z,\tau ) = \int_{\tau} ^{\tau  + T} 
\left( \, r(t) - z \cdot h(t - \tau) \right)
\left( \, \cc r (t) - \cc z \cdot \cc h (t - \tau) \right)
 \, dt \,.
\end{equation}
As shown in \citeref{176},
a stationary point can be determined by setting
\begin{equation}
\label{ }
0 = \frac{\partial }{ {\partial \cc z } }\varepsilon (z, \cc z,\tau )
= -  \int_{\tau} ^{\tau  + T} 
\left( \, r(t) - z \cdot h(t - \tau) \right)
\cc h (t - \tau)
 \, dt \,.
\end{equation}
Solving for $z$, this gives \eqref{eq:LSsolnZ},
and substituting $\hat z$ into \eqref{eq:LSerror} yields \eqref{eq:LSsolnE}.


%\chapter{Performance of QAM}
%\label{sec:qam}
%
%When a decision variable $Q$ is Gaussian (or can be approximated as Gaussian),
%the probability of a wrong decision $\pe$ is strongly dominated by mistaking the nearest points
%in the signal constellation of $Q$ \citerefWloc{43}{Chap. 6}.
%Thus, constellations with the same minimum distance between points
%$d_{\min}$ have approximately the same $\pe$.
%An accurate proxy for $\pe$ is thus
%\begin{equation}
%\label{eq:snrQdef}
%\snr_{Q} \doteq \frac
%	{d_{\min}^{\,2}}
%	{\text{Var} [Q]}
%\,.
%\end{equation}
%Apply this insight to QAM, where the noise-free $Q = \sqrt{\recenergy} \, A_{k}$
%and the variance is $\text{Var} [Q] = N_{0}$.
%For larger $N$ the energy per symbol is minimized by arranging
%the $2^{N}$ points in a disk $|Q| \le R$ with radius $R$ and the greatest $d_{\min}$
%is achieved by spacing them on a uniform grid with spacing $d_{\min}$.
%The area per point is $d_{\min}^{\,2}$ and the total area is $\pi R^{2}$, and thus
%$2^N \cdot d_{\min}^{\,2} \approx \pi R^2 $.
%Assuming the constellation points are equally probable, the
%energy per symbol is $\recenergy \, \energy_{A} \approx R^{2} /2$, the second moment
%of a continuous random variable with a uniform distribution on the disk.
%Thus
%\begin{equation}
%\snr_{Q} \approx  
%\snrnorm =
%\frac{2 \pi \, \recenergy \, \energy_{A}}{2^{N} \, N_{0}} 
%= \frac{2 \pi}{2^{N}} \cdot \ecrs \,.
%\end{equation}
%Although adequate for our purposes,
%this approximation is crude for small $N$, but by direct calculation
%$\snr_{Q} = 4 \cdot \ecrs$ for $N=1$ and $\snr_{Q} = 2 \cdot \ecrs$ for $N=2$.
%
%The noise in \eqref{eq:mfoutput} can be written in terms of real and
%imaginary parts as  $M(t) = M_{r} (t) + i \, M_{i} (t)$.
%A full characterization of the distribution of $M(t)$ requires the
%autocorrelation and pseudo-autocorrelation \citerefWloc{43}{Section 3.2.8},
%\begin{subequations}
%\begin{align}
%\label{eq:auto}
%\rate_{M}  (\tau) &= E [ M(t+\tau) \cc M (t) ] = h(\tau) \convolve \cc h (-\tau) \\
%\label{eq:cauto}
%\tilde \rate_{M}  (\tau) &= E [ M(t+\tau) M (t) ] =  \cc h (\tau) \convolve \cc h (-\tau) \,.
%\end{align}
%\end{subequations}
%The Fourier transform of $\tilde \rate_{M} (\tau)$ from \eqref{eq:cauto} is $\cc H (-f) \, \cc H(f) = 0$,
%and since $H(f) = 0$ for $f<0$, it follows that $\tilde \rate_{M} (\tau) = 0$
%and $M(t)$ is circularly symmetric.
%$\rate_{M} (\tau)$ is illustrated in Figure \ref{fig:pulseAutoCorr}.
%The statistics of the real and imaginary are
%\begin{align*}
%&R_{r} (\tau) = E[ M_{r} (t+\tau) M_{r} (t) ] = E[ M_{i} (t+\tau) M_{i} (t) ] =
%\Re \{ R_{M} (\tau) \} /2 
%= \frac{\sin (2 \pi \, B \tau )}{4  \pi \,  B  \tau} \\
%&R_{ri}  (\tau) = E[ M_{r} (t+\tau) M_{i} (t) ] = 
% - \Im \{ R_{M} (\tau) \} 
% = \frac{\sin ^2(\pi \, B \tau )}{2  \pi  \, B \tau } \,.
%\end{align*}
%From \eqref{eq:auto}, $R_{M} (-\tau)= \cc R_{M} (\tau)$, and hence
%$R_{r} (-\tau) = R_{r} (\tau)$, $R_{ri} (-\tau) = - R_{ri} (\tau)$,
%and $R_{ri} (0) = 0$.
%Another property that will prove important is
%\begin{equation}
%\label{eq:corrcond}
%| R_{M} (\tau) |^{2}  = 4 \, R_{r}^{\,2} (\tau) + 4 \, R_{ri}^{\,2} (\tau) \le | R_{M} (0) |^{2}  = 4 \, | R_{r} (0) |^{2}  \,.
%\end{equation}
%
%\incfig
%	{pulseAutoCorr}
%	{1}
%	{Pulse autocorrelation $R_h (\tau)$ (real part on the left and imaginary part on the right) for $T=1$
%	and $B=10$. Note the symmetry of the real part and anti-symmetry of the imaginary part,
%	and also that the time duration of the autocorrelation is 
%	on the order of $2/B = 0.2$ seconds.}
%
%For communication, the decision variable is $Q = e^{-i \, \Theta} \, Z(0)$ from \eqref{eq:mfest},
%where $\Theta$ and the constellation of the $\{ A_{k} \}$ must be known and
%$\pe$ is approximately fixed when \eqref{eq:snrpamcommunication} 
%is satisfied.
%For discovery, the decision variable is $Q = | Z(0) |^{2}$ from \eqref{eq:ipdnod},
%and the statistics of $Q$ are not dependent on $\Theta$.
%$Q \ge 0$ has a non-central $\chi^{2}$ distribution, which approaches
%Gaussian for large non-centrality parameter (high SNR).
%Using \eqref{eq:snrQdef} and calculating the first and second moments of $Q$ leads to \eqref{eq:snrpamdiscovery}.
%
%For MCM discovery, assume $L$ energy estimates $\{ Q_m , \, 1 \le m \le L \}$
%of the form of \eqref{eq:ipdnod} corresponding to different symbol internals
%or different carriers.
%Because these are non-overlapping in time or frequency, these $Q_{m}$
%are independent and identically distributed.
%Thus
%\begin{equation*}
%E \left[ \sum_{m=1}^{L} Q_{m} \right] = L \cdot E [ Q_{m} ]
%\ \ \ \text{and} \ \ \ 
%\text{Var} \left[ \sum_{m=1}^{L} Q_{m} \right] = L \cdot \text{Var} [ Q_{m} ] \,,
%\end{equation*}
%and $\snr$ is increased by a factor of $L$.

%\chapter{Modulation}
%
%\section{Equivalent baseband model}
%
%A passband radio communication and its baseband equivalent is modeled in Figure \ref{fig:complexbaseband}.
%A complex-valued baseband input signal $s(t)$ with bandwidth $f \in [0,B]$ is modulated to passband with
%carrier frequency $f_{c}$ (which has an unknown phase $\theta$), and then demodulated and
%filtered to recover a complex-valued baseband signal $r(t)$.
%The reason the baseband signals $s(t)$ and $r(t)$ are permitted to be 
%complex-valued is that the real-valued passband
%signal $x(t)$ can actually accommodate two real-valued components, the in-phase and the quadrature,
%corresponding to modulation by two carriers with a relative $\pi/2$ radian phase shift.
%Taking the real-part $\Re \{ \cdot \}$ to obtain $x(t)$ introduces after demodulation component at
%$2 f_{c}$, and this is eliminated by a post-demodulation lowpass filter.
%For purposes of modeling (but not implementation) the $\Re \{ \cdot \}$ and lowpass filter
%can be omitted as shown in the second realization.
%This presumes that the passband ISM model accepts a complex-valued input, or specifically
%that there are two identical copies of this model, one applied to the real-part and other 
%applied to the imaginary part.
%Finally, an equivalent baseband model can always be derived as shown in the third realization.
%
%\incxy
%	[@C=.8cm] 
%	{complexbaseband}
%	{
%	Reduction of a practical passband channel for radio propagation
%	to an equivalent complex-valued baseband channel.
%	From top to bottom, a passband model with real-valued passband signal $x(t)$,
%	a passband model with complex-valued signal,
%	and an equivalent baseband model.
%	Real-valued signals are denoted by a single arrow, and complex-valued with a couple arrow.
%	}
%	{
% 	s(t) \ar@{=>}[r] 
%	&
%	*{\bigotimes} \ar@{=>}[r] 
%	&
%	*+<1pc>[F-,]{\Re \{ \cdot \}} \ar@{->}[r]^<<<<<{\displaystyle x(t)} 
%	&
%	*+<1pc>[F-,]{
%	\begin{matrix}
%	\text{ISM} \\
%	\text{model}
%	\end{matrix}
%	} \ar@{->}[r]^>>>>>{\displaystyle y(t)} 
%	&
%	*{\bigotimes} \ar@{=>}[r] 
%	&
%	*+<1pc>[F-,]{\begin{matrix}\text{LPF} \\ f \in [0,B] \end{matrix}} \ar@{=>}[r] 
%	&
%	r(t)
%	\\
%	& 
%	\displaystyle e^{\, i \, ( 2 \pi \, f_{c} t + \theta)} \ar@{=>}[u] 
%	&&&
%	\displaystyle e^{ - \, i \, 2 \pi \, f_{c} \, t } \ar@{=>}[u]
%	\\
%	&
%	s(t) \ar@{=>}[r] 
%	&
%	*{\bigotimes} \ar@{=>}[r]
%	&
%	*+<1pc>[F-,]{
%	\begin{matrix}
%	\text{ISM} \\
%	\text{model}
%	\end{matrix}
%	} \ar@{=>}[r] 
%	&
%	*{\bigotimes} \ar@{=>}[r]
%	&
%	r(t)
%	\\
%	&&
%	\displaystyle e^{\, i \, ( 2 \pi \, f_{c} t + \theta)} \ar@{=>}[u] 
%	&&
%	\displaystyle e^{ - \, i \, 2 \pi \, f_{c} \, t } \ar@{=>}[u]
%	\\
%	&&
%	s(t) \ar@{=>}[r] 
%	&
%	*+<1pc>[F-,]{
%	\begin{matrix}
%	\text{Baseband} \\
%	\text{ISM model}
%	\end{matrix}
%	} \ar@{=>}[r] 
%	&
%	r(t)
%	}
%
%	
%\section{Amplitude modulation}
%\label{sec:channelcoding}
%
%The transmitted baseband signal $s(t)$ must embed information in such a way that
%this information can be extracted from $r(t)$.
%A common way to accomplish this in terrestrial systems is to adjust the amplitude of
%waveform $s(t) = A \, \sqrt{ \recenergy} \, h(t)$
%where $A$ is the  \emph{data symbol} which conveys the information.
%It is assumed that $A \in \Omega$, where $\Omega$ is a finite symbol alphabet.
%An example from Section \ref{sec:infosignals} is \emph{on-off keying} (OOK) in which $\Omega = \{ 0,1 \}$.
%This communicates one bit of information (or more generally $\log_{\,2} N$ bits when the
%cardinality of $\Omega$ is $N$).
%
%The waveform $h(t)$ that is modulated by $A$ is of prime importance.
%It is assumed to have Fourier transform $H(t)$,
% unit energy (so that $\recenergy$ controls the signal energy),
%time duration $t \in [0,T]$, and bandwidth $f \in [0,B]$.
%The \emph{degrees of freedom} in $h(t)$
%is $K = B T$, and we must have that $K \ge 1$ \citeref{211}.
%Another important property of $h(t)$ is its correlation function
%\begin{equation}
%R_{h} (t) = h(t) \convolve \cc h (-t)
%\end{equation}
%which is also the inverse Fourier transform of $| H(f) |^{2}$.
%
%%\begin{equation}
%%\label{eq:reception}
%%R(t) =  \sqrt{\recenergy} \,  A \cdot h (t) + \sqrt{N_{0}} \, M(t) \,.
%%\end{equation}
%
%\section{Noise}
%
%An important and unavoidable impairment introduced by the ISM and
%in the receiver is noise\footnote{
%For signals (functions of time),
%upper case is used to denote randomness, and
%lower case to denote deterministic.
%For deterministic signals, upper case denotes an autocorrelation function or Fourier transform}
%$N(t)$.
%For our purpose $N(t)$ is assumed to be AWGN
%with a fixed power spectral density $N_{0}$ 
%(which has the units of watts per Hz, or Joules).
%Referencing this to baseband illustrates of how a baseband model
%is created, as shown in Figure \ref{fig:noisemodel}.
%
%\incxy
%	[@C=.4cm] 
%	{noisemodel}
%	{
%	On the left, baseband noise $M(t)$ is generated from passband AWGN
%	$N(t)$ by demodulation and lowpass filtering. The impulse response of the
%	lowpass filter is $f(t)$.
%	On the right, the lowpass filter is replaced by a matched filter $\cc h (-t)$, which is
%	permissible because the matched filter is also lowpass.
%	}
%	{
% 	N(t) \ar@{->}[r] 
%	&
%	*{\bigotimes} \ar@{=>}[r] 
%	&
%	*+<1pc>[F-,]{\begin{matrix} \text{Lowpass} \\ \text{filter} \\ f(t) \end{matrix}} \ar@{=>}[r] 
%	&
%	M(t)
%	&
%	N(t) \ar@{->}[r] 
%	&
%	*{\bigotimes} \ar@{=>}[r] 
%	&
%	*+<1pc>[F-,]{\begin{matrix} \text{Matched} \\ \text{filter} \\ \cc h(-t) \end{matrix}} \ar@{=>}[r] 
%	&
%	M(t) \convolve \cc h (-t)
%	\\
%	& 
%	\displaystyle e^{- \, i \,  2 \pi \, f_{c} t} \ar@{=>}[u] 
%	&&&&
%	\displaystyle e^{- \, i \,  2 \pi \, f_{c} t} \ar@{=>}[u]
%	}
%
%Quadrature-amplitude modulation (QAM) is
%the simplest and most widely used class of data modulation
%techniques in terrestrial systems.
%This simplicity renders QAM particularly amenable to 
%the absence of explicit coordination
%between transmitter and receiver designs \citeref{583}.
%A real-valued passband signal with carrier frequency
%$f_c$ and occupying bandwidth $f \in [f_c, \, f_c+B]$
%can be represented by an equivalent complex-valued baseband signal
%occupying bandwidth $f \in [0,\,B]$.
%In baseband form, the transmit signal $X(t)$ and receive signal $Y(t)$
%are modeled by \citeref{211}
%\begin{subequations}
%\begin{align}
%\label{eq:modulation}
%X(t) &= \sqrt{\recenergy} \, \sum_{k = -\infty}^{\infty} A_{k} \cdot h (t - k T) \\
%\label{eq:reception}
%Y(t) &= f(t) \convolve X(t) + \sqrt{N_{0}} \, N(t) + \sqrt{\sigma_{r}} \, r(t) \,.
%\end{align}
%\end{subequations}
%where ``$\convolve$'' denotes convolution and the constituent
%signals and parameters are defined in Table \ref{tbl:parameters}.
%The transmitter conveys $N$ bits of information for each $k$ by
%choosing $A_k$ from one of $2^N$ values in a complex-valued constellation
%such as those illustrated in Figure \ref{fig:threeConstellations}.
%The case of $N=1$,
%called binary-phase or \emph{biphase} modulation,
%is particularly important in the sequel.\footnote{
%Biphase is an example of binary antipodal modulation,
%where a waveform and its negative carry one bit of information.
%It is also called binary phase-shift keying (BPSK).}
%Performance metrics characterizing the quality of
%data sharing and parameters affecting these metrics
%are listed in Table \ref{tbl:performance}.
%
%\doctable
%	{\footnotesize}
%	{parameters}
%	{Signals and parameters of the modulated signal of \eqref{eq:modulation} and the
%	reception of \eqref{eq:reception}.}
%	{l l p{10cm}}
%	{
%	\textbf{Category} 
%	& \textbf{Parameter} 
%	& \textbf{Description} \\
%	\toprule
%	Signal & $h(t), \ H(f)$ & Unit-energy pulse used to represent one data symbol \\
%	\cmidrule{2-3}
%	& $A_k$ & One complex-valued data symbol at time $k$; \newline
%	Drawn from a complex-valued signal constellation 
%	(Figure \ref{fig:threeConstellations}) \\
%	\cmidrule{2-3}
%	& $f(t)$ & Impulse response of dispersion bandlimited to $f \in [0,B]$ \\
%	\cmidrule{2-3}
%	& $N(t)$ & Thermal (white Gaussian) noise from natural sources \newline
%	Power spectral density (watts per Hz) equal to constant unity \\
%	\cmidrule{2-3}
%	& $r(t)$ & Unit-energy unknown radio-frequency interference \\
%	\cmidrule{1-3}
%	Rate & $T$ &  Temporal spacing of data symbols; \newline
%	$h(t)$ is mostly confined to symbol interval $t \in [0,T]$; \newline
%	Validity of the matched filter depends on $T \le T_{c}$ \newline
%	$1/T \ \text{sec}^{-1}$ is the symbol rate \\
%	\cmidrule{2-3}
%	& $B$ &  Bandwidth of $h(t)$ and $X(t)$; 
%	$H(f)$ is confined to $f \in [0,B]$ \\
%	\cmidrule{2-3}
%	& $K$ & Degrees of freedom (DOF) in $h(t)$ where $K = B \, T \ge 1$; \newline
%	The immunity to RFI in receiver vicinity increases as $K \uparrow$ \\
%	\cmidrule{2-3}
%	& $N$ & Number of bits per symbol; 
%	\newline Each symbol $A_{k}$ is drawn from a constellation with $2^{N}$ points;
%	\newline Three examples are illustrated in Figure \ref{fig:threeConstellations} \\
%	\cmidrule{2-3}
%	& $\rate$ & Information rate in bits per sec, and equal to $N/T$ \\
%	\bottomrule
%	}
%
%\incfig
%	{threeConstellations}
%	{.6}
%	{
%	Examples of signal constellations with small $N$.
%	The $N=1$ and $N=2$ are examples of phase modulation,
%	since $A_k$ modifies the carrier phase but not amplitude.
%	The $N=3$ example modulates both amplitude and phase of the carrier.
%	For the lowest $\pe$ in AWGN, the points are spaced as
%	far apart as possible in the complex plane subject to a peak- or average-power constraint.
%	}

%\doctable
%	{\footnotesize}
%	{performance}
%	{A list of performance metrics affecting the quality of data sharing using
%	QAM modulation  (\eqref{eq:modulation} and \eqref{eq:reception})
%	and parameters affecting those metrics. 
%	Since propagation and noise vary depending on line-of-sight, 
%	the transmitter designer must focus on
%	a worst-case scenario.}
%	{p{1.5cm} l p{10cm}}
%	{
%	Receiver \newline sensitivity & $\recenergy$ & 
%	Minimum energy in received pulse $\sqrt{\recenergy} \, h(t)$; \newline
%	Pulse $h(t)$ is assumed to have unit energy; \newline
%	When $R_h (kT) = \delta_k$, $\recenergy$ equals minimum energy per symbol \\
%	\cmidrule{2-3}
%	& $\energy_{A}$ & Average energy of the data symbol $E|A_{k}|^{2}$; \newline
%	Total energy per symbol is $\recenergy \, \energy_{A}$ \\
%	\cmidrule{2-3}
%	& $\sigma_{r}$ & Received energy in the RFI; \newline
%	Interference $r(t)$ is assumed to have unit energy \\
%	\cmidrule{2-3}
%	& $\power$ & Average received signal power $\recenergy \, \energy_{A} /T$;\newline
%	Measured at input to baseband processing;\newline
%	Minimum value for the assumed maximum propagation \newline distance
%	and minimum receive antenna collection area \\
%	\cmidrule{2-3}
%	& $N_{0}$ & Power spectrum of additive AWGN; 
%	\newline Autocorrelation is $E[N(t) N(s)] = \delta (t-s)$ \\
%	\cmidrule{2-3}
%	& $\pe$ & During communication, design maximum error probability \\
%	\cmidrule{2-3}
%	& $\pfa$ & During discovery, design maximum false alarm probability \\
%	\cmidrule{2-3}
%	& $\pd$ & During discovery, design minimum detection probability \\
%	\cmidrule{1-3}
%	Dispersion & $f_{c}$ & Carrier frequency; lowest 
%	frequency in the passband signal \\
%	\cmidrule{2-3}
%	& $\dm$ & Dispersion measure; typically $10 < \dm < 1000$ \\
%	\cmidrule{2-3}
%	& $B_c$ & Coherence bandwidth defined in \eqref{eq:coherencebandwidth} \\
%	\cmidrule{2-3}
%	& $T_{c}$ & Coherence time over which the frequency-response $F(f)$ is valid \\
%	\cmidrule{2-3}
%	& $\tau_s$ & Delay spread defined in \eqref{eq:delayspread} \\
%	\bottomrule
%	}
	
%\section{The matched filter}
%\label{sec:mf}
%
%According to various criteria, the optimum processing to extract the
%data symbol $A$ from the received signal $R(t) = s(t) + M(t)$ is
%to apply $r(t)$ to a \emph{matched filter} (MF) with impulse response $\cc h (-t)$
%(and  frequency response $\cc H (f)$)
%and sample the result at $t=0$.
%As illustrated in Figure \ref{fig:noisemodel}, the MF can
%replace the lowpass filter, since it is also a lowpass filter.
%\begin{equation}
%\label{eq:MF}
%Z(t) = R(t) \convolve \cc h (-t)
%=  A \, \sqrt{\recenergy} \, R_{h} (t) + M(t) \convolve \cc h (-t) \,.
%\end{equation}
%Using a MF does require the receiver to correctly guess the
%$h(t)$ used by the transmitter.
%Other possibilities based on autocorrelation techniques have
%been suggested \citereftwo{581}{577}, but the price paid is considerable loss in
%detection sensitivity (higher transmit energy).
%Considerations of RFI does provide very specific guidance on the characteristics
%of $h(t)$ \citeref{211}; namely it should be spread spectrum,
%which means noise-like, with its energy spread
%uniformly over $t \in [0,T]$ and $f \in [0,B]$, and with large $K$.
%In fact $R_{h} (t)$ depends on only the magnitude spectrum,
%and the simplest value that meets the noise-like criterion is
%\begin{equation}
%\label{eq:flatmag}
%| H(f) | =
%\begin{cases}
%1/ \sqrt{B} \,, & 0 \le f \le B \\
%0 \,, & \text{otherwise}
%\end{cases}
%\,.
%\end{equation}
%Figure \ref{fig:bwIllustration} illustrates $R_h (t)$ for two values of $K$,
%where the larger $K$ results in a narrowing of $R_h (t)$ relative to $T$.
%
%\incfig
%	{bwIllustration}
%	{1}
%	{A plot of $R_h (t)$ in \eqref{eq:flatmag} with $T=1$ and
%	two values of $K = B T$.
%	The effect of increasing the bandwidth through $K$ is to narrow the autocorrelation.
%	In both cases, $R_h(kT) = \delta_k$.}
%
%Because $h(t)$ has unit energy, $R(0) = 1$ and thus
%\begin{equation}
%Z(0) = A \, \sqrt{\recenergy} + M
%\end{equation}
%where $M$ is a complex-valued zero-mean Gaussian random variable with
%variance $E |M|^{2} = N_{0}$.
%This model, although it can be used to make a decision on the value of $A$
%and hence the embedded information, does not take into account propagation
%effects through the ISM.
%These effects will now be addressed. 

%With additive AWGN, 
%a \emph{matched filter} (MF) for $h(t)$
%is a filter with impulse response $\cc h (-t)$
%and frequency response $\cc H (f)$.
%The MF is suitable for front-end processing regardless of $f(t)$
%\citereftwo{43}{211}.
%The response of a MF to $h(t)$ has Fourier transform $| H(f)  |^{\,2}$.
%The autocorrelation function $R_{h} (t)$ of $h(t)$
%equals either the inverse Fourier transform of  $| H(f)  |^{\,2}$
%or $R_h (t) = h(t) \convolve \cc h (-t)$.
%The transmitter should choose $h(t)$ such that
%$R_h (kT) = \delta_{k}$ so that, in the absence of dispersion,
%the MF output sampled at $t = kT$
%responds to only $h(t-kT)$ and none of the other translates of $h(t)$.
%A necessary condition is $K = B T \ge 1$.
%For convenience, we always choose $K$ to be an integer, in which case $K$
%is interpretated as the \emph{degrees of freedom} (DOF) in $h(t)$,
%equal to the number of complex-numbers required to fully specify
%the waveform $h(t)$.

%In spread spectrum \citeref{211}, $K \gg 1$ to gain RFI immunity \citeref{211}, and
%further $h(t)$ should be noise-like, 
%spreading its energy over both $t \in [0,T]$ and $f \in [0,B]$.
%For this purpose, \eqref{eq:flatmag} is an appropriate choice of $| H(f) |$
%because it spreads energy uniformly over $f \in [0,B]$, but the phase of $H(f)$ 
%(which does not affect $R_h (t)$) must be manipulated
%to also spread energy uniformly over $t \in [0,T]$.
%The MF is then a phase equalizer, gathering the energy up into a narrow pulse $R_{h} (t)$
%while robustly attenuating RFI.
%As dispersion does not affect RFI immunity, $\recenergy = 0$ is assumed in the sequel.
%
%Defining $Z(t)$ as the MF output and
%pulling out only the $k=0$ term\footnote{
%Ignoring the $k \ne 0$ terms is justified if there is no intersymbol interference (ISI) \citeref{43}.
%In the sequel, by constraining $B \le B_c$ the dispersion will be 
%much too small to result in ISI.}
%in \eqref{eq:reception},
%\begin{equation}
%\label{eq:mfoutput}
%Z(t) = \sqrt{\recenergy} \, A_{0} \, f(t) \convolve R_h (t) + \sqrt{N_{0}} \, M(t) \,,
%\end{equation}
%where $M(t) = N(t) \convolve \cc h (-t)$.
%The dispersion tends to 'smear out'' and broaden $R_{h} (t)$ by convolving with $f(t)$.
%Although Figure \ref{fig:impulseResponse} illustrates $f(t)$ for large dispersion,
%when the dispersion is small ($B \le B_{c}$)
%the effect is less severe as illustrated in Figure \ref{fig:IRvsB}
%where the magnitude (but not phase) is plotted.
%When $B \le B_{c}$ the dispersion can be ignored for both discovery
%and communication because $Z(0)$ is not appreciably affected by dispersion.
%In this case,
%\begin{equation}
%\label{eq:mfest}
%Z(0)
%= \sqrt{\recenergy} \cdot  e^{\,i\,\Theta} A_{k}  + \sqrt{N_{0}} \cdot M(0)
%\,,
%\end{equation}
%where $\Theta$ is an unknown phase.\footnote{
%This phase has two constituents, an unknown carrier phase
%and the phase of $f(t) \convolve R_{h} (t)$ (which depends on the
%precise value of $\dm$).
%}
%During communication, $\Theta$ must be estimated using available techniques \citerefWloc{43}{Chapter 15},
%after which 
%$e^{\,- i\,\Theta} Z(0)$ in \eqref{eq:mfest} is analyzed to identify the
%nearest constellation point.
%A rate-normalized SNR measure
%\begin{equation}
%\label{eq:snrpamcommunication}
%\snrnorm = \frac{2 \pi}{2^{N}} \cdot \ecrs
%\, \ \ \ \text{for} \ \ \ \ 
%\ecrs = \frac{\recenergy \, \energy_{A}}{N_{0}} \,,
%\end{equation}
%accurately predicts $\pe$ (Appendix \ref{sec:qam}),
%with typical values of $\snrnorm \approx 10$.
%Fixed $\pe$ requires that $\ecrs$ grow as $2^N$.
%Because it will be established that biphase ($N=1$) is an advantageous choice,
%this $\pe$ is plotted in Figure \ref{fig:pEvsSNR0}.
%
%\incfig
%	{pEvsSNR0}
%	{.8}
%	{A log plot of the error probability $\pe$ vs $\snr_0$ in dB
%	for biphase modulation with $A_{k} \in \pm 1$ and $\energy_{A} = 1$.
%	Note that $\snr_0 \approx 10$ dB or larger is required for reliability.}

\chapter{Statistical model for a coherence hole}
\label{sec:modelICH}

\section{Scintillation without modulation}
\label{sec:withoutmod}

The statistical properties of the model for an ICH given in \eqref{eq:ICHmodel}
will now be established.
Define the random variable $S$ as
\begin{equation}
S = \sum_{n=1}^{N} r_n \, e^{\,i\, (\Phi_{n}}
\end{equation}
where the $\{ r_n \}$ are fixed but unknown quantities
and the $\{ \Phi_n \}$ are independent and uniformly distributed.
By the Central Limit Theorem we can approximate $S$ as Gaussian
for reasonably large $N$.
It follows from independence and $\expec{e^{\,i\, \Phi_{m}}} = 0$ that $\expec{S}= 0$ and
\begin{equation}
\expec{S^{2}}  = 
\expec{ \sum_{n=1}^{N} \sum_{m=1}^{N} r_n \, r_m \, e^{\,i\, ( \Phi_{m} + \Phi_{n}} ) }
= \sum_{n=1}^{N} r_n^{\,2} \, \expec{e^{\,i\, 2 \Phi_{m}}} = 0 \,.
\end{equation}
This establishes that the $\Re \{ S \}$ and $\Im \{ S \}$ have equal variance and are uncorrelated and hence independent.
The variance of $S$ is
\begin{equation}
\expec{ | S |^{2}} = 
\expec{ \sum_{n=1}^{N} \sum_{m=1}^{N} r_n \, r_m \, e^{\,i\, ( \Phi_{m} - \Phi_{n}} ) }
= \sum_{n=1}^{N} r_n^{\,2} \,.
\end{equation}
For the $n \ne m$ terms, the expected values are zero due to independence, leaving
only the $n = m$ terms.

From \eqref{eq:noiseICH}, that $E |M|^2 = N_0$ is easily established.
More interesting is the conclusion that $\Re \{ M \}$ and $\Im \{ M \}$ have equal variance and are uncorrelated and hence independent.
This follows from
\begin{equation}
\expec{ M^2 } = 
N_0 \int_0^T e^{-\,i\,4 \pi \, f_c t} \, \left( \cc h (t) \right)^2 \, dt = 0 \,,
\end{equation}
where $\left( \cc h (t) \right)^2$ has bandwidth $2 B$, and after
modulation with carrier frequency $2 f_c$ its spectrum is guaranteed not to overlap
$f = 0$ and thus the integrand averages to zero.

%Finally, the phase of the signal term has been deliberately omitted in \eqref{eq:ICHmodel},
%because all the subsequent signal processing uses the magnitude of the MF output
%in order to be insensitive to this phase.
%To see why such a phase would make no difference in the statistics of $| z(0) |^{2}$,
%note that
%\begin{equation}
%| z(0) |^{2} =
%\left| \sqrt{\recenergy} \sqrt{\flux} e^{\,i\, \theta} + M \right|^{2}
%= \left|  \sqrt{\recenergy} \sqrt{\flux} +  e^{-\,i\, \theta} \, M \right|^{2} \,.
%\end{equation}
%The distribution of $M$ and $e^{-\,i\, \theta} \, M$ are identical for all values of $\theta$,
%and thus $M$ and $e^{-\,i\, \Theta} \, M$ have the same distribution for any
%random variable $\Theta$.

\section{Scintillation and amplitude modulation}
\label{sec:withmod}

Suppose $h(t)$ is amplitude modulated by $A$, and after matched filtering
the scintillation and noise result in \eqref{eq:singleIU},
where the flux for weak scattering given by \eqref{eq:ricianflux} is assumed.
Then the MF output is
\begin{equation}
Z = \sqrt{\recenergy} \cdot \left( \sqrt{\gamma} \, 
e^{\,i\,\Psi} \, \sigma_{s} + \sqrt{1 - \gamma} \, S \right) \, A + M \,,
\end{equation}
where $0 \le \gamma \le 1$ is the fraction of signal that arrives in the specular path.
Conditioned on a particular specular phase $\Psi = \psi$,
and writing the data symbol in polar coordinates $A = a \, e^{\,i\,\theta}$,
$Z$ becomes Gaussian with independent real- and imaginary parts,
and with first and second order statistics
\begin{align}
&\expec{\Re \{ Z \}} = \sqrt{\, \recenergy \, \gamma \,}  \, a \, \sigma_{s} \, \cos ( \psi + \theta )
\ \ \ \text{and} \ \ \ \  \expec{\Im \{ Z \}} = \sqrt{\, \recenergy \, \gamma \, } \, a \, \sigma_{s} \, \sin ( \psi + \theta )
\\
& \var{\Re \{ Z \}} = \var{\Im \{ Z \}} = \frac{\recenergy \, a^{2} \, (1 - \gamma ) \, \vs + N_{0}}{2} \,.
\end{align}
Observe that only $\expec{Z}$ (and not $\var{Z}$) is dependent on $\theta$.
When $\psi$ is unknown and uniformly distributed, $\expec{Z}$
yields no information on the value of $\theta$.
The conclusion is that any phase component in $A$ is rendered unobservable by scintillation
for any $\kappa$ and $\gamma$.
On the other hand $Q = |Z|^{2}$ makes a good real-valued decision variable
since its mean value includes a component of $a^{2}$ for any $0 \le \gamma \le 1$
(and in particular for strong scattering where $\gamma = 0$)
and any $\psi$, since
\begin{equation}
\expec{|Z|^{2}} = \recenergy \, a^{2} \, \vs + N_{0} \,.
\end{equation}
Particularly notable is the lack of dependence on $\gamma$,
or in other words the strength of the scattering.

\chapter{Two information units per coherence hole}
\label{sec:multiuse}

Assuming that it is supported by the size of an ICH,
more than one IU can be embedded within a single ICH,
thereby increasing the amount of information conveyed by that ICH.
The simplest case of two IU's per ICH illustrates most of the issues
that arise in attempting this.
Replace a single waveform $h(t)$ by a pair of waveforms
$h_{1} (t)$ and $h_{2} (t)$, each of which falls within the
\emph{same} ICH.
That is, each satisfies the $B \le B_{c}$ and $T \le T_{c}$ constraints,
which implies that any weighted superposition of these waveforms
satisfies the same constraints.
A transmitted signal $A_1 \, h_1 (t) + A_2 \, h_2 (t)$
can then convey more information in a pair of data symbols $A_{1}$ and $A_{2}$.

The receiver must sort out the two individual data symbols, and this is simpler
if $h_1 (t)$ and $h_2 (t)$ are chosen to be orthogonal, or
\begin{equation}
\label{eq:orthogonality}
\int h_1 (t) \, \cc h_2 (t) \, dt = 0 \,.
\end{equation}
Then, in the absence of ISM impairments a filter matched to
$h_1 (t)$ will have zero response to $h_2 (t)$ and vice versa.
The simplest and most obvious way to insure \eqref{eq:orthogonality}
is to choose the two waveforms to be non-overlapping in
time and/or spectrum, even while they fall in a common ICH.
For example, for some $h(t)$ choose $h_m (t) = h(t - \tau_m) \, e^{\,i\, 2 \pi \, f_m t}$
for $|\tau_2 - \tau_1| > T$, $|f_2 - f_1| > B$, or both.
The case $|t_2 - t_1| > T$ and $f_1 = f_2$ 
is called \emph{time division multiplexing} (TDM),
and the case $|f_2 - f_1| > B$ and $\tau_1 = \tau_2$
is called \emph{frequency-division multiplexing} (FDM).
It is also possible to choose time/frequency
overlapping waveforms and still satisfy \eqref{eq:orthogonality}.

The output of two MF's, one matched to $h_1 (t)$ and the other
matched to $h_2 (t)$ will generalize from \eqref{eq:singleIU} to
\begin{equation}
\label{eq:dualIU}
Z_1 =  \sqrt{\recenergy} \, \sqrt{\flux_{1}} \, e^{\,i\,\theta_{1}} \, A_1 + M_1
\ \ \ \ \text{and} \ \ \ \ 
Z_2 = \sqrt{\recenergy} \, \sqrt{\flux_{2}} \, e^{\,i\,\theta_{2}} \, A_2 + M_2 \,.
\end{equation}
Note that phase terms $e^{\,i\,\theta_{1}}$ and $e^{\,i\,\theta_{2}}$ have been included, because this is
an instance where the phase shift caused by scintillation may make a difference.
In particular, because of \eqref{eq:orthogonality} that $Z_1$ has no term
proportional to $A_2$, and likewise for $Z_2$ and $A_1$.
For this model to be valid, care must be exercised to insure
that a filter matched to $h_1 (t)$ does not respond to
$h_2 (t)$ post-ISM, and a filter matched to $h_2 (t)$ does not respond to
$h_1 (t)$ post-ISM.
To render \eqref{eq:dualIU} valid for TDM 
may require that $|t_2 - t_1|$ be increased, in effect putting in an additional
guard time between $h_1 (t)$ and $h_2 (t)$.
Similarly, to render 
\eqref{eq:dualIU} valid for FDM may require an increase in $|f_2 - f_1|$.

The $M_m$ in \eqref{eq:dualIU} are mutually independent due to
assumption \eqref{eq:orthogonality}.
However, the joint statistics of the scintillation amplitudes
$\sqrt{\flux_{1}}$ and $\sqrt{\flux_{2}}$ depends on circumstances.
The magnitude $|S|$ generally varies fairly slowly with time,
and also in frequency,
so if $|\tau_2 - \tau_2|$ is small (on the order of seconds to minutes)
and $f_1 = f_2$ then $\sqrt{\flux_{1}} \approx \sqrt{\flux_{1}}$.
However, $\arg S$ varies much more rapidly, and thus no
relationship of $\arg S_1$ and $\arg S_2$ can be counted on
unless $|\tau_2 - \tau_1| < T_c$ and $|f_2 - f_1| < B_c$;
that is, unless the two IU's fall within a single ICH.

When no two IU's fall within a single ICH, this is called a
\emph{single-use ICH}; otherwise, it is called a \emph{multi-use ICH}.
Single-use is simpler, which may be an advantage during discovery.
In Chapter \ref{sec:fundamental} it will be shown that fundamental
limits in power efficiency can be reached with a single-use ICH.
Also, the single-use ICH can have better consistent RFI
immunity (Section \ref{sec:rfi}).
On the other hand, the multi-use ICH
can relax the requirement that $h(t)$ be guessed by the
receiver by substituting autocorrelation algorithms \citereftwo{581}{577},
although this comes at a very substantial penalty in power efficiency
for $K \gg 1$ \citeref{626}.
The multi-use ICH also has better spectral efficiency.

\chapter{Search granularity in dilation and frequency}
\label{sec:searchgranulatiry}

Any mismatch between the time dilation parameter $\beta$ used in the
implementation of the MF and the actual value of $\beta$ results in incoherence.
The same is true for any mismatch between the carrier frequency $f_{1}$ and reality.
These sources of incoherence are totally under the control of the receiver in its
choice of a granularity in a search over these parameters.
Hence we don't put them in the same category as natural sources of incoherence.

\section{Time dilation error}

Since a search over $\beta$ will generally need a small range,
write it as $\beta = 1 + \delta$, and ask how $\delta \ne 0$ affects coherence.
This can be studied by assuming that $r(t) = h(t)$ but the MF used
is $\cc h (- (1+\Delta \delta) t)$.
%An example of time-varying delay is time dilation, in which the receiver
%replaces $h(t)$ by $h( (1 + \delta) \, t )$ when it performs matched filtering.
%The parameter $\delta \approx 0$
%is called the \emph{dilation error}, and is
%inevitable since for any assumed signal waveform $h(t)$
%the receiver has no knowledge of the rate or speed with which the signal
%is transmitted.
%Often the receiver can infer a range of dilations based on other considerations, such as the
%size of the coherence hole and the signaling technique in use,
%but precise information is never available.
%The receiver must then search over the uncertain range in order to find a close enough
%approximation.
The largest acceptable value of $| \Delta \delta |$ depends to some extent on $h(t)$.
We now show that for a signal
of the form of \eqref{eq:flatmag}, the MF output is affected very little when $| \Delta \delta | \ll 1/ \pi K$.
Thus the fractional dilation offset is on the order of $1/\pi K$, which implies that
an $h(t)$ with larger $K$ requires a finer-grain search over the dilation parameter.
Time dilation error is a factor in both time and frequency coherence, since a given error $\Delta \delta$
places an error on the product $K = B T$.

The Fourier transform of $h ((1+ \Delta \delta) t)$ is $H(f/ (1+ \Delta \delta))$.
Assume that $\Delta \delta > 0$ (the final result is the same for $\Delta \delta < 0$).
Then the MF output is
\begin{equation}
Z = \int_{0}^{B/(1+\Delta \delta)} H(f) \, \cc H \left( \frac{f}{1+\Delta \delta}  \right) \, df
=  \frac{1}{B} \, \int_{0}^{B/(1+\Delta \delta)} \exp \{ i \left( \phi(f) - \phi \left( \frac{f}{1+\Delta \delta} \right) \right) \, df
\end{equation}
The group delay $\tau (f)$ is defined by \eqref{eq:delayFromPhase}.
Since $h(t)$ is confined to $t \in [0,T]$, it follows that $0 \le \tau (f) \le T$.
The sensitivity of $Z$ to $\Delta \delta$ can be gauged by the derivative
\begin{equation}
v = \left. \frac{\partial Z}{\partial \Delta \delta} \right|_{\Delta \delta = 0} 
= \frac{i}{B} \, \int_{0}^{B} f \frac{\partial \phi (f)}{\partial f}  \, df - 1
= \frac{- i \, 2 \pi}{B} \, \int_{0}^{B} f \, \tau (f) \, df -1
\end{equation}
where
\begin{equation}
0 \le  \int_{0}^{B} f \, \tau (f) \, df \le \frac{B^{2} T}{2} 
\ \ \ \ \text{or} \ \ \ \ \ 
1 \le | v |^{2} \le 1 + \pi^{2} \, K^{2} \,.
\end{equation}
Thus, $|Z|$ is relatively little affected if  $\Delta \delta | v | \ll 1$ or
$\Delta \delta \ll 1/ \pi K$.

\section{Carrier frequency offset}

As with delay and dilation, the receiver will calculate the MF output for
discrete values of carrier frequency.
In Figure \ref{fig:coherenceholetest}
there may be a mismatch $\Delta \ecrb$ between reality and the receiver's assumption.
In this case, the MF output becomes 
\begin{equation}
Z = \int_{0}^{T} | h(t) |^{2} e^{-\,i\,2 \pi \, \Delta \ecrb \, f_{c} \, t} \, dt \,.
\end{equation}
The offset will have an insignificant effect of $Z$ if
the total phase shift is much less than $\pi$,
or $| \Delta \ecrb | \ll 1/2 f_{c} T$.
Time coherence is maintained if
the absolute carrier frequency spacing is small relative to $1/T$.

\chapter{Capacity of an ICH-structured communication} 
\label{sec:capacity}

%The channel capacity of a flat Rayleigh fading channel is known \citeref{622}, so
%we adapt (and simplify) this result by assuming unconstrained bandwidth.
%The continuous-time model employed in \citeref{622} is
%\begin{equation}
%\label{eq:ctchan}
%V_{t} = R_{t} \, e^{\,i\, \Theta_{t}} \, U_{t} + N_{t}
%\end{equation}
%where $R_{t}$ is the fading magnitude and $\Theta_{t}$ is the phase.
%The power average power of $U_{t}$ is constrained to be $\power$,
%which implies that $\power$ is the average received signal power
%in the absence of fading ($R \equiv 1$).
%While the transmitter is ignorant of the current value of $R_{t}$,
%it is assumed that the transmitter and receiver both know the distribution of
%$\{ R_{t}, \Theta_{t}, M_{t} \}$ and also that the receiver knows
%(or can form an accurate estimate of) $R_{t}$.
%Under these assumptions, the average capacity is
%\begin{equation}
%\capacity = \expec{ 
%B \, \log_{\,2} \left( 1 + \frac{R^{\,2} \, \power}{N_0 \, B} \right)
%}
% \,,
%\end{equation}
%where the expectation $\expec{\cdot}$ is over the $R$ ensemble.
%Our interest is in unconstrained bandwidth,
%\begin{equation}
%\lim_{B \to \infty}
%\expec{ 
%B \, \log_{\,2} \left( 1 + \frac{R^{\,2} \, \power}{N_0 \, B} \right)
%}
%=
%\expec{ 
%\frac{R^{\,2} \, \power}{N_0 \, \log_e 2}
%}
%= 
%\frac{ \vs \, \power}{N_{0} \, \log_{\,e} 2}
% \,.
%\end{equation}
 
%Define a capacity $\capacity_r$
%conditioned on scintillation magnitude $R = r$,
%\begin{equation}
%\capacity_r = B \, \log_{\,2} \left( 1 + \frac{r^{\,2} \, \power}{N_0 \, B} \right) \,.
%\end{equation}
%If $f_R (r)$ is the probability density of $R$, then under the assumptions above
%the actual capacity is the average
%with respect to the distribution of $R$,
%\begin{equation}
%\label{eq:ctrfcapacity}
%\capacity = \lim_{B \to \infty}
%\int \capacity_r \, f_R (r) \, dr =
%\int \frac{r^2 \, \power}{N_0 \, \log_{\,e} 2} \, f_R (r) \, dr =
%\frac{ \vs \, \power}{N_{0} \, \log_{\,e} 2} \,.
%\end{equation}

The ergotic capacity of a discrete-time communication
channel based on the repetitive transmission of information units
each falling within a single-use ICH as described in Chapter \ref{sec:channelmodelstructure}.
An appropriate model is a generalization of \eqref{eq:sequenceIU}
to transmit a sequence $\{ U_{k} \}$ at the input, yielding an output sequence
\begin{equation}
V_{k} = \sqrt{\flux_{k}} \, U_{k} + M_{k} \,,
\end{equation}
where the input signal power is constrained by $\expec{|U_{k}|^{2}} \le \recenergy$.
The key assumption is that the ICH's corresponding to the different $k_{1}$
and $k_{2}$ are non-overlapping in both time and frequency for $k_{1} \ne k_{2}$, so that the
$\{ M_{k} \}$ are statistically independent.
If the rate at which ICH's are invoked is $F$,
the average power is constrained $\power = F \, \recenergy$.
For each individual channel use $k$, the
maximum mutual information is \citerefWloc{43}{Section 4.2.3}
\begin{equation}
\expec{
\log_{\,2} \left( 1 + \frac{\flux \, \recenergy}{N_0} \right)
}\,.
\end{equation}
The expectation is over the random ensemble for $\flux$.
The ergotic capacity is
$F$ times the maximum mutual information per channel use,
and since the bandwidth $B$ is considered to be unconstrained
we can allow $F$ to grow arbitrarily.
As $F$ grows, $\recenergy$ and the per-use capacity shrink,
but the overall capacity approaches a maximum,
\begin{equation} 
\capacity =
\expec{
F \, \log_{\,2} \left( 1 + \frac{\flux  \, \power}{F \, N_0} \right) 
}
\underset{F \to \infty}{\longrightarrow}
\expec{ 
\frac{ \flux \, \power \, \log_{2} e}{N_0}
}
= 
\frac{ \power \, \vs \, \log_{2} e}{N_{0}} \,.
\end{equation}
This is identical to \eqref{eq:scincapacity}, and thus the ICH-structured
capacity is the same as that of the continuous-time channel with noise and scintillation.

%For any $R$ the random quantity being averaged
%is monotonically increasing with $F$, so $E [\cdot]$ has that
%property and thus $C$ is monotonically increasing with $F$.
%capacity corresponds to $F \to \infty$.
%Since bandwidth is unconstrained, then so too is $F$,
%and thus capacity is
%\begin{equation}
%E \left[
%F \, \log_{\,2} \left( 1 + \frac{R^{\,2} \, \power}{N_0 F} \right) 
%\right]\,.
%\end{equation}
%
%\begin{equation}
%\label{eq:dtrfcapacity}
%\capacity =  \lim_{F \to \infty}
%\int \capacity_r \, f_R (r) \, dr =
%\int \frac{r^2 \, \power}{N_0 \, \log_{\,e} 2} \, f_R (r) \, dr =
%\frac{ \vs \, \power}{N_{0} \, \log_{\,e} 2} \,.
%\end{equation}
%The equality of \eqref{eq:ctrfcapacity} and \eqref{eq:dtrfcapacity} establishes that
%structuring the signal based on the ICH does not affect the capacity.
%If $\capacity_{\text{ISM}}$ is the capacity of the actual ISM, 
%then $\capacity_{\text{ISM}} \le \capacity$ since the ISM introduces other impairments in addition to
%flat Rayleigh fading.
%Since our ICH scheme is a viable technique for the ISM, in fact $\capacity_{\text{ISM}} = \capacity$.
	
\chapter{Coin tossing analogy}
\label{sec:cointossing}

Although it doesn't apply directly to interstellar communication, the
 analogy between the discovery of a continuous-time signal $h(t)$ in AWGN
 and the discovery of a specific binary sequence in the presence of noise created by
 random coin tosses may be helpful to intuition.
 This analogy explains in a simple and less-mathematical way why the shape of $h(t)$ \emph{doesn't} matter for
 detection in noise, and also why the shape of $h(t)$ \emph{does} matter with respect to interference immunity.
 
\section{Discrete matched filter}

Consider a reception which consists of a sequence of $K$ 
elements, where each element is either a HEAD or a TAIL,
\begin{equation}
r_{k} =
\begin{cases}
\ \ h_{k} \,, & \text{signal} \\
\ \ n_{k} \,, & \text{noise} \,.
\end{cases}
\end{equation}
We know that $n_{k}$ is generated randomly by nature, and can be modeled as
a sequence of statistically independent fair coin tosses.
Thus, each possible sequence $\{ n_{k} , \, 1 \le k \le K \}$ is equally likely
with probability $2^{\,- K}$.
In the other case, signal $\{ h_{k} , \, 1 \le k \le K \}$ is presumed to have been generated
by some technological means, rather than a natural process.
Our goal is to observe $\{ r_{k} , \, 1 \le k \le K \}$ and make a decision between
signal and noise.
One might surmise that one distinguishing characteristic of a technologically-generated
signal is that it was generated by an algorithm, or sequence of steps that could
be executed by a software program or generated by a piece of Boolean hardware.

Unfortunately there is no practical way to identify whether 
$\{ r_{k}  \}$ was generated by an algorithm, without making much
stronger assumptions about the characteristics of that algorithm.
For example, if the Boolean hardware consisted of a memory storing a sequence
$\{ h_{k} \}$, then that hardware could generate literally any
sequence $\{ r_{k} \}$.
If no assumptions are made, any $\{ r_{k} \}$ could have been generated
by noise with probability $2^{\,-K}$.

If on the other hand, if it is known that the signal is a single unique sequence
(or this is correctly guessed),
then the detection algorithm can simply compare $\{ r_{k} \}$ to that $\{ h_{k} \}$
and declare signal if there is agreement in all $K$ positions of the sequence.
In that case, the probability of detection is $\pd = 1$.
On the other hand, the detector will incorrectly declare signal if $\{ n_{k} \}$ happens to
replicate $\{ r_{k} \}$ precisely, which occurs with probability $2^{\,-K}$.
Thus, the false alarm probability is $\pfa = 2^{\,-K}$.
The important point is that this detector performance does not depend on
the signal sequence $\{ h_{k} \}$, because the noise $\{ n_{k} \}$ is completely random
and it can replicate any $\{ h_{k} \}$ with the same probability.
This is analogous to our result that the waveform $h(t)$ does not matter
in the presence of AWGN (which is also completely random).

Suppose due to our uncertainty about  $\{ h_{k} \}$, we allow the signal to be
any one of $N > 1$ specific sequences (or corresponding algorithms).
In this case it remains that $\pd = 1$ if one of those sequences is valid.
However, $\pfa$ increases with $N$, since  $\{ n_{k} \}$ can more easily replicate
one of $N$ sequences. In the limit as $N \to 2^{K}$, $\pfa \to 1$.
This illustrates why the detector must keep $N$ small to keep $\pfa$ under control.

%The first case to consider is where the algorithm is unknown.
%There is no way to tell for sure, because the random generation can result in the observed
%sequence with probability $2^{-K}$.
%However, there are telltale signs that a sequence is not randomly generated based on the
%presence of recognizable patterns.
%For example, a sequence consisting of $K/2$ zeros followed by $K/2$ ones is less likely to
%have been generated randomly than a sequence that shows no discernible pattern.
%This method cannot, however, be applied to distinguishing coin tosses from an
%algorithm, because there are algorithms (called pseudorandom generators) that generate
%sequences that reliably meet all tests of randomness.
%For example, a binary expansion of the irrational number $\pi$ has this characteristic.
%Thus, if we truly know nothing about the algorithm used, then we have to conclude that
%\emph{any} sequence $\esv r$ is potentially algorithmic.
%
%Now change the premise to say that the goal is to distinguish a random sequence from
%a \emph{specific} sequence $\{ h_{k} ,\, \ 1 \le k \le K \}$.
%This is much easier, because a simple pattern matching can be applied.
%For example, merely calculate the number of places where $\{ r_{k} \, \ 1 \le k \le K \}$
%and $\{ h_{k} \, \ 1 \le k \le K \}$ agree.
%This is the matched filter test for this problem.
%If the sequence was in fact $\{ h_{k} \, \ 1 \le k \le K \}$, then the result will be $K$ matches precisely.
%However, if the result is $K$ matches, we cannot be certain that the sequence was not generated
%randomly, since a random sequence will match $K$ times with probability $2^{-K}$,
%and this will be true regardless of what $\{ h_{k} \, \ 1 \le k \le K \}$ we started with.
%The subtlety here is that it does not matter what $\{ h_{k} \, \ 1 \le k \le K \}$ was presumed.
%It can be all zero's, or all one's, or something that meets statistical tests of randomness
%like the binary expansion of $\pi$.
%The reliability of distinguishing it from randomness is the same; namely,
%we can say that it was algorithmic with a reliability on the order of one part in $2^{K}$.
%The reliability of the MF improves as $K$ increases, and if $K$ is large, it is pretty darn reliable.
%
%There is another lesson to take away from this analogy.
%In trying to distinguish nature (completely random coin tosses) from technology (algorithm), it is really helpful to have
%a \emph{unique} algorithm in mind, or at least a relatively small set of algorithms.

\section{Immunity to discrete interference}

Consider now a very different challenge,
\begin{equation}
r_{k} =
\begin{cases}
\ \ h_{k} \,, & \text{signal} \\
\ \ i_{k} \,, & \text{interferece} \,,
\end{cases}
\end{equation}
where the noise sequence has been replaced by
$\{ i_{k} , \, 1 \le k \le K \}$, an unknown interference.
(Interference, when present,
is likely to be much larger than the noise, and thus
it is not unreasonable to assume that the receiver has to deal
with interference, or noise, but not both at the same time.)
The question is how we can choose signal $\{ h_{k} \}$
to make it unlikely to be replicated by $\{ i_{k} \}$,
but without knowledge of $\{ i_{k} \}$.
The transmitter designers have no knowledge of the origin of $\{ i_{k} \}$,
and thus are unwilling to even make any assumptions about its statistics.
We define the transmitter's challenge as somehow choosing $\{ h_{k} \}$
so that the false alarm probability $\pfa = 2^{\,-K}$ is a constant,
independent of $\{ i_{k} \}$ and with the same $\pfa$ as we saw with noise.
As just seen, the choice of $\{ h_{k} \}$ doesn't matter when it comes to noise,
so the transmitter is free to choose $\{ h_{k} \}$ any way we choose.

The following way of choosing $\{ h_{k} \}$ satisfies our goals.
Choose $\{ h_{k} \}$ randomly by performing $K$ independent fair coin tosses.
Having determined $\{ h_{k} \}$ in this manner, the choice of $\{ h_{k} \}$ can be shared with the receiver.
(In practice $\{ h_{k} \}$ would be generated by a pseudo-random coin toss generator,
and the receiver would have to guess or infer that algorithm and generate the same
sequence $\{ h_{k} \}$ itself.)
 where it is compared with $\{ r_{k} \}$, our discrete MF algorithm.
Now $\pfa$ is the probability that $K$ coin tosses exactly match
$\{ i_{k} \}$, which is $\pfa = 2^{\,-K}$, the same for any $\{ i_{k} \}$.
Thus, the detector performance is identically the same for noise and interference,
regardless of the interference.
If $\{ h_{k} \}$ where chosen in any other way, such as another random ensemble
with different statistics, then some interferers $\{ i_{k} \}$ would
be replicated by $\{ h_{k} \}$ with higher probability than others.

\chapter{Analysis of communication reliability}
\label{sec:performancecalc}

As in discovery, we limit our analysis to the simpler Rayleigh fading case,
where closed-form results are obtainable.
Throughout a random variable $V$ will be a normalized complex-valued Gaussian random variable with
\begin{equation}
\expec{V} = \expec{V^{2}} = 0 \ \ \ \text{and} \ \ \ \expec{|V|^{2}} =2 \,.
\end{equation}
Then the random variable
\begin{equation}
X = \left| \sqrt{\xi} + V \right|^{2}
\end{equation}
is a non-central $\chi^2$ random variable with non-centrality parameter $\xi$
and two degrees of freedom.,
and for $\ecrb = 0$ it is a central $\chi^2$ random variable with two degrees of freedom.
Write this as $X \sim \chi^{2} (\xi)$, and let the
probability density and cumulative distribution functions be
$f (\xi,x)$ and $F (\xi,x)$.
The moment generating
function is
\begin{equation}
\mathcal M (\xi, t) = \expec{e^{t X}} = \frac{\displaystyle e^{\frac{ \xi  \, t}{1-2 \, t}}}{1-2 \, t}
\ \ \ \text{for} \ \ \  2\,  t < 1 \,.
\end{equation}


\section{Multilevel OOK}
\label{sec:multillevelOOK}

For amplitude modulation without channel coding,
and with a single-use ICH, the data symbol $A$ must be real-valued with $A \ge 0$.
Due to scintillation $S$, the MF output $Z$ offers no insight into the sign or phase of $A$.

In Section \ref{sec:channelcoding}, consider a more general data symbol constellation
$A_{k} \in \{  n , \, 0 \le n \le N-1 \}$.
If each point in the constellation is equally likely, then the average
energy in each symbol is
\begin{equation}
\recenergy \cdot \expec{A^{2}} = \recenergy \cdot \frac{(2 N - 1)(N-1)}{6}
\end{equation}
and the information embedded in each symbol is $\log_{\,2} N$.
The power efficiency is the
ratio the latter to the former, and it is maximized by $N = 2$.
For example, choosing $N=4$ (two bits per symbol) reduces the
power efficiency relative to $N=2$ by a factor of 3.5 (5.4 dB).

%\section{Determination of thresholds}
%
%From \eqref{eq:rayleighdist}, the outage probability is
%\begin{equation}
%\label{eq:outageprob}
%\po = \prob{ R < \oot }
%= 1 - e^{- \oot^{\,2} / \vs } \,.
%\end{equation}

%\section{Second-order statistics of MF output}
%
%The probability of error $\pe$ for the decision variable
% $Q$ defined in \eqref{eq:Qdec} can be estimated by making a Gaussian approximation.
%$Q$ has a non-central $\chi^{2}$ distribution.
%If $\snre$ is defined by \eqref{eq:snare}, the first and second-order moments of $Q$
%conditioned on data symbol $A = a$ are
%\begin{align}
%&\mu (a) =  2 + 2 \, a^{2} \, \ecrs \, \frac{\oot}{\vs} \\
%&\sigma^{2} (a) = 4 + 8 \, a^{2} \, \ecrs \, \frac{\oot}{\vs}\,.
%\end{align}
%The first and second order statistics of $Q^{2}$ are
%\begin{align}
%&\mu (r,a) = E[Q^{2} \left. \right| R = r , A = a ] = N_{0} + \recenergy \, r^{2} \, a^{2} \\
%&\sigma (r,a) = \sqrt{ \text{Var} \{ Q^{2}  \left. \right| R = r , A = a \} }
%= \sqrt{ N_{0} \left( N_{0} + 2 \, \recenergy \, r^{2} \, a^{2} \right) } \,.
%\end{align}

%\section{Detection probability}
%
%For $\pd$, the criterion $Q > \hht$ is equivalent to $Q^{2} > \hht^{\,2}$.
%Our objective is a snapshot at the threshold of outage $R = \oot$.
%Then,
%\begin{equation}
%\pd =
%\prob{ Q^{2} > \hht^{2} \left. \right| R = \oot, A = 1 } = 
%\prob{ \frac{Q^{2} - \mu (\oot, 1)}{\sigma (\oot,1)} > - \frac{\mu (\oot, 1) - \hht^{2}}{\sigma (\oot,1)} } \,.
%\end{equation}
%When $Q^{2}$ is assumed to be Gaussian,
%the l.h.s. is a zero-mean unit-variance Gaussian random variable, 
%so the value of $\pd$ is entirely represented by the
%quantity on the r.h.s.
%Assume that $\mu (\oot, 1) \ge \hht^{2}$, or in other words restrict consideration to
%the regime where $\pd \ge 1/2$.
%This is equivalent to $\left( 1+\ecrs > \log_{e} (1/\pfa) \right)$ for the $\ecrs$
%defined in \eqref{eq:snr0}.
%It is common to represent $\pd$ by the SNR measure
%\begin{equation}
%\snrd =
%\left( \frac{ \mu (\oot, 1) -  \hht^{2} }{\sigma (\oot,1)} \right)^{2}
%= \frac{\left(\recenergy \, \lambda _O^2-\lambda_H^2+
%N_{0}\right){}^2}{N_{0} \left(2 \, \recenergy \, \lambda_O^2+N_{0}\right)} \,.
%\end{equation}

%Assuming that any hit occurring when $A = 0$ is categorized as a false alarm,
%and that the detector is not penalized for failure to discover the signal during outages,
%at the threshold of outage ($R = \oot$) the discovery probability is
%\begin{align}
%\pd = \prob{ Q > \hht \left. \right| R = \oot , A = 1}
%&=  \prob{ \left| \sqrt{\recenergy} \, \oot + M \right| > \hht } \\
%&> \prob{ \Re \{ M \} > \hht - \sqrt{\recenergy} \, \oot }
% \,.
%\end{align}
%This lower bound is reasonably tight, so it will be used to characterize
%the tradeoff.
%\begin{equation}
%\snrd = \frac{ ( \hht - \sqrt{\recenergy} \, \oot )^2 }{N_0 /2}
%\end{equation}

\section{Probability of error of OOK}
\label{sec:peook}

Assume that detector distinguishes $A=0$ from $A =1$ by applying \eqref{eq:normalMFook}
to a threshold $\lambda$.
The decision threshold can be set halfway between the two mean values,
or $\lambda = 2 \, \ecro + 2$.
The error probability is then
\begin{align}
\pe &= 
\frac{1}{2} \cdot \prob{|V|^{2} > \lambda} +  \frac{1}{2} \cdot \prob{|\sqrt{4 \, \ecro} + V|^{2} \le \lambda} \\
&= \frac{1}{2} \cdot (1 - F(0, \, 2 \, \ecro + 2) ) +  \frac{1}{2} \cdot F(4 \, \ecro , \, 2 \, \ecro + 2) \,.
\end{align}

%Start with the simple OOK case.
%Our characterization of $\pe$ will be at the threshold of outage, so
%the decision variable is
%\begin{equation}
%|Z|^{2} = \left| \sqrt{\energy \, \oot} \, A + M \right|^{2} \,.
%\end{equation}
%Without changing $\pe$, this can be scaled to
%\begin{equation}
%|Z|^{2} = \left| \sqrt{2 \, \ecrs \, \oot} \, A + V \right|^{2}
%\end{equation}
%where $V$ is normalized as above.
%A reasonable threshold falls halfway between the mean values
%under $A = 0$ and $A = 1$, or $( 2 + \ecrs \, \oot$).
%Assuming $A = 0$ and $A = 1$ are equally likely, $\pe$ becomes
%\begin{equation}
%\pe = \frac{1}{2} \cdot ( 1 - F (0, 2 + \ecrs \, \oot ) ) +  \frac{1}{2} F ( 2 \, \ecrs \, \oot  , 2 + \ecrs \, \oot ) 
%\end{equation}
%When $\energy_{h} = 2 \, \energybit$, this becomes
%\begin{equation}
%\pe = \frac{1}{2} \cdot ( 1 - F (0, 2 + 2 \, \snr_{b} \, \oot ) ) +  \frac{1}{2} F ( 4 \, \snr_{b} \, \oot  , 2 + 2 \, \snr_{b} \, \oot ) 
%\end{equation}
%This is the value plotted in Figure \ref{fig:peOOKvsPPM}, where it is compared to PPM.

%and the threshold of decision is $\ddt$,
%the probability of error is
%\begin{equation}
%\pe = \frac{1}{2} \cdot \prob{| M |^{2} > \ddt}
%+ \frac{1}{2} \cdot \prob{ \left| \, \sqrt{ \recenergy \, \oot } + M \, \right|^{2} < \ddt } 
%\,,
%\end{equation}
%where $\oot$ is the received flux at the threshold of outage.
%Defining a normalized variable $V$ with real and imaginary parts
%that are unit-variance Gaussian, $\pe$ can be written as
%\begin{equation}
%\pe =  \frac{1}{2} \cdot \prob{| U |^{2} > \frac{ 2 \, \ddt}{N_{0}} }
%+ \frac{1}{2} \cdot \prob{ \left| \, \sqrt{2 \, \snro } + U \,  \right|^{2} <  \frac{ 2 \, \ddt}{N_{0}}  } 
%\end{equation}
%where $\snro$ is the SNR at the outage threshold and is defined in \eqref{eq:snro}.
%A reasonable choice for  $\oot$ is midway between the mean values, or
%$\ddt = N_{0} + 2 \recenergy \oot$, and with that choice $\pe$ becomes
%\begin{align}
%\pe &=  \frac{1}{2} \cdot \prob{| U |^{2} > 2 + \snro }
%+ \frac{1}{2} \cdot \prob{ \left| \, \sqrt{2 \, \snro } + U \,  \right|^{2} <  2 +\snro }  \\
%&= \frac{1}{2} \cdot \left( 1 - F_U (0,2 + \snro) \right)
%+ \frac{1}{2} \cdot F_U ( 2 \, \snro, 2 + \snro ) \,.
%\end{align}
%Note that $\pe$ is determined by the single parameter $\snro$, and thus
%keeping $\snro$ fixed (while other parameters are varied) will keep $\pe$ fixed.

%Since the distribution $Q$ can't be expressed in closed form,
% $\pe$ will be approximated assuming that $Q$ is
%Gaussian.
%
%
%Assume the threshold $\ddt$
% is positioned the same number of standard deviations $\alpha$ from the mean values,
% \begin{equation}
%\begin{matrix}
%\mu (0 ) + \alpha \cdot \sigma (0) = \ddt \\
%\mu (1) = \ddt + \alpha \cdot \sigma (1)
%\end{matrix}
%\ \ \ \ \ \text{or} \ \ \ \ 
%\alpha = \frac{\mu (1)-\mu (0 )}{\sigma (0) + \sigma (1)} \,.
%\end{equation}
%\begin{equation}
%\begin{matrix}
%\mu (\oot,0 ) + \alpha \cdot \sigma (\oot,0) = \ddt^{2} \\
%\mu (\oot,1) = \ddt^{2} + \alpha \cdot \sigma (\oot,1)
%\end{matrix}
%\ \ \ \ \ \text{or} \ \ \ \ 
%\alpha = \frac{\mu (\oot,1)-\mu (\oot,0 )}{\sigma (\oot,0) + \sigma (\oot,1)} \,.
%\end{equation}
%Assuming $A = \pm 1$ are equally likely,
%the probability of error
%\begin{align}
%\pe &\approx \frac{1}{2} \cdot \prob{\conditional{Q>\ddt}{A=0}}
%+  \frac{1}{2} \cdot \prob{\conditional{Q<\ddt}{A=1}} \\
%&= \frac{1}{2} \cdot \prob{\conditional{\frac{Q-\mu (0 )}{\sigma (0)}>\alpha}{A=0}}
%+ \frac{1}{2} \cdot  \prob{\conditional{\frac{Q-\mu (1 )}{\sigma (1)} < - \alpha}{A=1}} \\
%&=  \prob{\conditional{\frac{Q-\mu (0 )}{\sigma (0)}>\alpha}{A=0}} \,,
%\end{align}
%since the two types of error have equal probabilities.
%\begin{align}
%\pe &= \frac{1}{2} \cdot \prob{\conditional{Q^{2}>\ddt^{2}}{\hyp{0}}}
%+  \frac{1}{2} \cdot \prob{\conditional{Q^{2}<\ddt^{2}}{\hyp{1}}} \\
%&= \frac{1}{2} \cdot \prob{\conditional{\frac{Q-\mu (0 )}{\sigma (0)}>\alpha}{\hyp{0}}}
%+ \frac{1}{2} \cdot  \prob{\conditional{\frac{Q-\mu (1 )}{\sigma (1)} < - \alpha}{\hyp{1}}} \\
%&=  \prob{\conditional{\frac{Q-\mu (0 )}{\sigma (0)}>\alpha}{\hyp{0}}} \,,
%\end{align}
%since the two types of error have equal probabilities.
%This is expressed in terms of a normal Gaussian random variable (zero mean and unit variance),
%so $\pe$ can be represented by $\alpha$, which is given in \eqref{eq:alphape}.


%In this case $\pe$ can be represented by SNR
%\begin{equation}
%\snre = \left( \frac{\mu (\oot,1)-\mu (\oot,0 )}{\sigma (\oot,0) + \sigma (\oot,1)}
%\right)^{2}
%= \left(
%\frac{\recenergy \, \lambda _O^2}{\sqrt{N_{0} \left(2
%   \recenergy \, \lambda_O^2+N_{0}\right)}+\sqrt{N_{0}^2}}
%   \right)^{2} \,.
%\end{equation}
%Substituting from \eqref{eq:pfa}, \eqref{eq:outageprob} and \eqref{eq:snr0},
%$\snrd$ simplifies to \eqref{eq:snrd} and $\snre$ simplifies to \eqref{eq:snre}.
%Note also that $\pe = 1-\pd$ for the same SNR values $\snre = \snrd$,
%and thus both probabilities can share the same plot as in Figure \ref{fig:pEvsSNR}.

%\section{Independent observations during discovery}
%
%Assume $N$ independent observations $\{ Z_{1}, Z_{2}, \dots \, Z_{N} \}$ of a MF output,
%where each observation is a complex-valued random variable with statistics given by \eqref{eq:Zstats}.
%The overall probability of a miss $(1-\pd (N))$ probability that there is no hit in all $N$ observations is
%\begin{equation}
%1- \pd = \prob{ |Z_{1}| < \hht , |Z_{2}| < \hht, \dots \, |Z_{N}| < \hht}
%=  \left( \prob{ |Z| < \hht} \right)^{N} \,.
%\end{equation}
%Since $|Z|$ has a Rayleigh distribution,
%\begin{equation}
% \prob{ |Z| < \hht} = 1 - \exp \left\{ - \frac{\hht^{2}}{\recenergy \, \vs + N_{0}} \right\} \,.
%\end{equation}
%Thus,
%\begin{equation}
%\pd = 1 - \left(  1 - \exp \left\{ - \frac{\hht^{2}}{\recenergy \, \vs + N_{0}} \right\} \right)^{N}
%\overset{N \to \infty}{\longrightarrow} 1
%\end{equation}



%Substituting from \eqref{eq:pfa}, \eqref{eq:outageprob}, and \eqref{eq:snr0},
%this simplifies to
%\begin{equation}
%\snrd = \frac
%{\left( 1 + \log \pfa + \ecrs \right)^{2}}
%{1 + 2 \, \ecrs} \,.
%\end{equation}
%
%The $\pe$ is also a snap lot calculated for $R = \oot$, using a decision threshold $\ddt$.
%For this case the MF output is
%\begin{equation}
%Q = \left| \sqrt{\recenergy} \, \oot \, A + M \right| \,.
%\end{equation}
%The average of $Q^2$ under the two hypotheses is
%\begin{equation}
%E[ \, Q^2 \left. \right| A=0 \, ] = 
%\ \ \ \ \text{and} \ \ \ \ \
%E[ \, Q^2 \left. \right| A=1 \, ] =
%\end{equation}
%Although $Q^2$ is not Gaussian, in terms of understanding
%the tradeoffs between $\{ \}$ is expressed in the SNR
%\begin{equation}
%\snr = \frac{ 
%( E[ \, Q^2 \left. \right| A=1 \, ] - E[ \, Q^2 \left. \right| A=0 \, ] )^2 }
%{\text{Var} \{ Q^2 \}}
%\end{equation}
%
%There are two types of error.
%Conditioned on $A = 0$, $Q$ is Rayleigh,
%\begin{equation}
%\prob{Q > \ddt \left. \right| A = 0} = \exp \left\{ - \frac{\ddt^{\,2}}{N_{0}} \right\}
%\end{equation}
%Conditioned on $A = 1$, $Q$ is non-central $\chi$, which cannot be expressed in closed form.
%However, the error probability is easily bounded for the 
%regime of interest in which $\sqrt{\recenergy} \, \oot  > \ddt$,
%\begin{align}
%\prob{Q < \ddt  \left. \right| A = 1} &= \prob{ \left|  \sqrt{\recenergy} \, \oot + M \right| < \ddt} \\
%&\le 1 - \prob{ \left| M \right| <  \sqrt{\recenergy} \, \oot  - \ddt} = e^{ - ( \sqrt{\recenergy} \, \oot  - \ddt)^{2} / N_{0}}
%\,.
%\end{align}
%The two types of error are equally likely if the threshold is halfway between
%the two signal conditions, or $\ddt =  \sqrt{\recenergy} \, \oot / 2$.
%In that case,
%\begin{equation}
%\label{eq:ookpe}
%\pe < \exp \left\{ - \frac{\recenergy \oot^{\,2}}{4 \, N_{0}} \right\}
%\end{equation}
%Assuming equality in \eqref{eq:ookpe} and combining with \eqref{eq:outageprob},
%\eqref{eq:p0rate}, and \eqref{eq:erpower}
%results in \eqref{eq:powerefficbinary}.

%\begin{align}
%\pd = \prob{ Q > \hht \left. \right| R > \oot , A = 1}
%&=  \prob{ \left| \sqrt{\recenergy} \, R + M \right| > \hht \left. \right| R > \oot } \\
%& = \int_{\oot}^{\infty}  \prob{ \left| \sqrt{\recenergy} \, r + M \right| > \hht } \, f_{R} (r) \, dr \,.
%\end{align}
%Note that it is guaranteed that $ \sqrt{\recenergy} \, r > \hht$ within the limits of integration.
%Because of that, the integrand is bounded by
%\begin{equation}
% \prob{ \left| \sqrt{\recenergy} \, r + M \right| > \hht } >
%\prob{|M| <  \sqrt{\recenergy} \, r - \hht}
%= 1 -  \exp \left\{ - \frac{\left( \sqrt{\recenergy} \, r - \hht \right)^{2} }{N_{0}} \right\}
%\end{equation}



% from \eqref{eq:dtmodel} to a threshold for the signal magnitude $R = \oot$.
%The statistics of $Z$ do not depend on $\Theta$, and hence it is acceptable to set $\Theta = 0$.
%The resulting values under the two hypotheses is
%\begin{equation}
%|Z|^{2} = \begin{cases}
%\ | M |^{2} \,, & A = 0 \\
%\ \left| \sqrt{\recenergy} \, \oot + M \right|^{2} \,, & A = 1 \;.
%\end{cases}
%\end{equation}
%The distribution is non-central $\chi^{2}$, for which there is no closed form expression.
%While $\pe$ can be calculated numerically, for our purposes it should suffice
%to base our choice of thresholds on second-order statistics.
%Define 
%\begin{equation}
%E|Z|^2 = \begin{cases}
%\ \mu_0 \,, & A = 0 \\
%\ \mu_1 \,, & A = 1
%\end{cases}
%\ \ \ \text{and} \ \ \ \ 
%\text{Var} |Z|^2 = \begin{cases}
%\ \sigma_0^2 \,, & A = 0 \\
%\ \sigma_1^2 \,, & A = 1 \,,
%\end{cases}
%\end{equation}
%in which case
%\begin{equation}
%\mu_1 = \recenergy \, \oot^{\,2}+N_0
%\ \ \ \text{and} \ \ \ \ 
%\sigma_1^{\,2} = N_0 \left(2 \, \recenergy \, \oot^{\,2} + N_0 \right) \,.
%\end{equation}
%The regime of fixed error probability can be approximated
%by fixing the number of standard deviations between mean value and threshold.
%For a parameter $\alpha$ and for a decision threshold
%$\lambda_d$ that controls the probability of error,
%we choose $\oot$ such that
%\begin{equation}
%\lambda_d = \mu_0 + \alpha \cdot \sigma_0
%\ \ \ \text{and} \ \ \ \ 
%\mu_1 = \lambda_d + \alpha \cdot \sigma_1 \,.
%\end{equation}
%Eliminating $\lambda_d$,
%\begin{equation}
%\mu_1 - \mu_0 = \alpha \cdot ( \sigma_0 + \sigma_1) \,.
%\end{equation}
%Substituting for the moments, the received energy should be set at
%\begin{equation}
%\frac{\recenergy}{N_0} = \frac{2 \, \alpha ( \alpha + 1)}{\oot^{\,2}} \,.
%\end{equation}
%Simultaneous solution of this equation
%together with \eqref{eq:outageprob}, \eqref{eq:p0rate}, and \eqref{eq:erpower}
%results in \eqref{eq:powerefficbinary}.

%\chapter{Discovery in the presence of dispersion}
%\label{sec:ipd}
%
%The $\pfa$ and $\pd$ during discovery using estimate \eqref{eq:Q} will be characterized.
%The first issue is $\tmax$, because
%strictly speaking a bandlimited $R_h (t)$ cannot also be time-limited.
%The fraction of the energy in $R_{h} (t)$ falling in time window $t \in [ -\alpha/B , +\alpha/B ]$
%is plotted in Figure \ref{fig:energyVsTime}.
%Choosing $\tmax = 2\,\alpha /B + \tau_s$, only a fraction of a dB of the total energy is lost
%for $\alpha \ge 1$.
%It is assumed that the $t=0$ point in \eqref{eq:Q} coincides with the
%beginning of significant energy in $R_h (t)$, time shifting the signal if necessary.
%
%\incfig
%	{energyVsTime}
%	{.6}
%	{The fraction of the total energy in waveform $R_h (t)$
%	at the output of the matched filter
%	(expressed in dB)  in a time interval of
%	length $2 \alpha /B$ as a function of $\alpha$.
%	The choice $\alpha = 1$ (the entire main lobe),
%	captures all but a fraction of a dB of the energy.}
%
%Although $Q$ in \eqref{eq:Q} is not Gaussian, it can be approximated as such
%using \eqref{eq:snrQdef} as a proxy for $\pfa$ and $\pd$ with
%$d_{\min} = \left( E[Q] - \left. E[Q] \right|_{\recenergy = 0} \right)$.
%Assuming $\Theta = 0$, the moments are
%\begin{subequations}
%\begin{align}
%\label{eq:meanQ}
%&E[Q] = \int_{0}^{\tmax} E | Z(t) |^{2} \, dt \\
%\label{eq:varQ}
%&\text{Var} [Q] = \int_{0}^{\tmax} \int_{0}^{\tmax} 
%\left( 
%E \left[ | Z(u) |^{2} \cdot | Z(v) |^{2} \right] -
%E | Z(u) |^{2} \cdot E | Z(v) |^{2}
%\right) \, du \, dv \,.
%\end{align}
%\end{subequations}
%$\text{Var} [Q]$ depends on $\recenergy$, so there are actually two versions 
%of $\snr_{Q} $ in \eqref{eq:snrQdef} depending on whether $\recenergy = 0$ or 
%(the one used here) $\recenergy > 0$.
%Based on Appendix \ref{sec:qam},
%the covariance matrix of the noise is
%\begin{align}
%\notag
%&\esv M = \trans{[ \, M_{r} (u), \, M_{i} (u), \, M_{r} (v), \, M_{i} (v) \, ]} \\
%\label{eq:corrmatrix}
%&E [ \esv M \, \trans{\esv M} ] = 
%\begin{bmatrix}
%R_{r} (0) & 0 & R_{r} (u-v) & R_{ri} (u-v) \\
%0 & R_{r} (0) & - R_{ri} (u-v) & R_{r} (u-v) \\
%R_{r} (u-v) & - R_{ri} (u-v) & R_{r} (0) & 0 \\
%R_{ri} (u-v) & R_{r} (u-v) & 0 & R_{r} (0)
%\end{bmatrix}
%\,.
%\end{align}
%Substituting \eqref{eq:meanQ} and \eqref{eq:varQ} into \eqref{eq:snrQdef},
%\begin{align*}
%&E[Q] - \left. E[Q] \right|_{\recenergy = 0}  = \beta_{1} \, \recenergy \\
%&\text{Var} [Q] = \beta_{2} \, N_{0}^{\,2} + 2 \beta_{3} \, N_{0} \, \recenergy 
%\end{align*}
%where the constants are determined by the \eqref{eq:corrmatrix} and \eqref{eq:corrcond} as
%\begin{align*}
%&\beta_{1} = \int_{0}^{\tmax} | R_h (\tau) |^{2} \, d \tau 
%\approx 1/B
%\\
%&\beta_{2} =  \int_{0}^{\tmax} \int_{0}^{\tmax}  | R_h (u-v) |^{2}  \, du \, dv 
%\approx \tmax / B
%\\
%&\beta_{3} =  \int_{0}^{\tmax} \int_{0}^{\tmax} s(u,v)  \, du \, dv
%\approx 1/ B^{\,2}
%\\
%&s(u,v) =  R_{h,i} (u) \, R_{h,i} (u-v) \, R_{h,r} (v) +
%R_{h,i} (u) \, R_{h,i} (v) \, R_{h,r} (u-v) -
%\\
%&\ \ \ \ R_{h,i} (u-v) \, R_{h,i} (v) \, R_{h,r} (u) +
%R_{h,r} (u) \, R_{h,r} (u-v) \, R_{h,r} (v) \\
%&\ \ \ \ = \text{sinc} (\pi \, B \, u) \cdot \text{sinc} (\pi \, B \, v)  \cdot \text{sinc} (\pi \, B \, (u-v)) \,.
%\end{align*}
%The approximations assume that $|R_h (\tau)|^{2} \approx (1/B) \cdot \delta (\tau)$
%and that the integrals over $t \in [0,\tmax]$ can be approximated by
%integrals over $t \in [-\infty,\infty]$.
%Substituting into \eqref{eq:snrQdef} yields \eqref{eq:snrQ}.

\section{Probability of error of M-ary FSK}
\label{sec:peppm}

%A normalized version of \eqref{},
%\begin{equation}
%Z_m = \begin{cases}
%\sqrt{2 \, \log_{2} M \cdot \snr_{b}} + V_m \,, & m = M \\
%V_m \,, & 1 \le m \le M-1 \,.
%\end{cases}
%\end{equation}
%
%In \eqref{eq:peppm} $\pe$ is not affected if the variables are normalized,
%\begin{align}
%\label{eq:peppmnorm}
%1-\pe &= \prob{\max_{1 \le m \le M-1} | V_m |^2 < | V_{M} |^2} \\
%&= \prob{  \bigcap_{m=1}^{M-1} \left( | V_m |^2 < x \right)} f( 2 \, \log_{2} M \cdot \snr_{b} ,x)
%\end{align}
%By independence of the $\{ V_{m} \}$, 
%\begin{align}
%1-\pe &= F^{M-1} (0, x) \cdot f( 2 \, \log_{2} M \cdot \snr_{b} ,x) \\
%&=
%\end{align}
%
%
%
%Finally, this probability can be determined by conditioning on $| V_M |^2 = x$,
%\begin{align}
%\prob{ | V_{1} |^2 <| V_M |^2}
%&= F(0,x) f( 2 \log_{2} M \cdot \snr_{b}  , x) 
%= \left( 1 - e^{-x / 2}\right) \cdot f( 2 \log_{2} M \cdot \snr_{b}  , x) \\
%&= \mathcal M (-1/2, 2 \log_{2} M \cdot \snr_{b} ) \,.
%\end{align}
%Substituting for $\mathcal M ( \cdot, \cdot)$, \eqref{eq:peppmfinal} results.
%
%\section{Asympototic reliability of PPM on the AWGN channel}
%\label{sec:PPMonAWGN}

For M-ary FSK, we will determine an upper bound on $\pe$ that is tight for small $\pe$.
For the normalized MF outputs \eqref{eq:mfoutfsk} the symbol error probability of \eqref{eq:peppm} becomes
\begin{align}
P_{\text{S}} &=
\prob{
\max_{1 \le m \le M-1} | V_m |^2 > \left| \sqrt{2 \, \log_2 M \cdot \ecro} + V_{M} \right|^2
} \\
&= \prob{
\bigcup_{m = 1}^{M-1} \left( |V_m|^2 >  
\left| \sqrt{2 \, \log_2 M \, \ecro} + V_{M} \right|^2 \right)
} \\
&= \int_{0}^{\infty} \prob{ \bigcup_{m = 1}^{M-1} \left( |V_m|^2 >  x \right) }
f ( 2 \, \log_2 M \, \ecro , \, x ) \, dx
\,.
\end{align}
The union bound
replaces the union by a sum,
\begin{align}
\notag
P_{\text{S}}   &\le
\sum_{m = 1}^{M-1}  \int_{0}^{\infty} \prob{ |V_m|^2 > x } f ( 2 \, \log_2 M \, \ecro , x ) \, dx \\
\notag
 &= (M-1) \cdot  \int_{0}^{\infty} (1 - F(0,x) ) \cdot  f ( 2 \, \log_2 M \, \ecro  , x ) \, dx \\
 \notag
&= (M-1) \cdot \mathcal M ( 2 \, \log_2 M \, \ecro  \, , - 1/2 ) \\
\label{eq:bound1}
&= \frac{1}{2} \, (M-1) \, M^{-\frac{\ecro }{2 \, \log_{e} 2}}
 \,.
\end{align}
To calculate the bit error probability, 
conditional on there being a symbol error (and assuming $M$ is a power of two)
in any particular bit position in the symbol $M/2$ symbols disagree
and $M/2$ symbols agree (including the correct symbols).
Since all $M-1$ incorrect symbols are equally likely, the
conditional probability of bit error is $M/2$ divided by $M-1$, and
\begin{equation}
\label{eq:symboltobit}
\pe = \frac{M/2}{M-1} \cdot P_{\text{S}} \,.
\end{equation}
Combining \eqref{eq:bound1} and \eqref{eq:symboltobit} the result is \eqref{eq:peFSKbound}.

\chapter{Analysis of discovery}
\label{sec:discprob}

\section{Detection probability for single observation}
\label{sec:discprobsingle}

Consider the decision variable $Q$ is given by \eqref{eq:QR1K}.
An equivalent condition to $Q > \lambda$ is
\begin{equation}
\label{eq:discoverytest1}
(1 - \lambda) \cdot 
\left| \, \sqrt{\recenergy} \, \left( \sqrt{\,\gamma \,} \, \sigma_{s} \, e^{\,i\,\psi} + \sqrt{\,1-\gamma\,} \, S \right) + M_{1} \, \right|^{2} > \lambda \cdot \sum_{k=2}^{K} \left| M_{k} \right|^{2} 
\,.
\end{equation}
Specular phase $\psi$ does not affect the statistics, so set $\psi = 0$.
Define a normalized noise $V_{k} = M_{k} / \sqrt{N_{0}/2}$ with
unit-variance real and imaginary parts.
Then \eqref{eq:discoverytest1} becomes
\begin{equation}
\label{eq:discoverytest2}
\frac{1 - \lambda}{\lambda} \cdot V > W
\end{equation}
where
\begin{align}
V &= \left| \, \sqrt{\frac{2 \, \recenergy}{N_{0}}} \, \left( \sqrt{\,\gamma \,} \, \sigma_{s} + \sqrt{\,1-\gamma\,} \, S \right) + V_{1} \, \right|^{2} \\
W &=  \sum_{k=2}^{K} \left| V_{k} \right|^{2} 
\end{align}

The distribution $W$ is $\chi^{2}$ with $(2 \, K - 1)$ degrees of freedom,
and only the statistics of $V$ depend on the parameters of the model.
Since the statistics of $W$ are divorced from all the parameters, this
relation demonstrates how $Q$ is sensitive to the signal-to-noise ratio
$\ecrs$ rather than signal and noise energies individually.

%An equivalent condition to $Q > \lambda$ is
%\begin{equation}
%\label{eq:discoverytest}
%(1 - \lambda) \cdot 
%\left| \sqrt{\recenergy} \, S + M_{1} \right|^{2} > \lambda \cdot \sum_{k=2}^{K} \left| M_{k} \right|^{2} 
%\,.
%\end{equation}

\subsection{Rayleigh fading}
\label{sec:discoveryrayleigh}

For $\gamma = 0$, closed-form results for
false alarm probability $\pfa$ and detection probability $\pd$ can be obtained.
The simplification for this case is that $( \sqrt{2 \, \recenergy/N_{0}} \, S + V_{1} )$ is a zero-mean
Gaussian random variable with variance $2 \, (1+\ecrs)$.
Hence \eqref{eq:discoverytest2} can be rewritten as
\begin{equation}
\label{eq:V1W}
\alpha \cdot \left| U_{1} \right|^{2} 
 > W
 \ \ \ \text{for} \ \ \ \
\alpha = \frac{1-\lambda}{\lambda} \cdot (1 + \ecrs)
\end{equation}
where $U_{1}$ is also a Gaussian random variable
with unit-variance real- and imaginary parts.
In \eqref{eq:V1W}
$\left| U_{1} \right|^{2}$ is $\chi^{2}$ with two degrees of freedom
and $W$ is $\chi^{2}$ with $(2 \, K - 2)$ degrees of freedom.
The probability of event \eqref{eq:V1W} is readily determined,
\begin{equation}
\label{eq:probQgl}
\pd
= \int F \left( \frac{w}{\alpha}, \, 2 \right) \, f (w, \, 2 K - 2) \, dw
= \left( \frac{\alpha}{1+\alpha} \right)^{K-1} 
 \,,
\end{equation}
where $F (x,n)$ and $f (x,n)$ are the cumulative distribution
and probability density functions for a $\chi^{2}$ distribution with $n$ degrees of freedom.
Then $\pfa$ equals \eqref{eq:probQgl} for $\ecrs = 0$, and
eliminating  $\lambda$ from these two relations yields \eqref{eq:pdvspfa}.

When $N_{0}$ is known, the probability of $Q = |R_{1}|^{2} > \lambda$ is
\begin{equation}
\pd = F \left( \frac{2 \, \lambda}{\recenergy \, \vs + N_{0}} , \, 2 \right) =
\exp \left\{ - \frac{\lambda}{\recenergy \, \vs + N_{0}} \right\} \,.
\end{equation}
Eliminating $\lambda$ to solve for $\pd$ in terms of $\pfa$ yields \eqref{eq:asympPfaVsPd}.

\subsection{Rician fading}
\label{sec:discoveryrician}

When $\gamma > 0$, $V$ in \eqref{eq:discoverytest2} is non-central $\chi^{2}$
with two degrees of freedom.
There is no easy closed-form expression for $\pd$ as in the Rayleigh fading case.
Our intuition that Rayleigh fading is ''worst case'' in the sense of being more
difficult case to discover (because of the absence of a specular component)
can be confirmed by calculating a signal-to-noise ratio.
The first and second moments of $V$ are
\begin{align}
&\expec{V} = 2 \, ( 1 + \ecrs ) \\
&\var{V} =  4 \, \left( 1 + 2 \, \ecrs + (1 - \gamma^{2} ) \, \ecrs^{\,2} \right) 
\,.
\end{align}
A larger $\pd$ and smaller $\pfa$ are associated with
a bigger difference between mean values (signal plus noise vs noise alone) and
a smaller standard deviation.
These effects can be captured in a signal-to-noise ratio measure
\begin{equation}
\snr_{\text{Rice}} =
\frac{\left( \expec{V} - \left. \expec{V} \right|_{\recenergy=0} \right)^{\,2}}{\var{V}} 
= \frac{\ecrs^{\,2}}{1 + 2 \, \ecrs + (1 - \gamma^{2}) \, \ecrs^{\,2}}
\,.
\end{equation}
$\snr_{\text{Rice}}$ is plotted in Figure \ref{fig:snrRician} for different values of $\gamma$.
It is notable how small $\snr_{\text{Rice}}$ is for small values of $\gamma$.
This is the influence of the increasing prominence of outages when the
Rayleigh case is approached.
However, $\snr_{\text{Rice}}$ improves as $\gamma$ gets larger, reflecting the
increasing discovery reliability, particularly for larger $\ecrs$.

\incfig
	{snrRician}
	{.8}
	{
	A plot of $\snr_{\text{Rice}}$ in dB vs $\ecrs$ in dB for $\gamma=0$ to $1$
	in steps of $0.1$. For a larger specular component ($\gamma$ larger)
	$\snr_{\text{Rice}}$ gets larger, reflecting the increasing reliability in signal flux
	due to the increasing proportion of flux arriving in the specular component.
	}

\section{Detection probability for multiple independent observations}
\label{sec:Lobs}

%\newcommand{\pfaLone}{P_{\text{FA},L=1}}
%\newcommand{\pdLone}{P_{\text{D},L=1}}
%\newcommand{\pfaNone}{P_{\text{FA},N=1}}
%\newcommand{\pdNone}{P_{\text{D},N=1}}

The discovery relation of \eqref{eq:discoveryequation} and \eqref{eq:pfaavspfa} will now be derived.
Consider three granularities of observation:
(a) individual energy bundle, (b) one contiguous observation window, and (c)
the collection of $L$ observations.
It is assumed that the received flux remains constant over a contiguous observation window,
but is statistically independent from one observation window to the next.
Let the probabilities at granularity (a) be  $\{ \pfaa, \, \pda \}$
and at granularity (c) $\{ \pfa, \, \pd \}$.
Thus,  $\{ \pfa, \, \pd \}$ reflect the overall sensitivity of the $L$-observation detector.

\subsection{Granularity of individual energy bundle}

The relationship between $pfaa$ and $\pda$ is given by \eqref{eq:asympPfaVsPd}.

The false alarm probability in the detection of a single bundle is
\begin{equation}
\pfaa = \prob{  \left| V_{1} \right|^{2} > \frac{2 \, \lambda}{N_{0}}  }
= \exp \left\{ - \frac{\lambda}{N_{0}} \right\} \,,
\end{equation}
and thus the normalized threshold is determined as
\begin{equation}
\frac{\lambda}{N_{0}} = - \log_{e} \pfaa \,.
\end{equation}

%The relationship between $\pfaa$ and $\pda$ is given by
%\eqref{eq:asympPfaVsPd},
%\begin{equation}
%\label{eq:pfavspd}
%\pda = 
%\pfaa^{\, \frac{1}{1+ \ecrs}} \,.
%\end{equation}

\subsection{Granularity of individual observation}

Suppose that a beacon is present.
The number of energy bundles within a single observations is random whenever $\delta_{o} \ne 0$.
The locations where there are no energy bundles can be neglected, since they do not
contribute significantly to the detection probability.
Let random variable $J$ be the number of energy bundles falling in the observation.
%Conditional on $J$,
%the probability of a miss in this observation is
%\begin{equation}
%\label{eq:missoneobs}
%\prob{ \text{miss in one observation} \left. \right| J = k} = (1 - \pda )^{k} \,.
%\end{equation}
Define the miss probability at the granularity of an individual observation
and conditional on the number of energy bundles in the observation $J$
and the flux $\flux$ as
\begin{align}
P_{\text{M,b} \,|\, J, \flux} (j, f) &=
\prob{ \text{miss in one observation} \left. \right| J = j, \, \flux = f } \\
&=
\prob{ \bigcap_{l=1}^{j} \left( \left| \sqrt{2 \, \ecrs \,  f} + V_{l} \right|^{2} \le \frac{2 \, \lambda}{N_{0}} \right)  } \\
&= g( f  )^{\, j} \\
g( f ) &= \prob{  \left| \sqrt{2 \, \ecrs \, f} + V_{1} \right|^{2} \le \frac{2 \, \lambda}{N_{0}}  } ^{j}
\end{align}
The condition on $\flux$ can be removed by averaging over the flux,
\begin{equation}
P_{\text{M,b} \,|\, J} (j)
= \int_{0}^{\infty} g( f  )^{\, j}  \cdot f_{\flux} (f) \, df
\end{equation}


\subsection{Granularity of $L$ observations}

Assuming that the start time of an observation is random in relation to the
energy bundles in the beacon,
the distribution of $J$ is then
\begin{equation}
\label{eq:bundlesperobs}
\prob{J = k} =
\begin{cases}
1- \delta_{0} \,, & k = n_{0} \\
\delta_{0} \,, & k = n_{0}+1 \\
0 \,, & \text{otherwise} \,.
\end{cases} 
\end{equation}


Consider first the false alarm probability.
If $N$ is the total number of energy bundle locations at granularity (c),
the overall false alarm probability is
\begin{equation}
\label{eq:pfavspfaa}
1- \pfa = (1 - \pfaa)^{N}  \ \ \ \text{or}\ \ \ \ \pfa \approx N \cdot \pfaa \,.
\end{equation}
Typically $\pfaa$ is very small, so the approximation is very accurate.
The value of $N$ is
\begin{equation}
N = L \cdot \frac{T_{0}}{T} = L \cdot \left(  \frac{n_{0} + \delta_{0}}{\delta_{p}} +1 \right) \,,
\end{equation}
leading to \eqref{eq:pfaavspfa}.

Now consider the detection probability.
Within the $L$ observations, there are $I$
observations for which $J = n_{0}$ and
$(L - I)$ observations for which  $J = n_{0}+1$,
where $I$ has a binomial distribution.
Thus based on \eqref{eq:missoneobs} the overall probability of a miss is
\begin{align}
1 - \pd &= 
\sum_{i=0}^{L} P_{\text{M,b} \,|\, J} (n_{o})^{i} \,  P_{\text{M,b} \,|\, J} (n_{o}+1)^{L-i} \cdot
\begin{pmatrix} L \\ i \end{pmatrix}  \,  (1 - \delta_{o})^{\, i} \, \delta_{o}^{\,L- i} \\
\label{eq:pmfinal}
&= \left[ (1 - \delta_{o} ) \, P_{\text{M,b} \,|\, J} (n_{o}) + \delta_{o} \, P_{\text{M,b} \,|\, J} (n_{o}+1) \right]^{L}
\,.
\end{align}
Substituting for $P_{\text{M,b} \,|\, J} (\cdot)$ from \eqref{},
\begin{equation}
1 - \pd =
 \left[ \,
  \int_{0}^{\infty} 
  g( f  )^{\, n_{o}}  \cdot \left( 1 - (1 - \delta_{o}) \cdot g( f )^{\, n_{o}+1} \right)
  \cdot f_{\flux} (f) \, df  
\, \right]^{L}
\end{equation}


%\begin{equation}
%1 - \pd =
%\sum_{i=0}^{L} \left[ (1 - \pda )^{n_{o}} \right]^{i} \,  \left[ (1 - \pda )^{n_{o}+1} \right]^{L-i} \cdot
%\begin{pmatrix} L \\ i \end{pmatrix}  \,  (1 - \delta_{o})^{\, i} \, \delta_{o}^{\,L- i} 
%\end{equation}

Evaluating the sum and substituting from \eqref{eq:pfavspd} leads to \eqref{eq:discoveryequation}.

\subsection{Special case: $n_{o} = 0$}

For the simplest case of $n_{o} = 0$, there are either
zero or one energy bundles per observation, and these relations
can be expressed in closed form without the need to resort to numerical techniques.
Letting $T_{o} = 2 T$, then $n_{o} = 0$, the conclusion is that $\delta_{o} = \delta_{p}$.
Then the $\pfaa$ required to achieve an obverall false alarm probability $\pfa$ is
\begin{equation}
N = 2 \, L \ \ \ \ \text{and} \ \ \ \ \pfaa = \frac{\pfa}{2 \, L} \,.
\end{equation}

The only two relevant values of $J$ are $J=0$ (for which $P_{\text{M,b} \,|\, J, \flux} (0) = 1$
and $J = 1$, for which
\begin{align}
P_{\text{M,b} \,|\, J, \flux} (1) &=
\prob{  \left| \sqrt{2 \, \ecrs } \, S + V_{l} \right|^{2} \le \frac{2 \, \lambda}{N_{0}}  }
= \prob{  \left| \frac{\sqrt{2 \, \ecrs } \, S + V_{l} }{1 + \ecrs} \right|^{2} 
\le \frac{2 \, \lambda}{N_{0} \, (1 + \ecrs)}  }  \\
&= 1 - \exp \left\{ - \frac{\lambda}{N_{0} \, (1 + \ecrs)}  \right\} 
= 1 - \pfaa^{\, \frac{1}{1+\ecrs}} \,.
\end{align}
Substituting into \eqref{eq:pmfinal},
\begin{equation}
1 - \pd =
 \left[ 1 -  \delta_{p} \,  \pfaa^{\, \frac{1}{1+\ecrs}} \right]^{L}
\end{equation}


\section{Detection probability for multiple independent observations}

\newcommand{\pfaLone}{P_{\text{FA},L=1}}
\newcommand{\pdLone}{P_{\text{D},L=1}}
\newcommand{\pfaNone}{P_{\text{FA},N=1}}
\newcommand{\pdNone}{P_{\text{D},N=1}}

Consider $L$ statistically independent observations.
The probability of an energy bundle being present in a single observation is defined as $p_{s}$.
When an energy bundle is not present in a single observation present, the probability of false alarm is $\pfaLone$.
When an energy bundle is present in a single observation, the probability of detection is $\pdLone$.
After $L$ observations, a detection is defined as ''one or more energy bundles detected in
individual observations'', and this has probability $\pd$.
Let the overall false alarm probability after $L$ observations be $\pfa$.

Assuming only noise is present,
the overall false-alarm probability $\pfa$ is
\begin{equation}
\label{eq:pfaapprox}
1- \pfa = (1 - \pfaLone)^{L}  \ \ \ \text{or}\ \ \ \ \pfa \approx L \cdot \pfaLone \,.
\end{equation}
Typically $\pfaLone$ is very small, so the approximation is very accurate.

When signal is present, define $M \le L$ be the number of observations which contain an energy bundle.
Then $M$ has the binomial distribution
\begin{equation}
\prob{M = m} = \begin{pmatrix} L \\ m \end{pmatrix} \, p_{s}^{\,m} \, (1 - p_{s})^{\,L - m} \,.
\end{equation}
The $(L-M)$ observations that do not contain an energy bundle have negligible
effect on $\pd$ when $\pfaLone \approx 0$, so they can be neglected.
Conditional on $M = m$, the probability of detection is thus
\begin{equation}
1 - \pd \approx (1 - \pdLone)^m
\end{equation}
and removing the conditional by averaging over $M$, 
\begin{equation}
1 - \pd \approx
\sum_{m=0}^{L} \,
 ( 1 - \pdLone )^{\,m}
\cdot
\prob{M = m}
=
\left( 1 - p_{s} \, \pdLone \right)^L \,.
\end{equation}
The approximation comes from neglecting the possibility of a detection
caused by one or more false alarms in the $(L-M)$ observations not containing
an energy bundle, and will be accurate when $\pfaLone \approx 0$.

Now suppose each observation has the timing and duration shown in Figure \ref{}.
The duration of an energy bundle is $T$, the time from the beginning of one
 energy bundle to the next is $T_{p}$, and the duration of one observation is $T_{o}$.
 We will also assume that $T_{o} \le T_{p}$, so that only one energy bundle can be present
 in a single observation.
 Also assume that the timing of an observation is blind to the presence of energy bundles.
 In that case, the probability of an energy bundle falling entirely within an observation is
 \begin{equation}
p_{s} = \frac{T_{o} - T}{T_{p}} \,.
\end{equation}
It is convenient to define two duty cycles,
$\delta_{p} = T/T_{p}$ is the duration of an energy bundle expressed as a fraction of the
time between the beginning of one bundle to the next,
and $\delta_{o} = T/T_{o}$ is the duration of an energy bundle relative to the observation interval.
Then by assumption $\delta_{p} \le \delta_{o} \le 1$, and
 \begin{equation}
p_{s} =\delta_{p} \cdot \left( \frac{1}{\delta_{o}} - 1 \right) \le 1 - \delta_{p} \,,
\end{equation}
with equality when $\delta_{o} = \delta_{p}$ or in other words $T_{0} = T_{p}$.
Note that $p_{s} \to 0$ as $\delta_{o} \to 1$, because when $T_{0} = T$
 the observation interval would have to precisely line up with the energy bundle, which has
 probability zero.

Now focus on the determination of $\pfaLone$ and $\pdLone$.
Whenever $\delta_{0} < 1$, a single observation spans a greater time than
the duration of an energy bundle.
Assume for simplicity that $T_{o} = N \, T$ for some integer $N \ge 1$,
and hence $\delta_{o} = 1/N$.
Then assuming disjoint observations in the $N$ target locations,
\begin{equation}
1 - \pfaLone = (1 - \pfaNone )^{N}
\ \ \ \text{or}\ \ \ \ \pfaLone \approx N \cdot \pfaNone = \pfaNone / \delta_{o} \,.
\end{equation}
where $\pfaNone$ is the probability of false alarm when $N=1$.
The constraint that one and only one energy bundle can appear in a single observation
simplifies the calculation of $\pdLone$.
As before the small probability that a false alarm causes a detection can be neglected,
and subject to this approximation
\begin{equation}
\pdLone \approx \pdNone \,.
\end{equation}
The variable $\pdNone$ can be eliminating by substituting
from \eqref{eq:asympPfaVsPd},
\begin{equation}
\pdNone = 
\pfaNone^{\, \frac{1}{1+ \ecrs}} \,.
\end{equation}
Finally, expressing this in terms of $\pfa$,
\begin{equation}
\pd = 1 - \left(
1 -  \delta_{p} \cdot \left( \frac{1}{\delta_{o}} - 1 \right) \cdot 
\left( \frac{\delta_{o} \, \pfa }{L} \right)^{\, \frac{1}{1+ \ecrs}}
\right)^{L}
\end{equation}



and $\pfaLone$ can be eliminated using approximation \eqref{eq:pfaapprox},
resulting finally in \eqref{eq:discoveryequation}.


\chapter{Coherence bandwidth of plasma dispersion}
\label{sec:plasmaappx}

Integrating both sides of \eqref{eq:delayFromPhase},
the phase in \eqref{eq:passbanddispersiontf} is
\begin{equation}
\phi(f) = \phi (f_{c}) - 2 \pi \, \int_{f_{c}}^{f} \tau(u) \, du
= \phi (f_{c}) -  2 \pi \, \dc \, \dm \, \left( \frac{1}{f_{c}} - \frac{1}{f} \right)
\end{equation}
Expanding $\phi (f)$ in a Taylor series about $f = f_{c}$,
\begin{equation}
\label{eq:taylor}
\phi(f) =
\phi (f_{c}) -  2 \pi \, \dc \, \dm
\left(
\frac{f-f_{c}}{f_{c}^{\,2}} - \frac{(f-f_{c})^{2}}{f_{c}^{\,3}}  + \frac{(f-f_{c})^{3}}{f_{c}^{\,4}}  - \dots
\right) \,.
\end{equation}
The linear term is benign because it corresponds to a fixed group delay,
so the actual distortion is caused by the second-order and higher terms.
The second-order term (and hence the higher-order terms) 
have variation less than $\alpha \pi$ for $f \in [f_{c},f_{c}+B]$ if
\begin{equation}
2 \pi \, \dc \, \dm \,
\frac{ B^{2}}{f_{c}^{\,3}} \ll \alpha\, \pi
\end{equation}
which is yields \eqref{eq:dispersioncoherencebandwidth}.
In that case, \eqref{eq:taylor} becomes for $f \in [f_{c},f_{c}+B]$
\begin{equation}
\phi(f) \approx
\phi (f_{c}) -  2 \pi \, \tau (f_{c}) \cdot ( f - f_{c} ) \,.
\end{equation}
Thus, \eqref{eq:passbanddispersiontf} becomes
\begin{equation}
G(f)
\approx
e^{ \, i \, \phi (f_{c})}
\cdot
e^{ \, - i \, 2 \pi \, (f - f_{c})  \, \tau (f_{c})}
\,.
\end{equation}
The equivalent baseband transfer function is $G(f+f_{c})$, and this
too is illustrated in Figure \ref{fig:dispersion}.

\chapter{Partial equalization of plasma dispersion}
\label{sec:equalization}

Even though $\dm$ refers to a measurable physical property
pertaining to the line of sight between transmitter and receiver,
the state of knowledge of $\dm$
may be different at the transmitter and the receiver.
Astronomical observations provide
a priori knowledge about $\dm$ \citeref{213} in the form
of upper and lower bounds $\dm_{L} \le \dm \le \dm_{U}$.
The resulting uncertainty is captured by $\deltadm = (\dm_{U} - \dm_{L})$.
A more advanced civilization may possess tighter bounds
and a smaller $\deltadm$, but can probably never reduce the uncertainty entirely.

There is the possibility of equalization for any specific
value of $\dm$ by introducing by adding an artificial group delay such that
the artificial group delay plus the group delay corresponding to $\dm$
is constant over $f \in [0,B]$.
This can be done in either transmitter or receiver, and
the combined effect is indistinguishable from a benign fixed delay
which adds to the very large propagation delay.
Specifically a causal allpass filter with response
$F_{\text{eq}} (f) = \exp \{ i \, 2 \pi \, \phi_{eq} (f) \}$, where
\begin{equation}
\label{eq:preeq}
\tau_{\text{eq}} (f) = \dc \cdot \dm \cdot \left( \frac{1}{f_{c}^{\,2}} - \frac{1}{(f+f_{c})^{2}} \right)
\ \ \ \text{and} \ \ \ \ 
\frac{\phi_{\text{eq}} (f)}{2 \pi} = - \dc \cdot \dm \cdot \frac{f^{\,2}}{f_{c}^{\,2} \, (f+f_{c})} 
\end{equation}
placed before or after the dispersion results 
overall in a constant group delay $\dc \cdot \dm / f_{c}^{\,2}$.
Done in the transmitter, this pre-equalization has no effect on
the noise.
Done in the receiver, this post-equalization 
does change the noise \emph{waveform} but has no 
effect on the noise \emph{statistics} since $F_{\text{eq}} (f)$ is
an all pass (phase-only) filter \citerefWloc{43}{Chap. 8}.

An issue for the receiver to consider is whether or not the transmitter
has performed pre-equalization
$\dm_L$, after which $0 \le \dm \le \deltadm$.
Since $\deltadm < \dm_U$, this would increase the dispersion coherence bandwidth $B_0$.
Thus, a receiver estimating a range of $B_{0}$ for a given line of sight
prior to discovery may wish to consider two cases: with and without pre-equalization.

%In the following, an information-bearing signal will be tailored to $B_c$.
%Considering that the signal is determined by the transmitter alone, it is
%the transmitter's perception of $\dm_L$ and $\dm_U$ that matters.
%The transmitter may pre-equalize and tailor the signal bandwidth to 
% $B_c$ corresponding to $\deltadm$, or it may choose not to
%pre-equalize and use $\dm_U$ in determining $B_{c}$.
%The receiver must also take into account that its knowledge of 
%$\{ \dm_L , \,\dm_U \}$ inevitably differs from that of the transmitter.
%Following discovery and during communication, $\widehat \dm$
%can be used for post-equalization, which again has no effect on the
%noise statistics.
%For this reason, dispersion is an issue during
%discovery, but for most practical purposes should have no impact on communication.

\chapter{Referencing passband Doppler to baseband}
\label{sec:doppleranalysis}

The output of the channel before demodulation is
\begin{equation}
y(t) =
e^{\, i \, \theta } \cdot 
h \left( \left(1- \frac{v}{c} \right) \, t -\frac{a \cdot t^{\,2}}{2 \, c} \right) 
\cdot \exp \left(  \, i\, 2 \pi \, f_{c} \, \left(1- \frac{v}{c} \right) \, t \right) \cdot
\exp \left( \,- i\, \pi \, \frac{a \,  t^{\,2}}{\lambda_{c}}  \right) \,.
\end{equation}
Choosing the parameters of \eqref{eq:judiciousparam},
the matched filter output is
\begin{equation}
\label{eq:recconv}
 z \left( \frac{t}{1+\delta} \right)
= \frac{1}{1+\delta} \, e^{\, i \, \theta } 
\int
\exp \left( \, - \, i\, \pi \, \frac{a \,  v^{\,2}}{(1+ \delta)^{\,2} \, \lambda_{c}}  \right)
\cdot h \left( v -\frac{a \cdot v^{\,2}}{2 \, (1+\delta)^{\,2} \, c} \right)
\cdot \cc h ( v - t  )
\, dv \,.
\end{equation}
Since $| \delta | \ll 1$ the $(1+\delta)$ terms can safely be neglected,
and thus Figure \ref{fig:passbanddoppler} is a representation of
\eqref{eq:recconv} with $\delta = 0$.

\chapter{Coherence time with fading}
\label{sec:fadinganalysis}

The Fresnel approximation
expands the left side of \eqref{eq:dwv} in a Taylor series and retains terms 
up to $x^{2}$ and $t^{2}$.
The constant term is a flat delay and is discarded.
The result is the right side of \eqref{eq:dwv}
\begin{equation}
v(x) = v_{\parallel} - \frac{v_{\bot} x}{D_{2}} - \frac{v_{\parallel} x^{2}}{2 \, D_{2}^{\,2}}
\approx 
v_{\parallel} - \frac{v_{\bot} x}{D_{2}} \,.
\end{equation}
The fact that the net velocity $v(x)$ depends on $x$ limits the time coherence,
because different rays have slightly different Doppler shifts which causes their
superposition to change with time.

Within an ICH, where the distortion of $h(t)$ by plasma dispersion can be neglected,
the observer sees, associated with a ray through point $x$, the passband response
\begin{equation}
\Re \left\{ h \left( t - \frac{d(x) - v(x) \, t}{c} \right) 
\exp \left\{ \,i\,2 \pi \, f_{c} \, \left( t - \frac{d(x) - v(x) \, t}{c} \right) \right\} \right\} \,.
\end{equation}
Within an ICH, the effect of delay on $h(t)$ can be neglected, and thus the 
equivalent complex baseband signal is
\begin{equation}
\label{eq:threeterms}
h \left( t \right) \, \exp \{ - \,i\,2 \pi \, f_{c} \,d(x) / c) \} \, \exp \{ \,i\,2 \pi \, f_{c} \,v(x) \, t / c) \} \,.
\end{equation}
The first two terms in \eqref{eq:threeterms} are familiar,
but the third is the interesting one,
\begin{equation}
 \exp \{ \,i\,2 \pi \, f_{c} \,v(x) \, t / c) \} =
 \exp \{ \,i\,2 \pi \, f_{c} \,v_{\parallel} \, t / c) \} \exp \{ - \,i\,2 \pi \, f_{c} \,v_{\bot} \, x \, t / c \, D_{2}) \} \,.
\end{equation}
The effect of $v_{\parallel}$ can be compensated by a simple carrier frequency offset
as described in Section \ref{sec:doppler}.
That $v_{\parallel}$ can be rendered impotent in this manner is not surprising,
since this component of velocity aligned with the light of sight affects all rays
in the same way.
The second term is a time-varying phase at baseband which affects the
time coherence
unless the total phase shift it causes over $t \in [0, T]$, which is condition \eqref{eq:tcf}.


